2-adic Galois images of non-CM isogeny-torsion graphs

Let $\mathcal{E}$ be a $\mathbb{Q}$-isogeny class of elliptic curves defined over $\mathbb{Q}$ without CM. The isogeny graph associated to $\mathcal{E}$ is a graph which has a vertex for each elliptic curve in $\mathcal{E}$ and an edge for each $\mathbb{Q}$-isogeny of prime degree that maps one elliptic curve in $\mathcal{E}$ to another elliptic curve in $\mathcal{E}$, with the degree recorded as a label of the edge. An isogeny-torsion graph is an isogeny graph where, in addition, we label each vertex with the abstract group structure of the torsion subgroup over $\mathbb{Q}$ of the corresponding elliptic curve. Then, the main statement of the article is a classification of the $2$-adic image of Galois that occurs at each vertex of all isogeny-torsion graphs consisting of elliptic curves defined over $\mathbb{Q}$ without CM.

==> removed_stuff.tex <==
\iffalse

\begin{lemma}\label{2-adic images}

Let $E$ and $E'$ be non-CM elliptic curves defined over $\QQ$ that are $\QQ$-isogenous by an isogeny $\phi$ whose kernel is finite, cyclic, and $\QQ$-rational. Let $r$ be the non-negative integer such that $2^{r}$ is the greatest power of $2$ that divides the order of $\operatorname{Ker}(\phi)$. Suppose that $\rho_{E,2^{\infty}}(G_{\QQ})$ is a group of level $2^{m}$. Then $5 \geq m \geq r \geq 0$ and there is a basis of $E[2^{m}]$ such that $\overline{\rho}_{E,2^{m}}(G_{\QQ})$ is conjugate to
$$\left\langle
\begin{bmatrix} A_{1} & C_{1} \\ B_{1} & D_{1} \end{bmatrix},
\ldots,
\begin{bmatrix} A_{s} & C_{s} \\ B_{s} & D_{s} \end{bmatrix}
\right\rangle \subseteq \operatorname{GL}\left(2, \ZZ / 2^{5+r}\ZZ \right)$$
such that $2^{r}$ divides $C_{1}$, \ldots, $C_{s}$.

Moreover,


\begin{enumerate}
\item f
    \begin{itemize}
    \item if $m = 0$, then $\overline{\rho}_{E,2^{5+r}}(G_{\QQ}) = \operatorname{GL}\left(2, \ZZ / 2^{5+r} \ZZ\right)$,
    
    \item if $m=1$, then there is a basis $\left\{P_{2^{5+r}}, Q_{2^{5+r}}\right\}$ of $E\left[2^{5+r}\right]$ such that $\overline{\rho}_{E,2^{5+r}}(G_{\QQ})$ is conjugate to
    $$\left\langle
\begin{bmatrix} A_{1} & C_{1} \\ B_{1} & D_{1} \end{bmatrix},
\ldots,
\begin{bmatrix} A_{s} & C_{s} \\ B_{s} & D_{s} \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 2 & 1 \end{bmatrix}
\right\rangle \subseteq \operatorname{GL}\left(2, \ZZ / 2^{5+r}\ZZ \right)$$
such that $2^{r}$ divides $C_{1}$, \ldots, $C_{s}$,

\item and if $m \geq 2$, then there is a basis $\left\{P_{2^{5+r}}, Q_{2^{5+r}} \right\}$ of $E[2^{5+r}]$, such that $\overline{\rho}_{E,2^{5+r}}(G_{\QQ})$ is conjugate to
$$\left\langle
\begin{bmatrix} A_{1} & C_{1} \\ B_{1} & D_{1} \end{bmatrix},
\ldots,
\begin{bmatrix} A_{s} & C_{s} \\ B_{s} & D_{s} \end{bmatrix},
\begin{bmatrix} 1+2^{m} & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 2^{m} \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 2^{m} & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 1+2^{m} \end{bmatrix}
\right\rangle \subseteq \operatorname{GL}\left(2, \ZZ / 2^{5+r}\ZZ \right)$$
such that $2^{r}$ divides $C_{1}$, \ldots, $C_{s}$.
\end{itemize}

Let $Q_{2^{r}}$ be a point on $E$ that generates the subgroup $\operatorname{Ker}(\phi)$ of order $2^{r}$. Then there is a point $Q_{2^{m}}$ of order $2^{m}$ such that $\left\langle Q_{2^{m}} \right\rangle$ contains $Q_{2^{r}}$. Moreover, we can pick the basis of $E[2^{m+r}]$ in such a way that $\left\langle Q_{2^{r}} \right\rangle \subseteq \left\langle Q_{2^{m}} \right\rangle \subseteq \left\langle Q_{2^{m+r}} \right\rangle$.

\item Moreover, if

\begin{itemize}

\item $m \geq 2$, then $\overline{\rho}_{E',32}(G_{\QQ})$ is conjugate to
$$\left\langle
\begin{bmatrix} A_{1} & \frac{C_{1}}{2^{r}} \\ 2^{r} \cdot B_{1} & D_{1} \end{bmatrix},
\ldots,
\begin{bmatrix} A_{s} & \frac{C_{s}}{2^{r}} \\ 2^{r} \cdot B_{s} & D_{s} \end{bmatrix},
\begin{bmatrix} 1+2^{r} & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 2^{m-r} \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 2^{m+r} & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 1+2^{r} \end{bmatrix}
\right\rangle$$
\item $m = 1$, then $\overline{\rho}_{E',32}(G_{\QQ})$ is conjugate to
$$\left\langle
\begin{bmatrix} A_{1} & \frac{C_{1}}{2^{r}} \\ 2^{r} \cdot B_{1} & D_{1} \end{bmatrix},
\ldots,
\begin{bmatrix} A_{s} & \frac{C_{s}}{2^{r}} \\ 2^{r} \cdot B_{s} & D_{s} \end{bmatrix},
\begin{bmatrix} 1 & 2^{1-r} \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 2^{1+r} & 1 \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}
\right\rangle$$
\item $m = 0$, then $\overline{\rho}_{E',32}(G_{\QQ})$ is conjugate to $\operatorname{GL}(2, \ZZ / 32 \ZZ)$
\end{itemize}
\end{enumerate}

\end{lemma}

\begin{proof}
We break up the proof into steps.

\begin{enumerate}
\item By Theorem \ref{thm-rzb}, $\rho_{E,2^{\infty}}(G_{\QQ})$ is a group of level $2^{m}$ where $0 \leq m \leq 5$. If $m = 0$, then $\rho_{E,2^{\infty}}(G_{\QQ})$ is a group of level $1$, in other words, $\rho_{E,2^{\infty}}(G_{\QQ}) = \operatorname{GL}(2, \ZZ_{2})$ and so, $\overline{\rho}_{E,2}(G_{\QQ})$ is conjugate to $\operatorname{GL}(2, \ZZ / 2 \ZZ)$. If at the same time, $r$ is positive, then by Lemma \ref{Borel 2}, $\overline{\rho}_{E,2}(G_{\QQ})$ is conjugate to a subgroup of $\left\{\operatorname{Id}, \begin{bmatrix} 1 & 0 \\ 1 & 1 \end{bmatrix}\right\}$ which is a contradiction, hence, $r = 0$.

Now suppose that $r$ is a positive integer and assume by way of contradiction that $1 \leq m < m+1 \leq r$. Then by Lemma \ref{Borel 2}, $\overline{\rho}_{E,2^{r}}(G_{\QQ})$ is conjugate to a subgroup of $\operatorname{GL}\left(2, \ZZ / 2^{r} \ZZ\right)$ of the form
$$\left\langle
\begin{bmatrix} A_{1} & 0 \\ B_{1} & D_{1} \end{bmatrix},
\ldots,
\begin{bmatrix} A_{1} & 0 \\ B_{1} & D_{1} \end{bmatrix}
\right\rangle.$$
Next, $\overline{\rho}_{E,2^{m+1}}(G_{\QQ})$ and $\overline{\rho}_{E,2^{m}}(G_{\QQ})$ are simply the reductions of $\overline{\rho}_{E,2^{r}}(G_{\QQ})$ modulo $2^{m+1}$ and $2^{m}$ respectively. Hence, $\overline{\rho}_{E,2^{m+1}}(G_{\QQ})$ is conjugate to
$$\left\langle
\begin{bmatrix} A_{1} & 0 \\ B_{1} & D_{1} \end{bmatrix},
\ldots,
\begin{bmatrix} A_{1} & 0 \\ B_{1} & D_{1} \end{bmatrix}
\right\rangle \subseteq \operatorname{GL}(2, \ZZ / 2^{m+1} \ZZ)$$
and $\overline{\rho}_{E,2^{m}}(G_{\QQ})$ is conjugate to
$$\left\langle
\begin{bmatrix} A_{1} & 0 \\ B_{1} & D_{1} \end{bmatrix},
\ldots,
\begin{bmatrix} A_{1} & 0 \\ B_{1} & D_{1} \end{bmatrix}
\right\rangle \subseteq \operatorname{GL}(2, \ZZ / 2^{m} \ZZ).$$
By Lemma \ref{lifting with kernel} and Lemma \ref{kernel of pi 2},
if $m = 1$, then $\overline{\rho}_{E,2^{m+1}}(G_{\QQ}) = \overline{\rho}_{E,4}(G_{\QQ})$ is conjugate to
$$\left\langle
\begin{bmatrix} A_{1} & 0 \\ B_{1} & D_{1} \end{bmatrix},
\ldots,
\begin{bmatrix} A_{1} & 0 \\ B_{1} & D_{1} \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 2 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}
\right\rangle \subseteq \operatorname{GL}(2, \ZZ / 2^{m+1} \ZZ)$$
and if $m \geq 2$, then by Lemma \ref{lifting with kernel} and Lemma \ref{kernel of pi 1}, $\overline{\rho}_{E,2^{m+1}}(G_{\QQ})$ is conjugate to
$$\left\langle
\begin{bmatrix} A_{1} & 0 \\ B_{1} & D_{1} \end{bmatrix},
\ldots,
\begin{bmatrix} A_{1} & 0 \\ B_{1} & D_{1} \end{bmatrix},
\begin{bmatrix} 1+2^{m} & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 1+2^{m} \end{bmatrix},
\begin{bmatrix} 1 & 2^{m} \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 2^{m} & 1 \end{bmatrix}
\right\rangle \subseteq \operatorname{GL}(2, \ZZ / 2^{m+1} \ZZ).$$
In both cases of $m = 1$ or $m \geq 2$, there are contradictions due to the order of $\overline{\rho}_{E,2^{m+1}}(G_{\QQ})$ because of the presence of the matrix $\begin{bmatrix} 1 & 2^{m} \\ 0 & 1 \end{bmatrix}$. We continue with the proof of the classification of the generators of $\overline{\rho}_{E,2^{5+r}}(G_{\QQ})$ in the cases of level $2^{m}$.


If $m = 0$, then this part of the lemma is clear. We may suppose that $m$ is positive. The proof is similar to the proof of Lemma \ref{Borel 1}.

Let $Q_{2^{r}}$ be a point on $E$ of order $2^{r}$ that is contained in $\operatorname{Ker}(\phi)$. Let $Q_{2^{m}}$ be a point on $E$ such that $[2^{m-r}] \cdot Q_{2^{m}} = Q_{2^{r}}$. Let $P_{2^{m}}$ be a point on $E$ such that $E[2^{m}] = \left\langle P_{2^{m}}, Q_{2^{m}} \right\rangle$. Let $\sigma \in G_{\QQ}$. Then there are integers $A$, $B$, $C$, and $D$, such that $\sigma(P_{2^{m}}) = [A]P_{2^{m}} + [B]Q_{2^{m}}$ and $\sigma(Q_{2^{m}}) = [C]P_{2^{m}} + [D]Q_{2^{m}}$. Note that $\left\langle Q_{2^{r}} \right\rangle$ generates a $\QQ$-rational group. Then
$$\sigma(Q_{2^{r}}) = \sigma\left([2^{m-r}]Q_{2^{m}}\right) = [2^{m-r}]\sigma(Q_{2^{m}}) = [2^{m-r}]([C]P_{2^{m}} + [D]Q_{2^{m}}) = [2^{m-r}C]P_{2^{m}} + [D]Q_{2^{r}}.$$
As $[2^{m-r}C]P_{2^{m}} + [D]Q_{2^{r}}$ is an element of $\left\langle Q_{2^{r}} \right\rangle$, so is $[2^{m-r}C]P_{2^{m}}$. As $\left\langle P_{2^{m}} \right\rangle \cap \left\langle Q_{2^{m}} \right\rangle = \left\{ \mathcal{O} \right\}$, we have that $[2^{m-r}C]P_{2^{m}} = \mathcal{O}$ and hence, $2^{m}$ divides $2^{m-r}C$. Thus, $2^{r}$ divides $C$. Hence, $\overline{\rho}_{E,2^{m}}(G_{\QQ})$ is conjugate to a subgroup of $\operatorname{GL}(2, \ZZ / 2^{m} \ZZ)$ of the form
$$\left\langle
\begin{bmatrix} A_{1} & C_{1} \\ B_{1} & D_{1} \end{bmatrix},
\ldots
\begin{bmatrix} A_{s} & C_{s} \\ B_{s} & D_{s} \end{bmatrix}
\right\rangle$$
such that $2^{r}$ divides $C_{1}$, \ldots, $C_{s}$.

Note that $r+5 \geq 5 \geq m \geq r$. If $m = 1$, then by Lemma \ref{lifting with kernel}, there is a basis $\left\{P_{2^{5+r}}, Q_{2^{5+r}}\right\}$ of $E\left[2^{5+r}\right]$ with $\left\langle Q_{2^{r}} \right\rangle \subseteq \left\langle Q_{2^{m}} \right\rangle \subseteq \left\langle Q_{2^{r+5}} \right\rangle$, such that $\overline{\rho}_{E,2^{5+r}}(G_{\QQ})$ is conjugate to
$$\left\langle
\begin{bmatrix}
A_{1} & C_{1} \\ B_{1} & D_{1}
\end{bmatrix},
\ldots,
\begin{bmatrix}
A_{s} & C_{s} \\ B_{s} & D_{s}
\end{bmatrix},
\begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 2 & 1 \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}
\right\rangle$$
and if $m \geq 2$, then by Lemma \ref{lifting with kernel}, there is a basis $\left\{P_{2^{5+r}}, Q_{2^{5+r}}\right\}$ of $E[2^{5+r}]$, such that $\left\langle Q_{2^{r}} \right\rangle \subseteq \left\langle Q_{2^{m}} \right\rangle \subseteq \left\langle Q_{2^{r+5}} \right\rangle$ and
$\overline{\rho}_{E,2^{5+r}}(G_{\QQ})$ is conjugate to
$$\left\langle
\begin{bmatrix}
A_{1} & C_{1} \\ B_{1} & D_{1}
\end{bmatrix},
\ldots,
\begin{bmatrix}
A_{s} & C_{s} \\ B_{s} & D_{s}
\end{bmatrix},
\begin{bmatrix} 1 & 2^{m} \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 2^{m} & 1 \end{bmatrix},
\begin{bmatrix} 1+2^{m} & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 1+2^{m} \end{bmatrix}
\right\rangle.$$

\item We will prove that $E'[32] = \left\langle \phi([2^{r}]P_{2^{5+r}}), \phi(Q_{2^{5+r}})\right\rangle$ by proving that the order of both $\phi([2^{r}]P_{2^{5+r}})$ and $\phi(Q_{2^{5+r}})$ are equal to $32$ and that $\left\langle \phi([2^{r}]P_{2^{5+r}}) \right\rangle \cap \left\langle \phi(Q_{2^{5+r}}) \right\rangle = \left\{\mathcal{O}\right\}$.

We have $[32] \cdot ([2^{r}]\phi(P_{2^{5+r}})) = \phi([2^{5+r}]P_{2^{5+r}}) = \mathcal{O}$ and $[16] \cdot ([2^{r}]\phi(P_{2^{5+r}}) = \phi([2^{4+r}]P_{2^{5+r}})$. By Lemma \ref{generators of Z/2^NZ} and Remark \ref{remark generators of Z/2^NZ} $[2^{4+r}]P_{2^{5+r}} = P_{2}$ is not contained in $\left\langle Q_{2^{r}} \right\rangle$ and so, $[16] \cdot ([2^{r}]\phi(P_{2^{5+r}}) \neq \mathcal{O}$. Hence, the order of $[2^{r}]\phi(P_{2^{5+r}})$ is equal to $32$. Next, $[32] \cdot \phi(Q_{2^{5+r}}) = \phi([32]Q_{2^{5+r}}) = \mathcal{O}$ as $[32]Q_{2^{5+r}}$ is contained in $\left\langle Q_{2^{r}} \right\rangle$. Next, $[16] \cdot \phi(Q_{2^{5+r}}) = \phi([16]Q_{2^{5+r}})$. Note that the order of $[16]Q_{2^{5+r}}$ is equal to $2^{1+r}$ and hence, cannot be in $\left\langle Q_{2^{r}} \right\rangle$.

Assume by way of contradiction that $\left\langle \phi([2^{r}]P_{2^{r+5}}) \right\rangle \cap \left\langle \phi(Q_{2^{r+5}}) \right\rangle$ is not trivial. Then $\left\langle \phi(Q_{2^{r+5}}) \right\rangle$ and $\left\langle \phi([2^{r}]P_{2^{r+5}}) \right\rangle$ share a point of order $2$. The point of order $2$ in $\left\langle \phi([2^{r}]P_{2^{r+5}}) \right\rangle$ is $\phi([2^{4+r}]P_{2^{r+5}})$ and the point of order $2$ in $\left\langle \phi(Q_{2^{r+5}}) \right\rangle$ is $\phi([16]Q_{2^{r+5}})$. If they were equal, then $[2^{4+r}]P_{2^{r+5}} - [16]Q_{2^{r+5}} \in \left\langle Q_{2^{r}} \right\rangle \subseteq \left\langle Q_{2^{5+r}} \right\rangle$. Thus, $[2^{4+r}]P_{2^{r+5}} \in \left\langle Q_{2^{5+r}} \right\rangle$. As $\left\langle P_{2^{r+5}} \right\rangle \bigcap \left\langle Q_{2^{r+5}} \right\rangle = \left\{ \mathcal{O} \right\}$, we have that $[2^{4+r}]P_{2^{r+5}} \notin \left\langle Q_{2^{r+5}} \right\rangle$.

Let $\sigma \in G_{\QQ}$. Then there are integers $A$ and $B$ such that $\sigma(P_{2^{5+r}}) = [A]P_{2^{5+r}} + [B]Q_{2^{5+r}}$ and there are integers $C$ and $D$ such that $\sigma(Q_{2^{5+r}}) = [C]P_{2^{5+r}} + [D]Q_{2^{5+r}}$. Then
$$\sigma(\phi([2^{r}]P_{2^{5+r}})) = \phi([2^{r}]([A]P_{2^{5+r}}+[B]Q_{2^{5+r}})) = [A]\phi([2^{r}]P_{2^{5+r}}) + [2^{r}B]\phi(Q_{2^{5+r}})$$
$$\sigma(\phi(Q_{2^{r+5}})) = \phi(\sigma(Q_{2^{5+r}})) = \phi([C]P_{2^{5+r}} + [D]Q_{2^{5+r}}) = \phi([C]P_{2^{5+r}}) + [D]\phi(Q_{2^{5+r}}).$$
As $C$ is divisible by $2^{r}$, we have $C = \frac{C}{2^{r}} \cdot 2^{r}$ and so,
$$\phi([C]P_{2^{5+r}}) = \phi\left(\left[\frac{C}{2^{r}}\right][2^{r}]P_{2^{5+r}}\right) = \left[\frac{C}{2^{r}}\right]\phi([2^{r}]P_{2^{5+r}}).$$
In particular, in the case that $m = 0$, we have that $r = 0$ and by Lemma \ref{lifting with kernel}, $\overline{\rho}_{E,32}(G_{\QQ})$ is conjugate to $\overline{\rho}_{E',32}(G_{\QQ})$. The rest of the proof is clear due to Lemma \ref{kernel of pi 1}, Lemma \ref{kernel of pi 2}, and Lemma \ref{lifting with kernel}.
\end{enumerate}
\end{proof}
\fi



\iffalse

Note that the group $\operatorname{H}_{38}$ is a proper subgroup of $\operatorname{H}_{14}$. Hence, in order to prove that there is no non-CM elliptic curve $E/\QQ$ such that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to a subgroup of $\operatorname{H}_{38}$ and $\overline{\rho}_{E,3}(G_{\QQ})$ is conjugate to a subgroup of $\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$ simultaneously, it suffices to prove that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is not conjugate to a subgroup of $\operatorname{H}_{14}$ and $\overline{\rho}_{E,3}(G_{\QQ})$ is not conjugate to a subgroup of $\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$ simultaneously (see Table \ref{Modular curves of genus 1}).

Note that the group $\operatorname{H}_{46}$ is a proper subgroup of $\operatorname{H}_{18}$. Hence, in order to prove that there is no non-CM elliptic curve $E/\QQ$ such that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to a subgroup of $\operatorname{H}_{46}$ and $\overline{\rho}_{E,3}(G_{\QQ})$ is conjugate to a subgroup of $\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$ simultaneously, it suffices to prove that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is not conjugate to a subgroup of $\operatorname{H}_{18}$ and $\overline{\rho}_{E,3}(G_{\QQ})$ is not conjugate to a subgroup of $\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$ simultaneously (see Table \ref{Modular curves of genus 1}).

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.59}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \# & $\overline{\rho}_{E,3}(G_{\QQ})$ & $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ & $\textit{j}_{3}(E)$ & $\textit{j}_{2^{\infty}}(E)$ & $H$ & $l$ & $i$ & $g$ & LMFDB \\
    \hline
    \multirow{4}*{$1$} & \multirow{8}*{$\left\{ \begin{bmatrix} 1 & \ast \\ 0 & \ast \end{bmatrix} \right\}$} & \multirow{4}*{$\operatorname{H}_{8a}$} & \multirow{20}*{$\frac{(s+3)^{3}(s+27)}{s}$} & \multirow{8}*{$64 \cdot \frac{\left(t^{2}+3\right)^{3}}{\left(t-1\right)^{2}\left(t+1\right)^{2}}$} & \multirow{4}*{$\begin{bmatrix} 19 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 0 & 13 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 6 & 1 \end{bmatrix}$} & \multirow{4}*{$24$} & \multirow{4}*{$96$} & \multirow{4}*{$2$} & \multirow{4}*{\texttt{24.96.2.3}} \\
    & & & & & & & & & \\
    & & & & & & & & & \\
    & & & & & & & & & \\
    \cline{1-1}
    \cline{3-3}
    \cline{6-10}
    & & & & & & & & & \\
    \multirow{4}*{$2$} & & \multirow{4}*{$\operatorname{H}_{8b}$} & & & \multirow{4}*{$\begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 6 & 1 \end{bmatrix}$} & \multirow{4}*{$12$} & \multirow{4}*{$96$} & \multirow{4}*{$2$} & \multirow{4}*{\texttt{12.96.2.1}} \\
    & & & & & & & & & \\
    & & & & & & & & & \\
    & & & & & & & & & \\
    \cline{1-3}
    \cline{5-10}
    \multirow{4}*{$3$} & \multirow{12}*{$\left\{ \begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$} & \multirow{4}*{$\operatorname{H}_{24}$} & & \multirow{4}*{$256 \cdot \frac{\left(t^{2}-t+1\right)^{3} \cdot \left(t^{2}+t+1\right)^{3}}{t^{4}\left(t^{2}+1\right)^{2}}$} & \multirow{4}*{$\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 2 \\ 6 & 1 \end{bmatrix}$} & \multirow{4}*{$12$} & \multirow{4}*{$48$} & \multirow{4}*{$1$} & \multirow{4}*{\texttt{12.48.1.4}} \\
    & & & & & & & & & \\
    & & & & & & & & & \\
    & & & & & & & & & \\
    \cline{1-1}
    \cline{3-3}
    \cline{5-10}
    \multirow{4}*{$4$} & & \multirow{4}*{$\operatorname{H}_{38}$} & & \multirow{4}*{$64 \cdot \frac{(t^{4}-2t^{2}+4)^{3}}{t^{4}(t^{2}-2)^{2}}$} & \multirow{4}*{$\begin{bmatrix} 11 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 19 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 19 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 6 & 1 \end{bmatrix}$} & \multirow{4}*{$24$} & \multirow{4}*{$48$} & \multirow{4}*{$1$} & \multirow{4}*{\texttt{24.48.1.31}} \\
    & & & & & & & & & \\
    & & & & & & & & & \\
    & & & & & & & & & \\
    \cline{1-1}
    \cline{3-3}
    \cline{5-10}
    \multirow{4}*{$5$} & & \multirow{4}*{$\operatorname{H}_{46}$} & & \multirow{4}*{$64 \frac{\left(t^{4}+2t^{2}+4\right)^{3}}{t^{4}\left(t^{2}+2\right)^{2}}$} & \multirow{4}*{$\begin{bmatrix} 7 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 23 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 19 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 6 & 1 \end{bmatrix}$} & \multirow{4}*{$24$} & \multirow{4}*{$48$} & \multirow{4}*{$1$} & \multirow{4}*{\texttt{24.48.1.32}} \\
    & & & & & & & & & \\
    & & & & & & & & & \\
    & & & & & & & & & \\
    \hline
\end{tabular}}
\caption{product groups for $S$ graphs}
\label{product groups for S graphs}
\end{table}
\end{center}
Note that the group $\operatorname{H}_{24}$ is a proper subgroup of $\operatorname{H}_{11}$. Hence, in order to prove that there is no non-CM elliptic curve $E/\QQ$ such that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to a subgroup of $\operatorname{H}_{24}$ and $\overline{\rho}_{E,3}(G_{\QQ})$ is conjugate to a subgroup of $\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$ simultaneously, it suffices to prove that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is not conjugate to a subgroup of $\operatorname{H}_{11}$ and $\overline{\rho}_{E,3}(G_{\QQ})$ is not conjugate to a subgroup of $\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$ simultaneously (see Table \ref{Modular curves of genus 1}).

Note that the group $\operatorname{H}_{38}$ is a proper subgroup of $\operatorname{H}_{14}$. Hence, in order to prove that there is no non-CM elliptic curve $E/\QQ$ such that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to a subgroup of $\operatorname{H}_{38}$ and $\overline{\rho}_{E,3}(G_{\QQ})$ is conjugate to a subgroup of $\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$ simultaneously, it suffices to prove that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is not conjugate to a subgroup of $\operatorname{H}_{14}$ and $\overline{\rho}_{E,3}(G_{\QQ})$ is not conjugate to a subgroup of $\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$ simultaneously (see Table \ref{Modular curves of genus 1}).

Note that the group $\operatorname{H}_{46}$ is a proper subgroup of $\operatorname{H}_{18}$. Hence, in order to prove that there is no non-CM elliptic curve $E/\QQ$ such that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to a subgroup of $\operatorname{H}_{46}$ and $\overline{\rho}_{E,3}(G_{\QQ})$ is conjugate to a subgroup of $\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$ simultaneously, it suffices to prove that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is not conjugate to a subgroup of $\operatorname{H}_{18}$ and $\overline{\rho}_{E,3}(G_{\QQ})$ is not conjugate to a subgroup of $\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$ simultaneously (see Table \ref{Modular curves of genus 1}).
\fi

\iffalse
\begin{itemize}
    \item $R_{4}(10)$
    
    Let $B_{5} = \left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\} \subseteq \operatorname{GL}(2, \ZZ / 5 \ZZ)$. Then the modular curves generated by the product groups $B_{5} \times \operatorname{H}_{9}$, $B_{5} \times \operatorname{H}_{11}$, $B_{5} \times \operatorname{H}_{12}$, $B_{5} \times \operatorname{H}_{16}$, and $B_{5} \times \operatorname{H}_{18}$, are elliptic curves $\operatorname{X}$, such that the cardinality of $\operatorname{X}(\QQ)_{\text{tors}}$ is equal to the number of rational cusps on $\operatorname{X}$ (see Table \ref{Modular curves of genus 1} and Section \ref{Modular curves}).
    
    \item $R_{4}(6)$
    
    Let $B_{3} = \left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\} \subseteq \operatorname{GL}(2, \ZZ / 3 \ZZ)$. Then the modular curves generated by the product groups $B_{3} \times \operatorname{H}_{11}$, $B_{3} \times \operatorname{H}_{12}$, $B_{3} \times \operatorname{H}_{14}$, and $B_{3} \times \operatorname{H}_{18}$, are elliptic curves $\operatorname{X}$, such that the cardinality of $\operatorname{X}(\QQ)_{\text{tors}}$ is equal to the number of rational cusps on $\operatorname{X}$ (see Table \ref{Modular curves of genus 1} and Section \ref{Modular curves}).
\end{itemize}
\fi

\iffalse

\newpage


\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.5}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \# & $p$ & $\overline{\rho}_{E,p}(G_{\QQ})$ & $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ & $\textit{j}_{p}(E)$ & $\textit{j}_{2^{\infty}}(E)$ & $H$ & $l$ & $i$ & $g$ & LMFDB \\
    \hline
    \multirow{2}*{$1$} & \multirow{16}*{$5$} & \multirow{14}*{$\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$} & \multirow{2}*{$\operatorname{H}_{9}$} & \multirow{14}*{$\frac{\left(s^{2}+10s+5\right)^{3}}{s}$} & \multirow{2}*{$\frac{(t^{2}+48)^{3}}{t^{2}+64}$} & \multirow{2}*{$\begin{bmatrix} 1 & 1 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 13 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 11 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 10 & 1 \end{bmatrix}$} & \multirow{2}*{$20$} & \multirow{2}*{$36$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{20.36.1.3}} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$2$} & & & \multirow{2}*{$\operatorname{H}_{11}$} & & \multirow{2}*{$\frac{(t-4)^{3}(t+4)^{3}}{t^{2}}$} & \multirow{2}*{$\begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 13 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 9 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 13 \end{bmatrix}, \begin{bmatrix} 9 & 2 \\ 10 & 7 \end{bmatrix}$} & \multirow{2}*{$20$} & \multirow{2}*{$36$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{20.36.1.4}}\\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$3$} & & & \multirow{2}*{$\operatorname{H}_{12}$} & & \multirow{2}*{$\frac{(t^{2}+16)^{3}}{t^{2}}$} & \multirow{2}*{$\begin{bmatrix} 3 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 11 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 11 \end{bmatrix}, \begin{bmatrix} 11 & 1 \\ 10 & 1 \end{bmatrix}$} & \multirow{2}*{$20$} & \multirow{2}*{$36$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{20.36.1.2}} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$4$} & & & \multirow{2}*{$\operatorname{H}_{16}$} & & \multirow{2}*{$4 \cdot \frac{(t^{2}-24)^{3}}{t^{2}-32}$} & \multirow{2}*{$\begin{bmatrix} 1 & 1 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 31 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 33 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 11 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 31 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 10 & 1 \end{bmatrix}$} & \multirow{2}*{$40$} & \multirow{2}*{$36$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{40.36.1.1}}\\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$5$} & & & \multirow{2}*{$\operatorname{H}_{18}$} & & \multirow{2}*{$64 \cdot \frac{(t^{2}-2)^{3}}{t^{2}}$} &  \multirow{2}*{$\begin{bmatrix} 3 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 11 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 21 & 1 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 11 \end{bmatrix}, \begin{bmatrix} 1 & 31 \\ 0 & 31 \end{bmatrix}, \begin{bmatrix} 11 & 1 \\ 10 & 1 \end{bmatrix}$} & \multirow{2}*{$40$} & \multirow{2}*{$36$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{40.36.1.3}} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$6$} & & & \multirow{2}*{$\operatorname{H}_{23}$} & & \multirow{2}*{$-64 \cdot \frac{(t^{2}-3)^{3}(t^{2}+1)^{3}}{(t-1)^{4}(t+1)^{4}}$} & \multirow{2}*{$\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 13 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 11 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 10 & 1 \end{bmatrix}$} & \multirow{2}*{$20$} & \multirow{2}*{$72$} & \multirow{2}*{$3$} & \multirow{2}*{\texttt{20.72.3.6}} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$7$} & & & \multirow{2}*{$\operatorname{H}_{26}$} & & \multirow{2}*{$-64 \cdot \frac{(t-1)^{3}(t+1)^{3}(t^{2}+3)^{3}}{(t^{2}+1)^{4}}$} & \multirow{2}*{$\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 13 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 11 \end{bmatrix}, \begin{bmatrix} 11 & 1 \\ 10 & 1 \end{bmatrix}$} & \multirow{2}*{$20$} & \multirow{2}*{$72$} & \multirow{2}*{$3$} & \multirow{2}*{\texttt{20.72.3.3}} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{3-11}
    \multirow{2}*{$8$} & & \multirow{2}*{$\left\{\begin{bmatrix} 1 & \ast \\ 0 & \ast \end{bmatrix}\right\}$} & \multirow{2}*{$\operatorname{H}_{14}$} & \multirow{2}*{$\frac{(s^{4}-12s^{3}+14s^{2}+12s+1)^{3}}{s^{5}(s^{2}-11s-1)}$} & \multirow{2}*{$4 \cdot \frac{(t^{2}+8)^{3}}{t^{2}}$} & \multirow{2}*{$\begin{bmatrix} 31 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 11 & 1 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 3 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 1 & 11 \\ 0 & 11 \end{bmatrix}, \begin{bmatrix} 1 & 21 \\ 0 & 21 \end{bmatrix}, \begin{bmatrix} 11 & 1 \\ 10 & 1 \end{bmatrix}$} & \multirow{2}*{$40$} & \multirow{2}*{$144$} & \multirow{2}*{$3$} & \multirow{2}*{\texttt{40.72.3.27
'''}} \\
    & & & & & & & & & & \\
    \hline
    \multirow{2}*{$9$} & \multirow{18}*{$3$} & \multirow{14}*{$\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix}\right\}$} & \multirow{2}*{$\operatorname{H}_{11}$} & \multirow{18}*{$\frac{(s+3)^{3}(s+27)}{s}$} & \multirow{2}*{$\frac{(t-4)^{3}(t+4)^{3}}{t^{2}}$} & \multirow{2}*{$\begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 6 & 7 \end{bmatrix}$} & \multirow{2}*{$12$} & \multirow{2}*{$24$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{12.24.1.6}}\\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$10$} & & & \multirow{2}*{$\operatorname{H}_{12}$} & & \multirow{2}*{$\frac{(t^{2}+16)^{3}}{t^{2}}$} & \multirow{2}*{$\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 6 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 11 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 1 \\ 6 & 7 \end{bmatrix}$} & \multirow{2}*{$12$} & \multirow{2}*{$24$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{12.24.1.5}} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$11$} & & & \multirow{2}*{$\operatorname{H}_{14}$} & & \multirow{2}*{$4 \cdot \frac{(t^{2}+8)^{3}}{t^{2}}$} & \multirow{2}*{$\begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix}, \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 8 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 17 & 14 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 13 & 17 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 1 \\ 6 & 7 \end{bmatrix}$} & \multirow{2}*{$24$} & \multirow{2}*{$24$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{24.24.1.21}} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$12$} & & & \multirow{2}*{$\operatorname{H}_{18}$} & & \multirow{2}*{$64 \cdot \frac{(t^{2}-2)^{3}}{t^{2}}$} & \multirow{2}*{$\begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 7 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 19 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 6 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix}$} & \multirow{2}*{$24$} & \multirow{2}*{$24$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{24.24.1.22}} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$13$} & & & \multirow{2}*{$\operatorname{H}_{23}$} & & \multirow{2}*{$-64 \cdot \frac{(t^{2}-3)^{3}(t^{2}+1)^{3}}{(t-1)^{4}(t+1)^{4}}$} & \multirow{2}*{$\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 6 & 7 \end{bmatrix}$} & \multirow{2}*{$12$} & \multirow{2}*{$48$} & \multirow{2}*{$2$} & \multirow{2}*{\texttt{12.48.2.2}} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$14$} & & & \multirow{2}*{$\operatorname{H}_{26}$} & & \multirow{2}*{$-64 \cdot \frac{(t-1)^{3}(t+1)^{3}(t^{2}+3)^{3}}{(t^{2}+1)^{4}}$} & \multirow{2}*{$\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 11 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 1 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 2 \\ 6 & 11 \end{bmatrix}$} & \multirow{2}*{$12$} & \multirow{2}*{$48$} & \multirow{2}*{$2$} & \multirow{2}*{\texttt{12.48.2.1}}\\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$15$} & & & \multirow{2}*{$\operatorname{H}_{37}$} & & \multirow{2}*{$32 \cdot \frac{(448t^{4}+384t^{3}+176t^{2}+48t+7)^{3}}{(8t^{2}+4t+1)^{2}(8t^{2}+8t+1)^{4}}$} & \multirow{2}*{$\begin{bmatrix} 5 & 5 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 13 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 6 & 1 \end{bmatrix}$} & \multirow{2}*{$24$} & \multirow{2}*{$48$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{24.48.1.74}} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{3-4}
    \cline{6-11}
    \multirow{2}*{$16$} & & \multirow{4}*{$\left\{ \begin{bmatrix} 1 & \ast \\ 0 & \ast \end{bmatrix}\right\}$} & \multirow{2}*{$\operatorname{H}_{9a}$} & & \multirow{4}*{$\frac{(t^{2}+48)^{3}}{t^{2}+64}$} & \multirow{2}*{$\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 13 & 13 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 6 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 12 & 5 \end{bmatrix}$} & \multirow{2}*{$24$} & \multirow{2}*{$48$} & \multirow{2}*{$2$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{7-11}
    \multirow{2}*{$17$} & & & \multirow{2}*{$\operatorname{H}_{9b}$} & & & \multirow{2}*{$\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 13 & 6 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 6 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 6 & 11 \end{bmatrix}, \begin{bmatrix} 19 & 18 \\ 12 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 13 \\ 18 & 17 \end{bmatrix} $} & \multirow{2}*{$24$} & \multirow{2}*{$96$} & \multirow{2}*{$2$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
    \hline
    \end{tabular}}
\caption{product groups for $R_{4}$ graphs}
\label{product groups for R4 graphs}
\end{table}
\end{center}

\fi


\iffalse
$\operatorname{H}_{3a}$ Note that $\operatorname{H}_{3}$ is a group of level $4$. By Lemma \ref{lifting with kernel} and Lemma \ref{kernel of pi 2}, the full lift of $\operatorname{H}_{3}$ to level $32$ is conjugate to
$$\left\langle \begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 0 & 1 \\ 3 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix} , \begin{bmatrix} 1 & 0 \\ 4 & 1 \end{bmatrix} \right\rangle = \left\langle \begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 0 & 1 \\ 3 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix} \right\rangle \subseteq \operatorname{GL}(2, \ZZ / 32 \ZZ).$$
Thus, the quadratic twists of $\operatorname{H}_{3}$ are
\begin{center} $\operatorname{H}_{3}, \left\langle -\begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 0 & 1 \\ 3 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix} \right\rangle,
\left\langle \begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, -\begin{bmatrix} 0 & 1 \\ 3 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix} \right\rangle$, \end{center}

\begin{center}
$\left\langle \begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 0 & 1 \\ 3 & 1 \end{bmatrix}, -\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix} \right\rangle,
\left\langle -\begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, -\begin{bmatrix} 0 & 1 \\ 3 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix} \right\rangle, \left\langle -\begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 0 & 1 \\ 3 & 1 \end{bmatrix}, -\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix} \right\rangle$, \end{center}

\begin{center}
$\left\langle \begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, -\begin{bmatrix} 0 & 1 \\ 3 & 1 \end{bmatrix}, -\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix} \right\rangle,
\left\langle -\begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, -\begin{bmatrix} 0 & 1 \\ 3 & 1 \end{bmatrix}, -\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix} \right\rangle,
\left\langle \operatorname{H}_{3}, \operatorname{-Id} \right\rangle$
\end{center}
all of which are conjugate to one of three groups, $\operatorname{H}_{3}$, $\operatorname{H}_{3a} = \left\langle \begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, -\begin{bmatrix} 0 & 1 \\ 3 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix} \right\rangle$, and $\operatorname{H}_{3b} = \left\langle \begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 0 & 1 \\ 3 & 1 \end{bmatrix}, -\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix} \right\rangle$.
\fi

\iffalse
\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.48}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \# & $p$ & $\overline{\rho}_{E,p}(G_{\QQ})$ & $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ & $\textit{j}_{p}(E)$ & $\textit{j}_{2^{\infty}}(E)$ & $H$ & $l$ & $i$ & $g$ & LMFDB \\
    \hline
    \multirow{2}*{$1$} & \multirow{10}*{$13$} & \multirow{10}*{$\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$} & \multirow{2}*{$\operatorname{H}_{2}$} & \multirow{10}*{$\frac{(s^{2}+5s+13)(s^{4}+7s^{3}+20s^{2}+19s+1)^{3}}{s}$} & \multirow{2}*{$t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 3 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 2 & 1 \\ 13 & 1 \end{bmatrix}$} & \multirow{2}*{$26$} & \multirow{2}*{$28$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{26.28.1.1}} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$2$} & & & \multirow{2}*{$\operatorname{H}_{3}$} & & \multirow{2}*{$-t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 29 & 46 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix}, \begin{bmatrix} 4 & 1 \\ 39 & 1 \end{bmatrix}$} & \multirow{2}*{$52$} & \multirow{2}*{$28$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{52.28.1.1}} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$3$} & & & \multirow{2}*{$\operatorname{H}_{5}$} & & \multirow{2}*{$8t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 5 & 5 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 33 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 47 & 100 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 33 \end{bmatrix}, \begin{bmatrix} 8 & 1 \\ 65 & 1 \end{bmatrix} $} & \multirow{2}*{$104$} & \multirow{2}*{$28$} & \multirow{2}*{$1$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$4$} & & & \multirow{2}*{$\operatorname{H}_{7}$} & & \multirow{2}*{$\frac{32t-4}{t^{4}}$} & \multirow{2}*{$\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 47 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix}, \begin{bmatrix} 10 & 1 \\ 39 & 1 \end{bmatrix} $} & \multirow{2}*{$52$} & \multirow{2}*{$56$} & \multirow{2}*{$3$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$5$} & & & \multirow{2}*{$\operatorname{H}_{20}$} & & \multirow{2}*{$-4 \cdot \frac{(t^{2}-8t-11)(t^{2}-3)^{3}}{(t+1)^{4}}$} & \multirow{2}*{$\begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix}, \begin{bmatrix} 16 & 1 \\ 39 & 3 \end{bmatrix}, \begin{bmatrix} 9 & 9 \\ 39 & 36 \end{bmatrix}$} & \multirow{2}*{$52$} & \multirow{2}*{$112$} & \multirow{2}*{$7$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
    \hline
    \multirow{2}*{$6$} & \multirow{12}*{$7$} & \multirow{2}*{$\left\{ \begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$} & \multirow{2}*{$\operatorname{H}_{7}$} & \multirow{2}*{$\frac{(s^{2}+5s+1)^{3}(s^{2} + 13s + 49)}{s}$} & \multirow{2}*{$\frac{32t-4}{t^{4}}$} & \multirow{2}*{$\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 15 \end{bmatrix}, \begin{bmatrix} 10 & 21 \\ 7 & 1 \end{bmatrix}$} & \multirow{2}*{$28$} & \multirow{2}*{$32$} & \multirow{2}*{$2$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{3-11}
    \multirow{2}*{$7$} & & \multirow{10}*{$\left\{\begin{bmatrix} 1 & \ast \\ 0 & \ast \end{bmatrix} \right\}$} & \multirow{2}*{$\operatorname{H}_{2}$} & \multirow{10}*{$\frac{(s^{2}-s+1)^{3}(s^{6}-11s^{5}+30s^{4}-15s^{3}-10s^{2}+5s+1)^{3}}{(s-1)^{7}s^{7}(s^{3}-8s^{2}+5s+1)}$} & \multirow{2}*{$t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 8 & 11 \\ 7 & 1 \end{bmatrix}$} & \multirow{2}*{$14$} & \multirow{2}*{$96$} & \multirow{2}*{$2$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$8$} & & & \multirow{2}*{$\operatorname{H}_{3}$} & & \multirow{2}*{$-t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 15 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 6 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 8 & 9 \\ 7 & 1 \end{bmatrix}$} & \multirow{2}*{$28$} & \multirow{2}*{$96$} & \multirow{2}*{$2$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$9$} & & & \multirow{2}*{$\operatorname{H}_{4}$} & & \multirow{2}*{$-2t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 15 & 7 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 14 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 29 & 7 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 14 & 1 \end{bmatrix}, \begin{bmatrix} 29 & 0 \\ 49 & 1 \end{bmatrix} $} & \multirow{2}*{$56$} & \multirow{2}*{$96$} & \multirow{2}*{$2$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$10$} & & & \multirow{2}*{$\operatorname{H}_{5}$} & & \multirow{2}*{$8t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 29 & 5 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 15 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},  \begin{bmatrix} 8 & 1 \\ 49 & 1 \end{bmatrix}$} & \multirow{2}*{$56$} & \multirow{2}*{$96$} & \multirow{2}*{$2$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$11$} & & & \multirow{2}*{$\operatorname{H}_{20}$} & & \multirow{2}*{$-4 \cdot \frac{(t^{2}-8t-11)(t^{2}-3)^{3}}{(t+1)^{4}}$} & \multirow{2}*{$\begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 15 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 1 \\ 7 & 4 \end{bmatrix}$} & \multirow{2}*{$28$} & \multirow{2}*{$384$} & \multirow{2}*{$11$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
    \hline
    \multirow{2}*{$12$} & \multirow{14}*{$5$} & \multirow{12}*{$\left\{ \begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$} & \multirow{2}*{$\operatorname{H}_{2}$} & \multirow{12}*{$\frac{(s^{2}+10s+5)^{3}}{s}$} & \multirow{2}*{$t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 3 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 3 & 1 \\ 5 & 2 \end{bmatrix}$} & \multirow{2}*{$10$} & \multirow{2}*{$12$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{10.12.1.1}} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$13$} & & & \multirow{2}*{$\operatorname{H}_{3}$} & & \multirow{2}*{$-t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 13 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 17 & 6 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 13 \end{bmatrix}, \begin{bmatrix} 3 & 1 \\ 10 & 19 \end{bmatrix}, \begin{bmatrix} 4 & 1 \\ 15 & 1 \end{bmatrix}$} & \multirow{2}*{$20$} & \multirow{2}*{$12$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{20.12.1.1}} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$14$} & & & \multirow{2}*{$\operatorname{H}_{5}$} & & \multirow{2}*{$8t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 31 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 33 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 11 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 21 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 5 & 1 \end{bmatrix}$} & \multirow{2}*{$40$} & \multirow{2}*{$12$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{40.12.1.6}} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$15$} & & & \multirow{2}*{$\operatorname{H}_{20}$} & & \multirow{2}*{$-4 \cdot \frac{(t^{2}-8t-11)(t^{2}-3)^{3}}{(t+1)^{4}}$} & \multirow{2}*{$\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 13 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 11 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 5 & 1 \end{bmatrix}$} & \multirow{2}*{$20$} & \multirow{2}*{$48$} & \multirow{2}*{$3$} & \multirow{2}*{\texttt{20.48.3.2}} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$16$} & & & \multirow{2}*{$\operatorname{H}_{22}$} & & \multirow{2}*{$1728 \cdot \frac{(t^{2}-36t-162)(t^{2}+12t+30)^{3}}{(t^{2}-18)^{4}}$} & \multirow{2}*{$\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 33 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 31 & 31 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 31 & 35 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 11 \end{bmatrix}, \begin{bmatrix} 21 & 0 \\ 0 & 21 \end{bmatrix}, \begin{bmatrix} 31 & 0 \\ 5 & 1 \end{bmatrix}, \begin{bmatrix} 6 & 3 \\ 5 & 3 \end{bmatrix}$} & \multirow{2}*{$40$} & \multirow{2}*{$48$} & \multirow{2}*{$3$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{4-4}
    \cline{6-11}
    \multirow{2}*{$17$} & & & \multirow{2}*{$\operatorname{H}_{55}$} & & \multirow{2}*{$-2^{15} \cdot \frac{(2t-1)(2t^{2}-2t+1)^{3}(2t^{2}+2t-1)^{3}}{(2t^{2}-1)^{8}}$} & \multirow{2}*{$\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 33 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 31 & 35 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 23 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 11 \end{bmatrix}, \begin{bmatrix} 21 & 0 \\ 0 & 21 \end{bmatrix}, \begin{bmatrix} 8 & 15 \\ 5 & 1 \end{bmatrix}, \begin{bmatrix} 26 & 15 \\ 5 & 3 \end{bmatrix} $} & \multirow{2}*{$40$} & \multirow{2}*{$96$} & \multirow{2}*{$5$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{3-11}
    \multirow{2}*{$18$} & & \multirow{2}*{$\left\{ \begin{bmatrix} 1 & \ast \\ 0 & \ast \end{bmatrix} \right\}$} & \multirow{2}*{$\operatorname{H}_{7}$} & \multirow{2}*{$\frac{(s^{4}-12s^{3}+14s^{2}+12+1)^{3}}{s^{5}(s^{2}-11s-1)}$} & \multirow{2}*{$\frac{32t-4}{t^{4}}$} & \multirow{2}*{$\begin{bmatrix} 11 & 11 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 11 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 11 & 0 \\ 0 & 11 \end{bmatrix}, \begin{bmatrix} 11 & 0 \\ 5 & 1 \end{bmatrix}, \begin{bmatrix} 6 & 3 \\ 5 & 3 \end{bmatrix}$} & \multirow{2}*{$20$} & \multirow{2}*{$96$} & \multirow{2}*{$3$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
    \hline
    \multirow{2}*{$19$} & \multirow{4}*{$3$} & \multirow{2}*{$\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$} & \multirow{2}*{$\operatorname{H}_{7}$} & \multirow{4}*{$\frac{(s+3)^{3}(s+27)}{s}$} & \multirow{2}*{$\frac{32t-4}{t^{4}}$} & \multirow{2}*{$\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 7 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 7 & 2 \\ 3 & 1 \end{bmatrix}$} & \multirow{2}*{$12$} & \multirow{2}*{$16$} & \multirow{2}*{$1$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
    \cline{1-1}
    \cline{3-4}
    \cline{6-11}
    \multirow{2}*{$20$} & & \multirow{2}*{$\left\{\begin{bmatrix} 1 & \ast \\ 0 & \ast \end{bmatrix} \right\}$} & \multirow{2}*{$\operatorname{H}_{20a}$} & & \multirow{2}*{$-4 \cdot \frac{(t^{2}-8t-11)(t^{2}-3)^{3}}{(t+1)^{4}}$} & \multirow{2}*{$\begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 7 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 13 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 19 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 13 & 0 \\ 0 & 13 \end{bmatrix}, \begin{bmatrix} 13 & 13 \\ 3 & 4 \end{bmatrix}$} & \multirow{2}*{$24$} & \multirow{2}*{$128$} & \multirow{2}*{$1$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
    \hline
    \end{tabular}}
\caption{product groups for $L_{2}$ graphs}
\label{product groups for L2 graphs}
\end{table}
\end{center}
\fi

\iffalse
\begin{lemma}\label{H4 lemma}
Let $E/\QQ$ be a non-CM elliptic curve such that $\rho_{E,2^{\infty}}(G_{\QQ})$ is conjugate to the full lift of $\operatorname{H}_{4}$. Let $E^{\chi}$ be a quadratic twist of $E$. Then $\rho_{E^{\chi},2^{\infty}}(G_{\QQ})$ is conjugate to $\operatorname{H}_{4}$.
\end{lemma}

\begin{proof}
Note that $\operatorname{H}_{4} = \left\langle
\begin{bmatrix} 7 & 7 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 1 & 1 \end{bmatrix}
\right\rangle$ is a group of level $8$. By Lemma \ref{lifting with kernel} and Lemma \ref{kernel of pi 1}, $\overline{\rho}_{E,32}(G_{\QQ})$ is conjugate to
$$\widehat{H} = \left\langle
\begin{bmatrix} 7 & 7 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 1 & 1 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}
\right\rangle = \left\langle
\begin{bmatrix} 7 & 7 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 1 & 1 \end{bmatrix}
\right\rangle \subseteq \operatorname{GL}(2, \ZZ / 32 \ZZ).$$
Thus, the quadratic twists of $\widehat{H}$ are
\begin{center}
    $\widehat{H}$, $\left\langle
-\begin{bmatrix} 7 & 7 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 1 & 1 \end{bmatrix}
\right\rangle$, $\left\langle
\begin{bmatrix} 7 & 7 \\ 0 & 1 \end{bmatrix},
-\begin{bmatrix} 5 & 0 \\ 1 & 1 \end{bmatrix}
\right\rangle$, $\left\langle
-\begin{bmatrix} 7 & 7 \\ 0 & 1 \end{bmatrix},
-\begin{bmatrix} 5 & 0 \\ 1 & 1 \end{bmatrix}
\right\rangle$, and $\left\langle \widehat{H}, \operatorname{-Id} \right\rangle$.
\end{center}
A computation using Magma \cite{magma} reveals that all five groups are conjugate in $\operatorname{GL}(2, \ZZ / 32 \ZZ)$ to $\widehat{H}$.
\end{proof}
\fi

\iffalse
\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.62}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \# & $\overline{\rho}_{E,3}(G_{\QQ})$ & $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ & $\textit{j}_{3}(E)$ & $\textit{j}_{2^{\infty}}(E)$ & $H$ & $l$ & $i$ & $g$ & LMFDB \\
    \hline
    \multirow{4}*{$1$} & \multirow{8}*{$\left\{ \begin{bmatrix} \ast & 0 \\ 0 & \ast \end{bmatrix} \right\}$} & \multirow{4}*{$\operatorname{H}_{9}$} & \multirow{8}*{$27 \cdot \frac{(s+1)^{3}(s+3)^{3}(s^{2}+3)^{3}}{s^{3}(s^{2}+3s+3)^{3}}$} & \multirow{4}*{$\frac{(t^{2}+48)^{3}}{t^{2}+64}$} & \multirow{4}*{$\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 6 & 1 \end{bmatrix}$} & \multirow{4}*{$12$} & \multirow{4}*{$72$} & \multirow{4}*{$1$} & \multirow{4}*{\texttt{12.72.1.2}}\\
    & & & & & & & & & \\
    & & & & & & & & & \\
    & & & & & & & & & \\
    \cline{1-1}
    \cline{3-3}
    \cline{5-10}
    \multirow{4}*{$2$} & & \multirow{4}*{$\operatorname{H}_{15}$} & & \multirow{4}*{$64 \cdot \frac{(t^{2}+6)^{3}}{t^{2}+8}$} & \multirow{4}*{$\begin{bmatrix} 19 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 11 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 13 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 6 & 1 \end{bmatrix}$} & \multirow{4}*{$24$} & \multirow{4}*{$72$} & \multirow{4}*{$1$} & \multirow{4}*{---} \\
    & & & & & & & & & \\
    & & & & & & & & & \\
    & & & & & & & & & \\
    \hline
    \end{tabular}}
\caption{product groups for $R_{6}$ graphs}
\label{product groups for R6 graphs}
\end{table}
\end{center}
\fi

\iffalse

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.5}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \# & $p$ & $\overline{\rho}_{E,p}(G_{\QQ})$ & $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ & $\textit{j}_{p}(E)$ & $\textit{j}_{2^{\infty}}(E)$ & $H$ & $l$ & $i$ & $g$ & LMFDB \\
    \hline
    \multirow{2}*{$1$} & \multirow{4}*{$5$} & \multirow{4}*{$\left\{\begin{bmatrix} \ast & 0 \\ 0 & \ast \end{bmatrix} \right\}$} & \multirow{2}*{$\operatorname{H}_{4}$} & \multirow{4}*{$\frac{(s^{2}+5s+5)^{3}(s^{4}+5s^{2}+25)^{3}(s^{4}+5s^{3}+20s^{2}+25s+25)^{3}}{s^{5}(s^{4}+5s^{3}+15s^{2}+25s+25)^{5}}$} & \multirow{2}*{$-2t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 3 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 11 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 21 & 25 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 11 \end{bmatrix}, \begin{bmatrix} 21 & 0 \\ 0 & 21 \end{bmatrix}, \begin{bmatrix} 21 & 0 \\ 5 & 1 \end{bmatrix}$} & \multirow{2}*{$40$} & \multirow{2}*{$60$} & \multirow{2}*{$3$} & \multirow{2}*{---} \\
    & & & & & & & & & & \\
\cline{1-1}
\cline{4-4}
\cline{6-11}
    \multirow{2}*{$2$} & & & \multirow{2}*{$\operatorname{H}_{7}$} & & \multirow{2}*{$\frac{32t-4}{t^{4}}$} & \multirow{2}*{$\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 13 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 15 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 11 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 5 & 1 \end{bmatrix}, \begin{bmatrix} 18 & 5 \\ 15 & 1 \end{bmatrix}$} & \multirow{2}*{$20$} & \multirow{2}*{$120$} & \multirow{2}*{$7$} & \multirow{2}*{\texttt{20.120.7.7}} \\
    & & & & & & & & & & \\
    \hline
    \multirow{2}*{$3$} & \multirow{10}*{$3$} & \multirow{10}*{$\left\{ \begin{bmatrix} \ast & 0 \\ 0 & \ast \end{bmatrix} \right\}$} & \multirow{2}*{$\operatorname{H}_{2}$} & \multirow{10}*{$27 \cdot \frac{(s+1)^{3}(s+3)^{3}(s^{2}+3)^{3}}{s^{3}(s^{2}+3s+3)^{3}}$} & \multirow{2}*{$t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 2 & 3 \\ 3 & 1 \end{bmatrix}$} & \multirow{2}*{$6$} & \multirow{2}*{$24$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{6.24.1.2}} \\
    & & & & & & & & & & \\
\cline{1-1}
\cline{4-4}
\cline{6-11}
    \multirow{2}*{$4$} & & & \multirow{2}*{$\operatorname{H}_{3}$} & & \multirow{2}*{$-t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 9 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 3 & 1 \end{bmatrix}$} & \multirow{2}*{$12$} & \multirow{2}*{$24$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{12.24.1.3}} \\
    & & & & & & & & & & \\
\cline{1-1}
\cline{4-4}
\cline{6-11}
\multirow{2}*{$5$} & & & \multirow{2}*{$\operatorname{H}_{4}$} & & \multirow{2}*{$-2t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 19 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 11 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 15 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 13 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 3 & 1 \end{bmatrix}$} & \multirow{2}*{$24$} & \multirow{2}*{$24$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{24.24.1.1}} \\
& & & & & & & & & & \\
\cline{1-1}
\cline{4-4}
\cline{6-11}
\multirow{2}*{$6$} & & & \multirow{2}*{$\operatorname{H}_{5}$} & & \multirow{2}*{$8t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 7 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 15 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 13 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 3 & 1 \end{bmatrix}$} & \multirow{2}*{$24$} & \multirow{2}*{$24$} & \multirow{2}*{$1$} & \multirow{2}*{\texttt{24.24.1.2}} \\
& & & & & & & & & & \\
\cline{1-1}
\cline{4-4}
\cline{6-11}
\multirow{2}*{$7$} & & & \multirow{2}*{$\operatorname{H}_{20}$} & & \multirow{2}*{$-4 \cdot \frac{(s^{2}-8s-11)(s^{2}-3)^{3}}{(s+1)^{4}}$} & \multirow{2}*{$\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 9 & 1 \end{bmatrix}$} & \multirow{2}*{$12$} & \multirow{2}*{$96$} & \multirow{2}*{$5$} & \multirow{2}*{\texttt{12.96.5.3}} \\
& & & & & & & & & & \\
\hline
    \end{tabular}}
\caption{product groups for $L_{3}$ graphs}
\label{product groups for L3 Graphs}
\end{table}
\end{center}

\fi

\iffalse

\begin{remark}
The intersection $\operatorname{X}$ of the modular curve generated by the split Cartan group modulo $3$, $\left\{\begin{bmatrix} \ast & 0 \\ 0 & \ast \end{bmatrix} \right\} \subseteq \operatorname{GL}(2, \ZZ / 3 \ZZ)$ and the subgroup $\operatorname{H}_{5}$ of $\operatorname{GL}(2, \ZZ / 8 \ZZ)$ is a curve of genus $1$ and rank $1$. The elliptic curve with LMFDB label \texttt{576a3} is isomorphic to $\operatorname{X}$. Moreover, the elliptic curve $\operatorname{576a3}$ has CM by $-3$.

We will investigate the modular curves $C$ from Table \ref{Modular curves of genus 1} of rank $0$ such that the number of $\QQ$-rational cusps is less than the order of $C(\mathbb{Q})_{\text{tors}}$.

\begin{itemize}

\item $\operatorname{H}_{11}$ and $\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}_{3}$

Let $C$ be the modular curve with LMFDB label \texttt{12.24.1.6}. Then $C$ has a plane model
$$C : x^{3}-x^{2}z-24xz^{2}+y^{2}z-36z^{3} = 0$$
with $\textit{j}$-map
$$\textit{j} = 1728 + \frac{(x^{2} - 12z^{2})^{2}  (x^{4} - 24x^{2}z^{2} - 72xz^{3} - 72z^{4})^{2}}{(x - 6z)  (x + 3z)^{2}  (x + 2z)^{3}  z^{6}}.$$
Using Magma, we see that $C$ is isomorphic to the elliptic curve with LMFDB label \texttt{48.a3}. Moreover, $C$ has eight points defined over $\QQ$, namely,
$$(x,y,z) = (-6,12,1), (6,0,1), (0,-6,1), (0,1,0), (-3,0,1), (0,6,1), (-6,-12,1), (-2,0,1).$$
The \textit{j}-invariant corresponding to those points are, respectively,
$$54000, \infty, 0, \infty, \infty, 0, 54000, \infty.$$
Thus, if $E/\QQ$ is a non-CM elliptic curve with a $\QQ$-rational subgroup of order $3$, then $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is not conjugate to a subgroup of $\operatorname{H}_{11}$.

\item $\operatorname{H}_{7}$ and $\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix}\right\}_{5}$

Let $C$ be the modular curve with LMFDB label \texttt{20.24.1.1}. Then $C$ has the plane model
$$C : 4x^{3}z-20x^{2}z^{2}-32xyz^{2}-80xz^{3}+y^{4}+160yz^{3}+400z^{4} = 0$$
with \textit{j}-map
$$\textit{j} = \frac{(x^{2} - 20z^{2})^{3}}{(x - 5z)z^{5}}.$$
Using Magma, we see that $C$ is isomorphic to the elliptic curve with LMFDB label \texttt{80.a4}. Moreover, $C$ has four points defined over $\QQ$, namely,
$$\left(-\frac{5}{4}, -\frac{5}{2}, 1\right), \left(-15, 10, 1\right), \left(1,0,0\right), \left(5,0,1\right).$$
The \textit{j}-invariant corresponding to these points are, respectively,
$$\frac{1026895}{1024}, -\frac{1723025}{4}, \infty, \infty.$$
Both of the rational \textit{j}-invariants correspond to elliptic curves over $\QQ$ in the $\QQ$-isogeny class with LMFDB label \texttt{14450.h}.

\item $\operatorname{H}_{7}$ and $\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix}\right\}_{3}$

Let $C$ be the modular curve with LMFDB label \texttt{12.16.1.1}. Then $C$ has the plane model
$$C : x^{2}z^{2}+2xy^{2}z+8xyz^{2}+30xz^{3}+y^{4}-6y^{2}z^{2}-24yz^{3}-99z^{4} = 0$$
with \textit{j}-map
$$\textit{j} = \frac{(x+24z)x^{3}}{(x-3z)z^{3}}.$$
Using Magma, we see that $C$ is isomorphic to the elliptic curve with LMFDB label \texttt{48.a6}. Moreover, $C$ has eight points defined over $\QQ$, namely,
$$(-24,9,1), \left(-\frac{69}{4},-\frac{9}{2}, 1 \right), (-24,-3,1), (1,0,0), (0,-3,1), (3,0,1), (-240,9,1), (-33,0,1).$$
The \textit{j}-invariant corresponding to these points are, respectively,
$$0, \frac{109503}{64}, 0, \infty, 0, \infty, -12288000, -\frac{35937}{4}.$$
The \textit{j}-invariants, $\frac{109503}{64}$ and $-\frac{35937}{4}$ correspond to elliptic curves over $\QQ$ in the $\QQ$-isogeny class with LMFDB label \texttt{162.a}. The \textit{j}-invariants $0$ and $-12288000$ correspond to elliptic curves over $\QQ$ with CM.
\end{itemize}

\end{remark}

\newpage

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.45}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \# & graph & $p$ & $\overline{\rho}_{E,p}(G_{\QQ})$ & $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ & $\textit{j}_{p}(E)$ & $\textit{j}_{2^{\infty}}(E)$ & $H$ & $g$ & \#$\operatorname{X}_{\operatorname{H}}(\QQ)$ & \# $\QQ$-cusps & LMFDB \\
    \hline
    \multirow{2}*{$1$} & \multirow{4}*{$S$} & \multirow{4}*{$3$} & \multirow{4}*{$\left\{\begin{bmatrix} 1 & \ast \\ 0 & \ast \end{bmatrix}\right\}$} & \multirow{2}*{$\operatorname{H}_{8a}$} & \multirow{4}*{$\frac{(s+3)^{3}(s+27)}{s}$} & \multirow{4}*{$64 \cdot \frac{(t^{2}+3)^{3}}{(t-1)^{2}(t+1)^{2}}$} & \multirow{2}*{$\begin{bmatrix} 19 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 0 & 13 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 6 & 1 \end{bmatrix}$} & \multirow{2}*{$2$} & \multirow{2}*{---} & \multirow{2}*{$6$} & \multirow{2}*{\texttt{24.96.2.3}} \\
    & & & & & & & & & & & \\
    \cline{1-1}
    \cline{5-5}
    \cline{8-12}
    \multirow{2}*{$2$} & & & & \multirow{2}*{$\operatorname{H}_{8b}$} & & & \multirow{2}*{$\begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 6 & 1 \end{bmatrix}$} & \multirow{2}*{$2$} & \multirow{2}*{---} & \multirow{2}*{$6$} & \multirow{2}*{\texttt{12.96.2.1}} \\
    & & & & & & & & & & & \\
    \hline
    \multirow{2}*{$3$} & \multirow{6}*{$R_{4}(2p)$} & \multirow{2}*{$5$} & \multirow{6}*{$\left\{\begin{bmatrix} 1 & \ast \\ 0 & \ast \end{bmatrix}\right\}$} & \multirow{2}*{$\operatorname{H}_{14}$} & \multirow{2}*{$\frac{(s^{4}-12s^{3}+14s^{2}+12s+1)^{3}}{s^{5}(s^{2}-11s-1)}$} & \multirow{2}*{$4 \cdot \frac{(t^{2}+8)^{3}}{t^{2}}$} & \multirow{2}*{$\begin{bmatrix} 31 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 11 & 1 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 3 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 1 & 11 \\ 0 & 11 \end{bmatrix}, \begin{bmatrix} 1 & 21 \\ 0 & 21 \end{bmatrix}, \begin{bmatrix} 11 & 1 \\ 10 & 1 \end{bmatrix}$} & \multirow{2}*{$3$} & \multirow{2}*{---} & \multirow{2}*{$4$} & \multirow{2}*{\texttt{40.144.3.87}} \\
    & & & & & & & & & & & \\
    \cline{1-1}
    \cline{3-3}
    \cline{5-12}
    \multirow{2}*{$4$} & & \multirow{4}*{$3$} & & \multirow{2}*{$\operatorname{H}_{9a}$} & \multirow{4}*{$\frac{(s+3)^{3}(s+27)}{s}$} & \multirow{4}*{$\frac{(t^{2}+48)^{3}}{t^{2}+64}$} & \multirow{2}*{$\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 13 & 13 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 6 & 11 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 12 & 5 \end{bmatrix}$} & \multirow{2}*{$2$} & \multirow{2}*{---} & \multirow{2}*{$2$} & \multirow{2}*{\texttt{24.96.2.100}} \\
    & & & & & & & & & & & \\
    \cline{1-1}
    \cline{5-5}
    \cline{8-12}
    \multirow{2}*{$5$} & & & & \multirow{2}*{$\operatorname{H}_{9b}$} & & & \multirow{2}*{$\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 13 & 6 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 6 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 6 & 11 \end{bmatrix}, \begin{bmatrix} 19 & 18 \\ 12 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 13 \\ 18 & 17 \end{bmatrix} $} & \multirow{2}*{$2$} & \multirow{2}*{---} & \multirow{2}*{$2$} & \multirow{2}*{\texttt{24.96.2.99}} \\
    & & & & & & & & & & & \\
    \hline
    \multirow{2}*{$6$} & \multirow{12}*{$L_{2}(p)$} & \multirow{2}*{$13$} & \multirow{4}*{$\left\{ \begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$} & \multirow{4}*{$\operatorname{H}_{7}$} & \multirow{2}*{$\frac{(s^{2}+5s+13)(s^{4}+7s^{3}+20s^{2}+19s+1)^{3}}{s}$} & \multirow{4}*{$\frac{32t-4}{t^{4}}$} & \multirow{2}*{$\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 47 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix}, \begin{bmatrix} 10 & 1 \\ 39 & 1 \end{bmatrix}$} & \multirow{2}*{$3$} & \multirow{2}*{---} & \multirow{2}*{$2$} & \multirow{2}*{\texttt{52.56.3.1}} \\
    & & & & & & & & & & & \\
    \cline{1-1}
    \cline{3-3}
    \cline{6-6}
    \cline{8-12}
    \multirow{2}*{$7$} & & \multirow{2}*{$7$} & & & \multirow{2}*{$\frac{(s^{2}+5s+1)^{3}(s^{2} + 13s + 49)}{s}$} & & \multirow{2}*{$\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 15 \end{bmatrix}, \begin{bmatrix} 10 & 21 \\ 7 & 1 \end{bmatrix}$} & \multirow{2}*{$2$} & \multirow{2}*{---} & \multirow{2}*{$2$} & \multirow{2}*{\texttt{28.32.2.1}} \\
    & & & & & & & & & & & \\
    \cline{1-1}
    \cline{3-12}
    \multirow{2}*{$8$} & & \multirow{8}*{$7$} & \multirow{8}*{$\left\{\begin{bmatrix} 1 & \ast \\ 0 & \ast \end{bmatrix} \right\}$} & \multirow{2}*{$\operatorname{H}_{2}$} & \multirow{8}*{$\frac{(s^{2}-s+1)^{3}(s^{6}-11s^{5}+30s^{4}-15s^{3}-10s^{2}+5s+1)^{3}}{(s-1)^{7}s^{7}(s^{3}-8s^{2}+5s+1)}$} & \multirow{2}*{$t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 8 & 11 \\ 7 & 1 \end{bmatrix}$} & \multirow{2}*{$2$} & \multirow{2}*{---} & \multirow{2}*{$3$} & \multirow{2}*{\texttt{14.96.2.1}} \\
    & & & & & & & & & & & \\
    \cline{1-1}
    \cline{5-5}
    \cline{7-12}
    \multirow{2}*{$9$} & & & & \multirow{2}*{$\operatorname{H}_{3}$} & & \multirow{2}*{$-t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 15 & 3 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 6 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 8 & 9 \\ 7 & 1 \end{bmatrix}$} & \multirow{2}*{$2$} & \multirow{2}*{---} & \multirow{2}*{$3$} & \multirow{2}*{\texttt{28.96.2.7}} \\
    & & & & & & & & & & & \\
    \cline{1-1}
    \cline{5-5}
    \cline{7-12}
    \multirow{2}*{$10$} & & & & \multirow{2}*{$\operatorname{H}_{4}$} & & \multirow{2}*{$-2t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 15 & 7 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 14 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 29 & 7 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 14 & 1 \end{bmatrix}, \begin{bmatrix} 29 & 0 \\ 49 & 1 \end{bmatrix} $} & \multirow{2}*{$2$} & \multirow{2}*{---} & \multirow{2}*{$3$} & \multirow{2}*{\texttt{56.96.2.6}}\\
    & & & & & & & & & & & \\
    \cline{1-1}
    \cline{5-5}
    \cline{7-12}
    \multirow{2}*{$11$} & & & & \multirow{2}*{$\operatorname{H}_{5}$} & & \multirow{2}*{$8t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 29 & 5 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 15 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},  \begin{bmatrix} 8 & 1 \\ 49 & 1 \end{bmatrix}$} & \multirow{2}*{$2$} & \multirow{2}*{---} & \multirow{2}*{$3$} & \multirow{2}*{\texttt{56.96.2.3}} \\
    & & & & & & & & & & & \\
    \hline
    \multirow{2}*{$12$} & \multirow{2}*{$L_{2}(p^{2})$} & \multirow{2}*{$5$} & \multirow{2}*{$\left\{\begin{bmatrix} \ast & 0 \\ 0 & \ast \end{bmatrix} \right\}$} & \multirow{2}*{$\operatorname{H}_{4}$} & \multirow{2}*{$\frac{(s^{2}+5s+5)^{3}(s^{4}+5s^{2}+25)^{3}(s^{4}+5s^{3}+20s^{2}+25s+25)^{3}}{s^{5}(s^{4}+5s^{3}+15s^{2}+25s+25)^{5}}$} & \multirow{2}*{$-2t^{2}+1728$} & \multirow{2}*{$\begin{bmatrix} 3 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 11 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 21 & 25 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 11 \end{bmatrix}, \begin{bmatrix} 21 & 0 \\ 0 & 21 \end{bmatrix}, \begin{bmatrix} 21 & 0 \\ 5 & 1 \end{bmatrix}$} & \multirow{2}*{$3$} & \multirow{2}*{---} & \multirow{2}*{$2$} & \multirow{2}*{\texttt{40.60.3.1}} \\
    & & & & & & & & & & & \\
\hline
    \end{tabular}}
\caption{Modular curves of higher genus}
\label{Modular curves of higher genus}
\end{table}
\end{center}

\begin{itemize}

\item Curves of genus $2$

Let $E/\QQ$ be an elliptic curve with \textit{j}-invariant equal to $\frac{-38575685889}{16384}$ or $\frac{351}{4}$. Then $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to a subgroup of $\operatorname{H}_{20}$ of index $1$ or $2$ and $\overline{\rho}_{E,7}(G_{\QQ})$ is conjugate to $B_{7} = \left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix}\right\}$. Let $C$ be the curve that parametrizes non-CM elliptic curves $E/\QQ$ such that $E$ has a $\QQ$-rational subgroup of order $7$ and $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to a subgroup of $\operatorname{H}_{7}$. Then by the RSVZB code, $C$ has two $\QQ$-rational cusps. We claim that $C(\QQ)$ has four points. Note that $C$ is a hyperelliptic curve of genus $2$ and the Jacobian $J$ of the hyperelliptic curve that $C$ is isomorphic to is of rank $1$. Using Chabauty's method on a point on $J$ of infinite order, we see that $C(\QQ)$ has four total points, two of which are cusps by RSVZB code, and the other two correspond to elliptic curves over $\QQ$ with \textit{j}-invariant equal to $\frac{-38575685889}{16384}$ or $\frac{351}{4}$.

Let $C$ be the curve that parametrizes non-CM elliptic curves $E / \QQ$ such that $\overline{\rho}_{E,7}(G_{\QQ})$ is conjugate to a subgroup of $\left\{\begin{bmatrix} \pm 1 & \ast \\ 0 & \ast \end{bmatrix} \right\}$ and $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to $\operatorname{H}_{2}$, $\operatorname{H}_{3}$, $\operatorname{H}_{4}$, or $\operatorname{H}_{5}$. Then $C$ is a curve of genus $2$ with a Jacobian of rank $0$. Using Chabauty's method (using the command Chabauty0 on the Jacobian of the hyperelliptic curve that $C$ is isomorphic to), we determine that $C$ contains three points defined over $\QQ$. Code by RSVZB determines that all three points are cusps.

\item Curves of genus $3$
\end{itemize}
\fi


\newpage

\iffalse
\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.33}{
    \begin{tabular}{|c|c|c|c|c|}
\hline
Isogeny Graph & Isogeny-Torsion Graph & $E_{1}$ & $E_{2}$ & Example Isogeny Class \\
\hline
\multirow{86}*{\includegraphics[scale=0.1]{L22 graph.png}} & \multirow{86}*{$([2],[2])$} & $\operatorname{H}_{26}$ & $\operatorname{H}_{28}$ & \texttt{468.e} \\
\cline{3-5}
& & $\operatorname{H}_{73}$ & $\operatorname{H}_{90}$ & \texttt{16940.b} \\
\cline{3-5}
& & $\operatorname{H}_{68}$ & $\operatorname{H}_{74}$ & \texttt{16810.c} \\
\cline{3-5}
& & $\operatorname{H}_{81}$ & $\operatorname{H}_{83}$ & \texttt{202496.e} \\
\cline{3-5}
& & $\operatorname{H}_{220}$ & $\operatorname{H}_{232}$ & \texttt{4352.f} \\
\cline{3-5}
& & $\operatorname{H}_{218}$ & $\operatorname{H}_{237}$ & \texttt{147712.d} \\
\cline{3-5}
& & $\operatorname{H}_{281}$ & $\operatorname{H}_{349}$ & \texttt{122740.j} \\
\cline{3-5}
& & $\operatorname{H}_{350}$ & $\operatorname{H}_{284}$ & $y^2 = x^3 - 1725814293280x + 872648220992027997$ \\
\cline{3-5}
& & $\operatorname{H}_{9b}$ & $\operatorname{H}_{10b}$ & \texttt{1600.t} \\
\cline{3-5}
& & $\operatorname{H}_{37b}$ & $\operatorname{H}_{42b}$ & \texttt{640.g} \\
\cline{3-5}
& & $\operatorname{H}_{108e}$ & $\operatorname{H}_{123f}$ & \texttt{1664.e} \\
\cline{3-5}
& & $\operatorname{H}_{108f}$ & $\operatorname{H}_{123b}$ & \texttt{1664.r} \\
\cline{3-5}
& & $\operatorname{H}_{238b}$ & $\operatorname{H}_{239a}$ & \texttt{128.d} \\
\cline{3-5}
& & $\operatorname{H}_{238c}$ & $\operatorname{H}_{239d}$ & \texttt{128.b} \\
\cline{3-5}
& & $\operatorname{H}_{9d}$ & $\operatorname{H}_{10d}$ & \texttt{136.a} \\
\cline{3-5}
& & $\operatorname{H}_{37d}$ & $\operatorname{H}_{42d}$ & \texttt{640.h} \\
\cline{3-5}
& & $\operatorname{H}_{108b}$ & $\operatorname{H}_{123d}$ & \texttt{1664.o} \\
\cline{3-5}
& & $\operatorname{H}_{108d}$ & $\operatorname{H}_{123c}$ & \texttt{1664.d} \\
\cline{3-5}
& & $\operatorname{H}_{238a}$ & $\operatorname{H}_{239b}$ & \texttt{128.c} \\
\cline{3-5}
& & $\operatorname{H}_{238d}$ & $\operatorname{H}_{239c}$ & \texttt{128.a} \\
\cline{3-5}
& & $\operatorname{H}_{23}$ & $\operatorname{H}_{43}$ & \texttt{1176.b} \\
\cline{3-5}
& & $\operatorname{H}_{64}$ & $\operatorname{H}_{64}$ & \texttt{424830.dp} \\
\cline{3-5}
& & $\operatorname{H}_{65}$ & $\operatorname{H}_{71}$ & \texttt{867.a} \\
\cline{3-5}
& & $\operatorname{H}_{68}$ & $\operatorname{H}_{74}$ & \texttt{16810.c} \\
\cline{3-5}
& & $\operatorname{H}_{69}$ & $\operatorname{H}_{91}$ & \texttt{11109.g} \\
\cline{3-5}
& & $\operatorname{H}_{76}$ & $\operatorname{H}_{82}$ & \texttt{19200.a} \\
\cline{3-5}
& & $\operatorname{H}_{77}$ & $\operatorname{H}_{80}$ & \texttt{5376.c} \\
\cline{3-5}
& & $\operatorname{H}_{191}$ & $\operatorname{H}_{196}$ & \texttt{294.b} \\
\cline{3-5}
& & $\operatorname{H}_{216}$ & $\operatorname{H}_{224}$ & \texttt{13056.e} \\
\cline{3-5}
& & $\operatorname{H}_{318}$ & $\operatorname{H}_{328}$ & \texttt{76614.h} \\
\cline{3-5}
& & $\operatorname{H}_{289}$ & $\operatorname{H}_{320}$ & \texttt{4046.n} \\
\cline{3-5}
& & $\operatorname{H}_{619}$ & $\operatorname{H}_{649}$ & \texttt{17918.c} \\
\cline{3-5}
& & $\operatorname{H}_{76a}$ & $\operatorname{H}_{82b}$ & \texttt{2304.k} \\
\cline{3-5}
& & $\operatorname{H}_{76b}$ & $\operatorname{H}_{82c}$ & \texttt{768.b} \\
\cline{3-5}
& & $\operatorname{H}_{76c}$ & $\operatorname{H}_{82d}$ & \texttt{2304.f} \\
\cline{3-5}
& & $\operatorname{H}_{76d}$ & $\operatorname{H}_{82a}$ & \texttt{768.g} \\
\cline{3-5}
& & $\operatorname{H}_{6}$ & $\operatorname{H}_{6}$ & \texttt{69.a} \\
\cline{3-5}
& & $\operatorname{H}_{14}$ & $\operatorname{H}_{14}$ & \texttt{1152.n} \\
\cline{3-5}
& & $\operatorname{H}_{15}$ & $\operatorname{H}_{19}$ & \texttt{102.a} \\
\cline{3-5}
& & $\operatorname{H}_{16}$ & $\operatorname{H}_{17}$ & \texttt{46.a} \\
\cline{3-5}
& & $\operatorname{H}_{18}$ & $\operatorname{H}_{18}$ & \texttt{490.f} \\
\cline{3-5}
& & $\operatorname{H}_{12}$ & $\operatorname{H}_{12}$ & \texttt{2200.i} \\
\cline{3-5}
& & $\operatorname{H}_{30}$ & $\operatorname{H}_{30}$ & \texttt{63075.t} \\
\cline{3-5}
& & $\operatorname{H}_{31}$ & $\operatorname{H}_{31}$ & \texttt{2312.c} \\
\cline{3-5}
& & $\operatorname{H}_{40}$ & $\operatorname{H}_{40}$ & \texttt{16128.bi} \\
\cline{3-5}
& & $\operatorname{H}_{89}$ & $\operatorname{H}_{93}$ & \texttt{4056.k} \\
\cline{3-5}
& & $\operatorname{H}_{103}$ & $\operatorname{H}_{104}$ & \texttt{4225.e} \\
\cline{3-5}
& & $\operatorname{H}_{295}$ & $\operatorname{H}_{297}$ & $y^{2} = x^{3} + x^{2} - 6740460588x - 200219177111472$ \\
\cline{3-5}
& & $\operatorname{H}_{556}$ & $\operatorname{H}_{563}$ & \texttt{200.b} \\
\cline{3-5}
& & $\operatorname{H}_{558}$ & $\operatorname{H}_{566}$ & \texttt{3362.c} \\
\cline{3-5}
& & $\operatorname{H}_{40a}$ & $\operatorname{H}_{40b}$ & \texttt{1792.e} \\
\cline{3-5}
& & $\operatorname{H}_{40c}$ & $\operatorname{H}_{40c}$ & \texttt{12544.e} \\
\cline{3-5}
& & $\operatorname{H}_{40d}$ & $\operatorname{H}_{40d}$ & \texttt{12544.p} \\
\cline{3-5}
& & $\operatorname{H}_{11}$ & $\operatorname{H}_{11}$ & \texttt{2772.m} \\
\cline{3-5}
& & $\operatorname{H}_{26}$ & $\operatorname{H}_{28}$ & \texttt{468.e} \\
\cline{3-5}
& & $\operatorname{H}_{29}$ & $\operatorname{H}_{41}$ & \texttt{17664.f} \\
\cline{3-5}
& & $\operatorname{H}_{35}$ & $\operatorname{H}_{49}$ & \texttt{300.d} \\
\cline{3-5}
& & $\operatorname{H}_{39}$ & $\operatorname{H}_{45}$ & \texttt{1575.g} \\
\cline{3-5}
& & $\operatorname{H}_{47}$ & $\operatorname{H}_{47}$ & \texttt{1800.w} \\
\cline{3-5}
& & $\operatorname{H}_{50}$ & $\operatorname{H}_{50}$ & \texttt{71148.s} \\
\cline{3-5}
& & $\operatorname{H}_{63}$ & $\operatorname{H}_{70}$ & \texttt{2400.p} \\
\cline{3-5}
& & $\operatorname{H}_{97}$ & $\operatorname{H}_{97}$ & $y^{2} = x^{3} - 558481500x - 5079892400000$ \\
\cline{3-5}
& & $\operatorname{H}_{105}$ & $\operatorname{H}_{112}$ & \texttt{4606.e} \\
\cline{3-5}
& & $\operatorname{H}_{106}$ & $\operatorname{H}_{111}$ & \texttt{2016.c} \\
\cline{3-5}
& & $\operatorname{H}_{107}$ & $\operatorname{H}_{110}$ & \texttt{3038.c} \\
\cline{3-5}
& & $\operatorname{H}_{109}$ & $\operatorname{H}_{124}$ & \texttt{700.f} \\
\cline{3-5}
& & $\operatorname{H}_{113}$ & $\operatorname{H}_{114}$ & $y^{2} + xy = x^{3} - x^{2} - 785472x - 267747760$ \\
\cline{3-5}
& & $\operatorname{H}_{288}$ & $\operatorname{H}_{323}$ & $y^{2} + xy = x^{3} + x^{2} - 1163177961056300788x - 365926510640189061755312483$ \\
\cline{3-5}
& & $\operatorname{H}_{291}$ & $\operatorname{H}_{324}$ & $y^{2} + xy + y = x^{3} + x^{2} - 70411166718x + 7186776239309115$ \\
\cline{3-5}
& & $\operatorname{H}_{302}$ & $\operatorname{H}_{326}$ & $y^{2} = x^{3} + x^{2} - 7859386910x - 268185327947856$ \\
\cline{3-5}
& & $\operatorname{H}_{304}$ & $\operatorname{H}_{309}$ & \texttt{6128.y} \\
\cline{3-5}
& & $\operatorname{H}_{308}$ & $\operatorname{H}_{312}$ & \texttt{173600.bn2} \\
\cline{3-5}
& & $\operatorname{H}_{76d}$ & $\operatorname{H}_{82a}$ & \texttt{768.g} \\
\cline{3-5}
& & $\operatorname{H}_{76a}$ & $\operatorname{H}_{82b}$ & \texttt{2304.k} \\
\cline{3-5}
& & $\operatorname{H}_{76b}$ & $\operatorname{H}_{82c}$ & \texttt{768.b} \\
\cline{3-5}
& & $\operatorname{H}_{76c}$ & $\operatorname{H}_{82d}$ & \texttt{2304.f} \\
\cline{3-5}
& & $\operatorname{H}_{9}$ & $\operatorname{H}_{10}$ & \texttt{325.d} \\
\cline{3-5}
& & $\operatorname{H}_{37}$ & $\operatorname{H}_{42}$ & \texttt{4480.a} \\
\cline{3-5}
& & $\operatorname{H}_{108}$ & $\operatorname{H}_{123}$ & \texttt{10880.ba} \\
\cline{3-5}
& & $\operatorname{H}_{238}$ & $\operatorname{H}_{239}$ & \texttt{1152.r} \\
\cline{3-5}
& & $\operatorname{H}_{9c}$ & $\operatorname{H}_{10a}$ & \texttt{52.a} \\
\cline{3-5}
& & $\operatorname{H}_{9a}$ & $\operatorname{H}_{10c}$ & \texttt{676.c} \\
\cline{3-5}
& & $\operatorname{H}_{37a}$ & $\operatorname{H}_{42a}$ & \texttt{3200.f} \\
\cline{3-5}
& & $\operatorname{H}_{37c}$ & $\operatorname{H}_{42c}$ & \texttt{3200.w} \\
\cline{3-5}
& & $\operatorname{H}_{108a}$ & $\operatorname{H}_{123e}$ & \texttt{21632.bc} \\
\cline{3-5}
& & $\operatorname{H}_{108c}$ & $\operatorname{H}_{123a}$ & \texttt{21632.bl} \\
\hline
\end{tabular}}
\caption{2-adic Images of $L_{2}(2)$ Graphs}
\label{2-adic Images of L22 Graphs}
\end{table}
\end{center}
\fi

\iffalse
G2:=GL(2,Integers(2));
G4:=GL(2,Integers(4));

/*$E$ has full two-torsion*/
G:=sub<G4|[3,0,0,1],[1,0,2,1],[1,0,0,3],[1,2,0,1]>;
S:=Subgroups(G);
Slist:=[s`subgroup : s in S];

/*$E$ does not have a $4$-isogeny*/
nolist:={};
A:=sub<G4|[3,0,0,1],[1,1,0,1],[1,0,0,3]>;
AA:=Subgroups(A);
AAA:=[s`subgroup : s in AA];
for s in Slist do
for a in AAA do
if IsConjugate(G4,a,s) then
nolist:=nolist join {s};
end if;
end for;
end for;
Slist:=[s:s in Slist|not s in nolist];

/* one group per conjugacy class */
nolist:={};
for i in [1..#Slist-1] do
for j in [i+1..#Slist] do
if IsConjugate(G4,Slist[i],Slist[j]) then
nolist:=nolist join {Slist[j]};
end if;
end for;
end for;
Slist:=[s : s in Slist | s notin nolist];

/* full determinant mod-4 */
Slist:=[s:s in Slist | #{Determinant(g) : g in s} eq 2];

/*representatives of complex conjugation mod-4*/
A:=sub<G4|[1,0,0,3]>;
B:=sub<G4|[1,1,0,3]>;
        
Alist:={};
for i in [1..#Slist] do
Ni:=Slist[i];
SNi:=Subgroups(Ni);
SNiList:=[s`subgroup : s in SNi];
SNiList:=[s : s in SNiList | #s eq 2];
for s in SNiList do
if IsConjugate(G4,s,A) then
Alist:=Alist join {Ni};
end if;
end for;
end for;

Blist:={};
for i in [1..#Slist] do
Ni:=Slist[i];
SNi:=Subgroups(Ni);
SNiList:=[s`subgroup : s in SNi];
SNiList:=[s : s in SNiList | #s eq 2];
for s in SNiList do
if IsConjugate(G4,s,B) then
Blist:=Blist join {Ni};
end if;
end for;
end for;

Slist:=[s:s in Slist | s in Alist or s in Blist];

/* $\phi_{P_{2}}(Q_{4})$ is not defined over $\Q$ */
nolist:={};
H:=sub<G4|[1,2,0,1],[3,0,0,1],[1,0,2,1]>;
HH:=Subgroups(H);
HHH:=[s`subgroup : s in HH];
for s in Slist do
for h in HHH do
if IsConjugate(G4,s,h) then
nolist:=nolist join {h};
end if;
end for;
end for;
Slist:=[s:s in Slist|not s in nolist];

/* $\phi_{P_{2}}(P_{4}+Q_{4})$ is not defined over $\Q$ */
nolist:={};
H:=sub<G4|[3,0,0,1],[1,2,0,1],[1,0,2,3],[1,2,2,3],[3,0,2,3],[3,2,2,3]>;
HH:=Subgroups(H);
HHH:=[s`subgroup : s in HH];
for s in Slist do
for h in HHH do
if IsConjugate(G4,s,h) then
nolist:=nolist join {h};
end if;
end for;
end for;
Slist:=[s:s in Slist|not s in nolist];

/* $\phi_{Q_{2}}(P_{4})$ is not defined over $\Q$ */
nolist:={};
H:=sub<G4|[1,0,2,1],[1,2,0,1],[1,0,0,3]>;
HH:=Subgroups(H);
HHH:=[s`subgroup : s in HH];
for s in Slist do
for h in HHH do
if IsConjugate(G4,s,h) then
nolist:=nolist join {h};
end if;
end for;
end for;
Slist:=[s:s in Slist|not s in nolist];

/* $\phi_{Q_{2}}(P_{4}+Q_{4})$ is not defined over $\Q$ */
nolist:={};
H:=sub<G4|[1,0,0,3],[1,0,2,1],[3,2,0,1],[3,2,0,3],[3,2,2,1],[3,2,2,3]>;
HH:=Subgroups(H);
HHH:=[s`subgroup : s in HH];
for s in Slist do
for h in HHH do
if IsConjugate(G4,s,h) then
nolist:=nolist join {h};
end if;
end for;
end for;
Slist:=[s:s in Slist|not s in nolist];

/* $\phi_{P_{2}+Q_{2}}(P_{4})$ is not defined over $\Q$ */
nolist:={};
H:=sub<G4|[3,0,2,1],[1,0,0,3],[1,2,0,1]>;
HH:=Subgroups(H);
HHH:=[s`subgroup : s in HH];
for s in Slist do
for h in HHH do
if IsConjugate(G4,s,h) then
nolist:=nolist join {h};
end if;
end for;
end for;
Slist:=[s:s in Slist|not s in nolist];

/* $\phi_{P_{2}+Q_{2}}(Q_{4})$ is not defined over $\Q$ */
nolist:={};
H:=sub<G4|[3,0,0,1],[1,0,2,1],[1,2,0,3]>;
HH:=Subgroups(H);
HHH:=[s`subgroup : s in HH];
for s in Slist do
for h in HHH do
if IsConjugate(G4,s,h) then
nolist:=nolist join {h};
end if;
end for;
end for;
Slist:=[s:s in Slist|not s in nolist];

list:={};
for s in Slist do
list:=list join {sub<G4|[Transpose(x) : x in Generators(s)]>};
end for;
Slist:=[s : s in list];

\fi



\iffalse
m:=4;
Gm:=GL(2,Integers(4));

load "/users/garenchiloyan/desktop/gl2data";
load "/users/garenchiloyan/desktop/gl2finedata";
load "/users/garenchiloyan/desktop/curvelist1.txt";
load "/users/garenchiloyan/desktop/curvelist2.txt";

yesno:=0;
for G in Slist do
for i:=1 to #newsublist do
grp:=newsublist[i];
if grp[2] gt 4 then
Ggrp:=sub<Gm|Generators(grp[3])>;
if IsConjugate(Gm,G,Ggrp) then
print "Yes, image does occur, for newsublist group #", i;
yesno:=1;
end if;
end if;
if grp[2] eq 2 then
Ggrp:=sub<Gm|Generators(grp[3]),[[1,2,0,1],[1+2,0,0,1],[1,0,0,1+2]\
,[1,0,2,1]]>;
if IsConjugate(Gm,G,Ggrp) then
print "Yes, image does occur, for newsublist group #", i;
yesno:=1;
end if;
end if;
if grp[2] eq 4 then
Ggrp:=sub<Gm|Generators(grp[3]),[[1,4,0,1],[1+4,0,0,1],[1,0,0,1+4]\
,[1,0,4,1]]>;
if IsConjugate(Gm,G,Ggrp) then
print "Yes, image does occur, for newsublist group #", i;
yesno:=1;
end if;
end if;
end for;
for i:=1 to #finesublist do
grp:=finesublist[i];
if grp[3] gt 4 then
Ggrp:=sub<Gm|Generators(grp[4])>;
if IsConjugate(Gm,G,Ggrp) then
print "Yes, image does occur, for finesublist group#", i;
E:=EllipticCurve(curvelist2[i][2]);
I:=IsogenousCurves(E);
print G,[GroupName(TorsionSubgroup(A)) : A in I];
yesno:=1;
end if;
end if;
if grp[3] eq 4 then
Ggrp:=sub<Gm|Generators(grp[4]),[[1,4,0,1],[1+4,0,0,1],[1,0,0,1+4]\
,[1,0,4,1]]>;
if IsConjugate(Gm,G,Ggrp) then
print "Yes, image does occur, for finesublist group #", i;
E:=EllipticCurve(curvelist2[i][2]);
I:=IsogenousCurves(E);
print G,[GroupName(TorsionSubgroup(A)) : A in I];
yesno:=1;
end if;
end if;
if grp[3] eq 2 then
Ggrp:=sub<Gm|Generators(grp[4]),[[1,2,0,1],[1+2,0,0,1],[1,0,0,1+2]\
,[1,0,2,1]]>;
if IsConjugate(Gm,G,Ggrp) then
print "Yes, image does occur, for finesublist group #", i;
E:=EllipticCurve(curvelist2[i][2]);
I:=IsogenousCurves(E);
print G,[GroupName(TorsionSubgroup(A)) : A in I];
yesno:=1;
end if;
end if;
end for;
end for;

\fi

\iffalse
	
	By Lemma \ref{coprime twists}, there is a quadratic twist $E^{(d)}$ of $E$ such that the image of the mod-$3$ Galois representation attached to $E$ is conjugate to $\mathcal{B}_{3}'$ and the image of the mod-$4$ Galois representation attached to $E^{(d)}$ contains $-I$ and the image of the mod-$8$ Galois representation attached to $E^{(d)}$ contains $-I$. Running a MAGMA code, we see that there are two admissible subgroups of $\operatorname{GL}(2, \ZZ / 4 \ZZ)$ that contain $-I$ modulo $4$ and reduce modulo $2$ to the trivial group. They are, $\operatorname{H}_{8}$ and $\operatorname{H}_{24}$. Running another MAGMA code, we see that there are four admissible subgroups of $\operatorname{GL}(2, \ZZ / 8 \ZZ)$ that contain $-I$ and reduce modulo $2$ to the trivial group. They are, $\operatorname{H}_{8}$, $\operatorname{H}_{24}$, $\operatorname{H}_{38}$, and $\operatorname{H}_{46}$.
	
	If the image of the mod-$3$ Galois representation attached to $E$ is conjugate to a subgroup of $\mathcal{B}_{3}'$, then the image of the mod-$4$ Galois representation attached to $E$ is not conjugate to a subgroup of $\operatorname{H}_{24}$ (see Section 13 of \cite{gcal-r}).
	
	
	By the classification of adelic images of Galois, there are no non-cuspidal, $\QQ$-rational points on the modular curves defined by $\operatorname{H}_{24} \times \operatorname{B}_{3}'$, $\operatorname{H}_{38} \times \operatorname{B}_{3}'$, or $\operatorname{H}_{46} \times \operatorname{B}_{3}'$. This shows that the image of the $2$-adic Galois representation attached to $E$ is conjugate to a subgroup $H$ of $\operatorname{GL}(2, \ZZ_{2})$ such that $\left\langle H, -I \right\rangle = H_{8}$. There are two subgroups $H$ of $\operatorname{GL}(2, \ZZ / 4 \ZZ)$ in the RZB database such that $\left\langle H, -I \right\rangle = H_{8}$, namely, $H_{8b}$ and $H_{8d}$. There are two subgroups $H$ of $\operatorname{GL}(2, \ZZ / 8 \ZZ)$ in the RZB database such that $\left\langle H, -I \right\rangle = H_{8}$, namely, $H_{8a}$ and $H_{8c}$. Of course, $H_{8}$ is the only subgroup of $\operatorname{GL}(2, \ZZ / 2 \ZZ)$ such that adjoining $-I$ is equal to $H_{8}$.
	
	By the classification of adelic images of Galois, there are no non-cuspidal, $\QQ$-rational points on the modular curves defined by $\operatorname{H}_{8a} \times \operatorname{B}_{3}$ or $\operatorname{H}_{8b} \times \operatorname{B}_{3}$.
	

	\begin{proof}
	
	Let $E/\QQ$ be an elliptic curve with full two-torsion defined over $\QQ$. Let $\mathcal{E}$ be the $\QQ$-isogeny class of $E$. Suppose that the isogeny-torsion graph associated to $\mathcal{E}$ is of type $S$.
	
	First, suppose the isogeny-torsion graph associated to $\mathcal{E}$ is $\mathcal{S}^{1}$ or $\mathcal{S}^{2}$. Running a MAGMA code (pasted below)
	
	
	G2:=GL(2,Integers(2));
G4:=GL(2,Integers(4));

/*$E$ has full two-torsion and $\phi_{Q_{2}}(P_{4})$ is defined over $\Q$*/
G:=sub<G4|[1,0,2,1],[1,0,0,3],[1,2,0,1]>;
S:=Subgroups(G);
Slist:=[s`subgroup : s in S];

/*$E$ does not have a $4$-isogeny*/
nolist:={};
A:=sub<G4|[3,0,0,1],[1,1,0,1],[1,0,0,3]>;
AA:=Subgroups(A);
AAA:=[s`subgroup : s in AA];
for s in Slist do
for a in AAA do
if IsConjugate(G4,a,s) then
nolist:=nolist join {s};
end if;
end for;
end for;
Slist:=[s:s in Slist|not s in nolist];

/* one group per conjugacy class */
nolist:={};
for i in [1..#Slist-1] do
for j in [i+1..#Slist] do
if IsConjugate(G4,Slist[i],Slist[j]) then
nolist:=nolist join {Slist[j]};
end if;
end for;
end for;
Slist:=[s : s in Slist | s notin nolist];

/* full determinant mod-4 */
Slist:=[s:s in Slist | #{Determinant(g) : g in s} eq 2];

/*representatives of complex conjugation mod-4*/
A:=sub<G4|[1,0,0,3]>;
B:=sub<G4|[1,1,0,3]>;
        
Alist:={};
for i in [1..#Slist] do
Ni:=Slist[i];
SNi:=Subgroups(Ni);
SNiList:=[s`subgroup : s in SNi];
SNiList:=[s : s in SNiList | #s eq 2];
for s in SNiList do
if IsConjugate(G4,s,A) then
Alist:=Alist join {Ni};
end if;
end for;
end for;

Blist:={};
for i in [1..#Slist] do
Ni:=Slist[i];
SNi:=Subgroups(Ni);
SNiList:=[s`subgroup : s in SNi];
SNiList:=[s : s in SNiList | #s eq 2];
for s in SNiList do
if IsConjugate(G4,s,B) then
Blist:=Blist join {Ni};
end if;
end for;
end for;

Slist:=[s:s in Slist | s in Alist or s in Blist];

/* $\phi_{P_{2}}(P_{4}+Q_{4})$ is not defined over $\Q$ */
nolist:={};
H:=sub<G4|[1,2,0,1],[1,0,2,3],[1,2,2,3]>;
HH:=Subgroups(H);
HHH:=[s`subgroup : s in HH];
for s in Slist do
for h in HHH do
if IsConjugate(G4,s,h) then
nolist:=nolist join {h};
end if;
end for;
end for;
Slist:=[s:s in Slist|not s in nolist];

/* $\phi_{P_{2}+Q_{2}}(Q_{4})$ is not defined over $\Q$ */
nolist:={};
H:=sub<G4|[1,0,2,1],[1,2,0,3]>;
HH:=Subgroups(H);
HHH:=[s`subgroup : s in HH];
for s in Slist do
for h in HHH do
if IsConjugate(G4,s,h) then
nolist:=nolist join {h};
end if;
end for;
end for;
Slist:=[s:s in Slist|not s in nolist];

list:={};
for s in Slist do
list:=list join {sub<G4|[Transpose(x) : x in Generators(s)]>};
end for;
Slist:=[s : s in list];

followed by calling groups from RZB database, code below,

/* RZB Database */

m:=4;
Gm:=GL(2,Integers(m));

load "/users/garenchiloyan/desktop/gl2data";
load "/users/garenchiloyan/desktop/gl2finedata";
load "/users/garenchiloyan/desktop/curvelist1.txt";
load "/users/garenchiloyan/desktop/curvelist2.txt";

yesno:=0;
for G in Slist do
for i:=1 to #newsublist do
grp:=newsublist[i];
if grp[2] gt 4 then
Ggrp:=sub<Gm|Generators(grp[3])>;
if IsConjugate(Gm,G,Ggrp) then
print "Yes, image does occur, for newsublist group #", i;
yesno:=1;
end if;
end if;
if grp[2] eq 2 then
Ggrp:=sub<Gm|Generators(grp[3]),[[1,2,0,1],[1+2,0,0,1],[1,0,0,1+2]\
,[1,0,2,1]]>;
if IsConjugate(Gm,G,Ggrp) then
print "Yes, image does occur, for newsublist group #", i;
yesno:=1;
end if;
end if;
if grp[2] eq 4 then
Ggrp:=sub<Gm|Generators(grp[3]),[[1,4,0,1],[1+4,0,0,1],[1,0,0,1+4]\
,[1,0,4,1]]>;
if IsConjugate(Gm,G,Ggrp) then
print "Yes, image does occur, for newsublist group #", i;
yesno:=1;
end if;
end if;
end for;
for i:=1 to #finesublist do
grp:=finesublist[i];
if grp[3] gt 4 then
Ggrp:=sub<Gm|Generators(grp[4])>;
if IsConjugate(Gm,G,Ggrp) then
print "Yes, image does occur, for finesublist group#", i;
E:=EllipticCurve(curvelist2[i][2]);
I:=IsogenousCurves(E);
print G,[GroupName(TorsionSubgroup(A)) : A in I];
yesno:=1;
end if;
end if;
if grp[3] eq 4 then
Ggrp:=sub<Gm|Generators(grp[4]),[[1,4,0,1],[1+4,0,0,1],[1,0,0,1+4]\
,[1,0,4,1]]>;
if IsConjugate(Gm,G,Ggrp) then
print "Yes, image does occur, for finesublist group #", i;
E:=EllipticCurve(curvelist2[i][2]);
I:=IsogenousCurves(E);
print G,[GroupName(TorsionSubgroup(A)) : A in I];
yesno:=1;
end if;
end if;
if grp[3] eq 2 then
Ggrp:=sub<Gm|Generators(grp[4]),[[1,2,0,1],[1+2,0,0,1],[1,0,0,1+2]\
,[1,0,2,1]]>;
if IsConjugate(Gm,G,Ggrp) then
print "Yes, image does occur, for finesublist group #", i;
E:=EllipticCurve(curvelist2[i][2]);
I:=IsogenousCurves(E);
print G,[GroupName(TorsionSubgroup(A)) : A in I];
yesno:=1;
end if;
end if;
end for;
end for;

we see that (naively), the image of the mod-$4$ Galois representation attached to $E$ is conjugate to one of two groups : $\operatorname{H}_{8d}$ and $\operatorname{H}_{24d}$. Note that $\left\langle \operatorname{H}_{24d}, -I \right\rangle = \operatorname{H}_{24}$. Work from \cite{gcal-r} (see subsection 11.3) proved that the image of the $2$-adic Galois representation attached to an elliptic curve over $\QQ$ with a $3$-isogeny is not conjugate to a subgroup of $\operatorname{H}_{24}$. Hence, the image of the mod-$4$ Galois representation attached to $E$ is conjugate to $\operatorname{H}_{8d}$. We must prove that the image of the mod-$4$ Galois representation attached to $E$ is of level $4$.

There are six subgroups of $\operatorname{GL}(2, \ZZ / 8 \ZZ)$ that reduce down mod-$4$ to $\operatorname{H}_{8d}$, namely, $\operatorname{H}_{38a}$, $\operatorname{H}_{38c}$, $\operatorname{H}_{38d}$, $\operatorname{H}_{46a}$, $\operatorname{H}_{46c}$, and $\operatorname{H}_{46d}$. Note that $\left\langle \operatorname{H}_{38a}, -I \right\rangle = \left\langle \operatorname{H}_{38c}, -I \right\rangle = \left\langle \operatorname{H}_{38d}, -I \right\rangle$ and $\left\langle \operatorname{H}_{46a}, -I \right\rangle = \left\langle \operatorname{H}_{46c}, -I \right\rangle = \left\langle \operatorname{H}_{46d}, -I \right\rangle$. In other words, if the image of the mod-$8$ Galois representation attached elliptic curve over $\QQ$ is conjugate to $\operatorname{H}_{38a}$, then after quadratic twisting, the image of the mod-$8$ Galois representation attached to the quadratic twist is conjugate to $\operatorname{H}_{38c}$ or $\operatorname{H}_{38d}$. The same can be true if the image of the mod-$8$ Galois representation attached to an elliptic curve is conjugate to $\operatorname{H}_{46a}$.

The model for $\operatorname{X}_{38d}$ is $y^{2} = x^{3} + A(t)x + B(t)$ where
\begin{center} $A(t) = -27t^{4}+54t^{2}-108$ and $B(t) = 54t^{6}-162t^{4}-324t^{2}+432$ \end{center}
with \textit{j}-invariant equal to $64 \cdot \frac{(t^{4}-2t^{2}+4)^{3}}{t^{4} \cdot (t^{2}-2)^{2}}$. An elliptic curve over $\QQ$ with a $3$-isogeny has \textit{j}-invariant equal to $27 \cdot\frac{(s+1)(s+9)^{3}}{s^{3}}$ for some non-zero rational number $s$. Homogenizing and setting these two terms equal, we have an equality
$$64 \cdot \frac{(t^{4}-2t^{2}z^{2}+4z^{4})^{3}}{z^{4} \cdot t^{4} \cdot (t^{2}-2z^{2})^{2}} = 27 \cdot\frac{(s+z)(s+9z)^{3}}{z \cdot s^{3}}.$$
We get a projective curve
$$C : 64 \cdot s^{3} \cdot (t^{4}-2t^{2}z^{2}+4z^{4})^{3} - 27 \cdot z^{3} \cdot t^{4} \cdot (t^{2}-2z^{2})^{2} \cdot (s+z) \cdot (s+9z)^{3} = 0.$$
Using code from Magma, (pasted below)

we get that $C$ is a curve of genus $1$ with three rational points, namely, $(0,0,1)$, $(0,1,0)$, and $(1,0,0)$.

The model for $\operatorname{X}_{46d}$ is $y^{2} = x^{3} + A(t)x + B(t)$ where
\begin{center}
    $A(t) = -27t^{4}-54t^{2}-108$ and $B(t) = 54t^{6}+162t^{4}-324t^{2}-432$
\end{center}
with \textit{j}-invariant equal to $64 \cdot \frac{(t^{4}+2t^{2}+4)^{3}}{t^{4} \cdot (t^{2}+2)^{2}}$. An elliptic curve over $\QQ$ with a $3$-isogeny has \textit{j}-invariant equal to $27 \cdot\frac{(s+1)(s+9)^{3}}{s^{3}}$ for some non-zero rational number $s$. Homogenizing and setting these two terms equal, we have an equality
$$64 \cdot \frac{(t^{4}+2t^{2}z^{2}+4z^{4})^{3}}{z^{4} \cdot t^{4} \cdot (t^{2}+2z^{2})^{2}} = 27 \cdot\frac{(s+z)(s+9z)^{3}}{z \cdot s^{3}}.$$
We get a projective curve
$$C : 64 \cdot s^{3} \cdot (t^{4}+2t^{2}z^{2}+4z^{4})^{3} - 27 \cdot z^{3} \cdot t^{4} \cdot (t^{2}+2z^{2})^{2} \cdot (s+z) \cdot (s+9z)^{3}.$$
Using similar code from Magma, we get that $C$ is a curve of genus $1$ with three $\QQ$-rational points, namely, $(0,0,1)$, $(0,1,0)$, and $(1,0,0)$.

Now let us say that the isogeny-torsion graph of $\mathcal{E}$ is $\mathcal{S}^{3}$ or $\mathcal{S}^{4}$. Running a Magma code (pasted below)


followed by calling groups from the RZB database, (code below)

we see that the image of the $2$-adic Galois representation attached to $E$ is conjugate to one of $\operatorname{H}_{8}$, $\operatorname{H}_{8a}$, $\operatorname{H}_{8b}$, or $\operatorname{H}_{8c}$, along with groups that reduce mod-$4$ or mod-$8$ to a group that is conjugate to a subgroup of $\operatorname{H}_{24}$, $\operatorname{H}_{38}$, or $\operatorname{H}_{46}$.

Notice that
$$\left\langle \operatorname{H}_{8a}, -I \right\rangle = \left\langle \operatorname{H}_{8b}, -I \right\rangle = \left\langle \operatorname{H}_{8c}, -I \right\rangle = \left\langle \operatorname{H}_{8d}, -I \right\rangle = \operatorname{H}_{8}.$$
In other words, $\operatorname{X}_{8a}$, $\operatorname{X}_{8b}$, $\operatorname{X}_{8c}$, $\operatorname{X}_{8d}$, and $\operatorname{X}_{8}$ are quadratic twists and their \textit{j}-invariants are equal. Moreover, $\operatorname{H}_{8a}$, $\operatorname{H}_{8b}$, $\operatorname{H}_{8c}$, $\operatorname{H}_{8d}$, and $\operatorname{H}_{8}$ are the only quadratic twists of $\operatorname{H}_{8}$, as each subgroup of $H_{8}$ of index $2$ without $-I$ is conjugate to one of $\operatorname{H}_{8a}$, $\operatorname{H}_{8b}$, $\operatorname{H}_{8c}$, or $\operatorname{H}_{8d}$. Using the previous part of the proof, the image of the mod-$4$ Galois representation attached to an elliptic curve over $\QQ$ with a $3$-isogeny cannot be conjugate to a subgroup of $\operatorname{H}_{24}$, and the image of the mod-$8$ Galois representation cannot be conjugate to a subgroup of $\operatorname{H}_{38}$ or $\operatorname{H}_{46}$.

\end{proof}

\begin{remark}
Let $E/\QQ$ be an elliptic curve such that the image of the $2$-adic Galois representation to $E$ is conjugate to $\operatorname{H}_{8}$. Consider the following models of $\operatorname{X}_{8a}$, $\operatorname{X}_{8b}$, $\operatorname{X}_{8c}$, and $\operatorname{X}_{8d}$.

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.7}{
    \begin{tabular}{|c|c|c|c|}
    \hline
    Model & RZB & $A(t)$ & $B(t)$\\
    \hline
    \multirow{4}*{$y^{2} = x^{3} + A(t)x + B(t)$} & $\operatorname{X}_{8a}$ & $-3^{3} \cdot (t^{2}+3)(t-1)^{2}(t+1)^{2}$ & $2 \cdot 3^{3} \cdot t(t-3)(t+3)(t-1)^{3}(t+1)^{3}$ \\
    \cline{2-4}
    & $\operatorname{X}_{8b}$ & $-2^{2} \cdot 3^{3} \cdot (t^{2}+3)(t-1)^{2}(t+1)^{2}$ & $2^{4} \cdot 3^{3} \cdot t(t-3)(t+3)(t-1)^{3}(t+1)^{3}$ \\
    \cline{2-4}
    & $\operatorname{X}_{8c}$ & $-3^{3} \cdot (t^{2}+3)$ & $2 \cdot 3^{3} \cdot t(t-3)(t+3)$ \\
    \cline{2-4}
    & $\operatorname{X}_{8d}$ & $-2^{2} \cdot 3^{3} \cdot (t^{2}+3)$ & $2^{4} \cdot 3^{3} \cdot t(t-3)(t+3)$\\
    \hline
    \end{tabular}}
    \end{table}
    \end{center}
\end{remark}

Notice that each of the polynomials $A(t)$ are even polynomials and each of the polynomials $B(t)$ are odd polynomials. Hence, the quadratic twist of $\operatorname{X}_{8a}$ by $-1$ is $\operatorname{X}_{8a}$, the quadratic twist of $\operatorname{X}_{8b}$ by $-1$ is $\operatorname{X}_{8b}$, etc. The quadratic twist of $\operatorname{X}_{8}$ by $1$ is the same as twisting $\operatorname{X}_{8}$ twice by $-1$. As $\operatorname{X}_{8a}$, $\operatorname{X}_{8b}$, $\operatorname{X}_{8c}$, $\operatorname{X}_{8d}$, and $\operatorname{X}_{8}$ are the only quadratic twists of $\operatorname{X}_{8}$, this means that the quadratic twist of $\operatorname{X}_{8}$ by $-1$ is $\operatorname{X}_{8}$. Next, the quadratic twist of $\operatorname{X}_{8a}$ by $2$ is $\operatorname{X}_{8b}$ and vise versus, the quadratic twist of $\operatorname{X}_{8c}$ by $2$ is $\operatorname{X}_{8d}$ and vise versus, and the quadratic twist of $\operatorname{X}_{8}$ by $2$ is $\operatorname{X}_{8}$.

There are $31$ subgroups of $\operatorname{H}_{8}$ of index $2$. Hence, there are $31$ quadratic subfields of $\QQ(E[8])$. If $\QQ(\sqrt{m})$ and $\QQ(\sqrt{n})$ are distinct quadratic subfields of $\QQ(E[8])$, then $\QQ(\sqrt{mn})$ is a quadratic subfield of $\QQ(E[8])$. A combinatorial argument shows that the $31$ quadratic subfields of $\QQ(E[8])$ are of the form $\QQ(\sqrt{d})$ where $d$ is a product of the numbers $-1$, $2$, $a$, $b$, and $c$, where $a$, $b$, and $c$ are squarefree integers greater than $2$.

There are two subgroups of $\operatorname{H}_{8}$ that are conjugate to $\operatorname{H}_{8a}$, namely,
\begin{itemize}
    \item $\left\langle
    \begin{bmatrix} 1 & 0 \\
    0 & 3\end{bmatrix},
    -\begin{bmatrix} 1 & 0 \\
    0 & 7\end{bmatrix},
    -\begin{bmatrix} 3 & 0 \\
    0 & 1\end{bmatrix},
    \begin{bmatrix} 7 & 0 \\
    0 & 1\end{bmatrix}
    -\begin{bmatrix} 1 & 2 \\
    0 & 1\end{bmatrix},
    -\begin{bmatrix} 1 & 0 \\
    2 & 1\end{bmatrix},
    \right\rangle$
    
    \vspace{5mm}
    
    \item $\left\langle
    -\begin{bmatrix} 1 & 0 \\
    0 & 3\end{bmatrix},
    \begin{bmatrix} 1 & 0 \\
    0 & 7\end{bmatrix},
    \begin{bmatrix} 3 & 0 \\
    0 & 1\end{bmatrix},
    -\begin{bmatrix} 7 & 0 \\
    0 & 1\end{bmatrix},
    -\begin{bmatrix} 1 & 2 \\
    0 & 1\end{bmatrix},
    -\begin{bmatrix} 1 & 0 \\
    2 & 1\end{bmatrix}
    \right\rangle$
\end{itemize}

\vspace{5mm}

There are six subgroups of $\operatorname{H}_{8}$ that are conjugate to $\operatorname{H}_{8c}$, namely,

\begin{itemize}
    \item $\left\langle
    \begin{bmatrix} 1 & 0 \\
    0 & 3\end{bmatrix},
    -\begin{bmatrix} 1 & 0 \\
    0 & 7\end{bmatrix},
    -\begin{bmatrix} 3 & 0 \\
    0 & 1\end{bmatrix},
    \begin{bmatrix} 7 & 0 \\
    0 & 1\end{bmatrix},
    \begin{bmatrix} 1 & 2 \\
    0 & 1 \end{bmatrix},
    -\begin{bmatrix} 1 & 0 \\
    2 & 1\end{bmatrix}
    \right\rangle$
    
    \vspace{5mm}
    
    \item $\left\langle
    -\begin{bmatrix} 1 & 0 \\
    0 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\
    0 & 7\end{bmatrix},
    \begin{bmatrix} 3 & 0 \\
    0 & 1\end{bmatrix},
    -\begin{bmatrix} 7 & 0 \\
    0 & 1\end{bmatrix},
    \begin{bmatrix} 1 & 2 \\
    0 & 1\end{bmatrix},
    -\begin{bmatrix} 1 & 0 \\
    2 & 1\end{bmatrix}
    \right\rangle$
    
    \vspace{5mm}
    
    \item $\left\langle
    \begin{bmatrix} 1 & 0 \\
    0 & 3\end{bmatrix},
    -\begin{bmatrix} 1 & 0 \\
    0 & 7\end{bmatrix},
    -\begin{bmatrix} 3 & 0 \\
    0 & 1\end{bmatrix}
    \begin{bmatrix} 7 & 0 \\
    0 & 1\end{bmatrix},
    -\begin{bmatrix} 1 & 2 \\
    0 & 1\end{bmatrix},
    \begin{bmatrix} 1 & 0 \\
    2 & 1 \end{bmatrix}
    \right\rangle$
    
    
    \vspace{5mm}
    
    \item $\left\langle
    -\begin{bmatrix} 1 & 0 \\
    0 & 3\end{bmatrix},
    \begin{bmatrix} 1 & 0 \\
    0 & 7 \end{bmatrix},
    \begin{bmatrix} 3 & 0 \\
    0 & 1\end{bmatrix},
    -\begin{bmatrix} 7 & 0 \\
    0 & 1\end{bmatrix},
    -\begin{bmatrix} 1 & 2 \\
    0 & 1\end{bmatrix},
    \begin{bmatrix} 1 & 0 \\
    2 & 1\end{bmatrix}
    \right\rangle$
    
    \vspace{5mm}
    
    \item $\left\langle
    \begin{bmatrix} 1 & 0 \\
    0 & 3 \end{bmatrix},
    -\begin{bmatrix} 1 & 0 \\
    0 & 7\end{bmatrix},
    -\begin{bmatrix} 3 & 0 \\
    0 & 1\end{bmatrix},
    \begin{bmatrix} 7 & 0 \\
    0 & 1\end{bmatrix},
    \begin{bmatrix} 1 & 2 \\
    0 & 1\end{bmatrix},
    \begin{bmatrix} 1 & 0 \\
    2 & 1\end{bmatrix}
    \right\rangle$
    
    \vspace{5mm}
    
    \item $\left\langle
    -\begin{bmatrix} 1 & 0 \\
    0 & 3\end{bmatrix},
    \begin{bmatrix} 1 & 0 \\
    0 & 7\end{bmatrix},
    \begin{bmatrix} 3 & 0 \\
    0 & 1 \end{bmatrix},
    -\begin{bmatrix} 7 & 0 \\
    0 & 1\end{bmatrix},
    \begin{bmatrix} 1 & 2 \\
    0 & 1\end{bmatrix},
    \begin{bmatrix} 1 & 0 \\
    2 & 1\end{bmatrix},
    \right\rangle$
    
\end{itemize}

There are two subgroups of $\operatorname{H}_{8}$ that are conjugate to $\operatorname{H}_{8b}$, namely,

\begin{itemize}
    \item $\left\langle
    \begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 7 \end{bmatrix},
    -\begin{bmatrix} 3 & 0 \\ 0 & 1 \end{bmatrix}, 
    -\begin{bmatrix} 7 & 0 \\ 0 & 1 \end{bmatrix}, 
    -\begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix}, 
    -\begin{bmatrix} 1 & 0 \\ 2 & 1 \end{bmatrix}
    \right\rangle$
    
    \vspace{5mm}
    
    \item $\left\langle
    -\begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix},
    -\begin{bmatrix} 1 & 0 \\ 0 & 7 \end{bmatrix},
    \begin{bmatrix} 3 & 0 \\ 0 & 1 \end{bmatrix}, 
    \begin{bmatrix} 7 & 0 \\ 0 & 1 \end{bmatrix}, 
    -\begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix}, 
    -\begin{bmatrix} 1 & 0 \\ 2 & 1 \end{bmatrix}
    \right\rangle$
\end{itemize}

There are six subgroups of $\operatorname{H}_{8}$ that are conjugate to $\operatorname{H}_{8d}$, namely,

\begin{itemize}

    \item $\left\langle
    \begin{bmatrix} 1 & 0 \\
    0 & 3 \end{bmatrix}, 
    \begin{bmatrix} 1 & 0 \\
    0 & 7 \end{bmatrix},
    -\begin{bmatrix} 3 & 0 \\
    0 & 1 \end{bmatrix}, 
    -\begin{bmatrix} 7 & 0 \\
    0 & 1 \end{bmatrix}, 
    -\begin{bmatrix} 1 & 2 \\
    0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\
    2 & 1 \end{bmatrix}\right\rangle$
    
    \vspace{5mm}
    
    \item $\left\langle -\begin{bmatrix} 1 & 0 \\
    0 & 3 \end{bmatrix}, 
    -\begin{bmatrix} 1 & 0 \\
    0 & 7 \end{bmatrix},
    \begin{bmatrix} 3 & 0 \\
    0 & 1 \end{bmatrix}, 
    \begin{bmatrix} 7 & 0 \\
    0 & 1 \end{bmatrix}, 
    -\begin{bmatrix} 1 & 2 \\
    0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\
    2 & 1 \end{bmatrix}\right\rangle$
    
    \vspace{5mm}
    
    \item $\left\langle \begin{bmatrix} 1 & 0 \\
    0 & 3 \end{bmatrix}, 
    \begin{bmatrix} 1 & 0 \\
    0 & 7 \end{bmatrix},
    -\begin{bmatrix} 3 & 0 \\
    0 & 1 \end{bmatrix}, 
    -\begin{bmatrix} 7 & 0 \\
    0 & 1 \end{bmatrix}, 
    \begin{bmatrix} 1 & 2 \\
    0 & 1 \end{bmatrix},
    -\begin{bmatrix} 1 & 0 \\
    2 & 1 \end{bmatrix}\right\rangle$
    
    \vspace{5mm}
    
    \item $\left\langle -\begin{bmatrix} 1 & 0 \\
    0 & 3 \end{bmatrix}, 
    -\begin{bmatrix} 1 & 0 \\
    0 & 7 \end{bmatrix},
    \begin{bmatrix} 3 & 0 \\
    0 & 1 \end{bmatrix}, 
    \begin{bmatrix} 7 & 0 \\
    0 & 1 \end{bmatrix}, 
    \begin{bmatrix} 1 & 2 \\
    0 & 1 \end{bmatrix},
    -\begin{bmatrix} 1 & 0 \\
    2 & 1 \end{bmatrix}\right\rangle$
    
    \vspace{5mm}
    
    \item $\left\langle
    \begin{bmatrix} 1 & 0 \\
    0 & 3 \end{bmatrix}, 
    \begin{bmatrix} 1 & 0 \\
    0 & 7 \end{bmatrix},
    -\begin{bmatrix} 3 & 0 \\
    0 & 1 \end{bmatrix}, 
    -\begin{bmatrix} 7 & 0 \\
    0 & 1 \end{bmatrix}, 
    \begin{bmatrix} 1 & 2 \\
    0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\
    2 & 1 \end{bmatrix}\right\rangle$
    
    \vspace{5mm}
    
    \item $\left\langle
    -\begin{bmatrix} 1 & 0 \\
    0 & 3 \end{bmatrix}, 
    -\begin{bmatrix} 1 & 0 \\
    0 & 7 \end{bmatrix},
    \begin{bmatrix} 3 & 0 \\
    0 & 1 \end{bmatrix}, 
    \begin{bmatrix} 7 & 0 \\
    0 & 1 \end{bmatrix}, 
    \begin{bmatrix} 1 & 2 \\
    0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\
    2 & 1 \end{bmatrix}\right\rangle$
\end{itemize}
The remaining fifteen subgroups of $\operatorname{H}_{8}$ of index $2$ contain $-I$.
\fi

\iffalse
\newpage

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{1}{
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    Isogeny Graph & $A$ & $B$ & level & $H$ & $\operatorname{X}$ \\
    \hline
    \multirow{5}*{\includegraphics[scale=0.2]{Snew}} & \multirow{2}*{$\left\{\begin{bmatrix} 1 & \ast \\ 0 & \ast \end{bmatrix} \right\}$} & $\operatorname{H}_{8a}$ & 24 & H & X \\
    \cline{3-6}
    & & $\operatorname{H}_{8b}$ & 12 & H & X \\
    \cline{2-6}
    & \multirow{3}*{$\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix}\right\}$} & $\operatorname{H}_{24}$ & 12 & H & X \\
    \cline{3-6}
    & & $\operatorname{H}_{38}$ & 24 & H & X \\
    \cline{3-6}
    & & $\operatorname{H}_{46}$ & 24 & H & X \\
    \cline{1-6}
    \hline
\end{tabular}}
\caption{product groups table S}
\label{product groups table S}
\end{table}
\end{center}

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{1}{
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    Isogeny Graph & $A$ & $B$ & level & $H$ & $\operatorname{X}$ \\
    \hline
    \multirow{8}*{\includegraphics[scale=0.25]{r6new.jpg}} & \multirow{8}*{$\left\{\begin{bmatrix} \ast & 0 \\ 0 & \ast \end{bmatrix} \right\}$} & $\operatorname{H}_{9}$ & 12 & H & X \\
    \cline{3-6}
    & & $\operatorname{H}_{11}$ & 12 & H & X \\
    \cline{3-6}
    & & $\operatorname{H}_{12}$ & 12 & H & X \\
    \cline{3-6}
    & & $\operatorname{H}_{14}$ & 24 & H & X \\
    \cline{3-6}
    & & $\operatorname{H}_{15}$ & 24 & H & X \\
    \cline{3-6}
    & & $\operatorname{H}_{18}$ & 24 & H & X \\
    \cline{3-6}
    & & $\operatorname{H}_{23}$ & 12 & H & X \\
    \cline{3-6}
    & & $\operatorname{H}_{26}$ & 12 & H & X \\
    \hline
\end{tabular}}
\caption{product groups table R6}
\label{product groups table R6}
\end{table}
\end{center}

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{1}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    Isogeny Graph & $p$ & $A$ & $B$ & level & $H$ & $\operatorname{X}$ \\
    \hline
    \multirow{15}*{\includegraphics[scale=0.1]{r42p graph.png}} &
    \multirow{8}*{$5$} & \multirow{7}*{$\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix}\right\}$} & $\operatorname{H}_{9}$ & 20 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{11}$ & 20 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{12}$ & 20 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{16}$ & 40 & H & X \\
    \cline{3-7}
    & & $\left\{\begin{bmatrix} 1 & \ast \\ 0 & \ast \end{bmatrix}\right\}$ & $\operatorname{H}_{14}$ & 40 & H & X \\
    \cline{2-7}
    & \multirow{7}*{$3$} & \multirow{5}*{$\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix}\right\}$} & $\operatorname{H}_{37}$ & 24 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{11}$ & 12 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{12}$ & 12 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{14}$ & 24 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{18}$ & 24 & H & X \\
    \cline{3-7}
    & & \multirow{2}*{$\left\{\begin{bmatrix} 1 & \ast \\ 0 & \ast \end{bmatrix}\right\}$} & $\operatorname{H}_{9a}$ & 24 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{9b}$ & 24 & H & X \\
    \hline
\end{tabular}}
\caption{product groups table R4}
\label{product groups table R4}
\end{table}
\end{center}

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{1}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    Isogeny Graph & $p$ & $A$ & $B$ & level & $H$ & $\operatorname{X}$ \\
    \hline
    \multirow{12}*{\includegraphics[scale=0.1]{L3 Graph.png}} &
    \multirow{6}*{$3$} & \multirow{6}*{$\left\{\begin{bmatrix} \ast & 0 \\ 0 & \ast \end{bmatrix}\right\}$} & $\operatorname{H}_{2}$ & 6 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{3}$ & 12 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{4}$ & 24 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{5}$ & 24 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{7}$ & 12 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{20}$ & 12 & H & X \\
    \cline{2-7}
    & \multirow{6}*{$5$} & \multirow{6}*{$\left\{\begin{bmatrix} \ast & 0 \\ 0 & \ast \end{bmatrix}\right\}$} & $\operatorname{H}_{2}$ & 10 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{3}$ & 20 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{4}$ & 40 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{5}$ & 40 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{7}$ & 20 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{20}$ & 20 & H & X \\
    \cline{4-7}
    \hline
\end{tabular}}
\caption{product groups table L3p}
\label{product groups table L3p}
\end{table}
\end{center}

\newpage

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{1}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    Isogeny Graph & $p$ & $A$ & $B$ & level & $H$ & $\operatorname{X}$ \\
    \hline
    \multirow{25}*{\includegraphics[scale=0.1]{L2 Graph.png}} &
    \multirow{5}*{$13$} & \multirow{5}*{$\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix}\right\}$} & $\operatorname{H}_{2}$ & 26 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{3}$ & 54 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{5}$ & 104 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{7}$ & 52 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{20}$ & 52 & H & X \\
    \cline{2-7}
    & \multirow{9}*{$7$} & \multirow{3}*{$\left\{\begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix}\right\}$} & $\operatorname{H}_{7}$ & 28 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{22}$ & 56 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{55}$ & 56 & H & X \\
    \cline{3-7}
    & & \multirow{6}*{$\left\{\begin{bmatrix} 1 & \ast \\ 0 & \ast \end{bmatrix} \right\}$} & $\operatorname{H}_{2}$ & 14 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{3}$ & 28 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{4}$ & 56 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{5}$ & 56 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{7}$ & 28 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{20}$ & 28 & H & X \\
    \cline{2-7}
    & \multirow{7}*{$5$} & \multirow{6}*{$\left\{ \begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$} & $\operatorname{H}_{2}$ & 10 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{3}$ & 20 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{5}$ & 40 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{20}$ & 20 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{22}$ & 40 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{55}$ & 40 & H & X \\
    \cline{3-7}
    & & $\left\{ \begin{bmatrix} 1 & \ast \\ 0 & \ast \end{bmatrix} \right\}$ & $\operatorname{H}_{7}$ & 20 & H & X \\
    \cline{2-7}
    & \multirow{4}*{$3$} & \multirow{3}*{$\left\{ \begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\}$} & $\operatorname{H}_{7}$ & 12 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{22}$ & 24 & H & X \\
    \cline{4-7}
    & & & $\operatorname{H}_{55}$ & 24 & H & X \\
    \cline{3-7}
    & & $\left\{ \begin{bmatrix} 1 & \ast \\ 0 & \ast \end{bmatrix} \right\}$ & $\operatorname{H}_{20a}$ & 24 & H & X \\
    \hline
\end{tabular}}
\caption{product groups table L2p}
\label{product groups table L2p}
\end{table}
\end{center}

\newpage
====================================================

\newpage

Let $E/\QQ$ be an elliptic curve. Then $E$ has the structure of an abelian group. Let $N$ be a positive integer. The set of points on $E$ of order dividing $N$ with coordinates in $\overline{\QQ}$ is a group, denoted $E[N]$ and isomorphic to $\ZZ / N \ZZ \times \ZZ / N \ZZ$. An element of $E[N]$ is called an $N$-torsion point. The group $G_{\QQ}:= \operatorname{Gal}(\overline{\QQ}/\QQ)$ acts on $E[N]$ for all positive integers $N$. From this action, we have the mod-$N$ Galois representation attached to $E$:
$$ \overline{\rho}_{E,N} \colon G_{\QQ} \to \operatorname{Aut}(E[N]).$$
After identifying $E[N] \cong \ZZ / N \ZZ \times \ZZ / N \ZZ$ and fixing a basis of $E[N]$, we may consider the mod-$N$ Galois representation attached to $E$ as
$$ \overline{\rho}_{E,N} \colon G_{\QQ} \to \operatorname{GL}(2,\ZZ / N \ZZ).$$
Let $u$ be an element of $\left(\ZZ / N \ZZ \right)^{\times}$. By the properties of the Weil pairing, there exists an element of $\overline{\rho}_{E,N}(G_{\QQ})$ whose determinant is equal to $u$. Moreover, $\overline{\rho}_{E,N}(G_{\QQ})$ has an element that behaves like complex conjugation. If $E$ is non-CM, then by Lemma 2.8 of \cite{SZ}, $\overline{\rho}_{E,N}(G_{\Q})$ has an element conjugate to $\left(\begin{array}{cc}
    1 & 1 \\
    0 & -1
\end{array}\right)$ or $\left(\begin{array}{cc}
    1 & 0 \\
    0 & -1
\end{array}\right)$. If $E$ is CM, then the situation is a little more complicated.

Let $E/\QQ$ and $E'/\QQ$ be elliptic curves. An isogeny mapping $E$ to $E'$ is a non-constant rational morphism $\phi \colon E \to E'$ that maps the identity of $E$ to the identity of $E'$. An isogeny is a group homomorphism with a kernel of finite order. The degree of an isogeny agrees with the order of its kernel.

\begin{lemma}\label{generators of Z/ell^NZ}
	Let $\ell$ be a prime. Let $E/\QQ$ be an elliptic curve and let $P_{\ell}$ and $Q_{\ell}$ be points on $E$ of order $\ell$ that generate distinct groups of order $\ell$. For each integer $m \geq 2$, let $P_{\ell^{m}}, Q_{\ell^{m}} \in E$, such that $[\ell]P_{\ell^{m}} = P_{\ell^{m-1}}$ and $[\ell]Q_{\ell^{m}} = Q_{\ell^{m-1}}$. Then $E[\ell^{m}] = \left\langle P_{\ell^{m}}, Q_{\ell^{m}} \right\rangle$.
	\end{lemma}
	
	\begin{proof}
	Clearly, $P_{\ell^{m}}$ and $Q_{\ell^{m}}$ are points of order equal to $\ell^{m}$ for all positive integers $m$. It remains to prove that for each positive integer $m$, that $\left\langle P_{\ell^{m}} \right\rangle$ and $\left\langle Q_{\ell^{m}} \right\rangle$ intersect trivially.
	
	We proceed by induction. As $P_{\ell}$ and $Q_{\ell}$ generate distinct groups of prime order, $\left\langle P_{\ell} \right\rangle$ and $\left\langle Q_{\ell} \right\rangle$ intersect trivially. Now assume that for a fixed positive integer $m$, that $\left\langle P_{\ell^{m}} \right\rangle$ and $\left\langle Q_{\ell^{m}} \right\rangle$ intersect trivially. Both $\left\langle P_{\ell^{m+1}} \right\rangle$ and $\left\langle Q_{\ell^{m+1}} \right\rangle$ are cyclic groups of equal, $\ell$-power order. If $\left\langle P_{\ell^{m+1}} \right\rangle$ and $\left\langle Q_{\ell^{m+1}} \right\rangle$ intersect non-trivially, they would share a subgroup of order $\ell$.
	
	The subgroup of order $\ell$ in $\left\langle P_{\ell^{m+1}} \right\rangle$ is $\left\langle P_{\ell} \right\rangle$ and the subgroup of order $\ell$ in $\left\langle Q_{\ell^{m+1}} \right\rangle$ is $\left\langle Q_{\ell} \right\rangle$. As $\left\langle P_{\ell} \right\rangle \neq \left\langle Q_{\ell} \right\rangle$, the proof is finished.
	\end{proof}
	
	\begin{remark}
	Let $E/\QQ$ be an elliptic curve. For the rest of the paper, we will fix $P_{2}$ and $Q_{2}$ to designate two distinct points on $E$ of order $2$. For each positive integer $m$, we will denote $P_{2^{m}}$ and $Q_{2^{m}}$ to be points on $E$ such that $[2]P_{2^{m}} = P_{2^{m-1}}$ and $[2]Q_{2^{m}} = Q_{2^{m-1}}$. Then for each positive integer $m$, $E[2^{m}] = \left\langle P_{2^{m}}, Q_{2^{m}} \right\rangle$ because $\left\langle P_{2^{m}} \right\rangle$ and $\left\langle Q_{2^{m}} \right\rangle$ are two cyclic groups of order $2^{m}$ that intersect trivially. If $E$ has a point of order $2$ defined over $\QQ$, then we will say that $Q_{2}$ is defined over $\QQ$, if $E$ has a point of order $4$ defined over $\QQ$, we will say that $Q_{4}$ is defined over $\QQ$, and if $E$ has a point of order $8$ defined over $\QQ$, then we will say that $Q_{8}$ is defined over $\QQ$.

	\end{remark}
	

\begin{defn}
Let $E/\QQ$ be an elliptic curve. A subgroup $H$ of $E$ of finite order is said to be $\QQ$-rational if $\sigma(H) = H$ for all $\sigma \in G_{\QQ}$.
\end{defn}

\begin{remark}

Note that for an elliptic curve $E / \Q$, a group generated by a point $P$ on $E$ defined over $\QQ$ of finite order is certainly a $\Q$-rational group but in general, the elements of a $\QQ$-rational subgroup of $E$ need not be \textit{fixed} by $G_{\Q}$. For example, $E[3]$ is a $\Q$-rational group but certainly, the group $G_{\Q}$ fixes one or three of the nine points of $E[3]$ by Theorem \ref{thm-mazur}.
\end{remark}
	
\begin{lemma}[III.4.12, \cite{Silverman}]\label{Q-rational}
Let $E/\QQ$ be an elliptic curve. Then for each finite, cyclic, $\QQ$-rational subgroup $H$ of $E$, there is a unique elliptic curve defined over $\QQ$ up to isomorphism denoted $E / H$, and an isogeny $\phi_{H} \colon E \to E / H$ with kernel $H$.
\end{lemma}

\begin{remark}

Note that it is only the elliptic curve that is unique (up to isomorphism) but the isogeny is not. For any isogeny $\phi$, the isogeny $-\phi$ has the same domain, codomain, and kernel as $\phi$.

Moreover, for any positive integer $N$ the isogeny $\phi$ and the isogeny $[N] \circ \phi$ have the same domain and the same codomain. This is why the bijection in Lemma \ref{Q-rational} is with \textit{cyclic}, $\Q$-rational subgroups of an elliptic curve instead of with all $\QQ$-rational subgroups of an elliptic curve.
\end{remark}

\subsection{Quadratic Twists}

\begin{lemma}
Let $N$ be a positive integer and let $H$ be a subgroup of $\operatorname{GL}(2,\ZZ / N \ZZ)$ that does not contain $\operatorname{-Id}$. Let $H' = \left\langle \operatorname{-Id}, H \right\rangle$. Then $H' \cong \left\langle \operatorname{-Id} \right\rangle \times H$.
\end{lemma}

\begin{proof}
Define
$$\phi \colon \left\langle \operatorname{-Id} \right\rangle \times H \to H'$$
by $\phi(x,h) = xh$. This is a group homomorphism as $\operatorname{-Id}$ is in the center of $\operatorname{GL}(2,\Z/N\Z)$.

Let $(x,h) \in \left\langle \operatorname{-Id} \right\rangle \times H$ such that $\phi(x,h) = xh = \operatorname{Id}$. Then $h = x^{-1} = x$ as the order of $x$ is equal to $1$ or $2$. As $\operatorname{-Id} \notin H$, $h$ cannot be $\operatorname{-Id}$. Hence, $h = x = \operatorname{Id}$ and so, $\phi$ is injective. Finally, noting that all elements of $H'$ are of the form $\pm h$ for some $h \in H$, we have that $\phi$ is surjective. This proves that $\phi$ is an isomorphism.
\end{proof}

\begin{definition}
Let $\ell$ be a prime and let $G$ and $H$ be subgroups of $\operatorname{GL}(2, \ZZ_{\ell})$.Then we will say that $G$ is a quadratic twist of $H$ and $H$ is a quadratic twist of $G$ if $G$ is the same as $H$, up to multiplication of some elements of $H$ by $\operatorname{-Id}$. Note that if $\left\langle G, \operatorname{-Id} \right\rangle =  \left\langle H, \operatorname{-Id} \right\rangle$, then $H$ and $G$ are quadratic twists.
\end{definition}

\begin{lemma}
Let $N$ be a positive integer, let $H$ be a subgroup of $\operatorname{GL}(2,\Z/N\Z)$, and let $H' = \left\langle H, \operatorname{-Id} \right\rangle$. Let $\chi$ be a character of $H$ of degree two. Then $\chi(H) = H'$ or $\chi(H)$ is a subgroup of $H'$ of index $2$.
\end{lemma}

\begin{proof}

The character $\chi$ multiplies some elements of $H$ by $\operatorname{-Id}$. If $\operatorname{-Id} \in \chi(H)$, then we can multiply all of the elements of $H$ that $\chi$ multiplied by $\operatorname{-Id}$ by $\operatorname{-Id}$ again, and recoup all of the elements of $H$. Thus, $\chi(H)$ is a subgroup of $H'$ that contains both $\operatorname{-Id}$ and $H$ and so, $\chi(H) = H'$.

On the other hand, let us say that $\operatorname{-Id} \notin \chi(H)$. Let $\chi(H)' = \left\langle \chi(H), \operatorname{-Id} \right\rangle$. By the same argument from before, we can multiply all of the elements of $H$ that $\chi$ multiplied by $\operatorname{-Id}$ by $\operatorname{-Id}$ again, and recoup all of the elements of $H$ in $\chi(H)'$. In other words, $\chi(H)' = \left\langle \operatorname{-Id}, \chi(H) \right\rangle = \left\langle \operatorname{-Id}, H \right\rangle = H'$. By the previous lemma, $H' = \left\langle \chi(H), \operatorname{-Id} \right\rangle \cong \left\langle \operatorname{-Id} \right\rangle \times \chi(H)$ and $\chi(H)$ is a subgroup of $H'$ of index $2$.
\end{proof}

Let $E : y^{2} = x^{3} + Ax + B$ be an elliptic curve and let $d$ be a non-zero integer. Then we define the quadratic twist of $E$ by $d$ to be the elliptic curve $E^{(d)} : y^{2} = x^{3} + d^{2}Ax + d^{3}B$. Equivalently, we may define the quadratic twist of $E$ by $d$ to be the elliptic curve $E^{(d)} : dy^{2} = x^{3} + Ax + B$. Then $E$ is isomorphic to $E^{(d)}$ over $\QQ(\sqrt{d})$ by the map
$$\phi \colon E \to E^{(d)}$$
defined by fixing $\mathcal{O}$ and mapping any non-zero $(a,b)$ on $E$ to $\left(a,\frac{b}{\sqrt{d}}\right)$.

\begin{corollary}\label{subgroups of index 2 contain -Id}
Let $N$ be a positive integer and let $H$ be a subgroup of $\operatorname{GL}(2, \Z/N \Z)$ such that all subgroups of $H$ of index $2$ contain $\operatorname{-Id}$. Let $E/\Q$ be an elliptic curve such that $\overline{\rho}_{E,p}(G_{\Q})$ is conjugate to $H$. Let $E^{\chi}$ be a quadratic twist of $E$. Then $\overline{\rho}_{E^{\chi},p}(G_{\Q})$ is conjugate to $H$.
\end{corollary}

\begin{proof}
By our previous lemma, $\overline{\rho}_{E^{\chi},N}(G_{\Q})$ is conjugate to $H$ or conjugate to a subgroup of $H$ of index $2$. Moreover, $\overline{\rho}_{E^{\chi},N}(G_{\Q})$ is the same as $\overline{\rho}_{E,N}(G_{\Q}) = H$, up to multiplication of some elements of $H$ by $\operatorname{-Id}$. As all subgroups of $H$ of index $2$ contain $\operatorname{-Id}$, we can just multiply the elements of $\overline{\rho}_{E^{\chi},N}(G_{\Q})$ that $\chi$ multiplied by $\operatorname{-Id}$ again by $\operatorname{-Id}$ to recoup all elements of $H$. Hence, $\overline{\rho}_{E^{\chi},N}(G_{\QQ}) = H$.
\end{proof}

\begin{remark}
Let $N$ be a positive integer and let $H$ be a subgroup of $\operatorname{GL}(2, \Z/N\Z)$ that does not contain $\operatorname{-Id}$. Let $E/\Q$ be an elliptic curve such that $\overline{\rho}_{E,N}(G_{\QQ})$ is conjugate to $H' = \left\langle H, \operatorname{-Id} \right\rangle$. Then there is a quadratic twist $\chi$ such that $\overline{\rho}_{E^{chi},N}(G_{\QQ})$ is conjugate to $H$ (see Remark 1.1.3  and Section 10 in \cite{Rouse2021elladicIO}. Conversely, if $\overline{\rho}_{E,N}(G_{\QQ})$ is conjugate to $H$, then $\overline{\rho}_{E^{\chi},N}(G_{\QQ})$ is conjugate to $H'$ where $E^{\chi}$ is a quadratic twist of $E$ by a non-zero number $d$ such that $\QQ(E[N])$ does not contain $\QQ(\sqrt{d})$.
\end{remark}

\begin{remark}
Let $N$ be a positive integer. Let $E/\QQ$ be an elliptic curve such that $\overline{\rho}_{E,N}(G_{\Q})$ contains $\operatorname{-Id}$. Let $E^{\chi}$ be a quadratic twist of $E$. Then either $\overline{\rho}_{E,N}(G_{\Q}) = \overline{\rho}_{E^{\chi},N}(G_{\Q})$ or $\overline{\rho}_{E^{\chi},N}(G_{\Q})$ is an index-$2$ subgroup of $\overline{\rho}_{E,N}(G_{\Q})$ that does not contain $\operatorname{-Id}$. Moreover, for each index-$2$ subgroup $H$ of $\overline{\rho}_{E,N}(G_{\Q})$ that does not contain $\operatorname{-Id}$, there is a quadratic twist $E^{\chi}$ such that $\rho_{E^{\chi},N}(G_{\Q}) = H$.
\end{remark}

\subsection{Galois representations}

\begin{lemma}\label{order of 1+2^n}
Let $n$ be an integer greater than or equal to $2$. Then for each positive integer $r$, we have
$$(1+2^{n})^{2^{r}} = 1+2^{n+r}+s$$
where $s$ is a positive integer such that $v_{2}(s) \geq n+r+1$.
\end{lemma}

\begin{proof}

We proceed by induction on $r$. When $r = 1$, we have $(1+2^{n})^{2} = 1+2^{n+1}+2^{2n}$. As $n \geq 2$, we have $v_{2}(2^{2n}) = 2n = n + n \geq n+2 = n+r+1$. Now let $r \geq 2$ and suppose the lemma is true. Then
$$(1+2^{n})^{2^{r+1}} = \left(\left(1+2^{n}\right)^{2^{r}}\right)^{2} = (1+2^{n+r}+s)^{2} = 1+2^{n+r+1}+2s+2^{n+r+1}s+2^{2(n+r)}+s^{2}$$
where $s$ is a positive integer such that $v_{2}(s) \geq n+r+1$. It is clear that $m = 2s+2^{n+r+1}s+2^{2(n+r)}+s^{2}$ is a positive integer such that $v_{2}(m) \geq n+r+2$.

\end{proof}


\begin{lemma}\label{kernel of pi 1}
Let $m$ and $n$ be positive integers such that $m > n \geq 2$. Let $\pi \colon \operatorname{GL}\left(2, \ZZ / 2^{m} \ZZ\right) \to \operatorname{GL}\left(2, \ZZ / 2^{n} \ZZ\right)$ be the natural projection map.
\begin{enumerate}
    \item Then the order of $1+2^{n}$ in $\ZZ / 2^{m} \ZZ$ is equal to $2^{m-n}$,
    
    \item $\operatorname{Ker}(\pi) = \left\langle \begin{bmatrix} 1+2^{n} & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 1+2^{n} \end{bmatrix}, \begin{bmatrix} 1 & 2^{n} \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 2^{n} & 1 \end{bmatrix} \right\rangle$.
\end{enumerate}
\end{lemma}

\begin{proof} We break up the proof in steps.

\begin{enumerate}

    \item Note that $m-n$ is a positive integer. By the previous lemma,
    $$(1+2^{n})^{2^{m-n}} = 1+2^{m}+s$$
    for some positive integer $s$ such that $v_{2}(s) \geq m+1$. Reducing $(1+2^{n})^{2^{m-n}}$ modulo $2^{m}$, we have $\overline{(1+2^{n})^{2^{m-n}}} = \overline{1+2^{m}+s} = \overline{1}$. Thus, the order of $1+2^{n}$ is a power of $2$ less than or equal to $2^{m-n}$.
    
    If $m = n+1$, then $m-n-1 = 0$ and hence, $(1+2^{n})^{2^{m-n-1}} = 1+2^{n}$ which is not congruent to $1$ modulo $2^{m}$. Hence, the order of $1+2^{n}$ is equal to $2^{m-n}$ as in the lemma. If on the other hand, $m \geq n+1$, then $m-n-1$ is a positive integer and using the previous lemma again, we see that $$(1+2^{n})^{2^{m-n-1}} = 1+2^{m-1}+s$$
    where $s$ is a positive integer such that $v_{2}(s) \geq m$. Then reducing $(1+2^{n})^{2^{m-n-1}}$ modulo $2^{m}$, we get $\overline{(1+2^{n})^{2^{m-n-1}}} = \overline{1+2^{m-1}+s} = \overline{1 + 2^{m-1}}$ which is not congruent to $1$ modulo $2^{m}$. Thus, again, the order of $2^{n}$ modulo $2^{m}$ is equal to $2^{m-n}$.
    
    \item Let $\begin{bmatrix}
    A & B \\ C & D
    \end{bmatrix}$ be an element of $\operatorname{Ker}(\phi)$. Then $\begin{bmatrix}
    A-1 & B \\ C & D-1
    \end{bmatrix} \equiv \begin{bmatrix} 0 & 0 \\ 0 & 0 \end{bmatrix} \mod 2^{m}$. Clearly, $\operatorname{Ker}(\phi)$ is a group of order $\left(\frac{2^{m}}{2^{n}}\right)^{4} = 2^{4(m-n)}$. Let $G_{1} = \left\langle \begin{bmatrix} 1+2^{n} & 0 \\ 0 & 1 \end{bmatrix} \right\rangle$, let $G_{2} = \left\langle \begin{bmatrix} 1 & 2^{n} \\ 0 & 1 \end{bmatrix} \right\rangle$, let $G_{3} = \left\langle \begin{bmatrix} 1 & 0 \\ 2^{n} & 1 \end{bmatrix} \right\rangle$, and let $G_{4} = \left\langle \begin{bmatrix} 1 & 0 \\ 0 & 1 + 2^{n} \end{bmatrix} \right\rangle$. By the previous lemma, the order of $G_{1}$ and the order of $G_{4}$ are both equal to $2^{m-n}$. By another inductive argument, we can see that the order of $G_{2}$ and $G_{3}$ are both equal to $2^{m-n}$. For $i \in \{1, 2, 3, 4\}$ and $j \in \{1, 2, 3, 4\}$ with $j \neq i$, we have $G_{i} \cap G_{j} = \{\operatorname{Id}\}$. Thus, the group $\left\langle G_{1}, G_{2}, G_{3}, G_{4} \right\rangle$ is contained in $\operatorname{Ker}(\phi)$ and has order equal to $2^{4(m-n)}$.
    
    
\end{enumerate}
\end{proof}

\begin{lemma}\label{kernel of pi 2}
Let $m$ be an integer greater than or equal to $2$. Let $\pi \colon \operatorname{GL}(2, \ZZ / 2^{m} \ZZ) \to \operatorname{GL}(2, \ZZ / 2 \ZZ)$ be the natural projection map. Then

\begin{enumerate}
\item The order of $3$ in $\left(\ZZ / 2^{s} \ZZ\right)^{\times}$ is equal to $2^{s-2}$ for all $s \geq 3$

\item $5$ is not contained in the subgroup of $\left( \ZZ / 2^{d} \ZZ \right)^{\times}$ generated by $3$ for all $d \geq 3$ and $\left(\ZZ / 2^{d} \ZZ \right)^{\times} = \left\langle 3, 5 \right\rangle$.

\item $\operatorname{Ker}(\pi) = \left\langle \begin{bmatrix} 3 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 2 & 1 \end{bmatrix} \right\rangle$.
\end{enumerate}
\end{lemma}

\begin{proof} Again we break up the proof into steps.

\begin{enumerate}
    \item Consider $3 = 1+2$. We claim that the order of $3$ in $\left(\ZZ / 2^{s} \ZZ\right)^{\times}$ is equal to $2^{s-2}$ for all $s \geq 3$. Note that $3^{2} = 1+2^{3}$ so the claim is true when $s = 3$ so let $s \geq 4$. Let $r$ be a positive integer. Then by Lemma \ref{order of 1+2^n},
$$(1+2^{3})^{2^{r}} = 1+2^{3+r} + s$$
where $v_{2}(s) \geq 3+r+1$. Thus, the order of $1+2^{3}$ in $\left(\ZZ / 2^{s} \ZZ\right)^{\times}$ is equal to $2^{s-3}$. Hence, the order of $3$ in $\left(\ZZ / 2^{s} \ZZ\right)^{\times}$ is equal to $2^{s-2}$.

\item Assume by way of contradiction that there is an integer $d \geq 3$ such that $5 \in \left\langle 3 \right\rangle$ modulo $2^{d}$. Then $5$ is a $2$-power of $3$. So there is an integer $d \geq 3$ and a positive integer $r$ such that $5 = 3^{2^{r}} \mod 2^{d}$. Then $5 = (1+2)^{2^{r}} \mod 2^{d}$. If $r = 1$, then $5 = 9 \mod 2^{d}$ and so, $2^{d}$ divides $-4$ which is not true as $d \geq 3$. If $r = 2$, then $5 = 81 \mod 2^{d}$ which is not true. Thus, $r \geq 3$. So assume that
$$5 = (1+2)^{2^{r}} \mod 2^{d} = (1+2^{3})^{2^{r-1}} \mod 2^{d}$$
where $r \geq 3$. Then $5 = 1+2^{r+2}+s$ modulo $2^{d}$ where $s$ is a positive integer such that $v_{2}(s) \geq r+3$. Then $2^{d}$ divides $-4 + 2^{r+2} + s$. Note that $v_{2}(4) = 2$, $v_{2}(2^{r+2}) \geq 3$ and $v_{2}(s) \geq r+3$ and so, $v_{2}(-4+2^{r+2}+s) = 2$. Thus, $2^{d}$ does not divide $-4+2^{r+2}+s$.

The order of $\left(\ZZ / 2^{d}\right)^{\times}$ is equal to $2^{d-1}$. The order of $3$ in $\left(\ZZ / 2^{d} \right)^{\times}$ is equal to $2^{d-2}$ and $5$ is not contained in $\left\langle 3 \right\rangle$. Hence, $\left(\ZZ / 2^{d} \ZZ\right)^{\times} = \left\langle 3, 5 \right\rangle$.

\item Clearly, $\operatorname{Ker}(\pi)$ is the set of all matrices $\left\{\begin{bmatrix}
A & B \\ C & D
\end{bmatrix}\right\}$ where $A$ and $D$ are odd and $B$ and $C$ are even. Then $\operatorname{Ker}(\pi)$ is a group of order $2^{4(m-1)}$. Clearly the lemma is true when $m = 2$. Suppose that $m \geq 3$. Let $G_{1} = \left\langle \begin{bmatrix}
3 & 0 \\ 0 & 1
\end{bmatrix}, \begin{bmatrix}
5 & 0 \\ 0 & 1
\end{bmatrix} \right\rangle$, $G_{2} = \left\langle \begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix} \right\rangle$, $G_{3} = \left\langle\begin{bmatrix} 1 & 0 \\ 2 & 1 \end{bmatrix} \right\rangle$, and $G_{4} = \left\langle \begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix} \right\rangle$. For $i \in \{1, 2, 3, 4\}$, the order of $G_{i}$ is equal to $2^{m-1}$ and for $j \in \{1, 2, 3, 4\}$ and $i \neq j$, we have $G_{i} \bigcap G_{j} = \{\operatorname{Id}\}$. Thus, $\left\langle G_{1}, G_{2}, G_{3}, G_{4} \right\rangle$ is a subgroup of $\operatorname{Ker}(\pi)$ of order $2^{4(m-1)}$.
\end{enumerate}
\end{proof}

\begin{lemma}\label{lifting with kernel}

Let $E/\QQ$ be an elliptic curve and let $\ell$ be a prime number. Let $m$ and $n$ be non-negative integers. Let $\pi \colon \operatorname{GL}(2, \ZZ / \ell^{m+n} \ZZ) \to \operatorname{GL}(2, \ZZ / \ell^{n} \ZZ)$ be the natural projection map. Suppose that $\overline{\rho}_{E,\ell^{n}}(G_{\Q}) = \left\langle g_{1}, \ldots, g_{r} \right\rangle$. Then $\overline{\rho}_{E,\ell^{m+n}}(G_{\Q}) \subseteq \left\langle \widehat{g_{1}}, \ldots, \widehat{g_{r}}, \operatorname{Ker}(\pi) \right\rangle$ where $\widehat{g_{i}}$ is the same matrix as $g_{i}$ but viewed in $\operatorname{GL}(2, \ZZ / \ell^{m+n} \ZZ)$.

\end{lemma}

\begin{proof}

For $i \in \{1, \ldots, r\}$, $\pi(\widehat{g}_{i}) = g_{i}$. Let $x$ be a matrix in $\overline{\rho}_{E,\ell^{m+n}}(G_{\Q})$. Then $\pi(x) = y \in \left\langle g_{1}, \ldots, g_{r}\right\rangle$. Let $\widehat{y}$ be the product of those same matrices in $\operatorname{GL}(2, \ZZ / \ell^{n} \ZZ)$ but viewed in $\operatorname{GL}(2, \ZZ / \ell^{m+n} \ZZ)$. For example, if $y = g_{1} \cdot g_{3} \cdot g_{2} \cdot g_{1}^{-1}$, then let $\widehat{y} = \widehat{g_{1}} \cdot \widehat{g_{3}} \cdot \widehat{g_{2}} \cdot \widehat{g_{1}}^{-1}$. Then $\pi(x) = y = \pi(\widehat{y})$ and so, $x \cdot \widehat{y}^{-1} \in \operatorname{Ker}(\pi)$. Hence, $x \in \left\langle \widehat{g_{1}}, \ldots, \widehat{g_{r}}, \operatorname{Ker}(\pi) \right\rangle$.

\end{proof}

\begin{remark}

The lemma cannot be extended to say that $\overline{\rho}_{E,2^{m+n}}(G_{\QQ}) = \left\langle \widehat{g_{1}}, \ldots, \widehat{g_{r}}, \operatorname{Ker}(\pi) \right\rangle$ in general. For example, let $E$ be the elliptic curve with Weierstrass equation $y^2+xy+y=x^3+x^2-80x+242$. Then $E(\QQ)_{\text{tors}} \cong \ZZ / 4 \ZZ$. As $E$ has a single point of order $2$ defined over $\QQ$, $\overline{\rho}_{E,2}(G_{\QQ})$ is conjugate to $\left\langle \begin{bmatrix} 1 & 1 \\ 0 & 1 \end{bmatrix} \right\rangle$. Let $\pi \colon \operatorname{GL}(2, \ZZ / 4 \ZZ) \to \operatorname{GL}(2, \ZZ / 2 \ZZ)$ be the natural projection map. Then $\operatorname{Ker}(\pi) = \left\langle \begin{bmatrix}
3 & 0 \\ 0 & 1
\end{bmatrix}, \begin{bmatrix}
1 & 0 \\ 0 & 3
\end{bmatrix}, \begin{bmatrix}
1 & 2 \\ 0 & 1
\end{bmatrix}, \begin{bmatrix}
1 & 0 \\ 2 & 1
\end{bmatrix} \right\rangle$. On the other hand, $\overline{\rho}_{E,4}(G_{\QQ})$ is conjugate to a subgroup of $\mathcal{B}_{4} = \left\langle \begin{bmatrix} 1 & 1 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix} \right\rangle$. Note that $\operatorname{Ker}(\pi)$ is a group of order $16$ and $\mathcal{B}_{4}$ is a group of order $8$. Hence, $\operatorname{Ker}(\pi)$ is not contained in $\overline{\rho}_{E,4}(G_{\QQ})$.

\end{remark}

\begin{definition}

Let $E/\QQ$ be an elliptic curve and let $\ell$ be a prime number. Let $n$ be a positive integer and let $m$ be a non-negative integer. The full lift of $\overline{\rho}_{E,\ell^{n}}(G_{\QQ})$ to level $m+n$ is the group of all elements of $\operatorname{GL}(2, \ell^{m+n})(G_{\QQ})$ that reduce modulo $n$ to an element of $\overline{\rho}_{E,\ell^{n}}(G_{\QQ})$.

\end{definition}


\begin{definition}

Let $E/\QQ$ be an elliptic curve. Suppose that there is a non-negative integer $n$ such that for all non-negative integers, $m$, $\overline{\rho}_{E,\ell^{m+n}}(G_{\QQ})$ is the full lift of $\overline{\rho}_{E,\ell^{n}}(G_{\QQ})$ to level $m+n$. Moreover, suppose $n$ is the smallest such integer. Then we say that $\overline{\rho}_{E,\ell^{\infty}}(G_{\QQ})$ is a group of level $\ell^{n}$.

\end{definition}

\begin{lemma}\label{ell-adic images}

Let $E/\QQ$ and $E'/\QQ$ be elliptic curves that are isogenous by an isogeny $\phi$ whose kernel is finite, cyclic, and $\QQ$-rational. Let $\ell$ be a prime and let $r$ be the non-negative integer such that $\ell^{r}$ is the greatest power of $\ell$ that divides the order of $\operatorname{Ker}(\phi)$. Let $m$ be a non-negative integer. Then there is a basis $\{P_{\ell^{m+r}}, Q_{\ell^{m+r}}\}$ of $E[\ell^{m+r}]$ such that

\begin{enumerate}
\item if $\sigma$ is a Galois automorphism of $\QQ$, then $\overline{\rho}_{E,\ell^{m+r}}(\sigma) = \begin{bmatrix} A & C \\ B & D \end{bmatrix}$ such that $\ell^{r}$ divides $C$
\item $\{\phi([\ell^{r}]\phi(P_{\ell^{m+r}}), \phi(Q_{\ell^{m+r}}\}$ is a basis of $E'[\ell^{m}]$
\item $\overline{\rho}_{E',\ell^{m}}(\sigma) = \begin{bmatrix} A & \frac{C}{\ell^{r}} \\ \ell^{r} \cdot B & D \end{bmatrix}$
\end{enumerate}

\end{lemma}

\begin{proof}
We break up the proof into steps

\begin{enumerate}
\item Let $Q_{\ell^{r}}$ be an element of $\operatorname{Ker}(\phi)$ of order $\ell^{r}$ and let $Q_{\ell^{m+r}}$ be a point on $E$ such that $[\ell^{m}]Q_{\ell^{m+r}} = Q_{\ell^{r}}$. Let $P_{\ell^{m+r}}$ be a point on $E$ such that $E[\ell^{m+r}] = \left\langle P_{\ell^{m+r}}, Q_{\ell^{m+r}} \right\rangle$. Let $\sigma$ be a Galois automorphism of $\QQ$. Then there are integers $A$ and $B$ such that $\sigma(P_{\ell^{m+r}}) = [A]P_{\ell^{m+r}} + [B]Q_{\ell^{m+r}}$ and there are integers $C$ and $D$ such that $\sigma(Q_{\ell^{m+r}}) = [C]P_{\ell^{m+r}} + [D]Q_{\ell^{m+r}}$. Then
$$\sigma(Q_{\ell^{r}}) = \sigma([\ell^{m}]Q_{\ell^{m+r}}) = [\ell^{m}]\sigma(Q_{\ell^{m+r}}) = [\ell^{m}]([C]P_{\ell^{m+r}}+[D]Q_{\ell^{m+r}}) = [\ell^{m}C]P_{\ell^{m+r}} + [D]Q_{\ell^{r}}.$$
As $Q_{\ell^{r}}$ generates a $\QQ$-rational group, $[\ell^{m}C]P_{\ell^{m+r}} + [D]Q_{\ell^{r}} \in \left\langle Q_{\ell^{r}} \right\rangle \subseteq \left\langle Q_{\ell^{m+r}} \right\rangle$. Thus, $[\ell^{m} C]P_{\ell^{m+r}} \in \left\langle Q_{\ell^{m+r}} \right\rangle$. As $\left\langle P_{\ell^{m+r}} \right\rangle \bigcap \left\langle Q_{\ell^{m+r}} \right\rangle = \{\mathcal{O}\}$, we have that $[\ell^{m}C]P_{\ell^{m+r}} = \mathcal{O}$. Thus, $\ell^{m+r}$ divides $\ell^{m}C$ and hence, $\ell^{r}$ divides $C$.

\item We claim that $E'[\ell^{m}] = \left\langle \phi([\ell^{r}]P_{\ell^{m+r}}), \phi(Q_{\ell^{m+r}}) \right\rangle$. We claim that the order of $\phi([\ell^{r}]P_{\ell^{m+r}})$ and the order of $\phi(Q_{\ell^{m+r}})$ are both equal to $\ell^{m}$. Note that $[\ell^{m}]\phi([\ell^{r}]P_{\ell^{m+r}}) = \phi([\ell^{m+r}]P_{\ell^{m+r}}) = \mathcal{O}$. Next, $[\ell^{m}]\phi(Q_{\ell^{m+r}}) = \phi([\ell^{m}]Q_{\ell^{m+r}}) = \phi(Q_{\ell^{r}}) = \mathcal{O}$. Now let us say that there are integers $\alpha$ and $\beta$ such that $[\alpha]\phi([\ell^{r}]P_{\ell^{m+r}}) = [\beta]\phi(Q_{\ell^{m+r}})$. Then $\phi([\alpha\ell^{r}]P_{\ell^{m+r}}) = \phi([\beta]Q_{\ell^{m+r}})$. Hence, $[\alpha \ell^{r}]P_{\ell^{m+r}} - [\beta]Q_{\ell^{m+r}} \in \left\langle Q_{\ell^{r}} \right\rangle \subseteq \left\langle Q_{\ell^{m+r}} \right\rangle$ and hence, $[\alpha \ell^{r}]P_{\ell^{m+r}} \in \left\langle Q_{\ell^{m+r}} \right\rangle$. Thus, $[\alpha \ell^{r}]P_{\ell^{m+r}} = \mathcal{O}$ and hence, $[\alpha]\phi([\ell^{m}]P_{\ell^{m+r}}) = \phi([\alpha \ell^{m}]P_{\ell^{m+r}}) = \mathcal{O}$. This means that $\left\langle \phi([\ell^{r}]P_{\ell^{m+r}}) \right\rangle \bigcap \left\langle \phi(Q_{\ell^{m+r}}) \right\rangle = \{\mathcal{O}\}$.

\item Next, we see that
$$\sigma(\phi([\ell^{r}]P_{\ell^{m+r}})) = \phi([\ell^{r}]\sigma(P_{\ell^{m+r}})) = \phi([\ell^{r}]([A]P_{\ell^{m+r}}+[B]Q_{\ell^{m+r}})) = [A]\phi([\ell^{r}]P_{\ell^{m+r}})+[\ell^{r} \cdot B]\phi(Q_{\ell^{m+r}}).$$
Finally, we see that
$$\sigma(\phi(Q_{\ell^{m+r}})) = \phi(\sigma(Q_{\ell^{m+r}})) = \phi([C]P_{\ell^{m+r}}+[D]Q_{\ell^{m+r}})$$
$$= \phi\left(\left[\frac{C}{\ell^{r}}\right][\ell^{r}]P_{\ell^{m+r}}+[D]Q_{\ell^{m+r}}\right) = \left[\frac{C}{\ell^{r}}\right]\phi([\ell^{r}]P_{\ell^{m+r}})+[D]\phi(Q_{\ell^{m+r}}).$$
\end{enumerate}
\end{proof}

\begin{remark}
Let $E/\QQ$ and $E'/\QQ$ be elliptic curves. Let $\phi \colon E \to E'$ be a $\QQ$-isogeny with a finite, cyclic, $\QQ$-rational kernel. Then $\overline{\rho}_{E',\ell^{\infty}}(G_{\QQ})$ is determined by $\overline{\rho}_{E,\ell^{\infty}}(G_{\QQ})$ (and vice versa). Suppose that $\ell^{r}$ is the greatest power of $\ell$ that divides $\operatorname{Ker}(\phi)$. Let $m$ be a non-negative integer and suppose that we want to compute $\overline{\rho}_{E,2^{m}}(G_{\QQ})$. There is a basis $\{P_{\ell^{m+r}},Q_{\ell^{m+r}}\}$ of $E[\ell^{m+r}]$ such that $\overline{\rho}_{E,\ell^{m+r}}(G_{\QQ}) = \left\langle \begin{bmatrix} A_{1} & C_{1} \\ B_{1} & D_{1} \end{bmatrix}, \ldots, \begin{bmatrix} A_{s} & C_{s} \\ B_{s} & D_{s} \end{bmatrix} \right\rangle$ such that $\ell^{r}$ divides $C_{1}$, \ldots, $C_{s}$. Moreover, $\{\phi([\ell^{r}]P_{\ell^{m+r}}, \phi(Q_{\ell^{m+r}})\}$ is a basis of $E'[\ell^{m}]$. By Lemma \ref{ell-adic images}, with this basis, $\overline{\rho}_{E',\ell^{m}}(G_{\QQ}) = \left\langle \begin{bmatrix} A_{1} & \frac{C_{1}}{\ell^{r}} \\ \ell^{r} \cdot B_{1} & D_{1} \end{bmatrix}, \ldots, \begin{bmatrix} A_{s} & \frac{C_{s}}{\ell^{r}} \\ \ell^{r} \cdot B_{s} & D_{s} \end{bmatrix} \right\rangle$.

Let us say that $\overline{\rho}_{E,\ell^{\infty}}(G_{\QQ})$ is a group of level $\ell^{n}$ for some non-negative integer $n$. Then for all non-negative integers $k$, $\overline{\rho}_{E,\ell^{n+k}}(G_{\QQ})$ is simply the full lift of $\overline{\rho}_{E,\ell^{n}}(G_{\QQ})$ to level $k$. In other words, if we are given that the level of $\overline{\rho}_{E,\ell^{\infty}}(G_{\QQ})$ is equal to $n$ and if we are given $\overline{\rho}_{E,\ell^{n}}(G_{\QQ})$, then we can compute $\overline{\rho}_{E',\ell^{m}}(G_{\QQ})$ for all elliptic curves $E'$ that are $\QQ$-rational to $E$ and all non-negative integers $m$, using Lemma \ref{ell-adic images}.

\end{remark}

\begin{corollary}\label{coprime isogeny-degree}

Let $E/\QQ$ and $E'/\QQ$ be elliptic curves and let $\ell$ be a prime. Suppose that $E$ is $\QQ$-isogenous to $E'$ by an isogeny that is defined over $\QQ$ with a finite, cyclic kernel of degree not divisible by $\ell$. Then the image of the $\ell$-adic Galois representation attached to $E$ is conjugate to the image of the $\ell$-adic Galois representation attached to $E'$.

\end{corollary}

\begin{proof}

Use Lemma \ref{ell-adic images} with $r = 0$.

\end{proof}

\begin{corollary}\label{contains -Id}
 
Let $\ell$ be a prime and let $E/\QQ$ and $E'/\QQ$ be elliptic curves. Suppose that $E$ is $\QQ$-isogenous to $E'$ by an isogeny $\phi$ with a finite, cyclic, $\QQ$-rational kernel. Then $\overline{\rho}_{E,\ell^{\infty}}(G_{\QQ})$ contains $\operatorname{-Id}$ if and only if $\overline{\rho}_{E',\ell^{\infty}}(G_{\QQ})$ contains $\operatorname{-Id}$.
    
\end{corollary}

\begin{proof}

Let $r$ be the non-negative integer such that $\ell^{r}$ is the greatest power of $\ell$ that divides $\operatorname{Ker}(\phi)$. Let $m$ be a non-negative integer. As $\overline{\rho}_{E,\ell^{\infty}}(G_{\QQ})$ contains $\operatorname{-Id}$, so does $\overline{\rho}_{E,\ell^{m+r}}(G_{\QQ})$. As $\operatorname{-Id}$ is in the center of $\operatorname{GL}(2, \ZZ / \ell^{m+r} \ZZ)$, it does not matter what basis we use for $E[\ell^{m+r}]$. By Lemma \ref{ell-adic images}, $\operatorname{-Id}$ is an element of $\overline{\rho}_{E',\ell^{m}}(G_{\QQ})$.
\end{proof}

\newpage


\section{Elliptic curves, isogeny graphs, and isogeny-torsion graphs}\label{sec-preliminaries}

\begin{thm}[Mazur \cite{mazur1}]\label{thm-mazur}
		Let $E/\Q$ be an elliptic curve. Then
		\[
		E(\Q)_\tor\simeq
		\begin{cases}
		\Z/M\Z &\text{with}\ 1\leq M\leq 10\ \text{or}\ M=12,\ \text{or}\\
		\Z/2\Z\oplus \Z/2N\Z &\text{with}\ 1\leq N\leq 4.
		\end{cases}
		\]
	\end{thm}

The $\QQ$-rational points on the modular curves $\operatorname{X}_0(N)$ have been described completely in the literature, for all $N\geq 1$. One of the most important milestones in their classification was \cite{mazur1}, where Mazur dealt with the case when $N$ is prime. The complete classification of $\Q$-rational points on $\operatorname{X}_0(N)$, for any $N$, was completed due to work of Fricke, Kenku, Klein, Kubert, Ligozat, Mazur  and Ogg, among others (see the summary tables in \cite{lozano0}).
	
	\begin{thm}\label{thm-ratnoncusps} Let $N\geq 2$ be a number such that $\operatorname{X}_0(N)$ has a non-cuspidal $\Q$-rational point. Then:
		\begin{enumerate}
			\item $N\leq 10$, or $N= 12,13, 16,18$ or $25$. In this case $\operatorname{X}_0(N)$ is a curve of genus $0$ and its $\Q$-rational points form an infinite $1$-parameter family, or
			\item $N=11,14,15,17,19,21$, or $27$. In this case $\operatorname{X}_0(N)$ is a curve of genus $1$, i.e.,~$X_0(N)$ is an elliptic curve over $\Q$, but in all cases the Mordell-Weil group $\operatorname{X}_0(N)(\Q)$ is finite, or 
			
			\item $N=37,43,67$ or $163$. In this case $X_0(N)$ is a curve of genus $\geq 2$ and (by Faltings' theorem) there are only finitely many $\Q$-rational points, which are known explicitly.
		\end{enumerate} 
	\end{thm}
	
	
	\begin{defn}
		Let $E/\Q$ be an elliptic curve. We define $C(E)$ as the number of distinct $\Q$-rational cyclic subgroups of $E$ (including the identity subgroup), and we define $C_p(E)$ similarly to $C(E)$ but only counting $\Q$-rational cyclic subgroups of order a power of $p$, for each prime $p$. 
	\end{defn}

Notice that it follows from the definition that $C(E)=\prod_p C_p(E)$. 
	
	\begin{thm}[Kenku, \cite{kenku}]\label{thm-kenku} There are at most eight $\QQ$-isomorphism classes of elliptic curves in each $\QQ$-isogeny class. More concretely,  Then, $C(E)=\prod_p C_p(E)\leq 8$. Moreover, each factor $C_p(E)$ is bounded as follows:
		\begin{center}
			\begin{tabular}{c|ccccccccccccc}
				$p$ & $2$ & $3$ & $5$ & $7$ & $11$ & $13$ & $17$ & $19$ & $37$ & $43$ & $67$ & $163$ & \text{else}\\
				\hline 
				$C_p\leq $ & $8$ & $4$ & $3$ & $2$ & $2$ & $2$ & $2$ & $2$ & $2$ & $2$ & $2$ & $2$ & $1$.
			\end{tabular}
		\end{center}
		Moreover:
		\begin{enumerate}
			\item If $C_{p}(E) = 2$ for a prime $p$ greater than $7$, then $C_{q}(E) = 1$ for all other primes $q$. 
			\item Suppose $C_{7}(E) = 2$, then $C(E) \leq 4$. Moreover, we have $C_{3}(E) = 2$, or $C_{2}(E) = 2$, or $C(E) = 2$.
			\item $C_{5}(E) \leq 3$ and if $C_{5}(E) = 3$, then $C(E) = 3$.
			\item If $C_{5}(E) = 2$, then $C(E) \leq 4$. Moreover, either $C_{3}(E) = 2$, or $C_{2}(E) = 2$, or $C(E) = 2$. 
			\item $C_{3}(E) \leq 4$ and if $C_{3}(E) = 4$, then $C(E) = 4$. 
			\item If $C_{3}(E) = 3,$ then $C(E) \leq 6$. Moreover, $C_{2}(E) = 2$ or $C(E) = 3$.
			\item If $C_{3}(E) = 2$, then $C_{2}(E) \leq 4$.
		\end{enumerate}
	\end{thm}
	
	\begin{thm}[\cite{gcal-r}, Theorem 1.2]\label{thm-isogenygraphs}
	There are $26$ isomorphism types of isogeny graphs that are associated to elliptic curves defined over $\Q$. More precisely, there are $16$ types of (linear) $L_k$ graphs, $3$ types of (nonlinear two-primary torsion) $T_k$ graphs, $6$ types of (rectangular) $R_k$ graphs, and $1$ type of (special) $S$ graph. Moreover, there are $11$ isomorphism types of isogeny graphs that are associated to elliptic curves over $\QQ$ with complex multiplication, namely the types $L_2(p)$ for $p=2,3,11,19,43,67,163$, $L_4$, $T_4$, $R_4(6)$, and $R_4(14)$. Finally, the type $L_4$ occurs exclusively for elliptic curves with CM.
	\end{thm}
	
	Theorem \ref{thm-isogenygraphs} is simply a graphical reformulation of Theorem \ref{thm-kenku}. A detailed proof is found in Section 6 of \cite{gcal-r}. The main theorem of \cite{gcal-r} was the classification of the isogeny-torsion graphs that occur over $\QQ$.
	
	\begin{thm}[\cite{gcal-r}, Theorem 1.3] \label{thm-isogenytorsiongraphs} There are $52$ isomorphism types of isogeny-torsion graphs that are associated to elliptic curves defined over $\Q$. In particular, there are $23$ types of $L_k$ graphs, $13$ types of $T_k$ graphs, $12$ types of $R_k$ graphs, and $4$ types of $S$ graphs. Moreover, there are $16$ isomorphism types of isogeny-torsion graphs that are associated to elliptic curves over $\QQ$ with complex multiplication.
	\end{thm}
	
	\section{2-adic images attached to isogeny-torsion graphs without CM}
	
	The first task will be to classify the images of the $2$-adic Galois representations attached to non-CM isogeny-torsion graphs of $L_{1}, L_{2}(2)$, $T_{4}$, $T_{6}$, and $T_{8}$ type; these are the isogeny-torsion graphs of $2$-primary degree. All arrangements of $2$-adic images attached to $\QQ$-isogeny classes of elliptic curves over $\QQ$ is an arrangement coming from one of these five types of graphs. Each non-CM isogeny-torsion graph over $\QQ$ has one of the five isogeny-torsion graphs, as its largest $2$-adic subgraph. Let $\mathcal{E}$ be a $\QQ$-isogeny class of elliptic curves over $\QQ$ and let $\mathcal{G}$ be the isogeny-torsion graph associated to $\mathcal{E}$. Then if no elliptic curve in $\mathcal{E}$ has a point of order $2$ then $L_{1}$ is the largest $2$-adic subgraph of $\mathcal{G}$. If all elliptic curves in $\mathcal{E}$ have a point of order $2$ defined over $\QQ$ and no elliptic curve in $\mathcal{E}$ has full two-torsion defined over $\QQ$, then $L_{2}(2)$ is the largest $2$-adic subgraph of $\mathcal{G}$. If $\mathcal{E}$ contains an elliptic curve $E\QQ$ with full two-torsion defined over $\QQ$ but $E$ does not have a $\QQ$-rational subgroup of order $4$, then $T_{4}$ is the largest $2$-adic subgraph of $\mathcal{G}$. If $\mathcal{E}$ contains two and only two elliptic curves over $\QQ$ with full two-torsion defined over $\QQ$ and a cyclic, $\QQ$-rational subgroup of order $4$, then $\mathcal{G}$ is of type $T_{6}$. If $\mathcal{E}$ contains three distinct elliptic curves with full two-torsion defined over $\QQ$, then $\mathcal{G}$ is of $T_{8}$ type.
	
	The process is the following: if $E/\QQ$ is an elliptic curve such that the $\QQ$-isogeny class of $E$ contains one and only one curve, then the isogeny-torsion graph associated to (the $\QQ$-isogeny class of) $E$ is of $L_{1}$ type and the $2$-adic image attached to $E$ is the $\QQ$-adic image attached to the isogeny-torsion graph of $E$. Otherwise, let $\mathcal{G}$ be an isogeny-torsion graph of $L_{2}(2)$, $T_{4}$, $T_{6}$, or $T_{8}$ type. We use the image of the $2$-adic Galois representation of one of the curves in $\mathcal{G}$ to compute the image of all of the others. Actually, our work is mostly cut out for us. The LMFDB \cite{lmfdb} has classified the images of $2$-adic Galois representation of all isogeny-torsion graphs of $T_{8}$ type. The LMFDB has classified the images of $2$-adic Galois representation of all but one isogeny-torsion graph of $T_{6}$ type, all but four isogeny-torsion graphs of $T_{4}$ type, and all but seven isogeny-torsion graphs of $L_{2}(2)$ type.
	
	\begin{lemma}\label{2-adic image corollary 1}
	Let $E/\QQ$ be an elliptic curve with a point $Q_{2}$ of order $2$ defined over $\QQ$. Then there is a basis $\{P_{64}, Q_{64}\}$ of $E[64]$ such that $\overline{\rho}_{E,64}(G_{\QQ}) = \left\langle \begin{bmatrix} A_{1} & C_{1} \\ B_{1} & D_{1} \end{bmatrix}, \ldots, \begin{bmatrix}
	A_{s} & C_{s} \\ B_{s} & D_{s}
	\end{bmatrix} \right\rangle$ where $2$ divides $C_{1}$, \ldots, $C_{s}$. Moreover, $\overline{\rho}_{E / \left\langle Q_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to $\left\langle \begin{bmatrix} A_{1} & \frac{C_{1}}{2} \\ 2 \cdot B_{1} & D_{1} \end{bmatrix}, \ldots, \begin{bmatrix}
	A_{s} & \frac{C_{s}}{2} \\ 2 \cdot B_{s} & D_{s}
	\end{bmatrix} \right\rangle$.
	\end{lemma}
	
	\begin{proof}
	This follows from the first and third parts of Lemma \ref{ell-adic images} with $\ell = 2$.
	\end{proof}
	
	\begin{lemma}\label{2-adic image corollary 2}
	
	Let $E/\QQ$ be an elliptic curve with full two-torsion defined over $\QQ$. Then there is a basis $\{P_{64}, Q_{64}\}$ of $E[64]$ such that $\overline{\rho}_{E,64} = \left\langle \begin{bmatrix}
	A_{1} & C_{1} \\ B_{1} & D_{1}
	\end{bmatrix}, \ldots, \begin{bmatrix} A_{s} & C_{s} \\ B_{s} & D_{s} \end{bmatrix} \right\rangle$ where $A_{1}$, \ldots, $A_{s}$, $D_{1}$, \ldots, $D_{s}$ are odd and $B_{1}$, \ldots, $B_{s}$, $C_{1}$, \ldots, $C_{s}$ are even. Moreover,
	\begin{enumerate}
	
	    \item $\overline{\rho}_{E / \left\langle Q_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to $\left\langle \begin{bmatrix} A_{1} & \frac{C_{1}}{2} \\ 2 \cdot B_{1} & D_{1} \end{bmatrix}, \ldots, \begin{bmatrix}
	A_{s} & \frac{C_{s}}{2} \\ 2 \cdot B_{s} & D_{s}
	\end{bmatrix} \right\rangle$.
	
	    \item $\overline{\rho}_{E / \left\langle P_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to $\left\langle \begin{bmatrix} D_{1} & \frac{B_{1}}{2} \\ 2 \cdot C_{1} & A_{1} \end{bmatrix}, \ldots, \begin{bmatrix}
	    D_{s} & \frac{B_{s}}{2} \\ 2 \cdot C_{s} & A_{s}
	    \end{bmatrix} \right\rangle$.
	    
	    \item $\overline{\rho}_{E / \left\langle P_{2} + Q_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to $\left\langle \begin{bmatrix} A_{1}-B_{1} & \frac{A_{1}+C_{1}-B_{1}-D_{1}}{2} \\ 2 \cdot B_{1} & B_{1}+D_{1} \end{bmatrix}, \ldots, \begin{bmatrix} A_{s}-B_{s} & \frac{A_{s}+C_{s}-B_{s}-D_{s}}{2} \\ 2 \cdot B_{s} & B_{s}+D_{s} \end{bmatrix} \right\rangle$.
	    
	\end{enumerate}
	
	\end{lemma}
	
	\begin{proof}
	
	Let $P_{64}$ be a point on $E$ such that $[32]P_{64} = P_{2}$ and let $Q_{64}$ be a point on $E$ such that $[32]Q_{64} = Q_{2}$. Let $\sigma$ be a Galois automorphism. Then there are integers $A$ and $B$ such that $\sigma(P_{64}) = [A]P_{64}+[B]Q_{64}$. Note that as $P_{2}$ is defined over $\QQ$,
	$$P_{2} = \sigma(P_{2}) = \sigma([32]P_{64}) = [32]\sigma(P_{64}) = [32]([A]P_{64}+[B]Q_{64}] = [A]P_{2}+[B]Q_{2}.$$
	Then $A$ must be odd and $B$ must be even. A very similar computation shows that there is an even integer $C$ and an odd integer $D$ such that $\sigma(Q_{64}) = [C]P_{64}+[D]Q_{64}$. We break up the rest of the proof into steps.
	
	\begin{enumerate}
	    \item The first part follows from the first and third parts of Lemma \ref{ell-adic images} with $\ell = 2$ and $r = 1$.
	    
	    \item If we rewrite $E[64] = \left\langle Q_{64}, P_{64} \right\rangle$, then $\overline{\rho}_{E,64}(\sigma) = \begin{bmatrix} D & B \\ C & A \end{bmatrix}$. The rest of the part of the theorem follows from the first and third parts of Lemma \ref{ell-adic images} with $\ell = 2$ and $r = 1$.
	    
	    \item Note that $\sigma(P_{64}) = [A]P_{64}+[B]Q_{64} = [A-B]P_{64}+[B](P_{64}+Q_{64})$ and
	    $$\sigma(P_{64}+Q_{64}) = [A+C]P_{64}+[B+D]Q_{64} = [A+C-B-D]P_{64}+[B+D](P_{64}+Q_{64}).$$
	    As $A$ and $D$ are odd and $B$ and $C$ are even, $A+C-B-D$ is even. If we rewrite $E[64] = \left\langle P_{64}, P_{64}+Q_{64} \right\rangle$, then $\overline{\rho}_{E,64}(\sigma) = \begin{bmatrix} A-B & A+C-B-D \\ B & B+D \end{bmatrix}$. Then by Lemma \ref{ell-adic images} with $\ell = 2$, $\overline{\rho}_{E / \left\langle P_{2} + Q_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to $\left\langle \begin{bmatrix} A_{1}-B_{1} & \frac{A_{1}+C_{1}-B_{1}-D_{1}}{2} \\ 2 \cdot B_{1} & B_{1}+D_{1} \end{bmatrix}, \ldots, \begin{bmatrix} A_{s}-B_{s} & \frac{A_{s}+C_{s}-B_{s}-D_{s}}{2} \\ 2 \cdot B_{s} & B_{s}+D_{s} \end{bmatrix} \right\rangle$ and $r = 1$.
	\end{enumerate}
	
	\end{proof}
	
	\begin{lemma}\label{2-adic image corollary 3}
	Let $E/\QQ$ be an elliptic curve with full two-torsion defined over $\QQ$ and a cyclic, $\QQ$-rational, subgroup of order $4$, generated by a point $Q_{4}$ on $E$. Then there is a basis $\{P_{128}, Q_{128}\}$ of $E[128]$ such that $\overline{\rho}_{E,128}(G_{\QQ}) = \left\langle \begin{bmatrix} A_{1} & C_{1} \\ B_{1} & D_{1} \end{bmatrix}, \ldots, \begin{bmatrix} A_{s} & C_{s} \\ B_{s} & D_{s} \end{bmatrix} \right\rangle$ where $A_{1}$, \ldots, $A_{s}$, $D_{1}$, \ldots, $D_{s}$ are odd, $B_{1}$, \ldots, $B_{s}$ are even, and $C_{1}$, \ldots, $C_{s}$ are divisible by $4$. Moreover,
	\end{lemma}
	
	\begin{enumerate}
	    \item $\overline{\rho}_{E/\left\langle Q_{4} \right\rangle,32}(G_{\QQ})$ is conjugate to $\left\langle \begin{bmatrix} A_{1} & \frac{C_{1}}{4} \\ 4 \cdot B_{1} & D_{1} \end{bmatrix}, \ldots, \begin{bmatrix} A_{s} & \frac{C_{s}}{4} \\ 4 \cdot B_{s} & D_{s} \end{bmatrix} \right\rangle$.
	    
	    \item $\overline{\rho}_{E / \left\langle P_{2}+Q_{4} \right\rangle,32}(G_{\QQ})$ is conjugate to $\left\langle \begin{bmatrix} A_{1} & \frac{C_{1}}{4} \\ 4 \cdot B_{1} & D_{1} \end{bmatrix}, \ldots, \begin{bmatrix} A_{s} & \frac{C_{s}}{4} \\ 4 \cdot B_{s} & D_{s} \end{bmatrix} \right\rangle$
	\end{enumerate}
	
	\begin{proof}
	By Lemma \ref{ell-adic images} with $\ell = 2$ and $r = 1$ and again with $\ell = 2$ and $r = 2$, there is a basis $\{P_{128}, Q_{128}\}$ of $E[128]$ such that for $\sigma \in G_{\QQ}$, $\sigma(P_{128}) = [A]P_{128} + [B]Q_{128}$ and $\sigma(Q_{128}) = [C]P_{128} + [D]Q_{128}$ such that $A$ and $D$ are odd, $2$ divides $B$, and $4$ divides $C$. Thus, there are integers $A_{1}$, \ldots, $A_{s}$, $B_{1}$, \ldots, $B_{s}$, $C_{1}$, \ldots, $C_{s}$, $D_{1}$, \ldots, $D_{s}$ such that $A_{1}$, \ldots, $A_{s}$, $D_{1}$, \ldots, $D_{s}$ are odd, $2$ divides $B_{1}$, \ldots, $B_{s}$ and $4$ divides $C_{1}$, \ldots, $C_{s}$ and $\overline{\rho}_{E,128}(G_{\QQ}) = \left\langle \begin{bmatrix} A_{1} & C_{1} \\ B_{1} & D_{1} \end{bmatrix}, \ldots, \begin{bmatrix} A_{s} & C_{s} \\ B_{s} & D_{s} \end{bmatrix} \right\rangle$. We break up the rest of the proof into steps.
	
	\begin{enumerate}
	\item By the third part of Lemma \ref{ell-adic images}, with $\ell = 2$ and $r = 2$, we have that $\overline{\rho}_{E / \left\langle Q_{4} \right\rangle,32}(G_{\QQ})$ is conjugate to $\left\langle \begin{bmatrix} A_{1} & \frac{C_{1}}{4} \\ 4 \cdot B_{1} & D_{1} \end{bmatrix}, \ldots, \begin{bmatrix} A_{s} & \frac{C_{s}}{4} \\ 4 \cdot B_{s} & D_{s} \end{bmatrix} \right\rangle$.
	
	\item Next, $P_{2}+Q_{4}$ also generates a $\QQ$-rational subgroup of $E$ of order $4$. Then $\{P_{128}, [2]P_{128}+Q_{128}\}$ is a basis of $E[128]$. With this basis, $\overline{\rho}_{E,128}(G_{\QQ})$ is conjugate to
	$$\left\langle
	\begin{bmatrix} A_{1}-2B_{1} & 2A_{1}+C_{1}-4B_{1}-2D_{1} \\ B_{1} & 2B_{1}+D_{1} \end{bmatrix}, \ldots, \begin{bmatrix} A_{s}-2B_{s} & 2A_{s}+C_{s}-4B_{s}-2D_{s} \\ B_{s} & 2B_{s}+D_{s} \end{bmatrix}
	\right\rangle.$$
	Note that for all $i = 1$, \ldots, $s$, $A_{i}$ and $D_{i}$ are odd, $B_{i}$ is even, and $D_{i}$ is divisible by $4$. Thus,  $2A_{i}+C_{i}-4B_{i}-2D_{i}$ is divisible by $4$ for all $i = 1$, \ldots, $s$. By Lemma \ref{ell-adic images} with $\ell = 2$ and $r = 2$, we have $\overline{\rho}_{E/\left\langle P_{2}+Q_{4} \right\rangle}(G_{\QQ})$ is conjugate to
	$$\left\langle
	\begin{bmatrix} A_{1}-2B_{1} & \frac{2A_{1}+C_{1}-4B_{1}-2D_{1}}{4} \\ 4 \cdot B_{1} & 2B_{1}+D_{1} \end{bmatrix}, \ldots, \begin{bmatrix} A_{s}-2B_{s} & \frac{2A_{s}+C_{s}-4B_{s}-2D_{s}}{4} \\ 4 \cdot B_{s} & 2B_{s}+D_{s} \end{bmatrix}
	\right\rangle.$$
	\end{enumerate}
	\end{proof}
    
    \subsection{Isogeny-torsion graphs of $L_{1}$ type}
    
    Table \ref{2-adic Images of L1 Graphs}  classifies the $2$-adic images of all elliptic curves over $\QQ$ in an isogeny-torsion graph of $L_{1}$ type. The groups of the form $\operatorname{H}_{n}$ come from the RZB and the notation right next to them come from the LMFDB nomenclature. There are $22$ distinct arrangements of $2$-adic groups, $14$ of these arrangements contain groups with $\operatorname{-Id}$. In other words, each of the $22$ arrangements of groups in Table \ref{2-adic Images of L22 Graphs} are a quadratic twist of one of the $14$ arrangements of groups that contain $\operatorname{-Id}$. Two examples do not appear in the LMFDB.
    
    The groups $\operatorname{H}_{1}$, $\operatorname{H}_{4}$, $\operatorname{H}_{5}$, $\operatorname{H}_{7}$, $\operatorname{H}_{22}$, $\operatorname{H}_{55}$, $\operatorname{H}_{56}$, $\operatorname{H}_{177}$, $\operatorname{H}_{178}$, and $\operatorname{H}_{441}$ have no non-trivial quadratic twists. In other words, these groups contain $\operatorname{-Id}$ and multiplying some elements of these groups by $\operatorname{-Id}$ does not generate a different group.
    
    The following shows the reduction containment of all of the groups in Table \ref{2-adic Images of L1 Graphs} with $\operatorname{-Id}$

\begin{center}    
\begin{tikzcd}
                     &                        & \operatorname{H}_{1} \arrow[ld, no head] \arrow[d, no head] \arrow[rd, no head] \arrow[lld, no head] \arrow[rrd, no head] \arrow[rrrd, no head] &                                             &                                            &                                 \\
\operatorname{H}_{2} & \operatorname{H}_{3}   & \operatorname{H}_{4}                                                                      & \operatorname{H}_{5}                        & \operatorname{H}_{7} \arrow[ld, no head] \arrow[rd, no head] & \operatorname{H}_{20}           \\
                     &                        &                                                                                           & \operatorname{H}_{22} \arrow[ld, no head] \arrow[rd, no head] &                                            & \operatorname{H}_{55} \arrow[d, no head] \\
                     &                        & \operatorname{H}_{56} \arrow[ld, no head] \arrow[rd, no head]                                               &                                             & \operatorname{H}_{57}                      & \operatorname{H}_{441}          \\
                     & \operatorname{H}_{177} &                                                                                           & \operatorname{H}_{178}                      &                                            &                                
\end{tikzcd}
\end{center}
    
    \begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.7}{
    \begin{tabular}{|c|c|c|}

\hline

Isogeny-Torsion Graph & $E$ & Example Isogeny Class \\
    \hline
\multirow{22}*{$([1])$} & $\operatorname{H}_{1}$ & \texttt{37.a} \\
\cline{2-3}
& $\operatorname{H}_{2} = \texttt{2.2.0.1}$ & \texttt{392.a} \\
\cline{2-3}
& $\operatorname{H}_{2a} = \texttt{4.4.0.2}$ & \texttt{392.c} \\
\cline{2-3}
& $\operatorname{H}_{2b} = \texttt{8.4.0.1}$ & \texttt{3136.b} \\
\cline{2-3}
& $\operatorname{H}_{3} = \texttt{4.2.0.1}$ & \texttt{567.a} \\
\cline{2-3}
& $\operatorname{H}_{3a} = \texttt{4.4.0.3}$ & \texttt{2738.b} \\
\cline{2-3}
& $\operatorname{H}_{3b} = \texttt{8.4.0.2}$ & \texttt{2116.c} \\
\cline{2-3}
& $\operatorname{H}_{4} = \texttt{8.2.0.1}$ & \texttt{200.a} \\
\cline{2-3}
& $\operatorname{H}_{5} = \texttt{8.2.0.2}$ & \texttt{1682.a} \\
\cline{2-3}
& $\operatorname{H}_{7} = \texttt{4.4.0.1}$ & \texttt{216.a} \\
\cline{2-3}
& $\operatorname{H}_{20} = \texttt{4.8.0.2}$ & \texttt{648.d} \\
\cline{2-3}
& $\operatorname{H}_{20a} = \texttt{8.16.0.3}$ & \texttt{5184.u} \\
\cline{2-3}
& $\operatorname{H}_{20b} = \texttt{4.16.0.2}$ & \texttt{648.b} \\
\cline{2-3}
& $\operatorname{H}_{22} = \texttt{8.8.0.1}$ & \texttt{44800.r} \\
\cline{2-3}
& $\operatorname{H}_{55} = \texttt{8.16.0.1}$ & \texttt{3388.f} \\
\cline{2-3}
& $\operatorname{H}_{56} = \texttt{16.16.0.1}$ & \texttt{3628800.bg} \\
\cline{2-3}
& $\operatorname{H}_{57} = \texttt{16.16.0.2}$ & \texttt{6400.b} \\
\cline{2-3}
& $\operatorname{H}_{57a} = \texttt{32.32.0.3}$ & \texttt{6400.p} \\
\cline{2-3}
& $\operatorname{H}_{57b} = \texttt{32.32.0.4}$ & \texttt{6400.c} \\
\cline{2-3}
& $\operatorname{H}_{177}$ & $y^{2} = x^{3} - 340750x - 76560000$ \\
\cline{2-3}
& $\operatorname{H}_{178} = \texttt{32.32.0.1}$ & \texttt{20736.e} \\
\cline{2-3}
& $\operatorname{H}_{441}$ & $y^{2}+y = x^{3} - 3014658660x+150916472601529$ \\
\hline
\end{tabular}}
\caption{2-adic Images of $L_{1}$ Graphs}
\label{2-adic Images of L1 Graphs}
\end{table}
\end{center}

    
    \subsection{Isogeny-torsion graphs of $L_{2}(2)$ type}
    
    \begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.33}{
    \begin{tabular}{|c|c|c|c|c|}
\hline
Isogeny Graph & Isogeny-Torsion Graph & $E_{1}$ & $E_{2}$ & Example Isogeny Class \\
\hline
\multirow{80}*{\includegraphics[scale=0.1]{L22 graph.png}} & \multirow{80}*{$([2],[2])$} & $\operatorname{H}_{6} = \texttt{2.3.0.1}$ & $\operatorname{H}_{6} = \texttt{2.3.0.1}$ & \texttt{69.a} \\
\cline{3-5}
& & $\operatorname{H}_{9} = \texttt{4.6.0.3}$ & $\operatorname{H}_{10} = \texttt{4.6.0.5}$ & \texttt{325.d} \\
\cline{3-5}
& & $\operatorname{H}_{9a} = \texttt{8.12.0.24}$ & $\operatorname{H}_{10c} = \texttt{8.12.0.38}$ & \texttt{676.c} \\
\cline{3-5}
& & $\operatorname{H}_{9b} = \texttt{8.12.0.23}$ & $\operatorname{H}_{10b} = \texttt{4.12.0.6}$ & \texttt{1600.t} \\
\cline{3-5}
& & $\operatorname{H}_{9c} = \texttt{8.12.0.22}$ & $\operatorname{H}_{10a} = \texttt{8.12.0.37}$ & \texttt{52.a} \\
\cline{3-5}
& & $\operatorname{H}_{9d} = \texttt{8.12.0.21}$ & $\operatorname{H}_{10d} = \texttt{4.12.0.12}$ & \texttt{136.a} \\
\cline{3-5}
& & $\operatorname{H}_{11} = \texttt{4.6.0.4}$ & $\operatorname{H}_{11} = \texttt{4.6.0.4}$ & \texttt{2772.m} \\
\cline{3-5}
& & $\operatorname{H}_{12} = \texttt{4.6.0.2}$ & $\operatorname{H}_{12} = \texttt{4.6.0.2}$ & \texttt{2200.i} \\
\cline{3-5}
& & $\operatorname{H}_{14} = \texttt{8.6.0.2}$ & $\operatorname{H}_{14} = \texttt{8.6.0.2}$ & \texttt{1152.n} \\
\cline{3-5}
& & $\operatorname{H}_{15} = \texttt{8.6.0.4}$ & $\operatorname{H}_{19} = \texttt{8.6.0.5}$ & \texttt{102.a} \\
\cline{3-5}
& & $\operatorname{H}_{16} = \texttt{8.6.0.1}$ & $\operatorname{H}_{17} = \texttt{8.6.0.6}$ & \texttt{46.a} \\
\cline{3-5}
& & $\operatorname{H}_{18} = \texttt{8.6.0.3}$ & $\operatorname{H}_{18} = \texttt{8.6.0.3}$ & \texttt{490.f} \\
\cline{3-5}
& & $\operatorname{H}_{23} = \texttt{4.12.0.11}$ & $\operatorname{H}_{43} = \texttt{8.12.0.27}$ & \texttt{1176.b} \\
\cline{3-5}
& & $\operatorname{H}_{26} = \texttt{4.12.0.5}$ & $\operatorname{H}_{28} = \texttt{8.12.0.33}$ & \texttt{468.e} \\
\cline{3-5}
& & $\operatorname{H}_{29} = \texttt{8.12.0.35}$ & $\operatorname{H}_{41} = \texttt{8.12.0.36}$ & \texttt{17664.f} \\
\cline{3-5}
& & $\operatorname{H}_{30} = \texttt{8.12.0.17}$ & $\operatorname{H}_{30} = \texttt{8.12.0.17}$ & \texttt{63075.t} \\
\cline{3-5}
& & $\operatorname{H}_{31} = \texttt{8.12.0.18}$ & $\operatorname{H}_{31} = \texttt{8.12.0.18}$ & \texttt{2312.c} \\
\cline{3-5}
& & $\operatorname{H}_{35} = \texttt{8.12.0.32}$ & $\operatorname{H}_{49} = \texttt{8.12.0.28}$ & \texttt{300.d} \\
\cline{3-5}
& & $\operatorname{H}_{37} = \texttt{8.12.0.26}$ & $\operatorname{H}_{42} = \texttt{8.12.0.39}$ & \texttt{4480.a} \\
\cline{3-5}
& & $\operatorname{H}_{37a} = \texttt{16.24.0.30}$ & $\operatorname{H}_{42a} = \texttt{16.24.0.44}$ & \texttt{3200.f} \\
\cline{3-5}
& & $\operatorname{H}_{37b} = \texttt{8.24.0.126}$ & $\operatorname{H}_{42b} = \texttt{8.24.0.43}$ & \texttt{640.g} \\
\cline{3-5}
& & $\operatorname{H}_{37c} = \texttt{16.24.0.29}$ & $\operatorname{H}_{42c} = \texttt{16.24.0.43}$ & \texttt{3200.w} \\
\cline{3-5}
& & $\operatorname{H}_{37d} = \texttt{8.24.0.124}$ & $\operatorname{H}_{42d} = \texttt{8.24.0.85}$ & \texttt{640.h} \\
\cline{3-5}
& & $\operatorname{H}_{39} = \texttt{8.12.0.29}$ & $\operatorname{H}_{45} = \texttt{8.12.0.31}$ & \texttt{1575.g} \\
\cline{3-5}
& & $\operatorname{H}_{40} = \texttt{8.12.0.19}$ & $\operatorname{H}_{40} = \texttt{8.12.0.19}$ & \texttt{16128.bi} \\
\cline{3-5}
& & $\operatorname{H}_{40a} = \texttt{16.24.0.23}$ & $\operatorname{H}_{40b} = \texttt{16.24.0.24}$ & \texttt{1792.e} \\
\cline{3-5}
& & $\operatorname{H}_{40c} = \texttt{16.24.0.26}$ & $\operatorname{H}_{40c} = \texttt{16.24.0.26}$ & \texttt{12544.e} \\
\cline{3-5}
& & $\operatorname{H}_{40d} = \texttt{16.24.0.25}$ & $\operatorname{H}_{40d} = \texttt{16.24.0.25}$ & \texttt{12544.p} \\
\cline{3-5}
& & $\operatorname{H}_{47} = \texttt{8.12.0.30}$ & $\operatorname{H}_{47} = \texttt{8.12.0.30}$ & \texttt{1800.w} \\
\cline{3-5}
& & $\operatorname{H}_{50} = \texttt{8.12.0.34}$ & $\operatorname{H}_{50} = \texttt{8.12.0.34}$ & \texttt{71148.s} \\
\cline{3-5}
& & $\operatorname{H}_{63} = \texttt{8.24.0.135}$ & $\operatorname{H}_{70} = \texttt{8.24.0.131}$ & \texttt{2400.p} \\
\cline{3-5}
& & $\operatorname{H}_{64} = \texttt{8.24.0.79}$ & $\operatorname{H}_{64} = \texttt{8.24.0.79}$ & \texttt{424830.dp} \\
\cline{3-5}
& & $\operatorname{H}_{65} = \texttt{8.24.0.84}$ & $\operatorname{H}_{71} = \texttt{8.24.0.127}$ & \texttt{867.a} \\
\cline{3-5}
& & $\operatorname{H}_{68} = \texttt{8.24.0.82}$ & $\operatorname{H}_{74} = \texttt{8.24.0.39}$ & \texttt{16810.c} \\
\cline{3-5}
& & $\operatorname{H}_{69} = \texttt{8.24.0.83}$ & $\operatorname{H}_{91} = \texttt{8.24.0.128}$ & \texttt{11109.g} \\
\cline{3-5}
& & $\operatorname{H}_{73} = \texttt{8.24.0.41}$ & $\operatorname{H}_{90} = \texttt{8.24.0.136}$ & \texttt{16940.b} \\
\cline{3-5}
& & $\operatorname{H}_{76} = \texttt{8.24.0.80}$ & $\operatorname{H}_{82} = \texttt{8.24.0.130}$ & \texttt{19200.a} \\
\cline{3-5}
& & $\operatorname{H}_{76a} = \texttt{8.48.0.207}$ & $\operatorname{H}_{82b} = \texttt{16.48.0.246}$ & \texttt{2304.k} \\
\cline{3-5}
& & $\operatorname{H}_{76b} = \texttt{8.48.0.206}$ & $\operatorname{H}_{82c} = \texttt{16.48.0.247}$ & \texttt{768.b} \\
\cline{3-5}
& & $\operatorname{H}_{76c} = \texttt{8.48.0.208}$ & $\operatorname{H}_{82d} = \texttt{16.48.0.245}$ & \texttt{2304.f} \\
\cline{3-5}
& & $\operatorname{H}_{76d} = \texttt{8.48.0.205}$ & $\operatorname{H}_{82a} = \texttt{16.48.0.244}$ & \texttt{768.g} \\
\cline{3-5}
& & $\operatorname{H}_{77} = \texttt{8.24.0.129}$ & $\operatorname{H}_{80} = \texttt{8.24.0.81}$ & \texttt{5376.c} \\
\cline{3-5}
& & $\operatorname{H}_{81} = \texttt{8.24.0.137}$ & $\operatorname{H}_{83} = \texttt{8.24.0.37}$ & \texttt{202496.e} \\
\cline{3-5}
& & $\operatorname{H}_{89} = \texttt{8.24.0.122}$ & $\operatorname{H}_{93} = \texttt{8.24.0.119}$ & \texttt{4056.k} \\
\cline{3-5}
& & $\operatorname{H}_{97}$ & $\operatorname{H}_{97}$ & $y^{2} = x^{3} - 558481500x - 5079892400000$ \\
\cline{3-5}
& & $\operatorname{H}_{103} = \texttt{16.24.0.21}$ & $\operatorname{H}_{104} = \texttt{16.24.0.22}$ & \texttt{4225.e} \\
\cline{3-5}
& & $\operatorname{H}_{105} = \texttt{16.24.0.33}$ & $\operatorname{H}_{112} = \texttt{16.24.0.36}$ & \texttt{4606.e} \\
\cline{3-5}
& & $\operatorname{H}_{106} = \texttt{16.24.0.31}$ & $\operatorname{H}_{111} = \texttt{16.24.0.38}$ & \texttt{2016.c} \\
\cline{3-5}
& & $\operatorname{H}_{107} = \texttt{16.24.0.34}$ & $\operatorname{H}_{110} = \texttt{16.24.0.35}$ & \texttt{3038.c} \\
\cline{3-5}
& & $\operatorname{H}_{108} = \texttt{16.24.0.41}$ & $\operatorname{H}_{123} = \texttt{16.24.0.28}$ & \texttt{10880.ba} \\
\cline{3-5}
& & $\operatorname{H}_{108a} = \texttt{32.48.0.24
}$ & $\operatorname{H}_{123e} = \texttt{32.48.0.20}$ & \texttt{21632.bc} \\
\cline{3-5}
& & $\operatorname{H}_{108b} = \texttt{16.48.0.80}$ & $\operatorname{H}_{123d} = \texttt{16.48.0.236}$ & \texttt{1664.o} \\
\cline{3-5}
& & $\operatorname{H}_{108c} = \texttt{32.48.0.23}$ & $\operatorname{H}_{123a} = \texttt{32.48.0.19}$ & \texttt{21632.bl} \\
\cline{3-5}
& & $\operatorname{H}_{108d} = \texttt{16.48.0.81}$ & $\operatorname{H}_{123c} = \texttt{16.48.0.237}$ & \texttt{1664.d} \\
\cline{3-5}
& & $\operatorname{H}_{108e} = \texttt{16.48.0.24}$ & $\operatorname{H}_{123f} = \texttt{16.48.0.241}$ & \texttt{1664.e} \\
\cline{3-5}
& & $\operatorname{H}_{108f} = \texttt{16.48.0.23}$ & $\operatorname{H}_{123b} = \texttt{16.48.0.240}$ & \texttt{1664.r} \\
\cline{3-5}
& & $\operatorname{H}_{109} = \texttt{16.24.0.37}$ & $\operatorname{H}_{124} = \texttt{16.24.0.32}$ & \texttt{700.f} \\
\cline{3-5}
& & $\operatorname{H}_{113}$ & $\operatorname{H}_{114}$ & $y^{2} + xy = x^{3} - x^{2} - 785472x - 267747760$ \\
\cline{3-5}
& & $\operatorname{H}_{191} = \texttt{8.48.0.203}$ & $\operatorname{H}_{196} = \texttt{8.48.0.204}$ & \texttt{294.b} \\
\cline{3-5}
& & $\operatorname{H}_{216} = \texttt{16.48.0.242}$ & $\operatorname{H}_{224} = \texttt{16.48.0.79}$ & \texttt{13056.e} \\
\cline{3-5}
& & $\operatorname{H}_{218} = \texttt{16.48.0.248}$ & $\operatorname{H}_{237} = \texttt{16.48.0.21}$ & \texttt{147712.d} \\
\cline{3-5}
& & $\operatorname{H}_{220} = \texttt{16.48.0.249}$ & $\operatorname{H}_{232} = \texttt{16.48.0.22}$ & \texttt{4352.f} \\
\cline{3-5}
& & $\operatorname{H}_{238} = \texttt{32.48.0.21}$ & $\operatorname{H}_{239} = \texttt{32.48.0.18}$ & \texttt{1152.r} \\
\cline{3-5}
& & $\operatorname{H}_{238a} = \texttt{32.96.0.25}$ & $\operatorname{H}_{239b} = \texttt{32.96.0.102}$ & \texttt{128.c} \\
\cline{3-5}
& & $\operatorname{H}_{238b} = \texttt{32.96.0.1}$ & $\operatorname{H}_{239a} = \texttt{32.96.0.106}$ & \texttt{128.d} \\
\cline{3-5}
& & $\operatorname{H}_{238c} = \texttt{32.96.0.3}$ & $\operatorname{H}_{239d} = \texttt{32.96.0.108}$ & \texttt{128.b} \\
\cline{3-5}
& & $\operatorname{H}_{238d} = \texttt{32.96.0.27}$ & $\operatorname{H}_{239c} = \texttt{32.96.0.104}$ & \texttt{128.a} \\
\cline{3-5}
& & $\operatorname{H}_{281} = \texttt{16.48.1.146}$ & $\operatorname{H}_{349} = \texttt{16.48.1.5}$ & \texttt{122740.j} \\
\cline{3-5}
& & $\operatorname{H}_{284}$ & $\operatorname{H}_{350}$ & $y^2 = x^3 - 1725814293280x + 872648220992027997$ \\
\cline{3-5}
& & $\operatorname{H}_{288}$ & $\operatorname{H}_{323}$ & $y^{2} + xy = x^{3} + x^{2} - 1163177961056300788x - 365926510640189061755312483$ \\
\cline{3-5}
& & $\operatorname{H}_{289} = \texttt{16.48.1.118}$ & $\operatorname{H}_{320} = \texttt{16.48.1.35}$ & \texttt{4046.n} \\
\cline{3-5}
& & $\operatorname{H}_{291}$ & $\operatorname{H}_{324}$ & $y^{2} + xy + y = x^{3} + x^{2} - 70411166718x + 7186776239309115$ \\
\cline{3-5}
& & $\operatorname{H}_{295}$ & $\operatorname{H}_{297}$ & $y^{2} = x^{3} + x^{2} - 6740460588x - 200219177111472$ \\
\cline{3-5}
& & $\operatorname{H}_{302}$ & $\operatorname{H}_{326}$ & $y^{2} = x^{3} + x^{2} - 7859386910x - 268185327947856$ \\
\cline{3-5}
& & $\operatorname{H}_{304} = \texttt{16.48.1.129}$ & $\operatorname{H}_{309} = \texttt{16.48.1.136}$ & \texttt{16128.y} \\
\cline{3-5}
& & $\operatorname{H}_{308} = \texttt{16.48.1.132}$ & $\operatorname{H}_{312} = \texttt{16.48.1.133}$ & \texttt{173600.bn} \\
\cline{3-5}
& & $\operatorname{H}_{318} = \texttt{16.48.1.40}$ & $\operatorname{H}_{328} = \texttt{16.48.1.113}$ & \texttt{76614.h} \\
\cline{3-5}
& & $\operatorname{H}_{556} = \texttt{16.96.3.346}$ & $\operatorname{H}_{563} = \texttt{16.96.3.338}$ & \texttt{200.b} \\
\cline{3-5}
& & $\operatorname{H}_{558} = \texttt{16.96.3.343}$ & $\operatorname{H}_{566} = \texttt{16.96.3.335}$ & \texttt{3362.c} \\
\cline{3-5}
& & $\operatorname{H}_{619} = \texttt{32.96.3.230}$ & $\operatorname{H}_{649} = \texttt{32.96.3.82}$ & \texttt{17918.c} \\
\hline
\end{tabular}}
\caption{2-adic Images of $L_{2}(2)$ Graphs}
\label{2-adic Images of L22 Graphs}
\end{table}
\end{center}
    
Table \ref{2-adic Images of L22 Graphs} classifies the $2$-adic images of all elliptic curves over $\QQ$ in an isogeny-torsion graph of $L_{2}(2)$ type. The groups of the form $\operatorname{H}_{n}$ come from the RZB and the notation right next to them come from the LMFDB nomenclature. There are $80$ distinct arrangements of $2$-adic groups, $55$ of these arrangements contain groups with $\operatorname{-Id}$. In other words, each of the $80$ arrangements of groups in Table \ref{2-adic Images of L22 Graphs} are a quadratic twist of one of the $55$ arrangements of groups that contain $\operatorname{-Id}$.

There are seven arrangements of subgroups of $\operatorname{GL}(2, \ZZ_{2})$ that do not appear in the LMFDB. For all seven of the following cases, we will have $\QQ$-isogeny classes consisting of two elliptic curves, $E/\QQ$, which has a single point of order $2$, $Q_{2}$, defined over $\QQ$, and $E'/\QQ$. We will denote $E' = E / \left\langle Q_{2} \right\rangle$.

\begin{enumerate}
    \item $\operatorname{H}_{97} = \left\langle \begin{bmatrix} 1 & 3 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 3 \\ 2 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 1 \\ 6 & 3 \end{bmatrix} \right\rangle$
    
    Let $E/\QQ$ be an elliptic curve such that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to
    $\operatorname{H}_{97}$. Being careful of the right action in the RZB database, $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is actually conjugate to $H = \left\langle
    \begin{bmatrix} 1 & 0 \\ 3 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 2 \\ 3 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 6 \\ 1 & 3 \end{bmatrix}
    \right\rangle$. The RZB database says that $H$ is a group of level $8$. By the fact that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is a group of order $8$ and Lemma \ref{kernel of pi 1}, $\overline{\rho}_{E,64}(G_{\QQ})$ is conjugate to $\left\langle
    \begin{bmatrix} 1 & 0 \\ 3 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 2 \\ 3 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 6 \\ 1 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix}
    \right\rangle$.
    
    By Lemma \ref{2-adic image corollary 1}, we see that $\overline{\rho}_{E/\left\langle Q_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to the group $$\left\langle
    \begin{bmatrix} 1 & 0 \\ 6 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 1 \\ 6 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 3 \\ 2 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix}
    \right\rangle$$
    which is conjugate to $H$. Hence, $\overline{\rho}_{E/\left\langle Q_{2} \right\rangle,2^{\infty}}(G_{\QQ})$ is conjugate to $\operatorname{H}_{97}$ in the RZB database.
    
    \item $\operatorname{H}_{113} = \left\langle
    \begin{bmatrix} 1 & 3 \\ 12 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 1 \\ 12 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 4 & 5 \end{bmatrix},
    \begin{bmatrix} 1 & 3 \\ 14 & 7 \end{bmatrix}
    \right\rangle$
    
    Let $E/\QQ$ be an elliptic curve such that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to $\operatorname{H}_{113}$. Being careful of the right action in the RZB database, $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is actually conjugate to
    $$H = \left\langle \begin{bmatrix} 1 & 12 \\ 3 & 3 \end{bmatrix}, \begin{bmatrix} 1 & 12 \\ 1 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 4 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 14 \\ 3 & 7 \end{bmatrix} \right\rangle.$$
    The RZB database says that $H$ is a group of level $8$. By Lemma \ref{kernel of pi 1}, $\overline{\rho}_{E,64}(G_{\QQ})$ is conjugate to
    $$\left\langle \begin{bmatrix} 1 & 12 \\ 3 & 3 \end{bmatrix}, \begin{bmatrix} 1 & 12 \\ 1 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 4 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 14 \\ 3 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}, \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix} \right\rangle.$$
    By Lemma \ref{2-adic image corollary 1}, $\overline{\rho}_{E/\left\langle Q_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to
    $$\left\langle \begin{bmatrix} 1 & 6 \\ 6 & 3 \end{bmatrix}, \begin{bmatrix} 1 & 6 \\ 2 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 2 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 7 \\ 6 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}, \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix} \right\rangle$$
    which is conjugate to
    $$\left\langle
    \begin{bmatrix} 1 & 12 \\ 3 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 3 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 2 \\ 0 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 2 & 13 \end{bmatrix},
    \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}
    \right\rangle$$
    which is the full lift of $\left\langle
    \begin{bmatrix} 1 & 12 \\ 3 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 3 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 2 \\ 0 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 2 & 13 \end{bmatrix} \right\rangle$. The transpose of this group is conjugate to $\operatorname{H}_{114}$ in the RZB database.
    
    \item $\operatorname{H}_{284} = \left\langle
    \begin{bmatrix} 9 & 2 \\ 2 & 7 \end{bmatrix},
    \begin{bmatrix} 3 & 3 \\ 4 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 9 \\ 4 & 3 \end{bmatrix},
    \begin{bmatrix} 5 & 10 \\ 0 & 1 \end{bmatrix}
    \right\rangle$
    
    Let $E/\QQ$ be an elliptic curve such that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to $\operatorname{H}_{284}$. Being careful of the right action in the RZB database, $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to $H = \left\langle
    \begin{bmatrix} 9 & 2 \\ 2 & 7 \end{bmatrix},
    \begin{bmatrix} 3 & 4 \\ 3 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 4 \\ 9 & 3 \end{bmatrix},
    \begin{bmatrix} 5 & 0 \\ 10 & 1 \end{bmatrix}
    \right\rangle$. The RZB database says that $H$ is a group of level $16$. By Lemma \ref{kernel of pi 1}, $\overline{\rho}_{E,64}(G_{\QQ})$ is conjugate to
    $$\left\langle
    \begin{bmatrix} 9 & 2 \\ 2 & 7 \end{bmatrix},
    \begin{bmatrix} 3 & 4 \\ 3 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 4 \\ 9 & 3 \end{bmatrix},
    \begin{bmatrix} 5 & 0 \\ 10 & 1 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
    \right\rangle.$$
    By Lemma \ref{2-adic image corollary 1}, $\overline{\rho}_{E/\left\langle Q_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to
    $$\left\langle
    \begin{bmatrix} 9 & 1 \\ 4 & 7 \end{bmatrix},
    \begin{bmatrix} 3 & 2 \\ 6 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 2 \\ 18 & 3 \end{bmatrix},
    \begin{bmatrix} 5 & 0 \\ 20 & 1 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
    \right\rangle$$
    which is conjugate to
    $$\left\langle
    \begin{bmatrix} 1 & 10 \\ 3 & 15 \end{bmatrix},
    \begin{bmatrix} 1 & 2 \\ 6 & 11 \end{bmatrix},
    \begin{bmatrix} 1 & 12 \\ 5 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 2 \\ 2 & 11 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
    \right\rangle$$
    which is the full lift of $\left\langle
    \begin{bmatrix} 1 & 10 \\ 3 & 15 \end{bmatrix},
    \begin{bmatrix} 1 & 2 \\ 6 & 11 \end{bmatrix},
    \begin{bmatrix} 1 & 12 \\ 5 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 2 \\ 2 & 11 \end{bmatrix} \right\rangle$ to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{350}$ in the RZB database.
    
    \item $\operatorname{H}_{288} = \left\langle
    \begin{bmatrix} 9 & 2 \\ 2 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 10 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 9 \\ 2 & 7 \end{bmatrix}
    \right\rangle$
    
    Let $E/\QQ$ be an elliptic curve such that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to $\operatorname{H}_{288}$. Being careful of the right action in the RZB databse, $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to $H = \left\langle \begin{bmatrix} 9 & 2 \\ 2 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 0 \\ 10 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 2 \\ 9 & 7 \end{bmatrix} \right\rangle$. The RZB database says that $H$ is a group of level $16$. By Lemma \ref{kernel of pi 1}, $\overline{\rho}_{2,64}(G_{\QQ})$ is conjugate to
    $$\left\langle \begin{bmatrix} 9 & 2 \\ 2 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 0 \\ 10 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 2 \\ 9 & 7 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
    \right\rangle.$$
    By Lemma \ref{2-adic image corollary 1}, $\overline{\rho}_{E/\left\langle Q_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to
    $$\left\langle \begin{bmatrix} 9 & 1 \\ 4 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 0 \\ 20 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 1 \\ 18 & 7 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
    \right\rangle$$
    which is conjugate to
    $$\left\langle \begin{bmatrix} 9 & 1 \\ 4 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 0 \\ 20 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 1 \\ 18 & 7 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
    \right\rangle$$
    which is the full lift of $\begin{bmatrix} 9 & 1 \\ 4 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 0 \\ 20 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 1 \\ 18 & 7 \end{bmatrix}$ to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{323}$ in the RZB database.
    
    \item $\operatorname{H}_{291} = \left\langle
    \begin{bmatrix} 9 & 0 \\ 8 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 10 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 13 \\ 2 & 3 \end{bmatrix},
    \begin{bmatrix} 7 & 5 \\ 8 & 1 \end{bmatrix}\right\rangle$
    
    Let $E/\QQ$ be an elliptic curve such that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to $\operatorname{H}_{291}$. Being careful of the right action in the RZB database, $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to $H = \left\langle
    \begin{bmatrix} 9 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 0 \\ 10 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 2 \\ 13 & 3 \end{bmatrix},
    \begin{bmatrix} 7 & 8 \\ 5 & 1 \end{bmatrix}
    \right\rangle$. The RZB database says that $H$ is a group of level $16$. By Lemma \ref{kernel of pi 1}, $\overline{\rho}_{E,64}(G_{\QQ})$ is conjugate to
    $$\left\langle \begin{bmatrix} 9 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 0 \\ 10 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 2 \\ 13 & 3 \end{bmatrix},
    \begin{bmatrix} 7 & 8 \\ 5 & 1 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix} \right\rangle.$$
    By Lemma \ref{2-adic image corollary 1}, $\overline{\rho}_{E/\left\langle Q_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to
    $$\left\langle
    \begin{bmatrix} 9 & 4 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 0 \\ 20 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 1 \\ 26 & 3 \end{bmatrix},
    \begin{bmatrix} 7 & 4 \\ 10 & 1 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix} \right\rangle$$
    which is conjugate to
    $$\left\langle
    \begin{bmatrix} 9 & 4 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 0 \\ 20 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 1 \\ 26 & 3 \end{bmatrix},
    \begin{bmatrix} 7 & 4 \\ 10 & 1 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix} \right\rangle$$
    which is the full lift of $\begin{bmatrix} 9 & 4 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 0 \\ 20 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 1 \\ 26 & 3 \end{bmatrix},
    \begin{bmatrix} 7 & 4 \\ 10 & 1 \end{bmatrix}$ to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{324}$ in the RZB database.
    
    \item $\operatorname{H}_{295} = \left\langle \begin{bmatrix} 7 & 14 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 7 & 0 \\ 0 & 7 \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 5 \\ 6 & 3 \end{bmatrix}  \right\rangle$
    
    Let $E/\QQ$ be an elliptic curve such that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to $\operatorname{H}_{295}$. Being careful of the right action in the RZB database, $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to $H = \left\langle
    \begin{bmatrix} 7 & 0 \\ 14 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 0 \\ 0 & 7 \end{bmatrix},
    \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 6 \\ 5 & 3 \end{bmatrix}
    \right\rangle$. The RZB database says that $H$ is a group of level $16$. By Lemma \ref{kernel of pi 1}, $\overline{\rho}_{E,64}(G_{\QQ})$ is conjugate to
    $$\left\langle
    \begin{bmatrix} 7 & 0 \\ 14 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 0 \\ 0 & 7 \end{bmatrix},
    \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 6 \\ 5 & 3 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
    \right\rangle.$$
    By Lemma \ref{2-adic image corollary 1}, $\overline{\rho}_{E/\left\langle Q_{2} \right\rangle, 32}(G_{\QQ})$ is conjugate to
    $$\left\langle
    \begin{bmatrix} 7 & 0 \\ 28 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 0 \\ 0 & 7 \end{bmatrix},
    \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 3 \\ 10 & 3 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
    \right\rangle$$
    which is conjugate to
    $$\left\langle
    \begin{bmatrix} 7 & 0 \\ 10 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 0 \\ 0 & 3 \end{bmatrix},
    \begin{bmatrix} 5 & 2 \\ 3 & 1 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
    \right\rangle$$
    which is the full lift of $\left\langle
    \begin{bmatrix} 7 & 0 \\ 10 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 0 \\ 0 & 3 \end{bmatrix},
    \begin{bmatrix} 5 & 2 \\ 3 & 1 \end{bmatrix}\right\rangle$ to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{297}$ in the RZB database.
    
    \item $\operatorname{H}_{302} = \left\langle
    \begin{bmatrix} 13 & 7 \\ 2 & 3 \end{bmatrix},
    \begin{bmatrix} 3 & 3 \\ 2 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 10 \\ 2 & 3 \end{bmatrix}
    \right\rangle$
    
    Let $E/\QQ$ be an elliptic curve such that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to $\operatorname{H}_{302}$. Being careful of the right action in the RZB database, $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to $H = \left\langle
    \begin{bmatrix} 13 & 2 \\ 7 & 3 \end{bmatrix},
    \begin{bmatrix} 3 & 2 \\ 3 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 2 \\ 10 & 3 \end{bmatrix}
    \right\rangle$. The RZB database say that $H$ is a group of level $16$. By Lemma \ref{kernel of pi 1}, $\overline{\rho}_{E,64}(G_{\QQ})$ is conjugate to
    $$\left\langle
    \begin{bmatrix} 13 & 2 \\ 7 & 3 \end{bmatrix},
    \begin{bmatrix} 3 & 2 \\ 3 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 2 \\ 10 & 3 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
    \right\rangle.$$
    By Lemma \ref{2-adic image corollary 1}, $\overline{\rho}_{E/\left\langle Q_{2} \right\rangle,32}(G_{\QQ})$ is
    $$\left\langle
    \begin{bmatrix} 13 & 1 \\ 14 & 3 \end{bmatrix},
    \begin{bmatrix} 3 & 1 \\ 6 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 1 \\ 20 & 3 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
    \right\rangle$$
    which is conjugate to
    $$\left\langle
    \begin{bmatrix} 15 & 4 \\ 13 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 2 \\ 2 & 3 \end{bmatrix},
    \begin{bmatrix} 13 & 4 \\ 10 & 1 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
    \right\rangle$$
    which is the full lift of $\left\langle
    \begin{bmatrix} 15 & 4 \\ 13 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 2 \\ 2 & 3 \end{bmatrix},
    \begin{bmatrix} 13 & 4 \\ 10 & 1 \end{bmatrix}
    \right\rangle$. The transpose of this group is conjugate to $\operatorname{H}_{326}$ in the RZB database.
    \end{enumerate}
    
    \newpage
    
    \subsection{Isogeny-torsion graphs of $T_{4}$ type}
    
    Table \ref{2-adic Images of T4 Graphs} classifies the $2$-adic images of all elliptic curves over $\QQ$ in an isogeny-torsion graph of $T_{4}$ type. The groups of the form $\operatorname{H}_{n}$ come from the RZB database and the notation right next to them come from the LMFDB nomenclature. There are $60$ distinct arrangements of $2$-adic groups, $10$ of these arrangements contain groups with $\operatorname{-Id}$. In other words, each of the $60$ arrangements of groups in Table \ref{2-adic Images of T4 Graphs} are a quadratic twist of one of the $10$ arrangements of groups that contain $\operatorname{-Id}$.
    
    There are four arrangements of subgroups of $\operatorname{GL}(2, \ZZ_{2})$ that do not appear in the LMFDB. For all four of the following cases, we will have $\QQ$-isogeny classes consisting of one elliptic curve $E/\QQ$ which has full two-torsion defined over $\QQ$. Moreover, the only finite, cyclic, $\QQ$-rational subgroups of $E$ are the ones generated by the $2$-torsion points, $\mathcal{O}$, $P_{2}$, $Q_{2}$, and $P_{2}+Q_{2}$.
    
    \begin{enumerate}
        \item $\operatorname{H}_{61f}$
        
        Suppose $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to the full lift of
        $$\operatorname{H}_{61f} =
        \left\langle
        \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix},
        \begin{bmatrix} 1 & 2 \\ 6 & 7 \end{bmatrix},
        \begin{bmatrix} 3 & 6 \\ 10 & 5 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 12 & 3 \end{bmatrix}
        \right\rangle.$$
        Being careful of the right action in the RZB database, $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is actually conjugate to the full lift of
        $$\left\langle
        \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix},
        \begin{bmatrix} 1 & 6 \\ 2 & 7 \end{bmatrix},
        \begin{bmatrix} 3 & 10 \\ 6 & 5 \end{bmatrix},
        \begin{bmatrix} 1 & 12 \\ 0 & 3 \end{bmatrix}
        \right\rangle.$$
        The RZB database says that $\operatorname{H}_{61f}$ is a group of level $16$. By Lemma \ref{kernel of pi 1}, $\overline{\rho}_{E,64}(G_{\QQ})$ is conjugate to
        $$\left\langle
        \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix},
        \begin{bmatrix} 1 & 6 \\ 2 & 7 \end{bmatrix},
        \begin{bmatrix} 3 & 10 \\ 6 & 5 \end{bmatrix},
        \begin{bmatrix} 1 & 12 \\ 0 & 3 \end{bmatrix}
        \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
        \right\rangle.$$
        \begin{itemize}
            \item $E/\left\langle P_{2} \right\rangle$
            
            By the second part of Lemma \ref{2-adic image corollary 2}, $\overline{\rho}_{E/\left\langle P_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to
            $$\left\langle
        \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 7 & 1 \\ 12 & 1 \end{bmatrix},
        \begin{bmatrix} 5 & 3 \\ 20 & 3 \end{bmatrix},
        \begin{bmatrix} 3 & 0 \\ 24 & 1 \end{bmatrix}
        \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}
        \right\rangle$$
        which is conjugate to
        $$\left\langle
        \begin{bmatrix} 3 & 4 \\ 9 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 20 \\ 3 & 5 \end{bmatrix},
        \begin{bmatrix} 3 & 28 \\ 21 & 7 \end{bmatrix},
        \begin{bmatrix} 3 & 12 \\ 9 & 3 \end{bmatrix} \right\rangle.$$
        The transpose of this group is conjugate to $\operatorname{H}_{116a}$ in the RZB database.
            
        \item $E/\left\langle Q_{2} \right\rangle$
            
        By the first part of Lemma \ref{2-adic image corollary 2}, $\overline{\rho}_{E / \left\langle Q_{2} \right\rangle, 32}(G_{\QQ})$ is conjugate to
            $$\left\langle
        \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix},
        \begin{bmatrix} 1 & 3 \\ 4 & 7 \end{bmatrix},
        \begin{bmatrix} 3 & 5 \\ 12 & 5 \end{bmatrix},
        \begin{bmatrix} 1 & 6 \\ 0 & 3 \end{bmatrix},
        \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
        \right\rangle$$
        which is conjugate to
        $$\left\langle
        \begin{bmatrix} 3 & 4 \\ 9 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 20 \\ 3 & 5 \end{bmatrix},
        \begin{bmatrix} 3 & 28 \\ 21 & 7 \end{bmatrix},
        \begin{bmatrix} 3 & 12 \\ 9 & 3 \end{bmatrix} \right\rangle.$$
        The transpose of this group is conjugate to $\operatorname{H}_{116a}$ in the RZB database.
            \item $E/\left\langle P_{2}+Q_{2} \right\rangle$
            
            By the third part of Lemma \ref{2-adic image corollary 2}, $\overline{\rho}_{E,32}(G_{\QQ})$ is conjugate to
            $$\left\langle
            \begin{bmatrix} 1 & -2 \\ 0 & 5 \end{bmatrix},
            \begin{bmatrix} -1 & -1 \\ 4 & 9 \end{bmatrix},
            \begin{bmatrix} -3 & 1 \\ 12 & 11 \end{bmatrix},
            \begin{bmatrix} 1 & 5 \\ 0 & 3 \end{bmatrix},
            \begin{bmatrix} 17 & 8 \\ 0 & 1 \end{bmatrix},
            \begin{bmatrix} 1 & -8 \\ 0 & 17 \end{bmatrix},
            \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
            \begin{bmatrix} -15 & -8 \\ 0 & 17 \end{bmatrix}
            \right\rangle$$
            which is conjugate to
            $$\left\langle
            \begin{bmatrix} 7 & 0 \\ 7 & 1 \end{bmatrix},
            \begin{bmatrix} 3 & 12 \\ 0 & 3 \end{bmatrix},
            \begin{bmatrix} 11 & 0 \\ 0 & 3 \end{bmatrix},
            \begin{bmatrix} 3 & 0 \\ 9 & 1 \end{bmatrix},
            \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
            \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
            \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
            \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
            \right\rangle$$
            which is the full lift of $\left\langle \begin{bmatrix} 7 & 0 \\ 7 & 1 \end{bmatrix},
            \begin{bmatrix} 3 & 12 \\ 0 & 3 \end{bmatrix},
            \begin{bmatrix} 11 & 0 \\ 0 & 3 \end{bmatrix},
            \begin{bmatrix} 3 & 0 \\ 9 & 1 \end{bmatrix} \right\rangle$ to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{95h}$ in the RZB database.
            
        \end{itemize}
        
        \item $\operatorname{H}_{209d}$
        
        Suppose $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to the full lift of
        $$\operatorname{H}_{209d} =
        \left\langle
        \begin{bmatrix} 1 & 2 \\ 14 & 5 \end{bmatrix},
        \begin{bmatrix} 3 & 0 \\ 12 & 5 \end{bmatrix},
        \begin{bmatrix} 3 & 0 \\ 0 & 7 \end{bmatrix}
        \right\rangle.$$
        Being careful of the right action of right action in the RZB database, $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is actually conjugate to the full lift of
        $$\left\langle
        \begin{bmatrix} 1 & 14 \\ 2 & 5 \end{bmatrix},
        \begin{bmatrix} 3 & 12 \\ 0 & 5 \end{bmatrix},
        \begin{bmatrix} 3 & 0 \\ 0 & 7 \end{bmatrix}
        \right\rangle.$$
        The RZB database says that $\operatorname{H}_{209d}$ is a group of level $16$. By Lemma \ref{kernel of pi 1}, $\overline{\rho}_{E,64}(G_{\QQ})$ is conjugate to
        $$\left\langle
        \begin{bmatrix} 1 & 14 \\ 2 & 5 \end{bmatrix},
        \begin{bmatrix} 3 & 12 \\ 0 & 5 \end{bmatrix},
        \begin{bmatrix} 3 & 0 \\ 0 & 7 \end{bmatrix},
        \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
        \right\rangle.$$
        \begin{itemize}
            \item $E/\left\langle P_{2} \right\rangle$
            
            By the second part of Lemma \ref{2-adic image corollary 2}, $\overline{\rho}_{E/\left\langle P_{2} \right\rangle, 32}(G_{\QQ})$ is conjugate to
            $$\left\langle
        \begin{bmatrix} 5 & 1 \\ 28 & 1 \end{bmatrix},
        \begin{bmatrix} 5 & 0 \\ 24 & 3 \end{bmatrix},
        \begin{bmatrix} 7 & 0 \\ 0 & 3 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}
        \right\rangle$$
        which is conjugate to
        $$\left\langle
        \begin{bmatrix} 3 & 0 \\ 12 & 7 \end{bmatrix},
        \begin{bmatrix} 1 & 20 \\ 3 & 5 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix}
        \right\rangle.$$
        The transpose of this group is conjugate to $\operatorname{H}_{241f}$ in the RZB database.
            
        \item $E/\left\langle Q_{2} \right\rangle$
        
        By the first part of Lemma \ref{2-adic image corollary 2}, $\rho_{E/\left\langle Q_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to
        $$\left\langle
        \begin{bmatrix} 1 & 7 \\ 4 & 5 \end{bmatrix},
        \begin{bmatrix} 3 & 6 \\ 0 & 5 \end{bmatrix},
        \begin{bmatrix} 3 & 0 \\ 0 & 7 \end{bmatrix},
        \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
        \right\rangle$$
        which is conjugate to
        $$\left\langle
        \begin{bmatrix} 3 & 0 \\ 12 & 7 \end{bmatrix},
        \begin{bmatrix} 1 & 20 \\ 3 & 5 \end{bmatrix},
        \begin{bmatrix} 3 & 0 \\ 0 & 1 \end{bmatrix}
        \right\rangle.$$
        The transpose of this group is conjugate to $\operatorname{H}_{241g}$ in the RZB database.
            
        \item $E/\left\langle P_{2}+Q_{2} \right\rangle$
        
        By the third part of Lemma \ref{2-adic image corollary 2}, $\overline{\rho}_{E / \left\langle P_{2}+Q_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to
        $$\left\langle
        \begin{bmatrix} -1 & 4 \\ 4 & 7 \end{bmatrix},
        \begin{bmatrix} 3 & 5 \\ 0 & 5 \end{bmatrix},
        \begin{bmatrix} 3 & -2 \\ 0 & 7 \end{bmatrix},
        \begin{bmatrix} 17 & 8 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & -8 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} -15 & -8 \\ 0 & 17 \end{bmatrix}
        \right\rangle$$
        which is conjugate to
        $$\left\langle
        \begin{bmatrix} 7 & 0 \\ 7 & 1 \end{bmatrix},
        \begin{bmatrix} 3 & 12 \\ 0 & 3 \end{bmatrix},
        \begin{bmatrix} 9 & 0 \\ 11 & 3 \end{bmatrix},
        \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
        \right\rangle$$
        which is the full lift of
        $$\left\langle
        \begin{bmatrix} 7 & 0 \\ 7 & 1 \end{bmatrix},
        \begin{bmatrix} 3 & 12 \\ 0 & 3 \end{bmatrix},
        \begin{bmatrix} 9 & 0 \\ 11 & 3 \end{bmatrix}
        \right\rangle$$
        to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{222d}$ in the RZB database.
        \end{itemize}
        
        \item $\operatorname{H}_{214a}$
        
        Suppose $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to the full lift of
            $$\operatorname{H}_{214a} = \left\langle
            \begin{bmatrix} 3 & 6 \\ 6 & 11 \end{bmatrix},
            \begin{bmatrix} 1 & 2 \\ 14 & 7 \end{bmatrix},
            \begin{bmatrix} 1 & 6 \\ 2 & 1 \end{bmatrix}
            \right\rangle.$$
        Being careful of the right action in the RZB database, $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is actually conjugate to the full lift of
        $$\left\langle
            \begin{bmatrix} 3 & 6 \\ 6 & 11 \end{bmatrix},
            \begin{bmatrix} 1 & 14 \\ 2 & 7 \end{bmatrix},
            \begin{bmatrix} 1 & 2 \\ 6 & 1 \end{bmatrix}
            \right\rangle.$$
            The RZB database says that $\operatorname{H}_{214a}$ is a group of level $16$. By Lemma \ref{kernel of pi 1}, $\overline{\rho}_{E,64}(G_{\QQ})$ is conjugate to
            $$\left\langle
            \begin{bmatrix} 3 & 6 \\ 6 & 11 \end{bmatrix},
            \begin{bmatrix} 1 & 14 \\ 2 & 7 \end{bmatrix},
            \begin{bmatrix} 1 & 2 \\ 6 & 1 \end{bmatrix},
            \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
            \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
            \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
            \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
            \right\rangle.$$
            
        \begin{itemize}
            \item $E/\left\langle P_{2} \right\rangle$
            
            By the first part of Lemma \ref{2-adic image corollary 2}, $\overline{\rho}_{E/ \left\langle P_{2} \right\rangle, 32}(G_{\QQ})$ is conjugate to
            $$\left\langle
            \begin{bmatrix} 11 & 3 \\ 12 & 3 \end{bmatrix},
            \begin{bmatrix} 7 & 1 \\ 28 & 1 \end{bmatrix},
            \begin{bmatrix} 1 & 3 \\ 4 & 1 \end{bmatrix},
            \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
            \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
            \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix},
            \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}
            \right\rangle$$
            which is conjugate to
            $$\left\langle
            \begin{bmatrix} 1 & 4 \\ 3 & 1 \end{bmatrix},
            \begin{bmatrix} 11 & 12 \\ 11 & 3 \end{bmatrix},
            \begin{bmatrix} 15 & 0 \\ 0 & 1 \end{bmatrix},
            \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
            \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
            \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
            \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
            \right\rangle$$
            which is the full lift of
            $$\left\langle \begin{bmatrix} 1 & 4 \\ 3 & 1 \end{bmatrix},
            \begin{bmatrix} 11 & 12 \\ 11 & 3 \end{bmatrix},
            \begin{bmatrix} 15 & 0 \\ 0 & 1 \end{bmatrix} \right\rangle$$
            to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{226b}$ in the RZB database.
            
            \item $E/\left\langle Q_{2} \right\rangle$
            
            By the first part of Lemma \ref{2-adic image corollary 2}, $\overline{\rho}_{E/\left\langle Q_{2} \right\rangle, 32}(G_{\QQ})$ is conjugate to
            $$\left\langle
            \begin{bmatrix} 3 & 3 \\ 12 & 11 \end{bmatrix},
            \begin{bmatrix} 1 & 7 \\ 4 & 7 \end{bmatrix},
            \begin{bmatrix} 1 & 1 \\ 12 & 1 \end{bmatrix},
            \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
            \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
            \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
            \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
            \right\rangle$$
            which is the full lift of
            $$\left\langle
            \begin{bmatrix} 1 & 4 \\ 3 & 1 \end{bmatrix},
            \begin{bmatrix} 11 & 12 \\ 11 & 3 \end{bmatrix},
            \begin{bmatrix} 7 & 4 \\ 7 & 1 \end{bmatrix} \right\rangle$$
            to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{226a}$ in the RZB database.
            \item $E/\left\langle P_{2}+Q_{2} \right\rangle$
            
            By the third part of Lemma \ref{2-adic image corollary 2}, $\overline{\rho}_{E / \left\langle P_{2}+Q_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to
            $$\left\langle 
            \begin{bmatrix} -3 & -4 \\ 12 & 17 \end{bmatrix},
            \begin{bmatrix} -1 & 3 \\ 4 & 9 \end{bmatrix},
            \begin{bmatrix} -5 & -2 \\ 12 & 7 \end{bmatrix},
            \begin{bmatrix} 17 & 8 \\ 0 & 1 \end{bmatrix},
            \begin{bmatrix} 1 & -8 \\ 0 & 17 \end{bmatrix},
            \begin{bmatrix} -15 & -8 \\ 0 & 17 \end{bmatrix},
            \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}
            \right\rangle$$
            which is conjugate to
            $$\left\langle 
            \begin{bmatrix} 3 & 4 \\ 3 & 13 \end{bmatrix},
            \begin{bmatrix} 3 & 0 \\ 6 & 3 \end{bmatrix},
            \begin{bmatrix} 3 & 0 \\ 3 & 13 \end{bmatrix},
            \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
            \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
            \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
            \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
            \right\rangle$$
            which is the full lift of
            $$\left\langle \begin{bmatrix} 3 & 4 \\ 3 & 13 \end{bmatrix},
            \begin{bmatrix} 3 & 0 \\ 6 & 3 \end{bmatrix},
            \begin{bmatrix} 3 & 0 \\ 3 & 13 \end{bmatrix} \right\rangle$$
            to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{231d}$ in the RZB database.
        \end{itemize}
        
        \item $\operatorname{H}_{214c}$
        
        Suppose that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to the full lift of
        $$\operatorname{H}_{214c} =
        \left\langle
        \begin{bmatrix} 3 & 12 \\ 0 & 3 \end{bmatrix},
        \begin{bmatrix} 1 & 4 \\ 0 & 15 \end{bmatrix},
        \begin{bmatrix} 1 & 2 \\ 2 & 9 \end{bmatrix}
        \right\rangle.$$
        Being careful of the right action in the RZB database, $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is actually conjugate to the full lift of
        $$\left\langle
        \begin{bmatrix} 3 & 0 \\ 12 & 3 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 4 & 15 \end{bmatrix},
        \begin{bmatrix} 1 & 2 \\ 2 & 9 \end{bmatrix}
        \right\rangle.$$
        The RZB database says that $\operatorname{H}_{214c}$ is a group of level $16$. By Lemma \ref{kernel of pi 1}, $\overline{\rho}_{E,64}(G_{\QQ})$ is conjugate to
        $$\left\langle
        \begin{bmatrix} 3 & 0 \\ 12 & 3 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 4 & 15 \end{bmatrix},
        \begin{bmatrix} 1 & 2 \\ 2 & 9 \end{bmatrix},
        \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
        \right\rangle.$$
        
        \begin{itemize}
            \item $E/\left\langle P_{2} \right\rangle$
            
            By the first part of Lemma \ref{2-adic image corollary 2}, $\overline{\rho}_{E / \left\langle P_{2} \right\rangle, 32}(G_{\QQ})$ is conjugate to
            $$\left\langle
        \begin{bmatrix} 3 & 6 \\ 0 & 3 \end{bmatrix},
        \begin{bmatrix} 15 & 2 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 9 & 1 \\ 4 & 1 \end{bmatrix},
        \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
        \right\rangle$$
        which is conjugate to
        $$\left\langle
        \begin{bmatrix} 3 & 0 \\ 6 & 3 \end{bmatrix},
        \begin{bmatrix} 9 & 4 \\ 9 & 1 \end{bmatrix},
        \begin{bmatrix} 15 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
        \right\rangle$$
        which is the full lift of
        $$\left\langle
        \begin{bmatrix} 3 & 0 \\ 6 & 3 \end{bmatrix},
        \begin{bmatrix} 9 & 4 \\ 9 & 1 \end{bmatrix},
        \begin{bmatrix} 15 & 0 \\ 0 & 1 \end{bmatrix} \right\rangle$$
        to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{226g}$ in the RZB database.
        
            \item $E/\left\langle Q_{2} \right\rangle$
            
            By the second part of Lemma \ref{2-adic image corollary 2}, $\overline{\rho}_{E/\left\langle Q_{2} \right\rangle, 32}(G_{\QQ})$ is conjugate to
            $$\left\langle
        \begin{bmatrix} 3 & 0 \\ 24 & 3 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 8 & 15 \end{bmatrix},
        \begin{bmatrix} 1 & 1 \\ 4 & 9 \end{bmatrix},
        \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
        \right\rangle$$
        which is conjugate to
        $$\left\langle
        \begin{bmatrix} 3 & 0 \\ 6 & 3 \end{bmatrix},
        \begin{bmatrix} 9 & 4 \\ 9 & 1 \end{bmatrix},
        \begin{bmatrix} 13 & 0 \\ 0 & 3 \end{bmatrix},
        \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
        \right\rangle$$
        which is the full lift of
        $$\left\langle
        \begin{bmatrix} 3 & 0 \\ 6 & 3 \end{bmatrix},
        \begin{bmatrix} 9 & 4 \\ 9 & 1 \end{bmatrix},
        \begin{bmatrix} 13 & 0 \\ 0 & 3 \end{bmatrix} \right\rangle$$
        to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{226f}$ in the RZB database.
        
            
        \item $E/\left\langle P_{2}+Q_{2} \right\rangle$
        
        By the third part of Lemma \ref{2-adic image corollary 2}, $\overline{\rho}_{E/\left\langle P_{2}+Q_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to
        $$\left\langle
        \begin{bmatrix} -9 & -6 \\ -8 & 15 \end{bmatrix},
        \begin{bmatrix} -3 & -9 \\ 8 & 19 \end{bmatrix},
        \begin{bmatrix} -1 & -4 \\ 4 & 11 \end{bmatrix},
        \begin{bmatrix} 17 & 8 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & -8 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} -15 & -8 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}
        \right\rangle$$
        which is conjugate to
        $$\left\langle
        \begin{bmatrix} 3 & 4 \\ 3 & 13 \end{bmatrix},
        \begin{bmatrix} 3 & 0 \\ 6 & 3 \end{bmatrix},
        \begin{bmatrix} 3 & 12 \\ 0 & 15 \end{bmatrix},
        \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
        \right\rangle$$
        which is the full lift of
        $$\left\langle
        \begin{bmatrix} 3 & 4 \\ 3 & 13 \end{bmatrix},
        \begin{bmatrix} 3 & 0 \\ 6 & 3 \end{bmatrix},
        \begin{bmatrix} 3 & 12 \\ 0 & 15 \end{bmatrix} \right\rangle$$
        to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{231b}$.
        \end{itemize}
    \end{enumerate}
    
    \begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.53}{
    \begin{tabular}{|c|c|c|c|c|c|c|}

\hline

Isogeny Graph & Isogeny-Torsion Graph & $E_{1}$ & $E_{2}$ & $E_{3}$ & $E_{4}$ & Example Isogeny Class \\
\hline
\multirow{60}*{\includegraphics[scale=0.1]{T4 Graph.png}} &

\multirow{7}*{$([2,2],[4],[4],[2])$} & $\operatorname{H}_{24e} = \texttt{4.24.0.7}$ & $\operatorname{H}_{27h} = \texttt{4.24.0.11}$ & $\operatorname{H}_{32l} = \texttt{8.24.0.47}$ & $\operatorname{H}_{32i} = \texttt{8.24.0.57}$ & \texttt{205a} \\
\cline{3-7}
& & $\operatorname{H}_{61h} = \texttt{8.48.0.40}$ & $\operatorname{H}_{95a} = \texttt{8.48.0.64}$ &  $\operatorname{H}_{116l} = \texttt{16.48.0.40}$ & $\operatorname{H}_{116i} = \texttt{16.48.0.56}$ & \texttt{291.b} \\
\cline{3-7}
& & $\operatorname{H}_{66e} = \texttt{8.48.0.37}$ & $\operatorname{H}_{79h} = \texttt{8.48.0.170}$ & $\operatorname{H}_{94d} = \texttt{8.48.0.62}$ & $\operatorname{H}_{79i} = \texttt{8.48.0.185}$ & \texttt{1120.i} \\
\cline{3-7}
& & $\operatorname{H}_{67c} = \texttt{8.48.0.39}$ & $\operatorname{H}_{60d} = \texttt{4.48.0.2}$ & $\operatorname{H}_{115e} = \texttt{16.48.0.39}$ & $\operatorname{H}_{115g} = \texttt{16.48.0.55}$ & \texttt{40.a} \\
\cline{3-7}
& & $\operatorname{H}_{209b} = \texttt{16.96.0.14}$ & $\operatorname{H}_{222a} = \texttt{16.96.0.31}$ & $\operatorname{H}_{241d} = \texttt{32.96.0.9}$ & $\operatorname{H}_{241c} = \texttt{32.96.0.17}$ & \texttt{514.b} \\
\cline{3-7}
& & $\operatorname{H}_{210b} = \texttt{16.96.0.13}$ & $\operatorname{H}_{221a} = \texttt{16.96.0.32}$ & $\operatorname{H}_{242d} = \texttt{32.96.0.10}$ & $\operatorname{H}_{242b} = \texttt{32.96.0.18}$ & \texttt{17.a} \\
\cline{3-7}
& & $\operatorname{H}_{214b} = \texttt{16.96.0.12}$ & $\operatorname{H}_{226d} = \texttt{16.96.0.132}$ & $\operatorname{H}_{231c} = \texttt{16.96.0.29}$ & $\operatorname{H}_{226c} = \texttt{16.96.0.176}$ & \text{84320.k} \\
\cline{2-7}

& \multirow{14}*{$([2,2],[4],[2],[2])$} & $\operatorname{H}_{8d} = \texttt{4.12.0.1}$ & $\operatorname{H}_{13h} = \texttt{4.12.0.7}$ & $\operatorname{H}_{13d} = \texttt{8.12.0.6}$ & $\operatorname{H}_{13f} = \texttt{4.12.0.8}$ & \texttt{33.a} \\
\cline{3-7}
& & $\operatorname{H}_{24d} = \texttt{4.24.0.4}$ & $\operatorname{H}_{32e} = \texttt{8.24.0.52}$ & $\operatorname{H}_{27d} = \texttt{8.24.0.68}$ & $\operatorname{H}_{32f} = \texttt{8.24.0.62}$ & \texttt{2200.e} \\
\cline{3-7}
& & $\operatorname{H}_{38a} = \texttt{8.24.0.5}$ & $\operatorname{H}_{34a} = \texttt{8.24.0.51}$ & $\operatorname{H}_{34d} = \texttt{8.24.0.61}$ & $\operatorname{H}_{44b} = \texttt{8.24.0.105}$ & \texttt{392.d} \\
\cline{3-7}
& & $\operatorname{H}_{38c} = \texttt{8.24.0.2}$ & $\operatorname{H}_{44c} = \texttt{8.24.0.49}$ & $\operatorname{H}_{34e} = \texttt{8.24.0.60}$ & $\operatorname{H}_{34h} = \texttt{8.24.0.101}$ & \texttt{112.b} \\
\cline{3-7}
& & $\operatorname{H}_{38d} = \texttt{8.24.0.1}$ & $\operatorname{H}_{34f} = \texttt{8.24.0.50}$ & $\operatorname{H}_{34g} = \texttt{8.24.0.103}$ & $\operatorname{H}_{44d} = \texttt{8.24.0.58}$ & \texttt{56.a} \\
\cline{3-7}
& & $\operatorname{H}_{46a} = \texttt{8.24.0.6}$ & $\operatorname{H}_{33c} = \texttt{8.24.0.54}$ & $\operatorname{H}_{33d} = \texttt{8.24.0.64}$ & $\operatorname{H}_{48b} = \texttt{8.24.0.106}$ & \texttt{288.b} \\
\cline{3-7}
& & $\operatorname{H}_{46c} = \texttt{8.24.0.3}$ & $\operatorname{H}_{48c} = \texttt{8.24.0.48}$ & $\operatorname{H}_{33f} = \texttt{8.24.0.63}$ & $\operatorname{H}_{33h} = \texttt{8.24.0.104}$ & \texttt{96.b} \\
\cline{3-7}
& & $\operatorname{H}_{46d} = \texttt{8.24.0.4}$ & $\operatorname{H}_{33e} = \texttt{8.24.0.53}$ & $\operatorname{H}_{33g} = \texttt{8.24.0.102}$ & $\operatorname{H}_{48d} = \texttt{8.24.0.59}$ & \texttt{66.b} \\
\cline{3-7}
& & $\operatorname{H}_{61d} = \texttt{8.48.0.21}$ & $\operatorname{H}_{116e} = \texttt{16.48.0.42}$ & $\operatorname{H}_{95e} = \texttt{8.48.0.193}$ & $\operatorname{H}_{116f} = \texttt{16.48.0.58}$ & \texttt{28227.e} \\
\cline{3-7}
& & $\operatorname{H}_{66d} = \texttt{8.48.0.19}$ & $\operatorname{H}_{79b} = \texttt{8.48.0.172}$ & $\operatorname{H}_{79d} = \texttt{8.48.0.187}$ & $\operatorname{H}_{94f} = \texttt{8.48.0.200}$ & \texttt{2240.l} \\
\cline{3-7}
& & $\operatorname{H}_{67b} = \texttt{8.48.0.22}$ & $\operatorname{H}_{115a} = \texttt{16.48.0.41}$ & $\operatorname{H}_{60b} = \texttt{8.48.0.5}$ & $\operatorname{H}_{115d} = \texttt{16.48.0.57}$ & \texttt{200.c} \\
\cline{3-7}
& & $\operatorname{H}_{209c} = \texttt{16.96.0.6}$ & $\operatorname{H}_{241e} = \texttt{32.96.0.11}$ & $\operatorname{H}_{222c} = \texttt{16.96.0.185}$ & $\operatorname{H}_{241h} = \texttt{32.96.0.19}$ & \texttt{132098.b} \\
\cline{3-7}
& & $\operatorname{H}_{210c} = \texttt{16.96.0.5}$ & $\operatorname{H}_{242h} = \texttt{32.96.0.12}$ & $\operatorname{H}_{221c} = \texttt{16.96.0.186}$ & $\operatorname{H}_{242e} = \texttt{32.96.0.20}$ & \texttt{289.a} \\
\cline{3-7}
& & $\operatorname{H}_{214d} = \texttt{16.96.0.4}$ & $\operatorname{H}_{226e} = \texttt{16.96.0.134}$ & $\operatorname{H}_{226h} = \texttt{16.96.0.178}$ & $\operatorname{H}_{231a} = \texttt{16.96.0.211}$ & \texttt{168640.bg} \\

\cline{2-7}

& \multirow{39}*{$([2,2],[2],[2],[2])$} & $\operatorname{H}_{8} = \texttt{2.6.0.1}$ & $\operatorname{H}_{13} = \texttt{4.6.0.1}$ & $\operatorname{H}_{13} = \texttt{4.6.0.1}$ & $\operatorname{H}_{13} = \texttt{4.6.0.1}$ & \texttt{315.a} \\
\cline{3-7}
& & $\operatorname{H}_{8a} = \texttt{8.12.0.2}$ & $\operatorname{H}_{13a} = \texttt{8.12.0.13}$ & $\operatorname{H}_{13a} = \texttt{8.12.0.13}$ & $\operatorname{H}_{13a} = \texttt{8.12.0.13}$ & \texttt{1800.c} \\
\cline{3-7}
& & $\operatorname{H}_{8b} = \texttt{4.12.0.2}$ & $\operatorname{H}_{13b} = \texttt{8.12.0.14}$ & $\operatorname{H}_{13b} = \texttt{8.12.0.14}$ & $\operatorname{H}_{13b} = \texttt{8.12.0.14}$ & \texttt{1089.j}\\
\cline{3-7}
& & $\operatorname{H}_{8c} = \texttt{8.12.0.1}$ & $\operatorname{H}_{13c} = \texttt{8.12.0.12}$ & $\operatorname{H}_{13e} = \texttt{8.12.0.8}$ & $\operatorname{H}_{13g} = \texttt{8.12.0.7}$ & \texttt{120.a} \\
\cline{3-7}
& & $\operatorname{H}_{24} = \texttt{4.12.0.4}$ & $\operatorname{H}_{27} = \texttt{4.12.0.9}$ & $\operatorname{H}_{32} = \texttt{8.12.0.10}$ & $\operatorname{H}_{32} = \texttt{8.12.0.10}$ & \texttt{1845.e} \\
\cline{3-7}
& & $\operatorname{H}_{24a} = \texttt{8.24.0.28}$ & $\operatorname{H}_{27b} = \texttt{8.24.0.65}$ & $\operatorname{H}_{32a} = \texttt{16.24.0.20}$ & $\operatorname{H}_{32a} = \texttt{16.24.0.20}$ & \texttt{7200.bz} \\
\cline{3-7}
& & $\operatorname{H}_{24b} = \texttt{8.24.0.34}$ & $\operatorname{H}_{27e} = \texttt{8.24.0.75}$ & $\operatorname{H}_{32h} = \texttt{16.24.0.18}$ & $\operatorname{H}_{32h} = \texttt{16.24.0.18}$ & \texttt{1025.c} \\
\cline{3-7}
& & $\operatorname{H}_{24c} = \texttt{8.24.0.29}$ & $\operatorname{H}_{27g} = \texttt{8.24.0.69}$ & $\operatorname{H}_{32j} = \texttt{8.24.0.112}$ & $\operatorname{H}_{32k} = \texttt{8.24.0.108}$ & \texttt{960.d} \\
\cline{3-7}
& & $\operatorname{H}_{24f} = \texttt{8.24.0.33}$ & $\operatorname{H}_{27f} = \texttt{4.24.0.9}$ & $\operatorname{H}_{32g} = \texttt{16.24.0.16}$ & $\operatorname{H}_{32g} = \texttt{16.24.0.16}$ & \texttt{936.h} \\
\cline{3-7}
& & $\operatorname{H}_{24g} = \texttt{8.24.0.27}$ & $\operatorname{H}_{27a} = \texttt{8.24.0.66}$ & $\operatorname{H}_{32b} = \texttt{16.24.0.19}$ & $\operatorname{H}_{32b} = \texttt{16.24.0.19}$ & \texttt{14400.ex} \\
\cline{3-7}
& & $\operatorname{H}_{24h} = \texttt{8.24.0.30}$ & $\operatorname{H}_{27c} = \texttt{8.24.0.73}$ & $\operatorname{H}_{32c} = \texttt{8.24.0.113}$ & $\operatorname{H}_{32d} = \texttt{8.24.0.109}$ & \texttt{2400.b} \\
\cline{3-7}
& & $\operatorname{H}_{38} = \texttt{8.12.0.3}$ & $\operatorname{H}_{34} = \texttt{8.12.0.9}$ & $\operatorname{H}_{34} = \texttt{8.12.0.9}$ & $\operatorname{H}_{44} = \texttt{8.12.0.15}$ & \texttt{350.b} \\
\cline{3-7}
& & $\operatorname{H}_{38b} = \texttt{8.24.0.7}$ & $\operatorname{H}_{34b} = \texttt{8.24.0.111}$ & $\operatorname{H}_{34c} = \texttt{8.24.0.107}$ & $\operatorname{H}_{44a} = \texttt{8.24.0.117}$ & \texttt{3136.q} \\
\cline{3-7}
& & $\operatorname{H}_{46} = \texttt{8.12.0.4}$ & $\operatorname{H}_{33} = \texttt{8.12.0.11}$ & $\operatorname{H}_{33} = \texttt{8.12.0.11}$ & $\operatorname{H}_{48} = \texttt{8.12.0.16}$ & \texttt{198.a} \\
\cline{3-7}
& & $\operatorname{H}_{46b} = \texttt{8.24.0.8}$ & $\operatorname{H}_{33a} = \texttt{8.24.0.114}$ & $\operatorname{H}_{33b} = \texttt{8.24.0.110}$ & $\operatorname{H}_{48a} = \texttt{8.24.0.118}$ & \texttt{576.h} \\
\cline{3-7}
& & $\operatorname{H}_{61}= \texttt{8.24.0.36}$ & $\operatorname{H}_{95} = \texttt{8.24.0.74}$ & $\operatorname{H}_{116} = \texttt{16.24.0.17}$ & $\operatorname{H}_{116} = \texttt{16.24.0.17}$ & \texttt{7275.i} \\
\cline{3-7}
& & $\operatorname{H}_{61a} = \texttt{16.48.0.16}$ & $\operatorname{H}_{95c} = \texttt{16.48.0.73}$ & $\operatorname{H}_{116h} = \texttt{32.48.0.13}$ & $\operatorname{H}_{116h} = \texttt{32.48.0.13}$ & \texttt{873.c} \\
\cline{3-7}
& & $\operatorname{H}_{61b} = \texttt{16.48.0.17}$ & $\operatorname{H}_{95d} = \texttt{16.48.0.72}$ & $\operatorname{H}_{116g} = \texttt{32.48.0.15}$ & $\operatorname{H}_{116g} = \texttt{32.48.0.15}$ & \texttt{6066.e} \\
\cline{3-7}
& & $\operatorname{H}_{61c} = \texttt{8.48.0.152}$ & $\operatorname{H}_{95f} = \texttt{8.48.0.191}$ & $\operatorname{H}_{116c} = \texttt{16.48.0.223}$ & $\operatorname{H}_{116d} = \texttt{16.48.0.219}$ & \texttt{161376.y} \\
\cline{3-7}
& & $\operatorname{H}_{61e} = \texttt{16.48.0.15}$ & $\operatorname{H}_{95g} = \texttt{16.48.0.75}$ & $\operatorname{H}_{116b} = \texttt{32.48.0.14}$ & $\operatorname{H}_{116b} = \texttt{32.48.0.14}$ & \texttt{84681.j} \\
\cline{3-7}
& & $\operatorname{H}_{61f}$ & $\operatorname{H}_{95h}$ & $\operatorname{H}_{116a}$ & $\operatorname{H}_{116a}$ & $y^{2} = x^{3} - 134002596x + 596756613760$ \\
\cline{3-7}
& & $\operatorname{H}_{61g} = \texttt{8.48.0.155}$ & $\operatorname{H}_{95b} = \texttt{8.48.0.59}$ & $\operatorname{H}_{116j} = \texttt{16.48.0.221}$ & $\operatorname{H}_{116k} = \texttt{16.48.0.217}$ & \texttt{7872.k} \\
\cline{3-7}
& & $\operatorname{H}_{66} = \texttt{8.24.0.31}$ & $\operatorname{H}_{79} = \texttt{8.24.0.115}$ & $\operatorname{H}_{79} = \texttt{8.24.0.115}$ & $\operatorname{H}_{94} = \texttt{8.24.0.70}$ & \texttt{10080.h} \\
\cline{3-7}
& & $\operatorname{H}_{66a} = \texttt{16.48.0.12}$ & $\operatorname{H}_{79e} = \texttt{16.48.0.229}$ & $\operatorname{H}_{79g} = \texttt{16.48.0.228}$ & $\operatorname{H}_{94a} = \texttt{16.48.0.66}$ & \texttt{39200.bo} \\
\cline{3-7}
& & $\operatorname{H}_{66b} = \texttt{8.48.0.153}$ & $\operatorname{H}_{79f} = \texttt{16.48.0.231}$ & $\operatorname{H}_{79f} = \texttt{16.48.0.231}$ & $\operatorname{H}_{94e} = \texttt{8.48.0.189}$ & \texttt{7840.m} \\
\cline{3-7}
& & $\operatorname{H}_{66c} = \texttt{16.48.0.11}$ & $\operatorname{H}_{79a} = \texttt{16.48.0.226}$ & $\operatorname{H}_{79c} = \texttt{16.48.0.227}$ & $\operatorname{H}_{94c} = \texttt{16.48.0.67}$ & \texttt{5600.j} \\
\cline{3-7}
& & $\operatorname{H}_{66f} = \texttt{8.48.0.150}$ & $\operatorname{H}_{79j} = \texttt{16.48.0.230}$ & $\operatorname{H}_{79j} = \texttt{16.48.0.230}$ & $\operatorname{H}_{94b} = \texttt{8.48.0.57}$ & \texttt{15680.cb} \\
\cline{3-7}
& & $\operatorname{H}_{67} = \texttt{8.24.0.35}$ & $\operatorname{H}_{60} = \texttt{4.24.0.2}$ & $\operatorname{H}_{115} = \texttt{16.24.0.15}$ & $\operatorname{H}_{115} = \texttt{16.24.0.15}$ & \texttt{360.a} \\
\cline{3-7}
& & $\operatorname{H}_{67a} = \texttt{8.48.0.156}$ & $\operatorname{H}_{60c} = \texttt{8.48.0.4}$ & $\operatorname{H}_{115f} = \texttt{16.48.0.220}$ & $\operatorname{H}_{115h} = \texttt{16.48.0.216}$ & \texttt{320.d} \\
\cline{3-7}
& & $\operatorname{H}_{67d} = \texttt{8.48.0.149}$ & $\operatorname{H}_{60a} = \texttt{8.48.0.6}$ & $\operatorname{H}_{115b} = \texttt{16.48.0.222}$ & $\operatorname{H}_{115c} = \texttt{16.48.0.218}$ & \texttt{1600.o} \\
\cline{3-7}
& & $\operatorname{H}_{209} = \texttt{16.48.0.19}$ & $\operatorname{H}_{222} = \texttt{16.48.0.77}$ & $\operatorname{H}_{241} = \texttt{32.48.0.11}$ & $\operatorname{H}_{241} = \texttt{32.48.0.11}$ & \texttt{4626.d} \\
\cline{3-7}
& & $\operatorname{H}_{209a} = \texttt{16.96.0.89}$ & $\operatorname{H}_{222b} = \texttt{16.96.0.24}$ & $\operatorname{H}_{241a} = \texttt{32.96.0.97}$ & $\operatorname{H}_{241b} = \texttt{32.96.0.93}$ & \texttt{16448.k} \\
\cline{3-7}
& & $\operatorname{H}_{209d}$ & $\operatorname{H}_{222d}$ & $\operatorname{H}_{241f}$ & $\operatorname{H}_{241g}$ & $y^{2} = x^{3} - 5794082476x + 169747287967440$ \\
\cline{3-7}
& & $\operatorname{H}_{210} = \texttt{16.48.0.20}$ & $\operatorname{H}_{221} = \texttt{16.48.0.76}$ & $\operatorname{H}_{242} = \texttt{32.48.0.12}$ & $\operatorname{H}_{242} = \texttt{32.48.0.12}$ & \texttt{153.c} \\
\cline{3-7}
& & $\operatorname{H}_{210a} = \texttt{16.96.0.90}$ & $\operatorname{H}_{221b} = \texttt{16.96.0.23}$ & $\operatorname{H}_{242a} = \texttt{32.96.0.94}$ & $\operatorname{H}_{242c} = \texttt{32.96.0.98}$ & \texttt{1088.i} \\
\cline{3-7}
& & $\operatorname{H}_{210d} = \texttt{16.96.0.86}$ & $\operatorname{H}_{221d} = \texttt{16.96.0.181}$ & $\operatorname{H}_{242f} = \texttt{32.96.0.96}$ & $\operatorname{H}_{242g} = \texttt{32.96.0.100}$ & \texttt{18496.i} \\
\cline{3-7}
& & $\operatorname{H}_{214} = \texttt{16.48.0.14}$ & $\operatorname{H}_{226} = \texttt{16.48.0.225}$ & $\operatorname{H}_{226} = \texttt{16.48.0.225}$ & $\operatorname{H}_{231} = \texttt{16.48.0.68}$ & \texttt{421600.o} \\
\cline{3-7}
& & $\operatorname{H}_{214a}$ & $\operatorname{H}_{226a}$ & $\operatorname{H}_{226b}$ & $\operatorname{H}_{231d}$ & $y^{2} = x^{3} - 248504206997764x - 1507817332544964967680$ \\
\cline{3-7}
& & $\operatorname{H}_{214c}$ & $\operatorname{H}_{226f}$ & $\operatorname{H}_{226g}$ & $\operatorname{H}_{231b}$ & \texttt{$y^{2} = x^{3} - 62126051749441x - 188477166568120620960$} \\
\hline
\end{tabular}}
\caption{2-adic Images of $T_{4}$ Graphs}
\label{2-adic Images of T4 Graphs}
\end{table}
\end{center}


	\newpage

\subsection{Isogeny-torsion graphs of $T_{6}$ type}

Table \ref{2-adic Images of T6 Graphs} classifies the $2$-adic images of all elliptic curves over $\QQ$ in an isogeny-torsion graph of $T_{6}$ type. The groups of the form $\operatorname{H}_{n}$ come from the RZB database and the notation right next to them comes from the LMFDB nomenclature. There are $81$ distinct arrangements of $2$-adic groups, which come from $7$ distinct arrangements with $\operatorname{-Id}$. In other words, each of the $81$ arrangements of $2$-adic images on an isogeny-torsion graph of $T_{6}$ is a quadratic twist of one of $7$ different isogeny-torsion graphs of $T_{6}$ type with $\operatorname{-Id}$. There are seven arrangements of subgroups of $\operatorname{GL}(2, \ZZ_{2})$ that do not appear in the LMFDB.

There is a single arrangement of subgroups of $\operatorname{GL}(2, \ZZ_{2})$ for an isogeny-torsion graph of $T_{6}$ type that does not appear in the LMFDB. Let $E/\QQ$ be an elliptic curve with full two-torsion such that the isogeny-torsion graph of the $\QQ$-isogeny class of $E$ is of $T_{6}$ type. Then the finite, cyclic, $\QQ$-rational subgroups of $E$ are generated by $\mathcal{O}$, $P_{2}$, $Q_{2}$, $P_{2}+Q_{2}$, $Q_{4}$, and $P_{2}+Q_{4}$. We will denote the elliptic curves in the $\QQ$-isogeny class of $E$ as $E$, $E/\left\langle P_{2} \right\rangle$, $E/\left\langle Q_{2} \right\rangle$, $E/\left\langle P_{2}+Q_{2} \right\rangle$, $E/\left\langle Q_{4} \right\rangle$, and $E/\left\langle P_{2}+Q_{4} \right\rangle$. Suppose $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to the full lift of
$$\operatorname{H}_{62j} = \left\langle \begin{bmatrix} 3 & 6 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 0 \\ 4 & 7 \end{bmatrix}
\right\rangle.$$
Being careful of the right action in the RZB database, $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is actually conjugate to
$$\left\langle
\begin{bmatrix} 3 & 0 \\ 6 & 7 \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 4 \\ 0 & 7 \end{bmatrix}
\right\rangle.$$
The RZB database says that $\operatorname{H}_{62j}$ is a group of level $8$. By Lemma \ref{kernel of pi 1}, $\overline{\rho}_{E,64}(G_{\QQ})$ and $\overline{\rho}_{E,128}(G_{\QQ})$ are both conjugate to the same group
$$\left\langle
\begin{bmatrix} 3 & 0 \\ 6 & 7 \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 4 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}
\right\rangle$$
but viewed in different ambient groups; the former in $\operatorname{GL}(2, \ZZ / 64 \ZZ)$ and the latter in $\operatorname{GL}(2, \ZZ / 128 \ZZ)$.
\begin{itemize}
    \item $E/\left\langle P_{2} \right\rangle$

    By the second part of Lemma \ref{2-adic image corollary 2}, $\overline{\rho}_{E/\left\langle P_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to
    $$\left\langle
\begin{bmatrix} 7 & 3 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 0 \\ 8 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}
\right\rangle$$
which is conjugate to
$$\left\langle
\begin{bmatrix} 7 & 8 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 8 \\ 5 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix}
\right\rangle$$
which is the full lift of $\left\langle
\begin{bmatrix} 7 & 8 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 8 \\ 5 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 7 \end{bmatrix}\right\rangle$ to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{78c}$ in the RZB database.

    \item $E/\left\langle P_{2}+Q_{2} \right\rangle$
    
    By the third part of Lemma \ref{2-adic image corollary 2}, $\overline{\rho}_{E/\left\langle P_{2}+Q_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to
    $$\left\langle
    \begin{bmatrix} -3 & -5 \\ 12 & 13  \end{bmatrix},
    \begin{bmatrix} 3 & -1 \\ 0 & 5  \end{bmatrix},
    \begin{bmatrix} 5 & 0 \\ 0 & 5  \end{bmatrix},
    \begin{bmatrix} 7 & 2 \\ 0 & 7  \end{bmatrix},
    \begin{bmatrix} 9 & 4 \\ 0 & 1  \end{bmatrix},
    \begin{bmatrix} 1 & -4 \\ 0 & 9  \end{bmatrix},
    \begin{bmatrix} 1 & 4 \\ 0 & 1  \end{bmatrix},
    \begin{bmatrix} -7 & -4 \\ 16 & 9  \end{bmatrix}
    \right\rangle$$
    which is conjugate to
    $$\left\langle
    \begin{bmatrix} 3 & 8 \\ 0 & 1  \end{bmatrix},
    \begin{bmatrix} 7 & 8 \\ 0 & 7  \end{bmatrix},
    \begin{bmatrix} 5 & 8 \\ 5 & 1  \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 3  \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1  \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17  \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1  \end{bmatrix}
    \right\rangle$$
    which is the full lift of $\left\langle \begin{bmatrix} 3 & 8 \\ 0 & 1  \end{bmatrix},
    \begin{bmatrix} 7 & 8 \\ 0 & 7  \end{bmatrix},
    \begin{bmatrix} 5 & 8 \\ 5 & 1  \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 3  \end{bmatrix} \right\rangle$ to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{75b}$ in the RZB database.
    \item $E/\left\langle Q_{2} \right\rangle$
    
    By the first part of Lemma \ref{2-adic image corollary 2}, $\overline{\rho}_{E/\left\langle Q_{2} \right\rangle,32}(G_{\QQ})$ is conjugate to
    $$\left\langle
\begin{bmatrix} 3 & 0 \\ 12 & 7 \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 2 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
\right\rangle$$
which is conjugate to
$$\left\langle
\begin{bmatrix} 1 & 4 \\ 2 & 7 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 3 & 4 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 7 & 0 \\ 6 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}
\right\rangle$$
which is the full lift of $\left\langle
\begin{bmatrix} 1 & 4 \\ 2 & 7 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 3 & 4 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 7 & 0 \\ 6 & 7 \end{bmatrix} \right\rangle$ to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{100d}$ in the RZB database.

\item $E/\left\langle P_{2}+Q_{4} \right\rangle$

By the second part of Lemma \ref{2-adic image corollary 3}, $\overline{\rho}_{E/\left\langle P_{2}+Q_{4} \right\rangle,32}(G_{\QQ})$ is conjugate to
$$\left\langle
\begin{bmatrix} -9 & -8 \\ 24 & 19 \end{bmatrix},
\begin{bmatrix} 3 & -1 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 1 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 4 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & -4 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} -15 & -8 \\ 0 & 17 \end{bmatrix}
\right\rangle$$
which is conjugate to
$$\left\langle
\begin{bmatrix} 1 & 8 \\ 1 & 7 \end{bmatrix},
\begin{bmatrix} 3 & 8 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 7 & 8 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 3 & 8 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
\begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
\right\rangle$$
which is the full lift of
$\left\langle
\begin{bmatrix} 1 & 8 \\ 1 & 7 \end{bmatrix},
\begin{bmatrix} 3 & 8 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 7 & 8 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 3 & 8 \\ 0 & 5 \end{bmatrix}
\right\rangle$ to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{117a}$ in the RZB database.


    \item $E/\left\langle Q_{4} \right\rangle$
    
    
    By the first part of Lemma \ref{2-adic image corollary 3}, $\overline{\rho}_{E/\left\langle Q_{4} \right\rangle,32}(G_{\QQ})$ is conjugate to
    $$\left\langle
\begin{bmatrix} 3 & 0 \\ 24 & 7 \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 1 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
\right\rangle$$
which is conjugate to
$$\left\langle
\begin{bmatrix} 3 & 0 \\ 3 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
\begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
\right\rangle$$
which is the full lift of $\left\langle \begin{bmatrix} 3 & 0 \\ 3 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 1 \end{bmatrix} \right\rangle$ to level $32$. The transpose of this group is conjugate to $\operatorname{H}_{117j}$ in the RZB database.

    
\end{itemize}

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.5}
\scalebox{0.3}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline

Isogeny Graph & Isogeny-Torsion Graph & $E_{1}$ & $E_{2}$ & $E_{3}$ & $E_{4}$ & $E_{5}$ & $E_{6}$ & Example Isogeny Class \\
\hline
\multirow{81}*{\includegraphics[scale=0.13]{T6 Graph.png}} &

\multirow{5}*{$([2,4],[8],[4],[2,2],[2],[2])$} & $\operatorname{H}_{98e} = \texttt{8.48.0.24}$ & $\operatorname{H}_{102p} = \texttt{8.48.0.159}$ & $\operatorname{H}_{120d} = \texttt{16.48.0.27}$ & $\operatorname{H}_{101d} = \texttt{8.48.0.34}$ & $\operatorname{H}_{122c} = \texttt{16.48.0.48}$ & $\operatorname{H}_{85l} = \texttt{8.48.0.177}$ & \texttt{21.a} \\
\cline{3-9}
& & $\operatorname{H}_{181e} = \texttt{8.96.0.38}$ & $\operatorname{H}_{223d} = \texttt{16.96.0.97}$ & $\operatorname{H}_{229g} = \texttt{16.96.0.99}$ & $\operatorname{H}_{203f} = \texttt{8.96.0.48}$ & $\operatorname{H}_{233a} = \texttt{16.96.0.136}$ & $\operatorname{H}_{199f} = \texttt{8.96.0.165}$ & \texttt{102.c} \\
\cline{3-9}
& & $\operatorname{H}_{188c} = \texttt{8.96.0.37}$ & $\operatorname{H}_{230e} = \texttt{16.96.0.98}$ & $\operatorname{H}_{236b} = \texttt{16.96.0.103}$ & $\operatorname{H}_{200b} = \texttt{8.96.0.50}$ & $\operatorname{H}_{202g} = \texttt{8.96.0.164}$ & $\operatorname{H}_{217c} = \texttt{16.96.0.137}$ & \texttt{42.a} \\
\cline{3-9}
& & $\operatorname{H}_{200a} = \texttt{8.96.0.33}$ & $\operatorname{H}_{202h} = \texttt{8.96.0.157}$ & $\operatorname{H}_{217b} = \texttt{16.96.0.91}$ & $\operatorname{H}_{188d} = \texttt{8.96.0.56}$ & $\operatorname{H}_{236h} = \texttt{16.96.0.147}$ & $\operatorname{H}_{230b} = \texttt{16.96.0.146}$ & \texttt{336.d} \\
\cline{3-9}
& & $\operatorname{H}_{204h} = \texttt{8.96.0.34}$ & $\operatorname{H}_{197h} = \texttt{8.96.0.155}$ & $\operatorname{H}_{234b} = \texttt{16.96.0.93}$ & $\operatorname{H}_{190d} = \texttt{8.96.0.53}$ & $\operatorname{H}_{219g} = \texttt{16.96.0.150}$ & $\operatorname{H}_{228h} = \texttt{16.96.0.142}$ & \texttt{48.a} \\
\cline{2-9}

& \multirow{8}*{$([2,4],[4],[4],[2,2],[2],[2])$} & $\operatorname{H}_{25n} = \texttt{4.24.0.5}$ & $\operatorname{H}_{36n} = \texttt{8.24.0.45}$ & $\operatorname{H}_{36n} = \texttt{8.24.0.45}$ & $\operatorname{H}_{25h} = \texttt{4.24.0.6}$ & $\operatorname{H}_{36l} = \texttt{8.24.0.55}$ & $\operatorname{H}_{36l} = \texttt{8.24.0.55}$ & \texttt{231.a} \\
\cline{3-9}
& & $\operatorname{H}_{62a} = \texttt{8.48.0.23}$ & $\operatorname{H}_{78j} = \texttt{8.48.0.158}$ & $\operatorname{H}_{75j} = \texttt{8.48.0.157}$ & $\operatorname{H}_{100h} = \texttt{8.48.0.36}$ & $\operatorname{H}_{117k} = \texttt{16.48.0.46}$ & $\operatorname{H}_{117k} = \texttt{16.48.0.46}$ & \texttt{3696.e} \\
\cline{3-9}
& & $\operatorname{H}_{87c} = \texttt{8.48.0.26}$ & $\operatorname{H}_{121d} = \texttt{16.48.0.30}$ & $\operatorname{H}_{86l} = \texttt{8.48.0.160}$ & $\operatorname{H}_{99h} = \texttt{8.48.0.31}$ & $\operatorname{H}_{119b} = \texttt{16.48.0.45}$ & $\operatorname{H}_{84l} = \texttt{8.48.0.175}$ & \texttt{120.b} \\
\cline{3-9}
& & $\operatorname{H}_{99g} = \texttt{8.48.0.27}$ & $\operatorname{H}_{119d} = \texttt{16.48.0.31}$ & $\operatorname{H}_{84k} = \texttt{8.48.0.162}$ & $\operatorname{H}_{87d} = \texttt{8.48.0.33}$ & $\operatorname{H}_{121c} = \texttt{16.48.0.47}$ & $\operatorname{H}_{86j} = \texttt{8.48.0.178}$ & \texttt{240.c} \\
\cline{3-9}
& & $\operatorname{H}_{100e} = \texttt{8.48.0.29}$ & $\operatorname{H}_{117d} = \texttt{16.48.0.29}$ & $\operatorname{H}_{117d} = \texttt{16.48.0.29}$ & $\operatorname{H}_{62b} = \texttt{8.48.0.30}$ & $\operatorname{H}_{78i} = \texttt{8.48.0.173}$ & $\operatorname{H}_{75i} = \texttt{8.48.0.174}$ & \texttt{1848.g} \\
\cline{3-9}
& & $\operatorname{H}_{101b} = \texttt{8.48.0.25}$ & $\operatorname{H}_{85k} = \texttt{8.48.0.161}$ & $\operatorname{H}_{122d} = \texttt{16.48.0.32}$ & $\operatorname{H}_{98h} = \texttt{8.48.0.32}$ & $\operatorname{H}_{120b} = \texttt{16.48.0.43}$ & $\operatorname{H}_{102o} = \texttt{8.48.0.176}$ & \texttt{210.c} \\
\cline{3-9}
& & $\operatorname{H}_{190c} = \texttt{8.96.0.42}$ & $\operatorname{H}_{219c} = \texttt{16.96.0.106}$ & $\operatorname{H}_{228b} = \texttt{16.96.0.110}$ & $\operatorname{H}_{204f} = \texttt{8.96.0.49}$ & $\operatorname{H}_{234a} = \texttt{16.96.0.135}$ & $\operatorname{H}_{197g} = \texttt{8.96.0.166}$ & \texttt{24.a} \\
\cline{3-9}
& & $\operatorname{H}_{203e} = \texttt{8.96.0.35}$ & $\operatorname{H}_{233b} = \texttt{16.96.0.94}$ & $\operatorname{H}_{199e} = \texttt{8.96.0.156}$ & $\operatorname{H}_{181f} = \texttt{8.96.0.55}$ & $\operatorname{H}_{223h} = \texttt{16.96.0.145}$ & $\operatorname{H}_{229c} = \texttt{16.96.0.151}$ & \texttt{816.b} \\
\cline{2-9}

& \multirow{24}*{$([2,2],[4],[2],[2,2],[2],[2])$} & $\operatorname{H}_{25i} = \texttt{4.24.0.3}$ & $\operatorname{H}_{36h} = \texttt{8.24.0.46}$ & $\operatorname{H}_{36f} = \texttt{8.24.0.56}$ & $\operatorname{H}_{25l} = \texttt{8.24.0.24}$ & $\operatorname{H}_{36m} = \texttt{16.24.0.4}$ & $\operatorname{H}_{36m} = \texttt{16.24.0.4}$ & \texttt{1287.e} \\
\cline{3-9}
& & $\operatorname{H}_{62e} = \texttt{8.48.0.8}$ & $\operatorname{H}_{78g} = \texttt{8.48.0.164}$ & $\operatorname{H}_{75f} = \texttt{8.48.0.180}$ & $\operatorname{H}_{100j} = \texttt{8.48.0.146}$ & $\operatorname{H}_{117l} = \texttt{16.48.0.183}$ & $\operatorname{H}_{117l} = \texttt{16.48.0.183}$ & \texttt{14784.ci} \\
\cline{3-9}
& & $\operatorname{H}_{62f} = \texttt{8.48.0.7}$ & $\operatorname{H}_{75g} = \texttt{8.48.0.163}$ & $\operatorname{H}_{78h} = \texttt{8.48.0.179}$ & $\operatorname{H}_{100i} = \texttt{8.48.0.148}$ & $\operatorname{H}_{117c} = \texttt{16.48.0.195}$ & $\operatorname{H}_{117c} = \texttt{16.48.0.195}$ & \texttt{14784.z} \\
\cline{3-9}
& & $\operatorname{H}_{87k} = \texttt{8.48.0.12}$ & $\operatorname{H}_{121f} = \texttt{16.48.0.37}$ & $\operatorname{H}_{86n} = \texttt{8.48.0.184}$ & $\operatorname{H}_{99o} = \texttt{8.48.0.125}$ & $\operatorname{H}_{119j} = \texttt{16.48.0.160}$ & $\operatorname{H}_{84d} = \texttt{16.48.0.148}$ & \texttt{600.c} \\
\cline{3-9}
& & $\operatorname{H}_{87l} = \texttt{8.48.0.15}$ & $\operatorname{H}_{86o} = \texttt{8.48.0.166}$ & $\operatorname{H}_{121e} = \texttt{16.48.0.52}$ & $\operatorname{H}_{99n} = \texttt{8.48.0.75}$ & $\operatorname{H}_{119l} = \texttt{16.48.0.88}$ & $\operatorname{H}_{84c} = \texttt{16.48.0.146}$ & \texttt{1200.o} \\
\cline{3-9}
& & $\operatorname{H}_{98m} = \texttt{8.48.0.9}$ & $\operatorname{H}_{102k} = \texttt{8.48.0.165}$ & $\operatorname{H}_{120h} = \texttt{16.48.0.49}$ & $\operatorname{H}_{101m} = \texttt{8.48.0.142}$ & $\operatorname{H}_{122l} = \texttt{16.48.0.114}$ & $\operatorname{H}_{85c} = \texttt{16.48.0.126}$ & \texttt{2352.v} \\
\cline{3-9}
& & $\operatorname{H}_{98n} = \texttt{8.48.0.11}$ & $\operatorname{H}_{120f} = \texttt{16.48.0.33}$ & $\operatorname{H}_{102l} = \texttt{8.48.0.182}$ & $\operatorname{H}_{101o} = \texttt{8.48.0.109}$ & $\operatorname{H}_{122k} = \texttt{16.48.0.174}$ & $\operatorname{H}_{85d} = \texttt{16.48.0.125}$ & \texttt{147.a} \\
\cline{3-9}
& & $\operatorname{H}_{99m} = \texttt{8.48.0.16}$ & $\operatorname{H}_{84p} = \texttt{8.48.0.168}$ & $\operatorname{H}_{119f} = \texttt{16.48.0.53}$ & $\operatorname{H}_{87p} = \texttt{8.48.0.101}$ & $\operatorname{H}_{121l} = \texttt{16.48.0.173}$ & $\operatorname{H}_{86d} = \texttt{16.48.0.137}$ & \texttt{2880.bb} \\
\cline{3-9}
& & $\operatorname{H}_{99p} = \texttt{8.48.0.10}$ & $\operatorname{H}_{119h} = \texttt{16.48.0.35}$ & $\operatorname{H}_{84o} = \texttt{8.48.0.181}$ & $\operatorname{H}_{87m} = \texttt{8.48.0.122}$ & $\operatorname{H}_{121k} = \texttt{16.48.0.113}$ & $\operatorname{H}_{86b} = \texttt{16.48.0.138}$ & \texttt{2880.x} \\
\cline{3-9}
& & $\operatorname{H}_{100a} = \texttt{8.48.0.17}$ & $\operatorname{H}_{117b} = \texttt{16.48.0.36}$ & $\operatorname{H}_{117i} = \texttt{16.48.0.51}$ & $\operatorname{H}_{62g} = \texttt{8.48.0.141}$ & $\operatorname{H}_{78d} = \texttt{16.48.0.212}$ & $\operatorname{H}_{75d} = \texttt{16.48.0.206}$ & \texttt{142296.bm} \\
\cline{3-9}
& & $\operatorname{H}_{101j} = \texttt{8.48.0.18}$ & $\operatorname{H}_{122f} = \texttt{16.48.0.38}$ & $\operatorname{H}_{85m} = \texttt{8.48.0.183}$ & $\operatorname{H}_{98o} = \texttt{8.48.0.66}$ & $\operatorname{H}_{102g} = \texttt{16.48.0.98}$ & $\operatorname{H}_{120j} = \texttt{16.48.0.84}$ & \texttt{63.a} \\
\cline{3-9}
& & $\operatorname{H}_{101l} = \texttt{8.48.0.13}$ & $\operatorname{H}_{85p} = \texttt{8.48.0.167}$ & $\operatorname{H}_{122e} = \texttt{16.48.0.54}$ & $\operatorname{H}_{98p} = \texttt{8.48.0.90}$ & $\operatorname{H}_{102h} = \texttt{16.48.0.100}$ & $\operatorname{H}_{120l} = \texttt{16.48.0.156}$ & \texttt{1008.l} \\
\cline{3-9}
& & $\operatorname{H}_{181a} = \texttt{8.96.0.19}$ & $\operatorname{H}_{223b} = \texttt{16.96.0.117}$ & $\operatorname{H}_{229b} = \texttt{16.96.0.171}$ & $\operatorname{H}_{203d} = \texttt{8.96.0.152}$ & $\operatorname{H}_{233e} = \texttt{16.96.0.271}$ & $\operatorname{H}_{199b} = \texttt{16.96.0.275}$ & \texttt{1734.j} \\
\cline{3-9}
& & $\operatorname{H}_{181b} = \texttt{8.96.0.26}$ & $\operatorname{H}_{229e} = \texttt{16.96.0.119}$ & $\operatorname{H}_{223f} = \texttt{16.96.0.165}$ & $\operatorname{H}_{203c} = \texttt{8.96.0.112}$ & $\operatorname{H}_{233f} = \texttt{16.96.0.235}$ & $\operatorname{H}_{199a} = \texttt{16.96.0.274}$ & \texttt{13872.bm} \\
\cline{3-9}
& & $\operatorname{H}_{188a} = \texttt{8.96.0.24}$ & $\operatorname{H}_{236a} = \texttt{16.96.0.123}$ & $\operatorname{H}_{230d} = \texttt{16.96.0.166}$ & $\operatorname{H}_{200f} = \texttt{8.96.0.128}$ & $\operatorname{H}_{202d} = \texttt{16.96.0.247}$ & $\operatorname{H}_{217f} = \texttt{16.96.0.305}$ & \texttt{2352.l} \\
\cline{3-9}
& & $\operatorname{H}_{188b} = \texttt{8.96.0.20}$ & $\operatorname{H}_{230h} = \texttt{16.96.0.118}$ & $\operatorname{H}_{236g} = \texttt{16.96.0.167}$ & $\operatorname{H}_{200e} = \texttt{8.96.0.110}$ & $\operatorname{H}_{202c} = \texttt{16.96.0.245}$ & $\operatorname{H}_{217h} = \texttt{16.96.0.213}$ & \texttt{294.g} \\
\cline{3-9}
& & $\operatorname{H}_{190a} = \texttt{8.96.0.21}$ & $\operatorname{H}_{219a} = \texttt{16.96.0.126}$ & $\operatorname{H}_{228e} = \texttt{16.96.0.162}$ & $\operatorname{H}_{204d} = \texttt{8.96.0.137}$ & $\operatorname{H}_{234g} = \texttt{16.96.0.270}$ & $\operatorname{H}_{197c} = \texttt{16.96.0.251}$ & \texttt{144.b} \\
\cline{3-9}
& & $\operatorname{H}_{190b} = \texttt{8.96.0.32}$ & $\operatorname{H}_{228a} = \texttt{16.96.0.130}$ & $\operatorname{H}_{219f} = \texttt{16.96.0.170}$ & $\operatorname{H}_{204a} = \texttt{8.96.0.107}$ & $\operatorname{H}_{234f} = \texttt{16.96.0.233}$ & $\operatorname{H}_{197d} = \texttt{16.96.0.249}$ & \texttt{72.a} \\
\cline{3-9}
& & $\operatorname{H}_{200c} = \texttt{8.96.0.13}$ & $\operatorname{H}_{202e} = \texttt{8.96.0.161}$ & $\operatorname{H}_{217d} = \texttt{16.96.0.157}$ & $\operatorname{H}_{188h} = \texttt{8.96.0.138}$ & $\operatorname{H}_{236f} = \texttt{16.96.0.277}$ & $\operatorname{H}_{230f} = \texttt{16.96.0.240}$ & \texttt{1344.i} \\
\cline{3-9}
& & $\operatorname{H}_{200d} = \texttt{8.96.0.11}$ & $\operatorname{H}_{217a} = \texttt{16.96.0.111}$ & $\operatorname{H}_{202f} = \texttt{8.96.0.168}$ & $\operatorname{H}_{188g} = \texttt{8.96.0.108}$ & $\operatorname{H}_{236c} = \texttt{16.96.0.217}$ & $\operatorname{H}_{230a} = \texttt{16.96.0.255}$ & \texttt{1344.q} \\
\cline{3-9}
& & $\operatorname{H}_{203a} = \texttt{8.96.0.14}$ & $\operatorname{H}_{233d} = \texttt{16.96.0.114}$ & $\operatorname{H}_{199g} = \texttt{8.96.0.169}$ & $\operatorname{H}_{181g} = \texttt{8.96.0.109}$ & $\operatorname{H}_{223e} = \texttt{16.96.0.239}$ & $\operatorname{H}_{229h} = \texttt{16.96.0.225}$ & \texttt{3264.bc} \\
\cline{3-9}
& & $\operatorname{H}_{203b} = \texttt{8.96.0.12}$ & $\operatorname{H}_{199h} = \texttt{8.96.0.160}$ & $\operatorname{H}_{233c} = \texttt{16.96.0.156}$ & $\operatorname{H}_{181h} = \texttt{8.96.0.131}$ & $\operatorname{H}_{223c} = \texttt{16.96.0.256}$ & $\operatorname{H}_{229d} = \texttt{16.96.0.289}$ & \texttt{3264.m} \\
\cline{3-9}
& & $\operatorname{H}_{204c} = \texttt{8.96.0.15}$ & $\operatorname{H}_{234c} = \texttt{16.96.0.113}$ & $\operatorname{H}_{197e} = \texttt{8.96.0.170}$ & $\operatorname{H}_{190g} = \texttt{8.96.0.144}$ & $\operatorname{H}_{219d} = \texttt{16.96.0.280}$ & $\operatorname{H}_{228c} = \texttt{16.96.0.300}$ & \texttt{192.b} \\
\cline{3-9}
& & $\operatorname{H}_{204b} = \texttt{8.96.0.9}$ & $\operatorname{H}_{197f} = \texttt{8.96.0.159}$ & $\operatorname{H}_{234d} = \texttt{16.96.0.155}$ & $\operatorname{H}_{190h} = \texttt{8.96.0.124}$ & $\operatorname{H}_{219h} = \texttt{16.96.0.220}$ & $\operatorname{H}_{228g} = \texttt{16.96.0.263}$ & \texttt{192.d} \\
\cline{2-9}

& \multirow{44}*{$([2,2],[2],[2],[2,2],[2],[2])$} & $\operatorname{H}_{25} = \texttt{4.12.0.3}$ & $\operatorname{H}_{36} = \texttt{8.12.0.5}$ & $\operatorname{H}_{36} = \texttt{8.12.0.5}$ & $\operatorname{H}_{25} = \texttt{4.12.0.3}$ & $\operatorname{H}_{36} = \texttt{8.12.0.5}$ & $\operatorname{H}_{36} = \texttt{8.12.0.5}$ & \texttt{3465.l} \\
\cline{3-9}
& & $\operatorname{H}_{25a} = \texttt{8.24.0.17}$ & $\operatorname{H}_{36r} = \texttt{16.24.0.14}$ & $\operatorname{H}_{36o} = \texttt{8.24.0.89}$ & $\operatorname{H}_{25k} = \texttt{8.24.0.9}$ & $\operatorname{H}_{36b} = \texttt{16.24.0.3}$ & $\operatorname{H}_{36a} = \texttt{8.24.0.87}$ & \texttt{693.d} \\
\cline{3-9}
& & $\operatorname{H}_{25b} = \texttt{8.24.0.11}$ & $\operatorname{H}_{36q} = \texttt{8.24.0.94}$ & $\operatorname{H}_{36p} = \texttt{16.24.0.9}$ & $\operatorname{H}_{25j} = \texttt{8.24.0.14}$ & $\operatorname{H}_{36s} = \texttt{8.24.0.93}$ & $\operatorname{H}_{36t} = \texttt{16.24.0.8}$ & \texttt{990.b} \\
\cline{3-9}
& & $\operatorname{H}_{25c} = \texttt{8.24.0.26}$ & $\operatorname{H}_{36j} = \texttt{16.24.0.11}$ & $\operatorname{H}_{36j} = \texttt{16.24.0.11}$ & $\operatorname{H}_{25f} = \texttt{8.24.0.19}$ & $\operatorname{H}_{36e} = \texttt{8.24.0.98}$ & $\operatorname{H}_{36c} = \texttt{8.24.0.96}$ & \texttt{990.c} \\
\cline{3-9}
& & $\operatorname{H}_{25d} = \texttt{8.24.0.16}$ & $\operatorname{H}_{36d} = \texttt{16.24.0.12}$ & $\operatorname{H}_{36d} = \texttt{16.24.0.12}$ & $\operatorname{H}_{25d} = \texttt{8.24.0.16}$ & $\operatorname{H}_{36d} = \texttt{16.24.0.12}$ & $\operatorname{H}_{36d} = \texttt{16.24.0.12}$ & \texttt{54450.bw} \\
\cline{3-9}
& & $\operatorname{H}_{25g} = \texttt{8.24.0.20}$ & $\operatorname{H}_{36i} = \texttt{8.24.0.95}$ & $\operatorname{H}_{36i} = \texttt{8.24.0.95}$ & $\operatorname{H}_{25e} = \texttt{8.24.0.21}$ & $\operatorname{H}_{36k} = \texttt{8.24.0.97}$ & $\operatorname{H}_{36k} = \texttt{8.24.0.97}$ & \texttt{6720.b} \\
\cline{3-9}
& & $\operatorname{H}_{25m} = \texttt{8.24.0.12}$ & $\operatorname{H}_{36g} = \texttt{16.24.0.10}$ & $\operatorname{H}_{36g} = \texttt{16.24.0.10}$ & $\operatorname{H}_{25m} = \texttt{8.24.0.12}$ & $\operatorname{H}_{36g} = \texttt{16.24.0.10}$ & $\operatorname{H}_{36g} = \texttt{16.24.0.10}$ & \texttt{53361.q} \\
\cline{3-9}
& & $\operatorname{H}_{62} = \texttt{8.24.0.22}$ & $\operatorname{H}_{78} = \texttt{8.24.0.100}$ & $\operatorname{H}_{75} = \texttt{8.24.0.99}$ & $\operatorname{H}_{100} = \texttt{8.24.0.25}$ & $\operatorname{H}_{117} = \texttt{16.24.0.5}$ & $\operatorname{H}_{117} = \texttt{16.24.0.5}$ & \texttt{5544.s} \\
\cline{3-9}
& & $\operatorname{H}_{62c} = \texttt{8.48.0.67}$ & $\operatorname{H}_{78e} = \texttt{8.48.0.214}$ & $\operatorname{H}_{75a} = \texttt{16.48.0.205}$ & $\operatorname{H}_{100c} = \texttt{8.48.0.128}$ & $\operatorname{H}_{117n} = \texttt{16.48.0.162}$ & $\operatorname{H}_{117o} = \texttt{16.48.0.115}$ & \texttt{8280.g} \\
\cline{3-9}
& & $\operatorname{H}_{62d} = \texttt{8.48.0.127}$ & $\operatorname{H}_{78f} = \texttt{8.48.0.223}$ & $\operatorname{H}_{75c} = \texttt{16.48.0.208}$ & $\operatorname{H}_{100b} = \texttt{8.48.0.68}$ & $\operatorname{H}_{117f} = \texttt{16.48.0.89}$ & $\operatorname{H}_{117e} = \texttt{16.48.0.172}$ & \texttt{16560.h} \\
\cline{3-9}
& & $\operatorname{H}_{62h} = \texttt{8.48.0.77}$ & $\operatorname{H}_{78b} = \texttt{16.48.0.211}$ & $\operatorname{H}_{75h} = \texttt{8.48.0.209}$ & $\operatorname{H}_{100f} = \texttt{8.48.0.78}$ & $\operatorname{H}_{117h} = \texttt{16.48.0.90}$ & $\operatorname{H}_{117m} = \texttt{16.48.0.112}$ & \texttt{25872.cs} \\
\cline{3-9}
& & $\operatorname{H}_{62i} = \texttt{8.48.0.102}$ & $\operatorname{H}_{78a} = \texttt{16.48.0.214}$ & $\operatorname{H}_{75e} = \texttt{8.48.0.232}$ & $\operatorname{H}_{100g} = \texttt{8.48.0.103}$ & $\operatorname{H}_{117p} = \texttt{16.48.0.161}$ & $\operatorname{H}_{117g} = \texttt{16.48.0.175}$ & \texttt{12936.m} \\
\cline{3-9}
& & $\operatorname{H}_{62j}$ & $\operatorname{H}_{78c}$ & $\operatorname{H}_{75b}$ & $\operatorname{H}_{100d}$ & $\operatorname{H}_{117a}$ & $\operatorname{H}_{117j}$ & $y^{2} = x^{3} + x^{2} - 87851969x - 102107357409$ \\
\cline{3-9}
& & $\operatorname{H}_{87} = \texttt{8.24.0.13}$ & $\operatorname{H}_{121} = \texttt{16.24.0.6}$ & $\operatorname{H}_{86} = \texttt{8.24.0.91}$ & $\operatorname{H}_{99} = \texttt{8.24.0.15}$ & $\operatorname{H}_{119} = \texttt{16.24.0.7}$ & $\operatorname{H}_{84} = \texttt{8.24.0.92}$ & \texttt{1989.e} \\
\cline{3-9}
& & $\operatorname{H}_{87a} = \texttt{8.48.0.70}$ & $\operatorname{H}_{121m} = \texttt{16.48.0.92}$ & $\operatorname{H}_{86g} = \texttt{16.48.0.136}$ & $\operatorname{H}_{99d} = \texttt{8.48.0.133}$ & $\operatorname{H}_{119n} = \texttt{16.48.0.118}$ & $\operatorname{H}_{84f} = \texttt{16.48.0.155}$ & \texttt{3600.t} \\
\cline{3-9}
& & $\operatorname{H}_{87b} = \texttt{8.48.0.116}$ & $\operatorname{H}_{121p} = \texttt{16.48.0.164}$ & $\operatorname{H}_{86e} = \texttt{16.48.0.141}$ & $\operatorname{H}_{99c} = \texttt{8.48.0.104}$ & $\operatorname{H}_{119p} = \texttt{16.48.0.178}$ & $\operatorname{H}_{84e} = \texttt{16.48.0.153}$ & \texttt{1800.n} \\
\cline{3-9}
& & $\operatorname{H}_{87e} = \texttt{8.48.0.118}$ & $\operatorname{H}_{121b} = \texttt{16.48.0.196}$ & $\operatorname{H}_{86i} = \texttt{8.48.0.228}$ & $\operatorname{H}_{99b} = \texttt{8.48.0.106}$ & $\operatorname{H}_{119a} = \texttt{16.48.0.184}$ & $\operatorname{H}_{84i} = \texttt{8.48.0.230}$ & \texttt{960.c} \\
\cline{3-9}
& & $\operatorname{H}_{87f} = \texttt{8.48.0.72}$ & $\operatorname{H}_{121a} = \texttt{16.48.0.182}$ & $\operatorname{H}_{86k} = \texttt{8.48.0.212}$ & $\operatorname{H}_{99a} = \texttt{8.48.0.135}$ & $\operatorname{H}_{119c} = \texttt{16.48.0.197}$ & $\operatorname{H}_{84j} = \texttt{8.48.0.221}$ & \texttt{960.j} \\
\cline{3-9}
& & $\operatorname{H}_{87g} = \texttt{8.48.0.99}$ & $\operatorname{H}_{121o} = \texttt{16.48.0.176}$ & $\operatorname{H}_{86f} = \texttt{16.48.0.142}$ & $\operatorname{H}_{99f} = \texttt{8.48.0.112}$ & $\operatorname{H}_{119o} = \texttt{16.48.0.165}$ & $\operatorname{H}_{84g} = \texttt{16.48.0.151}$ & \texttt{14400.db} \\
\cline{3-9}
& & $\operatorname{H}_{87h} = \texttt{8.48.0.111}$ & $\operatorname{H}_{121n} = \texttt{16.48.0.116}$ & $\operatorname{H}_{86h} = \texttt{16.48.0.143}$ & $\operatorname{H}_{99e} = \texttt{8.48.0.69}$ & $\operatorname{H}_{119m} = \texttt{16.48.0.93}$ & $\operatorname{H}_{84h} = \texttt{16.48.0.147}$ & \texttt{14400.cm} \\
\cline{3-9}
& & $\operatorname{H}_{87i} = \texttt{8.48.0.73}$ & $\operatorname{H}_{121j} = \texttt{16.48.0.91}$ & $\operatorname{H}_{86a} = \texttt{16.48.0.135}$ & $\operatorname{H}_{99j} = \texttt{8.48.0.134}$ & $\operatorname{H}_{119e} = \texttt{16.48.0.191}$ & $\operatorname{H}_{84n} = \texttt{8.48.0.222}$ & \texttt{720.d} \\
\cline{3-9}
& & $\operatorname{H}_{87j} = \texttt{8.48.0.119}$ & $\operatorname{H}_{121i} = \texttt{16.48.0.163}$ & $\operatorname{H}_{86c} = \texttt{16.48.0.140}$ & $\operatorname{H}_{99i} = \texttt{8.48.0.105}$ & $\operatorname{H}_{119g} = \texttt{16.48.0.202}$ & $\operatorname{H}_{84m} = \texttt{8.48.0.231}$ & \texttt{360.b} \\
\cline{3-9}
& & $\operatorname{H}_{87n} = \texttt{8.48.0.71}$ & $\operatorname{H}_{121h} = \texttt{16.48.0.200}$ & $\operatorname{H}_{86p} = \texttt{8.48.0.213}$ & $\operatorname{H}_{99l} = \texttt{8.48.0.136}$ & $\operatorname{H}_{119i} = \texttt{16.48.0.117}$ & $\operatorname{H}_{84a} = \texttt{16.48.0.154}$ & \texttt{4800.cd} \\
\cline{3-9}
& & $\operatorname{H}_{87o} = \texttt{8.48.0.117}$ & $\operatorname{H}_{121g} = \texttt{16.48.0.190}$ & $\operatorname{H}_{86m} = \texttt{8.48.0.229}$ & $\operatorname{H}_{99k} = \texttt{8.48.0.107}$ & $\operatorname{H}_{119k} = \texttt{16.48.0.177}$ & $\operatorname{H}_{84b} = \texttt{16.48.0.152}$ & \texttt{4800.r} \\
\cline{3-9}
& & $\operatorname{H}_{98} = \texttt{8.24.0.10}$ & $\operatorname{H}_{102} = \texttt{8.24.0.88}$ & $\operatorname{H}_{120} = \texttt{16.24.0.1}$ & $\operatorname{H}_{101} = \texttt{8.24.0.18}$ & $\operatorname{H}_{122} = \texttt{16.24.0.13}$ & $\operatorname{H}_{85} = \texttt{8.24.0.90}$ & \texttt{525.d} \\
\cline{3-9}
& & $\operatorname{H}_{98a} = \texttt{8.48.0.83}$ & $\operatorname{H}_{102b} = \texttt{16.48.0.105}$ & $\operatorname{H}_{120p} = \texttt{16.48.0.169}$ & $\operatorname{H}_{101c} = \texttt{8.48.0.126}$ & $\operatorname{H}_{122p} = \texttt{16.48.0.167}$ & $\operatorname{H}_{85f} = \texttt{16.48.0.129}$ & \texttt{28224.fk} \\
\cline{3-9}
& & $\operatorname{H}_{98b} = \texttt{8.48.0.85}$ & $\operatorname{H}_{102m} = \texttt{8.48.0.219}$ & $\operatorname{H}_{120c} = \texttt{16.48.0.192}$ & $\operatorname{H}_{101g} = \texttt{8.48.0.130}$ & $\operatorname{H}_{122b} = \texttt{16.48.0.185}$ & $\operatorname{H}_{85j} = \texttt{8.48.0.225}$ & \texttt{1344.g} \\
\cline{3-9}
& & $\operatorname{H}_{98c} = \texttt{8.48.0.94}$ & $\operatorname{H}_{102n} = \texttt{8.48.0.215}$ & $\operatorname{H}_{120a} = \texttt{16.48.0.180}$ & $\operatorname{H}_{101e} = \texttt{8.48.0.80}$ & $\operatorname{H}_{122a} = \texttt{16.48.0.194}$ & $\operatorname{H}_{85i} = \texttt{8.48.0.210}$ & \texttt{1344.s} \\
\cline{3-9}
& & $\operatorname{H}_{98d} = \texttt{8.48.0.92}$ & $\operatorname{H}_{120n} = \texttt{16.48.0.109}$ & $\operatorname{H}_{102a} = \texttt{16.48.0.107}$ & $\operatorname{H}_{101a} = \texttt{8.48.0.76}$ & $\operatorname{H}_{85e} = \texttt{16.48.0.124}$ & $\operatorname{H}_{122m} = \texttt{16.48.0.95}$ & \texttt{22050.df} \\
\cline{3-9}
& & $\operatorname{H}_{98f} = \texttt{8.48.0.65}$ & $\operatorname{H}_{102d} = \texttt{16.48.0.99}$ & $\operatorname{H}_{120m} = \texttt{16.48.0.85}$ & $\operatorname{H}_{101h} = \texttt{8.48.0.113}$ & $\operatorname{H}_{122o} = \texttt{16.48.0.119}$ & $\operatorname{H}_{85h} = \texttt{16.48.0.131}$ & \texttt{441.f} \\
\cline{3-9}
& & $\operatorname{H}_{98g} = \texttt{8.48.0.87}$ & $\operatorname{H}_{102c} = \texttt{16.48.0.103}$ & $\operatorname{H}_{120o} = \texttt{16.48.0.157}$ & $\operatorname{H}_{101f} = \texttt{8.48.0.100}$ & $\operatorname{H}_{122n} = \texttt{16.48.0.179}$ & $\operatorname{H}_{85g} = \texttt{16.48.0.130}$ & \texttt{7056.p} \\
\cline{3-9}
& & $\operatorname{H}_{98i} = \texttt{8.48.0.86}$ & $\operatorname{H}_{102e} = \texttt{16.48.0.104}$ & $\operatorname{H}_{120i} = \texttt{16.48.0.168}$ & $\operatorname{H}_{101n} = \texttt{8.48.0.129}$ & $\operatorname{H}_{122g} = \texttt{16.48.0.203}$ & $\operatorname{H}_{85o} = \texttt{8.48.0.226}$ & \texttt{4032.h} \\
\cline{3-9}
& & $\operatorname{H}_{98j} = \texttt{8.48.0.93}$ & $\operatorname{H}_{120e} = \texttt{16.48.0.198}$ & $\operatorname{H}_{102j} = \texttt{8.48.0.216}$ & $\operatorname{H}_{101i} = \texttt{8.48.0.81}$ & $\operatorname{H}_{85b} = \texttt{16.48.0.123}$ & $\operatorname{H}_{122j} = \texttt{16.48.0.94}$ & \texttt{1470.q} \\
\cline{3-9}
& & $\operatorname{H}_{98k} = \texttt{8.48.0.84}$ & $\operatorname{H}_{102i} = \texttt{8.48.0.220}$ & $\operatorname{H}_{120g} = \texttt{16.48.0.186}$ & $\operatorname{H}_{101k} = \texttt{8.48.0.131}$ & $\operatorname{H}_{122i} = \texttt{16.48.0.166}$ & $\operatorname{H}_{85a} = \texttt{16.48.0.128}$ & \texttt{5880.z} \\
\cline{3-9}
& & $\operatorname{H}_{98l} = \texttt{8.48.0.95}$ & $\operatorname{H}_{120k} = \texttt{16.48.0.108}$ & $\operatorname{H}_{102f} = \texttt{16.48.0.106}$ & $\operatorname{H}_{101p} = \texttt{8.48.0.79}$ & $\operatorname{H}_{85n} = \texttt{8.48.0.211}$ & $\operatorname{H}_{122h} = \texttt{16.48.0.188}$ & \texttt{2070.b} \\
\cline{3-9}
& & $\operatorname{H}_{181} = \texttt{8.48.0.89}$ & $\operatorname{H}_{223} = \texttt{16.48.0.101}$ & $\operatorname{H}_{229} = \texttt{16.48.0.132}$ & $\operatorname{H}_{203} = \texttt{8.48.0.137}$ & $\operatorname{H}_{233} = \texttt{16.48.0.213}$ & $\operatorname{H}_{199} = \texttt{8.48.0.224}$ & \texttt{306.b} \\
\cline{3-9}
& & $\operatorname{H}_{181c} = \texttt{8.96.0.104}$ & $\operatorname{H}_{223a} = \texttt{16.96.0.259}$ & $\operatorname{H}_{229f} = \texttt{16.96.0.229}$ & $\operatorname{H}_{203g} = \texttt{8.96.0.148}$ & $\operatorname{H}_{233h} = \texttt{16.96.0.272}$ & $\operatorname{H}_{199c} = \texttt{16.96.0.276}$ & \texttt{55488.cr} \\
\cline{3-9}
& & $\operatorname{H}_{181d} = \texttt{8.96.0.136}$ & $\operatorname{H}_{223g} = \texttt{16.96.0.244}$ & $\operatorname{H}_{229a} = \texttt{16.96.0.293}$ & $\operatorname{H}_{203h} = \texttt{8.96.0.111}$ & $\operatorname{H}_{233g} = \texttt{16.96.0.236}$ & $\operatorname{H}_{199d} = \texttt{16.96.0.273}$ & \texttt{55488.m} \\
\cline{3-9}
& & $\operatorname{H}_{188} = \texttt{8.48.0.97}$ & $\operatorname{H}_{236} = \texttt{16.48.0.120}$ & $\operatorname{H}_{230} = \texttt{16.48.0.102}$ & $\operatorname{H}_{200} = \texttt{8.48.0.96}$ & $\operatorname{H}_{202} = \texttt{8.48.0.217}$ & $\operatorname{H}_{217} = \texttt{16.48.0.204}$ & \texttt{126.a} \\
\cline{3-9}
& & $\operatorname{H}_{188e} = \texttt{8.96.0.129}$ & $\operatorname{H}_{236e} = \texttt{16.96.0.281}$ & $\operatorname{H}_{230c} = \texttt{16.96.0.260}$ & $\operatorname{H}_{200h} = \texttt{8.96.0.133}$ & $\operatorname{H}_{202a} = \texttt{16.96.0.248}$ & $\operatorname{H}_{217e} = \texttt{16.96.0.306}$ & \texttt{9408.n} \\
\cline{3-9}
& & $\operatorname{H}_{188f} = \texttt{8.96.0.106}$ & $\operatorname{H}_{236d} = \texttt{16.96.0.221}$ & $\operatorname{H}_{230g} = \texttt{16.96.0.243}$ & $\operatorname{H}_{200g} = \texttt{8.96.0.105}$ & $\operatorname{H}_{202b} = \texttt{16.96.0.246}$ & $\operatorname{H}_{217g} = \texttt{16.96.0.214}$ & \texttt{9408.bw} \\
\cline{3-9}
& & $\operatorname{H}_{190} = \texttt{8.48.0.138}$ & $\operatorname{H}_{219} = \texttt{16.48.0.127}$ & $\operatorname{H}_{228} = \texttt{16.48.0.150}$ & $\operatorname{H}_{204} = \texttt{8.48.0.88}$ & $\operatorname{H}_{234} = \texttt{16.48.0.210}$ & $\operatorname{H}_{197} = \texttt{8.48.0.218}$ & \texttt{600.h} \\
\cline{3-9}
& & $\operatorname{H}_{190e} = \texttt{8.96.0.113}$ & $\operatorname{H}_{219e} = \texttt{16.96.0.224}$ & $\operatorname{H}_{228d} = \texttt{16.96.0.303}$ & $\operatorname{H}_{204g} = \texttt{8.96.0.135}$ & $\operatorname{H}_{234h} = \texttt{16.96.0.269}$ & $\operatorname{H}_{197b} = \texttt{16.96.0.252}$ & \texttt{576.b} \\
\cline{3-9}
& & $\operatorname{H}_{190f} = \texttt{8.96.0.147}$ & $\operatorname{H}_{219b} = \texttt{16.96.0.284}$ & $\operatorname{H}_{228f} = \texttt{16.96.0.268}$ & $\operatorname{H}_{204e} = \texttt{8.96.0.103}$ & $\operatorname{H}_{234e} = \texttt{16.96.0.234}$ & $\operatorname{H}_{197a} = \texttt{16.96.0.250}$ & \texttt{576.d} \\
\hline
\end{tabular}}
\caption{2-adic Images of $T_{6}$ Graphs}
\label{2-adic Images of T6 Graphs}
\end{table}
\end{center}
	
	
	\subsection{Isogeny-torsion graphs of $T_{8}$ type}
	
	
	
Table \ref{2-adic Images of T8 Graphs} classifies the $2$-adic images of all elliptic curves over $\QQ$ in an isogeny-torsion graph of $T_{8}$ type. The groups of the form $\operatorname{H}_{n}$ come from the RZB database and the notation right next to them comes from the LMFDB nomenclature. There are $53$ distinct arrangements of $2$-adic groups, which come from $4$ distinct arrangements with $\operatorname{-Id}$. In other words, each of the $53$ arrangements of $2$-adic images on an isogeny-torsion graph of $T_{8}$ is a quadratic twist of one of $4$ different isogeny-torsion graphs of $T_{8}$ type with $\operatorname{-Id}$.
	
	
\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.5}
\scalebox{0.35}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline

Isogeny Graph & Isogeny-Torsion Graph & $E_{1}$ & $E_{2}$ & $E_{3}$ & $E_{4}$ & $E_{5}$ & $E_{6}$ & $E_{7}$ & $E_{8}$ & Example Isogeny Class \\
\hline
\multirow{53}*{\includegraphics[scale=0.15]{T8 Graph.png}} 

& $([2,8],[8],[8],[2,4],[4],[2,2],[2],[2])$ & $\operatorname{H}_{193n} = \texttt{8.96.0.40}$ & $\operatorname{H}_{235l} = \texttt{16.96.0.95}$ & $\operatorname{H}_{235l} = \texttt{16.96.0.95}$ & $\operatorname{H}_{189d} = \texttt{8.96.0.2}$ & $\operatorname{H}_{207n} = \texttt{16.96.0.25}$ & $\operatorname{H}_{192i} = \texttt{8.96.0.60}$ & $\operatorname{H}_{211m} = \texttt{16.96.0.149}$ & $\operatorname{H}_{211m} = \texttt{16.96.0.149}$ & \texttt{210.e} \\
\cline{2-11}

& $([2,4],[8],[4],[2,4],[4],[2,2],[2],[2])$ & $\operatorname{H}_{194l} = \texttt{8.96.0.39}$ & $\operatorname{H}_{213i} = \texttt{16.96.0.96}$ & $\operatorname{H}_{227i} = \texttt{16.96.0.107}$ & $\operatorname{H}_{183i} = \texttt{8.96.0.8}$ & $\operatorname{H}_{205h} = \texttt{8.96.0.102}$ & $\operatorname{H}_{208a} = \texttt{16.96.0.10}$ & $\operatorname{H}_{243g} = \texttt{32.96.0.14}$ & $\operatorname{H}_{243g} = \texttt{32.96.0.14}$ & \texttt{1230.f} \\
\cline{2-11}

& $([2,4],[4],[4],[2,4],[8],[2,2],[2],[2])$ & $\operatorname{H}_{215c} = \texttt{16.96.0.7}$ & $\operatorname{H}_{240l} = \texttt{32.96.0.5}$ & $\operatorname{H}_{240l} = \texttt{32.96.0.5}$ & $\operatorname{H}_{187d} = \texttt{8.96.0.3}$ & $\operatorname{H}_{195l} = \texttt{8.96.0.99}$ & $\operatorname{H}_{185h} = \texttt{8.96.0.58}$ & $\operatorname{H}_{225g} = \texttt{16.96.0.148}$ & $\operatorname{H}_{212h} = \texttt{16.96.0.153}$ & \texttt{15.a} \\
\cline{2-11}

& \multirow{4}*{$([2,4],[4],[4],[2,4],[4],[2,2],[2],[2])$} & $\operatorname{H}_{96t} = \texttt{8.48.0.28}$ & $\operatorname{H}_{118l} = \texttt{16.48.0.28}$ & $\operatorname{H}_{118l} = \texttt{16.48.0.28}$ & $\operatorname{H}_{58i} = \texttt{4.48.0.3}$ & $\operatorname{H}_{92h} = \texttt{8.48.0.60}$ & $\operatorname{H}_{96o} = \texttt{8.48.0.35}$ & $\operatorname{H}_{118i} = \texttt{16.48.0.44}$ & $\operatorname{H}_{118i} = \texttt{16.48.0.44}$ & \texttt{195.a} \\
\cline{3-11}
& & $\operatorname{H}_{185g} = \texttt{8.96.0.41}$ & $\operatorname{H}_{225h} = \texttt{16.96.0.104}$ & $\operatorname{H}_{212i} = \texttt{16.96.0.101}$ & $\operatorname{H}_{187k} = \texttt{8.96.0.1}$ & $\operatorname{H}_{195h} = \texttt{8.96.0.101}$ & $\operatorname{H}_{215l} = \texttt{16.96.0.9}$ & $\operatorname{H}_{240h} = \texttt{32.96.0.13}$ & $\operatorname{H}_{240h} = \texttt{32.96.0.13}$ & \texttt{240.d} \\
\cline{3-11}
& & $\operatorname{H}_{192g} = \texttt{8.96.0.43}$ & $\operatorname{H}_{211s} = \texttt{16.96.0.105}$ & $\operatorname{H}_{211s} = \texttt{16.96.0.105}$ & $\operatorname{H}_{189e} = \texttt{8.96.0.5}$ & $\operatorname{H}_{207l} = \texttt{16.96.0.28}$ & $\operatorname{H}_{193i} = \texttt{8.96.0.57}$ & $\operatorname{H}_{235i} = \texttt{16.96.0.143}$ & $\operatorname{H}_{235i} = \texttt{16.96.0.143}$ & \texttt{1680.j} \\
\cline{3-11}
& & $\operatorname{H}_{208c} = \texttt{16.96.0.8}$ & $\operatorname{H}_{243d} = \texttt{32.96.0.6}$ & $\operatorname{H}_{243d} = \texttt{32.96.0.6}$ & $\operatorname{H}_{183d} = \texttt{8.96.0.7}$ & $\operatorname{H}_{205i} = \texttt{8.96.0.100}$ & $\operatorname{H}_{194k} = \texttt{8.96.0.51}$ & $\operatorname{H}_{213h} = \texttt{16.96.0.144}$ & $\operatorname{H}_{227k} = \texttt{16.96.0.139}$ & \texttt{510.e} \\
\cline{2-11}

& \multirow{9}*{$([2,2],[4],[2],[2,2],[2],[2,2],[2],[2])$} & $\operatorname{H}_{96g} = \texttt{8.48.0.14}$ & $\operatorname{H}_{118f} = \texttt{16.48.0.34}$ & $\operatorname{H}_{118c} = \texttt{16.48.0.50}$ & $\operatorname{H}_{58c} = \texttt{8.48.0.48}$ & $\operatorname{H}_{92d} = \texttt{16.48.0.62}$ & $\operatorname{H}_{96p} = \texttt{16.48.0.5}$ & $\operatorname{H}_{118j} = \texttt{32.48.0.2}$ & $\operatorname{H}_{118j} = \texttt{32.48.0.2}$ & \texttt{7605.h} \\
\cline{3-11}
& & $\operatorname{H}_{185i} = \texttt{8.96.0.31}$ & $\operatorname{H}_{212g} = \texttt{16.96.0.121}$ & $\operatorname{H}_{225j} = \texttt{16.96.0.168}$ & $\operatorname{H}_{187h} = \texttt{8.96.0.77}$ & $\operatorname{H}_{195f} = \texttt{16.96.0.197}$ & $\operatorname{H}_{215d} = \texttt{16.96.0.35}$ & $\operatorname{H}_{240m} = \texttt{32.96.0.29}$ & $\operatorname{H}_{240m} = \texttt{32.96.0.29}$ & \texttt{75.b} \\
\cline{3-11}
& & $\operatorname{H}_{185l} = \texttt{8.96.0.27}$ & $\operatorname{H}_{225k} = \texttt{16.96.0.124}$ & $\operatorname{H}_{212f} = \texttt{16.96.0.173}$ & $\operatorname{H}_{187j} = \texttt{8.96.0.83}$ & $\operatorname{H}_{195b} = \texttt{16.96.0.199}$ & $\operatorname{H}_{215k} = \texttt{16.96.0.61}$ & $\operatorname{H}_{240d} = \texttt{32.96.0.79}$ & $\operatorname{H}_{240d} = \texttt{32.96.0.79}$ & \texttt{1200.e} \\
\cline{3-11}
& & $\operatorname{H}_{192j} = \texttt{8.96.0.30}$ & $\operatorname{H}_{211p} = \texttt{16.96.0.125}$ & $\operatorname{H}_{211c} = \texttt{16.96.0.169}$ & $\operatorname{H}_{189b} = \texttt{8.96.0.70}$ & $\operatorname{H}_{207c} = \texttt{16.96.0.191}$ & $\operatorname{H}_{193j} = \texttt{16.96.0.47}$ & $\operatorname{H}_{235j} = \texttt{32.96.0.37}$ & $\operatorname{H}_{235j} = \texttt{32.96.0.37}$ & \texttt{20160.cz} \\
\cline{3-11}
& & $\operatorname{H}_{193g} = \texttt{8.96.0.18}$ & $\operatorname{H}_{235f} = \texttt{16.96.0.115}$ & $\operatorname{H}_{235c} = \texttt{16.96.0.163}$ & $\operatorname{H}_{189c} = \texttt{8.96.0.89}$ & $\operatorname{H}_{207k} = \texttt{16.96.0.201}$ & $\operatorname{H}_{192h} = \texttt{16.96.0.78}$ & $\operatorname{H}_{211h} = \texttt{32.96.0.57}$ & $\operatorname{H}_{211h} = \texttt{32.96.0.57}$ & \texttt{1470.j} \\
\cline{3-11}
& & $\operatorname{H}_{194g} = \texttt{8.96.0.17}$ & $\operatorname{H}_{213k} = \texttt{16.96.0.116}$ & $\operatorname{H}_{227e} = \texttt{16.96.0.159}$ & $\operatorname{H}_{183j} = \texttt{8.96.0.80}$ & $\operatorname{H}_{205c} = \texttt{16.96.0.207}$ & $\operatorname{H}_{208i} = \texttt{16.96.0.70}$ & $\operatorname{H}_{243l} = \texttt{32.96.0.48}$ & $\operatorname{H}_{243l} = \texttt{32.96.0.48}$ & \texttt{50430.ba} \\
\cline{3-11}
& & $\operatorname{H}_{194h} = \texttt{8.96.0.25}$ & $\operatorname{H}_{227g} = \texttt{16.96.0.127}$ & $\operatorname{H}_{213f} = \texttt{16.96.0.164}$ & $\operatorname{H}_{183a} = \texttt{8.96.0.91}$ & $\operatorname{H}_{205b} = \texttt{16.96.0.209}$ & $\operatorname{H}_{208g} = \texttt{16.96.0.52}$ & $\operatorname{H}_{243p} = \texttt{32.96.0.82}$ & $\operatorname{H}_{243p} = \texttt{32.96.0.82}$ & \texttt{277440.dv} \\
\cline{3-11}
& & $\operatorname{H}_{208e} = \texttt{16.96.0.1}$ & $\operatorname{H}_{243b} = \texttt{32.96.0.8}$ & $\operatorname{H}_{243e} = \texttt{32.96.0.16}$ & $\operatorname{H}_{183c} = \texttt{8.96.0.65}$ & $\operatorname{H}_{205d} = \texttt{16.96.0.205}$ & $\operatorname{H}_{194d} = \texttt{16.96.0.38}$ & $\operatorname{H}_{213a} = \texttt{32.96.0.41}$ & $\operatorname{H}_{227d} = \texttt{32.96.0.69}$ & \texttt{130050.fr} \\
\cline{3-11}
& & $\operatorname{H}_{215g} = \texttt{16.96.0.2}$ & $\operatorname{H}_{240j} = \texttt{32.96.0.7}$ & $\operatorname{H}_{240f} = \texttt{32.96.0.15}$ & $\operatorname{H}_{187c} = \texttt{8.96.0.61}$ & $\operatorname{H}_{195c} = \texttt{16.96.0.195}$ & $\operatorname{H}_{185b} = \texttt{16.96.0.53}$ & $\operatorname{H}_{225b} = \texttt{32.96.0.49}$ & $\operatorname{H}_{212b} = \texttt{32.96.0.65}$ & \texttt{225.b} \\
\cline{2-11}

& \multirow{37}*{$([2,2],[2],[2],[2,2],[2],[2,2],[2],[2])$} & $\operatorname{H}_{96} = \texttt{8.24.0.23}$ & $\operatorname{H}_{118} = \texttt{16.24.0.2}$ & $\operatorname{H}_{118} = \texttt{16.24.0.2}$ & $\operatorname{H}_{58} = \texttt{4.24.0.8}$ & $\operatorname{H}_{92} = \texttt{8.24.0.67}$ & $\operatorname{H}_{96} = \texttt{8.24.0.23}$ & $\operatorname{H}_{118} = \texttt{16.24.0.2}$ & $\operatorname{H}_{118} = \texttt{16.24.0.2}$ & \texttt{6435.i} \\
\cline{3-11}
& & $\operatorname{H}_{96a} = \texttt{8.48.0.140}$ & $\operatorname{H}_{118e} = \texttt{16.48.0.199}$ & $\operatorname{H}_{118a} = \texttt{16.48.0.187}$ & $\operatorname{H}_{58f} = \texttt{8.48.0.51}$ & $\operatorname{H}_{92f} = \texttt{16.48.0.65}$ & $\operatorname{H}_{96j} = \texttt{16.48.0.8}$ & $\operatorname{H}_{118h} = \texttt{32.48.0.5}$ & $\operatorname{H}_{118h} = \texttt{32.48.0.5}$ & \texttt{486720.dr} \\
\cline{3-11}
& & $\operatorname{H}_{96b} = \texttt{16.48.0.9}$ & $\operatorname{H}_{118b} = \texttt{32.48.0.9}$ & $\operatorname{H}_{118b} = \texttt{32.48.0.9}$ & $\operatorname{H}_{58j} = \texttt{8.48.0.54}$ & $\operatorname{H}_{92e} = \texttt{8.48.0.55}$ & $\operatorname{H}_{96b} = \texttt{16.48.0.9}$ & $\operatorname{H}_{118b} = \texttt{32.48.0.9}$ & $\operatorname{H}_{118b} = \texttt{32.48.0.9}$ & \texttt{187200.hl} \\
\cline{3-11}
& & $\operatorname{H}_{96c} = \texttt{8.48.0.108}$ & $\operatorname{H}_{118s} = \texttt{16.48.0.171}$ & $\operatorname{H}_{118o} = \texttt{16.48.0.110}$ & $\operatorname{H}_{58b} = \texttt{8.48.0.42}$ & $\operatorname{H}_{92a} = \texttt{8.48.0.196}$ & $\operatorname{H}_{96r} = \texttt{16.48.0.4}$ & $\operatorname{H}_{118n} = \texttt{32.48.0.3}$ & $\operatorname{H}_{118n} = \texttt{32.48.0.3}$ & \texttt{585.g} \\
\cline{3-11}
& & $\operatorname{H}_{96d} = \texttt{16.48.0.1}$ & $\operatorname{H}_{118p} = \texttt{32.48.0.7}$ & $\operatorname{H}_{118p} = \texttt{32.48.0.7}$ & $\operatorname{H}_{58g} = \texttt{8.48.0.41}$ & $\operatorname{H}_{92j} = \texttt{16.48.0.59}$ & $\operatorname{H}_{96f} = \texttt{16.48.0.2}$ & $\operatorname{H}_{118r} = \texttt{32.48.0.6}$ & $\operatorname{H}_{118r} = \texttt{32.48.0.6}$ & \texttt{38025.cm} \\
\cline{3-11}
& & $\operatorname{H}_{96e} = \texttt{8.48.0.74}$ & $\operatorname{H}_{118t} = \texttt{16.48.0.87}$ & $\operatorname{H}_{118q} = \texttt{16.48.0.158}$ & $\operatorname{H}_{58k} = \texttt{8.48.0.47}$ & $\operatorname{H}_{92i} = \texttt{8.48.0.198}$ & $\operatorname{H}_{96m} = \texttt{16.48.0.7}$ & $\operatorname{H}_{118v} = \texttt{32.48.0.10}$ & $\operatorname{H}_{118v} = \texttt{32.48.0.10}$ & \texttt{975.i} \\
\cline{3-11}
& & $\operatorname{H}_{96h} = \texttt{16.48.0.10}$ & $\operatorname{H}_{118d} = \texttt{32.48.0.4}$ & $\operatorname{H}_{118d} = \texttt{32.48.0.4}$ & $\operatorname{H}_{58d} = \texttt{8.48.0.53}$ & $\operatorname{H}_{92c} = \texttt{8.48.0.192}$ & $\operatorname{H}_{96h} = \texttt{16.48.0.10}$ & $\operatorname{H}_{118d} = \texttt{32.48.0.4}$ & $\operatorname{H}_{118d} = \texttt{32.48.0.4}$ & \texttt{2925.d} \\
\cline{3-11}
& & $\operatorname{H}_{96i} = \texttt{8.48.0.147}$ & $\operatorname{H}_{118k} = \texttt{16.48.0.193}$ & $\operatorname{H}_{118k} = \texttt{16.48.0.193}$ & $\operatorname{H}_{58e} = \texttt{8.48.0.52}$ & $\operatorname{H}_{92g} = \texttt{8.48.0.195}$ & $\operatorname{H}_{96k} = \texttt{8.48.0.145}$ & $\operatorname{H}_{118g} = \texttt{16.48.0.181}$ & $\operatorname{H}_{118g} = \texttt{16.48.0.181}$ & \texttt{12480.n} \\
\cline{3-11}
& & $\operatorname{H}_{96l} = \texttt{8.48.0.110}$ & $\operatorname{H}_{118x} = \texttt{16.48.0.170}$ & $\operatorname{H}_{118x} = \texttt{16.48.0.170}$ & $\operatorname{H}_{58h} = \texttt{8.48.0.46}$ & $\operatorname{H}_{92k} = \texttt{16.48.0.64}$ & $\operatorname{H}_{96s} = \texttt{8.48.0.132}$ & $\operatorname{H}_{118w} = \texttt{16.48.0.159}$ & $\operatorname{H}_{118w} = \texttt{16.48.0.159}$ & \texttt{40560.h} \\
\cline{3-11}
& & $\operatorname{H}_{96n} = \texttt{8.48.0.143}$ & $\operatorname{H}_{118u} = \texttt{16.48.0.111}$ & $\operatorname{H}_{118u} = \texttt{16.48.0.111}$ & $\operatorname{H}_{58a} = \texttt{8.48.0.43}$ & $\operatorname{H}_{92b} = \texttt{16.48.0.61}$ & $\operatorname{H}_{96q} = \texttt{8.48.0.82}$ & $\operatorname{H}_{118m} = \texttt{16.48.0.86}$ & $\operatorname{H}_{118m} = \texttt{16.48.0.86}$ & \texttt{2535.k} \\
\cline{3-11}
& & $\operatorname{H}_{185} = \texttt{8.48.0.123}$ & $\operatorname{H}_{225} = \texttt{16.48.0.121}$ & $\operatorname{H}_{212} = \texttt{16.48.0.134}$ & $\operatorname{H}_{187} = \texttt{8.48.0.44}$ & $\operatorname{H}_{195} = \texttt{8.48.0.197}$ & $\operatorname{H}_{215} = \texttt{16.48.0.3}$ & $\operatorname{H}_{240} = \texttt{32.48.0.1}$ & $\operatorname{H}_{240} = \texttt{32.48.0.1}$ & \texttt{735.c} \\
\cline{3-11}
& & $\operatorname{H}_{185a} = \texttt{16.96.0.55}$ & $\operatorname{H}_{225d} = \texttt{32.96.0.50}$ & $\operatorname{H}_{212d} = \texttt{32.96.0.66}$ & $\operatorname{H}_{187b} = \texttt{8.96.0.69}$ & $\operatorname{H}_{195j} = \texttt{8.96.0.97}$ & $\operatorname{H}_{215e} = \texttt{16.96.0.49}$ & $\operatorname{H}_{240a} = \texttt{32.96.0.45}$ & $\operatorname{H}_{240n} = \texttt{32.96.0.83}$ & \texttt{2880.y} \\
\cline{3-11}
& & $\operatorname{H}_{185c} = \texttt{16.96.0.54}$ & $\operatorname{H}_{225a} = \texttt{32.96.0.52}$ & $\operatorname{H}_{212c} = \texttt{32.96.0.68}$ & $\operatorname{H}_{187f} = \texttt{8.96.0.62}$ & $\operatorname{H}_{195d} = \texttt{16.96.0.196}$ & $\operatorname{H}_{215f} = \texttt{16.96.0.67}$ & $\operatorname{H}_{240e} = \texttt{32.96.0.87}$ & $\operatorname{H}_{240i} = \texttt{32.96.0.91}$ & \texttt{14400.cj} \\
\cline{3-11}
& & $\operatorname{H}_{185d} = \texttt{16.96.0.56}$ & $\operatorname{H}_{225c} = \texttt{32.96.0.51}$ & $\operatorname{H}_{212a} = \texttt{32.96.0.67}$ & $\operatorname{H}_{187g} = \texttt{8.96.0.87}$ & $\operatorname{H}_{195i} = \texttt{8.96.0.172}$ & $\operatorname{H}_{215h} = \texttt{16.96.0.33}$ & $\operatorname{H}_{240b} = \texttt{32.96.0.77}$ & $\operatorname{H}_{240o} = \texttt{32.96.0.31}$ & \texttt{45.a} \\
\cline{3-11}
& & $\operatorname{H}_{185e} = \texttt{8.96.0.118}$ & $\operatorname{H}_{225i} = \texttt{16.96.0.222}$ & $\operatorname{H}_{212e} = \texttt{16.96.0.230}$ & $\operatorname{H}_{187l} = \texttt{8.96.0.78}$ & $\operatorname{H}_{195e} = \texttt{16.96.0.198}$ & $\operatorname{H}_{215j} = \texttt{16.96.0.69}$ & $\operatorname{H}_{240c} = \texttt{32.96.0.47}$ & $\operatorname{H}_{240c} = \texttt{32.96.0.47}$ & \texttt{4800.bz} \\
\cline{3-11}
& & $\operatorname{H}_{185f} = \texttt{8.96.0.149}$ & $\operatorname{H}_{225l} = \texttt{16.96.0.282}$ & $\operatorname{H}_{212l} = \texttt{16.96.0.295}$ & $\operatorname{H}_{187a} = \texttt{8.96.0.84}$ & $\operatorname{H}_{195a} = \texttt{16.96.0.200}$ & $\operatorname{H}_{215a} = \texttt{16.96.0.51}$ & $\operatorname{H}_{240p} = \texttt{32.96.0.81}$ & $\operatorname{H}_{240p} = \texttt{32.96.0.81}$ & \texttt{4800.t} \\
\cline{3-11}
& & $\operatorname{H}_{185j} = \texttt{8.96.0.122}$ & $\operatorname{H}_{225f} = \texttt{16.96.0.219}$ & $\operatorname{H}_{212j} = \texttt{16.96.0.291}$ & $\operatorname{H}_{187i} = \texttt{8.96.0.85}$ & $\operatorname{H}_{195k} = \texttt{8.96.0.175}$ & $\operatorname{H}_{215i} = \texttt{16.96.0.79}$ & $\operatorname{H}_{240g} = \texttt{32.96.0.85}$ & $\operatorname{H}_{240g} = \texttt{32.96.0.85}$ & \texttt{960.a} \\
\cline{3-11}
& & $\operatorname{H}_{185k} = \texttt{8.96.0.121}$ & $\operatorname{H}_{225e} = \texttt{16.96.0.278}$ & $\operatorname{H}_{212k} = \texttt{16.96.0.227}$ & $\operatorname{H}_{187e} = \texttt{8.96.0.86}$ & $\operatorname{H}_{195g} = \texttt{8.96.0.176}$ & $\operatorname{H}_{215b} = \texttt{16.96.0.81}$ & $\operatorname{H}_{240k} = \texttt{32.96.0.89}$ & $\operatorname{H}_{240k} = \texttt{32.96.0.89}$ & \texttt{960.l} \\
\cline{3-11}
& & $\operatorname{H}_{192} = \texttt{8.48.0.144}$ & $\operatorname{H}_{211} = \texttt{16.48.0.122}$ & $\operatorname{H}_{211} = \texttt{16.48.0.122}$ & $\operatorname{H}_{189} = \texttt{8.48.0.45}$ & $\operatorname{H}_{207} = \texttt{16.48.0.60}$ & $\operatorname{H}_{193} = \texttt{8.48.0.98}$ & $\operatorname{H}_{235} = \texttt{16.48.0.96}$ & $\operatorname{H}_{235} = \texttt{16.48.0.96}$ & \texttt{25410.bl} \\
\cline{3-11}
& & $\operatorname{H}_{192a} = \texttt{16.96.0.72}$ & $\operatorname{H}_{211q} = \texttt{16.96.0.315}$ & $\operatorname{H}_{211l} = \texttt{32.96.0.54}$ & $\operatorname{H}_{189f} = \texttt{16.96.0.17}$ & $\operatorname{H}_{207e} = \texttt{32.96.0.23}$ & $\operatorname{H}_{193e} = \texttt{16.96.0.43}$ & $\operatorname{H}_{235o} = \texttt{16.96.0.310}$ & $\operatorname{H}_{235s} = \texttt{32.96.0.35}$ & \texttt{7350.w} \\
\cline{3-11}
& & $\operatorname{H}_{192b} = \texttt{16.96.0.73}$ & $\operatorname{H}_{211b} = \texttt{32.96.0.53}$ & $\operatorname{H}_{211e} = \texttt{16.96.0.314}$ & $\operatorname{H}_{189g} = \texttt{16.96.0.18}$ & $\operatorname{H}_{207f} = \texttt{32.96.0.24}$ & $\operatorname{H}_{193f} = \texttt{16.96.0.44}$ & $\operatorname{H}_{235r} = \texttt{16.96.0.312}$ & $\operatorname{H}_{235p} = \texttt{32.96.0.34}$ & \texttt{1050.c} \\
\cline{3-11}
& & $\operatorname{H}_{192c} = \texttt{16.96.0.74}$ & $\operatorname{H}_{211f} = \texttt{32.96.0.56}$ & $\operatorname{H}_{211a} = \texttt{16.96.0.313}$ & $\operatorname{H}_{189n} = \texttt{16.96.0.15}$ & $\operatorname{H}_{207a} = \texttt{32.96.0.21}$ & $\operatorname{H}_{193l} = \texttt{16.96.0.41}$ & $\operatorname{H}_{235n} = \texttt{32.96.0.33}$ & $\operatorname{H}_{235m} = \texttt{16.96.0.309}$ & \texttt{3150.bp} \\
\cline{3-11}
& & $\operatorname{H}_{192d} = \texttt{16.96.0.71}$ & $\operatorname{H}_{211i} = \texttt{32.96.0.55}$ & $\operatorname{H}_{211o} = \texttt{16.96.0.316}$ & $\operatorname{H}_{189m} = \texttt{16.96.0.16}$ & $\operatorname{H}_{207b} = \texttt{32.96.0.22}$ & $\operatorname{H}_{193k} = \texttt{16.96.0.42}$ & $\operatorname{H}_{235t} = \texttt{32.96.0.36}$ & $\operatorname{H}_{235q} = \texttt{16.96.0.311}$ & \texttt{25200.p} \\
\cline{3-11}
& & $\operatorname{H}_{192e} = \texttt{8.96.0.123}$ & $\operatorname{H}_{211r} = \texttt{16.96.0.223}$ & $\operatorname{H}_{211g} = \texttt{16.96.0.283}$ & $\operatorname{H}_{189k} = \texttt{8.96.0.90}$ & $\operatorname{H}_{207g} = \texttt{16.96.0.202}$ & $\operatorname{H}_{193b} = \texttt{16.96.0.48}$ & $\operatorname{H}_{235h} = \texttt{32.96.0.39}$ & $\operatorname{H}_{235h} = \texttt{32.96.0.39}$ & \texttt{630.a} \\
\cline{3-11}
& & $\operatorname{H}_{192f} = \texttt{16.96.0.76}$ & $\operatorname{H}_{211n} = \texttt{32.96.0.60}$ & $\operatorname{H}_{211n} = \texttt{32.96.0.60}$ & $\operatorname{H}_{189j} = \texttt{8.96.0.64}$ & $\operatorname{H}_{207h} = \texttt{16.96.0.19}$ & $\operatorname{H}_{193d} = \texttt{16.96.0.45}$ & $\operatorname{H}_{235b} = \texttt{32.96.0.40}$ & $\operatorname{H}_{235b} = \texttt{32.96.0.40}$ & \texttt{4410.t} \\
\cline{3-11}
& & $\operatorname{H}_{192k} = \texttt{16.96.0.75}$ & $\operatorname{H}_{211k} = \texttt{32.96.0.59}$ & $\operatorname{H}_{211k} = \texttt{32.96.0.59}$ & $\operatorname{H}_{189a} = \texttt{8.96.0.63}$ & $\operatorname{H}_{207d} = \texttt{16.96.0.183}$ & $\operatorname{H}_{193h} = \texttt{16.96.0.46}$ & $\operatorname{H}_{235d} = \texttt{32.96.0.38}$ & $\operatorname{H}_{235d} = \texttt{32.96.0.38}$ & \texttt{141120.gt} \\
\cline{3-11}
& & $\operatorname{H}_{192l} = \texttt{8.96.0.125}$ & $\operatorname{H}_{211t} = \texttt{16.96.0.218}$ & $\operatorname{H}_{211t} = \texttt{16.96.0.218}$ & $\operatorname{H}_{189i} = \texttt{8.96.0.79}$ & $\operatorname{H}_{207m} = \texttt{16.96.0.187}$ & $\operatorname{H}_{193m} = \texttt{8.96.0.140}$ & $\operatorname{H}_{235g} = \texttt{16.96.0.237}$ & $\operatorname{H}_{235g} = \texttt{16.96.0.237}$ & \texttt{6720.bq} \\
\cline{3-11}
& & $\operatorname{H}_{192m} = \texttt{16.96.0.77}$ & $\operatorname{H}_{211d} = \texttt{32.96.0.58}$ & $\operatorname{H}_{211d} = \texttt{32.96.0.58}$ & $\operatorname{H}_{189h} = \texttt{8.96.0.71}$ & $\operatorname{H}_{207i} = \texttt{16.96.0.192}$ & $\operatorname{H}_{193c} = \texttt{8.96.0.127}$ & $\operatorname{H}_{235a} = \texttt{16.96.0.241}$ & $\operatorname{H}_{235e} = \texttt{16.96.0.257}$ & \texttt{47040.ha} \\
\cline{3-11}
& & $\operatorname{H}_{192n} = \texttt{8.96.0.153}$ & $\operatorname{H}_{211j} = \texttt{16.96.0.279}$ & $\operatorname{H}_{211j} = \texttt{16.96.0.279}$ & $\operatorname{H}_{189l} = \texttt{8.96.0.88}$ & $\operatorname{H}_{207j} = \texttt{16.96.0.188}$ & $\operatorname{H}_{193a} = \texttt{8.96.0.130}$ & $\operatorname{H}_{235k} = \texttt{16.96.0.253}$ & $\operatorname{H}_{235k} = \texttt{16.96.0.253}$ & \texttt{6720.j} \\
\cline{3-11}
& & $\operatorname{H}_{194} = \texttt{8.48.0.91}$ & $\operatorname{H}_{213} = \texttt{16.48.0.97}$ & $\operatorname{H}_{227} = \texttt{16.48.0.144}$ & $\operatorname{H}_{183} = \texttt{8.48.0.50}$ & $\operatorname{H}_{205} = \texttt{8.48.0.199}$ & $\operatorname{H}_{208} = \texttt{16.48.0.6}$ & $\operatorname{H}_{243} = \texttt{32.48.0.8}$ & $\operatorname{H}_{243} = \texttt{32.48.0.8}$ & \texttt{1530.b} \\
\cline{3-11}
& & $\operatorname{H}_{194a} = \texttt{16.96.0.37}$ & $\operatorname{H}_{213b} = \texttt{32.96.0.43}$ & $\operatorname{H}_{227c} = \texttt{32.96.0.71}$ & $\operatorname{H}_{183f} = \texttt{8.96.0.68}$ & $\operatorname{H}_{205a} = \texttt{16.96.0.206}$ & $\operatorname{H}_{208l} = \texttt{16.96.0.68}$ & $\operatorname{H}_{243f} = \texttt{32.96.0.88}$ & $\operatorname{H}_{243a} = \texttt{32.96.0.92}$ & \texttt{252150.c} \\
\cline{3-11}
& & $\operatorname{H}_{194b} = \texttt{16.96.0.39}$ & $\operatorname{H}_{213c} = \texttt{32.96.0.42}$ & $\operatorname{H}_{227b} = \texttt{32.96.0.70}$ & $\operatorname{H}_{183b} = \texttt{8.96.0.76}$ & $\operatorname{H}_{205k} = \texttt{8.96.0.171}$ & $\operatorname{H}_{208k} = \texttt{16.96.0.50}$ & $\operatorname{H}_{243n} = \texttt{32.96.0.84}$ & $\operatorname{H}_{243j} = \texttt{32.96.0.46}$ & \texttt{196800.ii} \\
\cline{3-11}
& & $\operatorname{H}_{194c} = \texttt{16.96.0.40}$ & $\operatorname{H}_{213d} = \texttt{32.96.0.44}$ & $\operatorname{H}_{227a} = \texttt{32.96.0.72}$ & $\operatorname{H}_{183g} = \texttt{8.96.0.96}$ & $\operatorname{H}_{205g} = \texttt{8.96.0.98}$ & $\operatorname{H}_{208f} = \texttt{16.96.0.34}$ & $\operatorname{H}_{243i} = \texttt{32.96.0.78}$ & $\operatorname{H}_{243o} = \texttt{32.96.0.32}$ & \texttt{6150.r} \\
\cline{3-11}
& & $\operatorname{H}_{194e} = \texttt{8.96.0.132}$ & $\operatorname{H}_{213l} = \texttt{16.96.0.254}$ & $\operatorname{H}_{227h} = \texttt{16.96.0.261}$ & $\operatorname{H}_{183k} = \texttt{8.96.0.75}$ & $\operatorname{H}_{205j} = \texttt{8.96.0.174}$ & $\operatorname{H}_{208j} = \texttt{16.96.0.80}$ & $\operatorname{H}_{243h} = \texttt{32.96.0.86}$ & $\operatorname{H}_{243h} = \texttt{32.96.0.86}$ & \texttt{16320.m} \\
\cline{3-11}
& & $\operatorname{H}_{194f} = \texttt{8.96.0.134}$ & $\operatorname{H}_{213g} = \texttt{16.96.0.238}$ & $\operatorname{H}_{227j} = \texttt{16.96.0.297}$ & $\operatorname{H}_{183e} = \texttt{8.96.0.74}$ & $\operatorname{H}_{205l} = \texttt{8.96.0.173}$ & $\operatorname{H}_{208h} = \texttt{16.96.0.82}$ & $\operatorname{H}_{243c} = \texttt{32.96.0.90}$ & $\operatorname{H}_{243c} = \texttt{32.96.0.90}$ & \texttt{16320.bw} \\
\cline{3-11}
& & $\operatorname{H}_{194i} = \texttt{8.96.0.126}$ & $\operatorname{H}_{213j} = \texttt{16.96.0.258}$ & $\operatorname{H}_{227l} = \texttt{16.96.0.301}$ & $\operatorname{H}_{183l} = \texttt{8.96.0.93}$ & $\operatorname{H}_{205e} = \texttt{16.96.0.210}$ & $\operatorname{H}_{208b} = \texttt{16.96.0.62}$ & $\operatorname{H}_{243k} = \texttt{32.96.0.80}$ & $\operatorname{H}_{243k} = \texttt{32.96.0.80}$ & \texttt{69360.q} \\
\cline{3-11}
& & $\operatorname{H}_{194j} = \texttt{8.96.0.139}$ & $\operatorname{H}_{213e} = \texttt{16.96.0.242}$ & $\operatorname{H}_{227f} = \texttt{16.96.0.265}$ & $\operatorname{H}_{183h} = \texttt{8.96.0.82}$ & $\operatorname{H}_{205f} = \texttt{16.96.0.208}$ & $\operatorname{H}_{208d} = \texttt{16.96.0.36}$ & $\operatorname{H}_{243m} = \texttt{32.96.0.30}$ & $\operatorname{H}_{243m} = \texttt{32.96.0.30}$ & \texttt{8670.v} \\
\cline{3-11}
\hline
\end{tabular}}
\caption{2-adic Images of $T_{8}$ Graphs}
\label{2-adic Images of T8 Graphs}
\end{table}
\end{center}

\newpage

\subsection{Isogeny-torsion graphs of $S$ type}

Table \ref{2-adic Images of S Graphs Table} contains the known examples of $2$-adic images associated to isogeny-torsion graphs of $S$ type. Clearly, all $2$-adic images come from Table \ref{2-adic Images of T4 Graphs} as the $2$-adic subgraph of an isogeny-torsion graph of $S$ type is of $T_{4}$ type. Let $E/\QQ$ be an elliptic curve such that $E$ has full two-torsion defined over $\QQ$ and a $\QQ$-rational subgroup of order $3$. Then $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to the full lift of a subgroup of $\operatorname{H}_{8}$. The RZB database says that there are four modular curves that cover $\operatorname{X}_{8}$ minimally whose generated groups contain $\operatorname{-Id}$: $\operatorname{X}_{24}$, $\operatorname{X}_{25}$, $\operatorname{X}_{38}$, and $\operatorname{X}_{46}$. The group $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is not conjugate to the full lift of a subgroup of $\operatorname{H}_{25}$ as $E$ does not have a cyclic, $\QQ$-rational subgroup of order $4$. There are no examples in the LMFDB of an elliptic curve over $\QQ$ with a $\QQ$-rational subgroup of order $3$, and $2$-adic image conjugate to $\operatorname{H}_{24}$, $\operatorname{H}_{38}$, or $\operatorname{H}_{46}$. Moreover, there are no examples in the LMFDB of an elliptic curve over $\QQ$ with a point of order $3$ defined over $\QQ$ and $2$-adic image conjugate to $\operatorname{H}_{8a}$ or $\operatorname{H}_{8b}$.


\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.7}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Isogeny Graph & $E_{1}$ & $E_{2}$ & $E_{3}$ & $E_{4}$ & $E_{5}$ & $E_{6}$ & $E_{7}$ & $E_{8}$ & Isogeny-Torsion Graph & Example Isogeny Class\\
    \hline
    \multirow{8}*{\includegraphics[scale=0.25]{Snew}} &
    \multirow{2}*{$\operatorname{H}_{8}$} & \multirow{2}*{$\operatorname{H}_{8}$} & \multirow{2}*{$\operatorname{H}_{13}$} & \multirow{2}*{$\operatorname{H}_{13}$} & \multirow{2}*{$\operatorname{H}_{13}$} & \multirow{2}*{$\operatorname{H}_{13}$} & \multirow{2}*{$\operatorname{H}_{13}$} & \multirow{2}*{$\operatorname{H}_{13}$} & $([2,6],[2,2],[6],[2],[6],[2],[6],[2])$ & \texttt{630.f} \\
    \cline{10-11}
    & & & & & & & & & $([2,2],[2,2],[2],[2],[2],[2],[2],[2])$ & \texttt{3630.w} \\
    \cline{2-11}
    & $\operatorname{H}_{8a}$ & $\operatorname{H}_{8a}$ & $\operatorname{H}_{13a}$ & $\operatorname{H}_{13a}$ & $\operatorname{H}_{13a}$ & $\operatorname{H}_{13a}$ & $\operatorname{H}_{13a}$ & $\operatorname{H}_{13a}$ & $([2,2],[2,2],[2],[2],[2],[2],[2],[2])$ & \texttt{450.d} \\
    \cline{2-11}
    & $\operatorname{H}_{8b}$ & $\operatorname{H}_{8b}$ & $\operatorname{H}_{13b}$ & $\operatorname{H}_{13b}$ & $\operatorname{H}_{13b}$ & $\operatorname{H}_{13b}$ & $\operatorname{H}_{13b}$ & $\operatorname{H}_{13b}$ & $([2,2],[2,2],[2],[2],[2],[2],[2],[2])$ & \texttt{14400.o} \\
    \cline{2-11}
    & \multirow{2}*{$\operatorname{H}_{8c}$} & \multirow{2}*{$\operatorname{H}_{8c}$} & \multirow{2}*{$\operatorname{H}_{13c}$} & \multirow{2}*{$\operatorname{H}_{13c}$} & \multirow{2}*{$\operatorname{H}_{13e}$} & \multirow{2}*{$\operatorname{H}_{13e}$} & \multirow{2}*{$\operatorname{H}_{13g}$} & \multirow{2}*{$\operatorname{H}_{13g}$} & $([2,6],[2,2],[6],[2],[6],[2],[6],[2])$ & \texttt{30.a} \\
    \cline{10-11}
    & & & & & & & & & $([2,2],[2,2],[2],[2],[2],[2],[2],[2])$ & \texttt{240.b} \\
    \cline{2-11}
    & \multirow{2}*{$\operatorname{H}_{8d}$} & \multirow{2}*{$\operatorname{H}_{8d}$} & \multirow{2}*{$\operatorname{H}_{13h}$} & \multirow{2}*{$\operatorname{H}_{13h}$} & \multirow{2}*{$\operatorname{H}_{13d}$} & \multirow{2}*{$\operatorname{H}_{13d}$} & \multirow{2}*{$\operatorname{H}_{13f}$} & \multirow{2}*{$\operatorname{H}_{13f}$} & $([2,6],[2,2],[12],[4],[6],[2],[6],[2])$ & \texttt{90.c} \\
    \cline{10-11}
    & & & & & & & & & $([2,2],[2,2],[4],[4],[2],[2],[2],[2])$ & \texttt{150.b} \\
    \hline

    
\end{tabular}}
\caption{2-adic Images of S Graphs}
\label{2-adic Images of S Graphs Table}
\end{table}
\end{center}

\subsection{Isogeny-torsion graphs of $R_{k}$ type}
Here we classify the $2$-adic images attached to isogeny-torsion graphs of $R_{6}$, $R_{4}(6)$, $R_{4}(10)$, $R_{4}(15)$, and $R_{4}(21)$ type.

\begin{itemize}
    \item Isogeny-torsion graphs of $R_{6}$ type
    
    \begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.7}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \hline
    
    Isogeny Graph & $E_{1}$ & $E_{2}$ & $E_{3}$ & $E_{4}$ & $E_{5}$ & $E_{6}$ & Isogeny-Torsion Graph & Example Isogeny Class \\
    \hline
    \multirow{4}*{\includegraphics[scale=0.25]{R6new.jpg}} & \multirow{2}*{$\operatorname{H}_{16}$} & \multirow{2}*{$\operatorname{H}_{17}$} & \multirow{2}*{$\operatorname{H}_{16}$} & \multirow{2}*{$\operatorname{H}_{17}$} & \multirow{2}*{$\operatorname{H}_{16}$} & \multirow{2}*{$\operatorname{H}_{17}$} & $([6],[6],[6],[6],[2],[2])$ & \texttt{14.a} \\
    \cline{8-9}
    & & & & & & & $([2],[2],[2],[2],[2],[2])$ & \texttt{98.a} \\
    \cline{2-9}
    & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & $([6],[6],[6],[6],[2],[2])$ & \texttt{2394.j} \\
    \cline{8-9}
    & & & & & & & $([2],[2],[2],[2],[2],[2])$ & \texttt{271950.do} \\
    \hline
    
	\end{tabular}}
\caption{2-adic Images of $R_{6}$ Graphs}
\label{2-adic Images of R6 Graphs Table}
\end{table}
\end{center}

Table \ref{2-adic Images of R6 Graphs Table} contains the known examples of the $2$-adic images attached to isogeny-torsion graphs of $R_{6}$ type.

Let $E/\QQ$ be an elliptic curve such that $E$ has a point of order $2$ defined over $\QQ$ and $E$ has two $\QQ$-rational subgroups of order $3$. Then $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to some subgroup of the full lift of $\operatorname{H}_{6}$. The RZB database says that the modular curves that minimally cover $\operatorname{X}_{6}$ are $\operatorname{X}_{i}$, where $i \in \{8, \ldots, 19\}$. By Table \ref{2-adic Images of L22 Graphs}, $\operatorname{H}_{9}$ is $\QQ$-isogenous to $\operatorname{H}_{10}$, $\operatorname{H}_{15}$ is $\QQ$-isogenous to $\operatorname{H}_{19}$, and $\operatorname{H}_{16}$ is $\QQ$-isogenous to $\operatorname{H}_{17}$. The modular curves in the RZB database that cover $\operatorname{X}_{16}$ minimally are $\operatorname{X}_{29}$, $\operatorname{X}_{38}$, $\operatorname{X}_{40}$, and $\operatorname{X}_{42}$. The only examples in the LMFDB of an elliptic curve like $E$ have $2$-adic image conjugate to $\operatorname{H}_{6}$, $\operatorname{H}_{16}$, or $\operatorname{H}_{17}$.

\item Isogeny-torsion graphs of $R_{4}$ type


\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.7}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    
    Isogeny Graph & $pq$ & $E_{1}$ & $E_{2}$ & $E_{3}$ & $E_{4}$ & Isogeny-Torsion Graph & Example Isogeny Class \\
    \hline
    \multirow{24}*{\includegraphics[scale=0.10]{Rk Graph.png}} & \multirow{2}*{$21$} & \multirow{2}*{$\operatorname{H}_{4}$} & \multirow{2}*{$\operatorname{H}_{4}$} & \multirow{2}*{$\operatorname{H}_{4}$} & \multirow{2}*{$\operatorname{H}_{4}$} & $([3],[3],[1],[1])$ & \texttt{162.b} \\
    \cline{7-8}
    & & & & & & $([1],[1],[1],[1])$ & \texttt{1296.f} \\
    \cline{2-8}
    & \multirow{3}*{$15$} & \multirow{3}*{$\operatorname{H}_{4}$} & 
    \multirow{3}*{$\operatorname{H}_{4}$} & \multirow{3}*{$\operatorname{H}_{4}$} & \multirow{3}*{$\operatorname{H}_{4}$} & $([5],[5],[1],[1])$ & \texttt{50.a} \\
    \cline{7-8}
    & & & & & & $([3],[3],[1],[1])$ & \texttt{50.b} \\
    \cline{7-8}
    & & & & & & $([1],[1],[1],[1])$ & \texttt{400.d} \\
    \cline{2-8}
    & \multirow{5}*{$10$} & \multirow{2}*{$\operatorname{H}_{15}$} & \multirow{2}*{$\operatorname{H}_{19}$} & \multirow{2}*{$\operatorname{H}_{15}$} & \multirow{2}*{$\operatorname{H}_{19}$} & $([10],[10],[2],[2])$ & \texttt{66.c} \\
    \cline{7-8}
    & & & & & & $([2],[2],[2],[2])$ & \texttt{198.c} \\
    \cline{3-8}
    & & $\operatorname{H}_{14}$ & $\operatorname{H}_{14}$ & $\operatorname{H}_{14}$ & $\operatorname{H}_{14}$ & $([2],[2],[2],[2])$ & \texttt{1734.d} \\
    \cline{3-8}
    & & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & $([10],[10],[2],[2])$ & \texttt{150.c} \\
\cline{7-8}
& & & & & & $([2],[2],[2],[2])$ & \texttt{150.a} \\
\cline{2-8}
& \multirow{14}*{$6$} & \multirow{2}*{$\operatorname{H}_{16}$} & \multirow{2}*{$\operatorname{H}_{17}$} & \multirow{2}*{$\operatorname{H}_{16}$} & \multirow{2}*{$\operatorname{H}_{17}$} & $([6],[6],[2],[2])$ & \texttt{34.a} \\
    \cline{7-8}
    & & & & & & $([2],[2],[2],[2])$ & \texttt{272.d} \\
    \cline{3-8}
    & & \multirow{2}*{$\operatorname{H}_{15}$} & \multirow{2}*{$\operatorname{H}_{19}$} & \multirow{2}*{$\operatorname{H}_{15}$} & \multirow{2}*{$\operatorname{H}_{19}$} & $([6],[6],[2],[2])$ & \texttt{66.a} \\
    \cline{7-8}
    & & & & & & $([2],[2],[2],[2])$ & \texttt{528.d} \\
    \cline{3-8}
    & & \multirow{2}*{$\operatorname{H}_{9d}$} & \multirow{2}*{$\operatorname{H}_{10d}$} & \multirow{2}*{$\operatorname{H}_{9d}$} & \multirow{2}*{$\operatorname{H}_{10d}$} & $([6],[6],[2],[2])$ & \texttt{130.a} \\
    \cline{7-8}
    & & & & & & $([2],[2],[2],[2])$ & \texttt{320.a} \\
    \cline{3-8}
    & & \multirow{2}*{$\operatorname{H}_{9c}$} & \multirow{2}*{$\operatorname{H}_{10a}$} & \multirow{2}*{$\operatorname{H}_{9c}$} & \multirow{2}*{$\operatorname{H}_{10a}$} & $([6],[6],[2],[2])$ & \texttt{20.a} \\
    \cline{7-8}
    & & & & & & $([2],[2],[2],[2])$ & \texttt{80.b} \\
    \cline{3-8}
    & & $\operatorname{H}_{9b}$ & $\operatorname{H}_{10b}$ & $\operatorname{H}_{9b}$ & $\operatorname{H}_{10b}$ & $([2],[2],[2],[2])$ & \texttt{1600.c} \\
    \cline{3-8}
    & & $\operatorname{H}_{9a}$ & $\operatorname{H}_{10c}$ & $\operatorname{H}_{9a}$ & $\operatorname{H}_{10c}$ & $([2],[2],[2],[2])$ & \texttt{100.a} \\
    \cline{3-8}
    & & \multirow{2}*{$\operatorname{H}_{9}$} & \multirow{2}*{$\operatorname{H}_{10}$} & \multirow{2}*{$\operatorname{H}_{9}$} & \multirow{2}*{$\operatorname{H}_{10}$} & $([6],[6],[2],[2])$ & \texttt{180.a} \\
    \cline{7-8}
    & & & & & & $([2],[2],[2],[2])$ & \texttt{650.l} \\
    \cline{3-8}
    & & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & $([6],[6],[2],[2])$ & \texttt{84.b} \\
    \cline{7-8}
    & & & & & & $([2],[2],[2],[2])$ & \texttt{336.b} \\
    \hline
    \end{tabular}}
\caption{2-adic Images of $R_{4}$ Graphs}
\label{2-adic Images of R4 Graphs Table}
\end{table}
\end{center}

Table \ref{2-adic Images of R4 Graphs Table} contains the known examples of $2$-adic images attached to isogeny-torsion graphs of $R_{4}$ type.

\begin{enumerate}
    \item Isogey-torsion graphs of $R_{4}(21)$ or $R_{4}(15)$ type
    
    Let $E/\QQ$ be an elliptic curve with a cyclic, $\QQ$-rational subgroup of order $15$ or $21$. Then $\textit{j}_{E} = \frac{-349938025}{8}$, $\frac{-121945}{32}$, $\frac{-25}{2}$, or $\frac{46969655}{32768}$ in the former case and $\frac{-189613868625}{128}$, $\frac{-1159088625}{2097152}$, $\frac{-140625}{8}$, or $\frac{3375}{2}$ in the latter.
    
    Let $E'$ be an elliptic curve in the $\QQ$-isogeny class with LMFDB notation \texttt{50.a}. Then $E'$ is $\QQ$-isogenous to one elliptic curve with \textit{j}-invariant equal to one of the four \textit{j}-invariants associated to an elliptic curve over $\QQ$ with a cyclic, $\QQ$-rational, subgroup of order $15$. Now let $E'$ be an elliptic curve in the $\QQ$-isogeny class with LMFDB notation \texttt{162.b}. Then $E'$ is $\QQ$-isogenous to one elliptic curve with \textit{j}-invariant equal to one of the four \textit{j}-invariants associated to an elliptic curve over $\QQ$ with a cyclic, $\QQ$-rational, subgroup of order $21$. By Corollary \ref{coprime isogeny-degree} with $\ell = 2$, all $2$-adic images attached to elliptic curves in \texttt{50.a} and \texttt{162.b} are the same. 
    
    The image of $\overline{\rho}_{E',2^{\infty}}(G_{\QQ})$ is conjugate to the full lift of $\operatorname{H}_{4} = \texttt{8.2.0.1}$. By Lemma \ref{kernel of pi 1}, $\overline{\rho}_{E',32}(G_{\QQ})$ is conjugate to
    $$\left\langle
    \begin{bmatrix} 7 & 0 \\ 7 & 1 \end{bmatrix},
    \begin{bmatrix} 5 & 1 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}
    \right\rangle.$$
    All quadratic twists of $\operatorname{H}_{4}$ contain $\operatorname{-Id}$. The elliptic curve $E$ is a quadratic twist of one of the elliptic curves in \texttt{50.a} or \texttt{162.b}. Thus, $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to $\operatorname{H}_{4}$.
    
    \item Isogeny-torsion graphs of $R_{4}(10)$ type
    
    Table \ref{2-adic Images of R4 Graphs Table} contain all of the known $2$-adic images attached to isogeny-torsion graphs of $R_{4}(10)$ type. The modular curves that cover $\operatorname{X}_{15}$ minimally are $\operatorname{X}_{41}$ and $\operatorname{X}_{46}$. Elliptic curves over $\QQ$ corresponding to $\operatorname{X}_{46}$ have full two-torsion defined over $\QQ$, hence, cannot have $\QQ$-rational subgroups of order $5$. The group $\operatorname{H}_{41}$ reduces mod-$4$ to $\operatorname{H}_{11}$. The modular curves that cover $\operatorname{X}_{14}$ minimally are $\operatorname{X}_{38}$ and $\operatorname{X}_{44}$. Elliptic curves corresponding to $\operatorname{X}_{38}$ have full two-torsion defined over $\QQ$ and hence, no $\QQ$-rational subgroup of order $5$. The group $\operatorname{H}_{44}$ reduces mod-$4$ to $\operatorname{H}_{13}$. The modular curves that cover $\operatorname{H}_{6}$ minimally are $\operatorname{H}_{i}$ where $i \in \{8, \ldots, 19\}$. The modular curves $\operatorname{H}_{8}$ and $\operatorname{H}_{13}$ correspond to elliptic curves over $\QQ$ with full two-torsion defined over $\QQ$ and a cyclic $\QQ$-rational subgroup of order $4$, respectively. Thus, by Theorem \ref{thm-kenku}, we can immediately eliminate the possibility of $\operatorname{H}_{8}$ and $\operatorname{H}_{13}$.
    
    By the fact that, $\operatorname{X}_{9}$ is $\QQ$-isogenous to $\operatorname{X}_{10}$, $\operatorname{X}_{15}$ is $\QQ$-isogenous to $\operatorname{X}_{19}$, and $\operatorname{X}_{16}$ is $\QQ$-isogenous to $\operatorname{X}_{17}$, we need to check if there exists an elliptic curve $E/\QQ$ such that $E$ contains a $\QQ$-rational subgroup of order $5$ and $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to the full lift of $\operatorname{H}_{k}$ where $k \in \{9, 11, 12, 15, 16, 18\}$. We also need to check if there is an elliptic curve $E/\QQ$ such that $E(\QQ)_{\text{tors}} \cong \ZZ / 10 \ZZ$ and $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to $\operatorname{H}_{14}$.
    
    \item Isogeny-torsion graphs of $R_{4}(6)$ type
    
    Table \ref{2-adic Images of R4 Graphs Table} contain all of the known $2$-adic images attached to isogeny-torsion graphs of $R_{4}(6)$ type. The process is very similar to the process used to find the $2$-adic images attached to isogeny-torsion graphs of $R_{6}$ type and $R_{4}(10)$ type.
    
    The modular curves that cover $\operatorname{X}_{16}$ minimally are $\operatorname{X}_{29}$, $\operatorname{X}_{38}$, $\operatorname{X}_{40}$, $\operatorname{X}_{42}$. Let $E/\QQ$ be an elliptic curve. If $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to the full lift of $\operatorname{H}_{29}$, then $\overline{\rho}_{E,4}(G_{\QQ})$ is conjugate to $\operatorname{H}_{11}$. If $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to the full lift of the full lift of $\operatorname{H}_{38}$, then $E$ has full two-torsion defined over $\QQ$. If $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to the full lift of $\operatorname{H}_{40}$, then $\overline{\rho}_{E,4}(G_{\QQ})$ is conjugate to $\operatorname{H}_{12}$.
    
    The modular curves that cover $\operatorname{X}_{15}$ minimally are $\operatorname{X}_{41}$ and $\operatorname{X}_{46}$. Let $E/\QQ$ be an elliptic curve. If $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to the full lift of $\operatorname{H}_{41}$, then $\overline{\rho}_{E,4}(G_{\QQ})$ is conjugate to $\operatorname{H}_{11}$. If $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to $\operatorname{H}_{46}$, then $E$ has full two-torsion defined over $\QQ$, which is not what we want here.
    
    The modular curves that cover $\operatorname{X}_{9}$ minimally are $\operatorname{X}_{24}$ and $\operatorname{X}_{37}$. Let $E/\QQ$ be an elliptic curve. If $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to the full lift of $\operatorname{H}_{24}$, then $E$ has full two-torsion defined over $\QQ$, which is not what we want here.
    
    We need to check if there is an elliptic curve $E/\QQ$ with a $\QQ$-rational subgroup of order $3$ such that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to the full lift of $\operatorname{H}_{11}$, $\operatorname{H}_{12}$, $\operatorname{H}_{14}$, $\operatorname{H}_{18}$ $\operatorname{H}_{37}$, or $\operatorname{H}_{42}$. Also, we need to check if there is an elliptic curve $E/\QQ$ such that $E(\QQ)_{\text{tors}} \cong \ZZ / 6 \ZZ$ such that $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to $\operatorname{H}_{9a}$ or $\operatorname{H}_{9b}$.
    
\end{enumerate}
\end{itemize}

\newpage
\subsection{Isogeny-torsion graphs of $L_{k}$ type}

Here we classify the $2$-adic images attached to isogeny-torsion graphs of $L_{2}(p)$ and $L_{3}(q^{2})$ type where $2 \leq p \leq 37$ and $q = 3$ or $5$.

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1}
\scalebox{0.7}{
    \begin{tabular}{|c|c|c|c|c|c|}

\hline

Isogeny Graph & $p$ & $E_{1}$ & $E_{2}$ & Isogeny-Torsion Graph & Example Isogeny Class \\
    \hline

\multirow{48}*{\includegraphics[scale=0.075]{L2 Graph.png}} & $37$ & $\operatorname{H}_{1}$ & $\operatorname{H}_{1}$ & $([1],[1])$ & \texttt{1225.b} \\
\cline{2-6}
& $17$ & $\operatorname{H}_{1}$ & $\operatorname{H}_{1}$ & $([1],[1])$ & \texttt{14450.b} \\
\cline{2-6}
& \multirow{2}*{$13$} & $\operatorname{H}_{1}$ & $\operatorname{H}_{1}$ & $([1],[1])$ & \texttt{147.b} \\
\cline{3-6}
& & $\operatorname{H}_{4}$ & $\operatorname{H}_{4}$ & $([1],[1])$ & \texttt{11094.g} \\
\cline{2-6}
& \multirow{3}*{$11$} & $\operatorname{H}_{3}$ & $\operatorname{H}_{3}$ & $([1],[1])$ & \texttt{121.a} \\
\cline{3-6}
& & $\operatorname{H}_{3a}$ & $\operatorname{H}_{3a}$ & $([1],[1])$ & \texttt{7744.c} \\
\cline{3-6}
& & $\operatorname{H}_{3b}$ & $\operatorname{H}_{3b}$ & $([1],[1])$ & \texttt{121.c} \\
\cline{2-6}
& \multirow{13}*{$7$} & \multirow{2}*{$\operatorname{H}_{1}$} & \multirow{2}*{$\operatorname{H}_{1}$} & $([7],[1])$ & \texttt{26.b} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{208.d} \\
\cline{3-6}
& & $\operatorname{H}_{2}$ & $\operatorname{H}_{2}$ & $([1],[1])$ & \texttt{1922.c} \\
\cline{3-6}
& & $\operatorname{H}_{2a}$ & $\operatorname{H}_{2a}$ & $([1],[1])$ & \texttt{3969.d} \\
\cline{3-6}
& & $\operatorname{H}_{2b}$ & $\operatorname{H}_{2b}$ & $([1],[1])$ & \texttt{1922.e} \\
\cline{3-6}
& & $\operatorname{H}_{3}$ & $\operatorname{H}_{3}$ & $([1],[1])$ & \texttt{507.b} \\
\cline{3-6}
& & $\operatorname{H}_{3a}$ & $\operatorname{H}_{3a}$ & $([1],[1])$ & \texttt{87616.w} \\
\cline{3-6}
& & $\operatorname{H}_{3b}$ & $\operatorname{H}_{3b}$ & $([1],[1])$ & \texttt{1369.d} \\
\cline{3-6}
& & $\operatorname{H}_{4}$ & $\operatorname{H}_{4}$ & $([1],[1])$ & \texttt{11094.i} \\
\cline{3-6}
& & $\operatorname{H}_{5}$ & $\operatorname{H}_{5}$ & $([1],[1])$ & \texttt{12482.f} \\
\cline{3-6}
& & $\operatorname{H}_{20}$ & $\operatorname{H}_{20}$ & $([1],[1])$ & \texttt{338.c} \\
\cline{3-6}
& & $\operatorname{H}_{20a}$ & $\operatorname{H}_{20a}$ & $([1],[1])$ & \texttt{10816.u1} \\
\cline{3-6}
& & $\operatorname{H}_{20b}$ & $\operatorname{H}_{20b}$ & $([1],[1])$ & \texttt{338.e} \\
\cline{2-6}
& \multirow{5}*{$5$} & \multirow{2}*{$\operatorname{H}_{1}$} & \multirow{2}*{$\operatorname{H}_{1}$} & $([5],[1])$ & \texttt{38.b} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{75.c} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{4}$} & \multirow{2}*{$\operatorname{H}_{4}$} & $([5],[1])$ & \texttt{38350.t} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{6400.d} \\
\cline{3-6}
& & $\operatorname{H}_{7}$ & $\operatorname{H}_{7}$ & $([1],[1])$ & \texttt{14450.h} \\
\cline{2-6}
& \multirow{23}*{$3$} & \multirow{2}*{$\operatorname{H}_{1}$} & \multirow{2}*{$\operatorname{H}_{1}$} & $([3],[1])$ & \texttt{44.a} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{176.a} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{2}$} & \multirow{2}*{$\operatorname{H}_{2}$} & $([3],[1])$ & \texttt{324.a} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{196.a} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{2a}$} & \multirow{2}*{$\operatorname{H}_{2a}$} & $([3],[1])$ & \texttt{196.b} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{784.d} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{2b}$} & \multirow{2}*{$\operatorname{H}_{2b}$} & $([3],[1])$ & \texttt{1922.b} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{3136.h} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{3}$} & \multirow{2}*{$\operatorname{H}_{3}$} & $([3],[1])$ & \texttt{324.d} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{242.b} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{3a}$} & \multirow{2}*{$\operatorname{H}_{3a}$} & $([3],[1])$ & \texttt{1058.b} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{5184.z} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{3b}$} & \multirow{2}*{$\operatorname{H}_{3b}$} & $([3],[1])$ & \texttt{242.a} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{1296.a} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{4}$} & \multirow{2}*{$\operatorname{H}_{4}$} & $([3],[1])$ & \texttt{350.e} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{350.a} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{5}$} & \multirow{2}*{$\operatorname{H}_{5}$} & $([3],[1])$ & \texttt{1682.b} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{1682.i} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{20}$} & \multirow{2}*{$\operatorname{H}_{20}$} & $([3],[1])$ & \texttt{162.a} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{1296.c} \\
\cline{3-6}
& & $\operatorname{H}_{20a}$ & $\operatorname{H}_{20a}$ & $([1],[1])$ & \texttt{5184.c} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{20b}$} & \multirow{2}*{$\operatorname{H}_{20b}$} & $([3],[1])$ & \texttt{162.d} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{1296.l} \\
\cline{3-6}
\hline
\end{tabular}}
\caption{2-adic Images of odd-degree $L_{2}$ Graphs}
\label{2-adic Images of L2 Graphs Table Odd}
\end{table}
\end{center}

\begin{itemize}
    \item Table \ref{2-adic Images of L2 Graphs Table Odd} contains the known $2$-adic images attached to isogeny-torsion graphs of $L_{2}(p)$ type where $p$ is an odd prime. 
    
    \begin{itemize}
        \item Isogeny-torsion graphs of $L_{2}(11)$ type
        
        Let $E/\QQ$ be a non-CM elliptic curve that contains a $\QQ$-rational subgroup of order $11$. Then $\textit{j}_{E} = -24729001$ or $\textit{j}_{E} = -121$. Consider the $\QQ$-isogeny class $\mathcal{E}$ with LMFDB label \texttt{121.a}. Then $\mathcal{E}$ contains two elliptic curves over $\QQ$, one with \textit{j}-invariant equal to $-24729001$ and another one with \textit{j}-invariant equal to $-121$. The image of the $2$-adic Galois representation attached to both of them is conjugate to the full lift of $\operatorname{H}_{3} = \texttt{4.2.0.1}$. Let $E/\QQ$ be an elliptic curve with a $\QQ$-rational subgroup of order $11$. Then $\overline{\rho}_{E,2^{\infty}}(G_{\QQ})$ is conjugate to the full lift of a quadratic twist of $\operatorname{H}_{3}$. The only possibilities are $\operatorname{H}_{3a}$ (see the $\QQ$-isogeny class with LMFDB label \texttt{7744.c}) and $\operatorname{H}_{3b}$ (see the $\QQ$-isogeny class with LMFDB label \texttt{121.c}).
        
        
        \end{itemize}
\end{itemize}

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.7}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    Isogeny Graph & $p$ & $E_{1}$ & $E_{2}$ & $E_{3}$ & Isogeny-Torsion Graph & Example Isogeny Class \\
    \hline
    \multirow{5}*{\includegraphics[scale=0.1]{L3 Graph.png}} & \multirow{2}*{$5$} & \multirow{2}*{$\operatorname{H}_{1}$} & \multirow{2}*{$\operatorname{H}_{1}$} & \multirow{2}*{$\operatorname{H}_{1}$} & $([5],[5],[1])$ & \texttt{11.a} \\
    \cline{6-7}
    & & & & & $([1],[1],[1])$ & \texttt{99.d} \\
    \cline{2-7}
    & \multirow{3}*{$3$} & \multirow{3}*{$\operatorname{H}_{1}$} & \multirow{3}*{$\operatorname{H}_{1}$} & \multirow{3}*{$\operatorname{H}_{1}$} & $([9],[3],[1])$ & \texttt{54.b} \\
    \cline{6-7}
    & & & & & $([3],[3],[1])$ & \texttt{19.a} \\
    \cline{6-7}
    & & & & & $([1],[1],[1])$ & \texttt{175.b} \\
    \hline
    
    
\end{tabular}}
\caption{2-adic Images of $L_{3}$ Graphs}
\label{2-adic Images of L3 Graphs Table}
\end{table}
\end{center}




KKKKKKKKKKKKKKKKKKK

\newpage


	
	\section{Isogeny-torsion graphs with complex multiplication}

Let $E/\QQ$ be an elliptic curve with CM. Then all elliptic curves over $\QQ$ that are $\QQ$-isogenous to $E$ have CM. Thus, it is natural to say that the isogeny-torsion graph associated to the $\QQ$-isogeny class of $E$ has CM. Here we classify the $2$-adic images of Galois attached to every vertex of an isogeny-torsion graph with CM. See Table \ref{tab-CMgraphs} for the classification of the isogeny-torsion graphs with CM. This same table appears as Table 5 in Section 4 of \cite{gcal-r}. Clearly, it is natural to classify the $2$-adic images of isogeny-torsion graphs with CM based on \textit{j}-invariant.

\begin{table}[h!]
 	\renewcommand{\arraystretch}{1.2}
 	\begin{tabular}{|c|c|c|c|c|c|}
 		\hline
 		$d_K$ & \multicolumn{2}{c|}{$j$} & Type & Torsion config. & LMFDB\\
 		\hline
 		\hline
 		\multirow{10}{*}{$-3$}  & \multirow{6}{*}{$0$} & $y^2=x^3+t^3, t=-3,1$  & $R_4(6)$ & $([6],[6],[2],[2])$ & \texttt{36.a4}\\
 		& &$y^2=x^3+t^3, t\neq -3,1$  & $R_4(6)$ & $([2],[2],[2],[2])$ & \texttt{144.a3}\\
 		& & $y^2=x^3+16t^3, t=-3,1$ & $L_4$ & $([3],[3],[3],[1])$ & \texttt{27.a3}\\
 		& & $y^2=x^3+16t^3, t\neq -3,1$  & $L_4$ & $([1],[1],[1],[1])$ & \texttt{432.e3}\\
 		& & $\!y^2=x^3+s^2,\,s^2\neq t^3,16t^3\!\!$  & $L_2(3)$ & $([3],[1])$ & \texttt{108.a2}\\
 		& & $\!y^2=x^3+s,\,s\neq t^3,16t^3\!\!$  & $L_2(3)$ & $([1],[1])$ & \texttt{225.c1}\\
 		\cline{2-6}
 		& \multirow{2}{*}{$2^4\cdot 3^3\cdot 5^3$} &  $y^2=x^3-15t^2x + 22t^3, t=1,3$ & $R_4(6)$ & $([6],[6],[2],[2])$ & \texttt{36.a1}\\
 		&  & $y^2=x^3-15t^2x + 22t^3, t\neq 1,3$ & $R_4(6)$ & $([2],[2],[2],[2])$ & \texttt{144.a1}\\
 		\cline{2-6}
 		& \multirow{2}{*}{$-2^{15}\cdot 3\cdot 5^3$} & $E^t, t=-3,1$ & $L_4$ & $([3],[3],[3],[1])$ & \texttt{27.a2}\\
 		& & $E^t, t\neq -3,1$ & $L_4$ & $([1],[1],[1],[1])$ & \texttt{432.e1}\\
 		\hline
 		\multirow{7}{*}{$-4$} & \multirow{4}{*}{$2^6\cdot 3^3$} & $y^2=x^3+tx, t=-1,4$  & $T_4$ & $([2,2],[4],[4],[2])$ & \texttt{32.a3}\\
 		& & $y^2=x^3+tx, t=-4,1$  & $T_4$ & $([2,2],[4],[2],[2])$ & \texttt{64.a3}\\
 		& & $y^2=x^3\pm t^2x, t\neq 1,2$  & $T_4$ & $([2,2],[2],[2],[2])$ & \texttt{288.d3}\\
 		& &  $y^2=x^3+sx$, $s\neq \pm t^2$  & $L_2(2)$ & $([2],[2])$ & \texttt{256.b1}\\
 		\cline{2-6}
 		& \multirow{3}{*}{$2^3\cdot 3^3\cdot 11^3$} & $y^2=x^3-11t^2x+14t^3, t=\pm 1$ & \multirow{3}{*}{$T_4$} & $([2,2],[4],[4],[2])$ & \texttt{32.a2}\\
 		& & $y^2=x^3-11t^2x+14t^3, t=\pm 2$ &  & $([2,2],[4],[2],[2])$ & \texttt{64.a1}\\
 		& & $y^2=x^3-11t^2x+14t^3, t\neq \pm 1, \pm 2$ &  & $([2,2],[2],[2],[2])$ & \texttt{288.d1}\\
 		\hline
 		\multirow{2}{*}{$-7$} & \multicolumn{2}{c|}{$-3^3\cdot 5^3$}  & \multirow{2}*{$R_4(14)$} & $([2],[2],[2],[2])$ & \texttt{49.a2}\\
 		& \multicolumn{2}{c|}{$3^3\cdot 5^3\cdot 17^3$} & & $([2],[2],[2],[2])$  & \texttt{49.a1}\\
 		\hline
 		$-8$ & \multicolumn{2}{c|}{$2^6\cdot 5^3$}  & $L_2(2)$ & $([2],[2])$ & \texttt{256.a1}\\
 		\hline
 		$-11$ & \multicolumn{2}{c|}{$-2^{15}$} & $L_2(11)$ & $([1],[1])$ & \texttt{121.b1}\\
 		\hline
 		$-19$ & \multicolumn{2}{c|}{$-2^{15}\cdot 3^3$} & $L_2(19)$ & $([1],[1])$ & \texttt{361.a1} \\
 		\hline
 		$-43$ & \multicolumn{2}{c|}{$-2^{18}\cdot 3^3\cdot 5^3$}  & $L_2(43)$ & $([1],[1])$ & \texttt{1849.b1}\\
 		\hline
 		$-67$ & \multicolumn{2}{c|}{$-2^{15}\cdot 3^3\cdot 5^3\cdot 11^3$}  & $L_2(67)$ & $([1],[1])$ & \texttt{4489.b1} \\
 		\hline
 		$-163$ & \multicolumn{2}{c|}{$-2^{18}\cdot 3^3\cdot 5^3\cdot 23^3\cdot 29^3$} & $L_2(163)$ & $([1],[1])$ & \texttt{26569.a1} \\
 		\hline
 	\end{tabular}
 	\caption{The list of rational $j$-invariants with CM and the possible isogeny-torsion graphs that occur, where $E^t$ denotes the curve $y^2=x^3-38880t^2x+2950992t^3$.}
 	\label{tab-CMgraphs}
 \end{table}
 
\begin{lemma}\label{lemma odd graphs}
Let $E/\QQ$ be an elliptic curve with complex multiplication. Suppose that $E$ does not have a point of order $2$ defined over $\QQ$. Then $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ contains $\operatorname{-Id}$.
\end{lemma}
 
\begin{proof}
By Table \ref{tab-CMgraphs}, $\textit{j}_{E} \neq 1728$. Let us first say that $\textit{j}_{E} = 0$. Then by Theorem 1.8 in \cite{al-rCMGRs}, $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ contains $\operatorname{-Id}$. Next, let us say that $\textit{j}_{E} = -12288000$. Then $E$ has contains a cyclic, $\QQ$-rational subgroup of order $27$ and the isogeny graph associated to $E$ is of $L_{4}$. Moreover, $E$ is $3$-isogenous to an elliptic curve with $\textit{j}$-invariant equal to $0$. By Lemma \ref{2-adic determination}, $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ contains $\operatorname{-Id}$. By Table \ref{tab-CMgraphs}, it remains to prove the lemma for when
$$\textit{j}_{E} \in \left\{-32768, -884736, -884736000, -147197952000, -262537412640768000 \right\}$$
corresponding to elliptic curves containing a $\QQ$-rational subgroup of order $11$, $19$, $43$, $67$, and $163$. Each such elliptic curve has CM by a quadratic imaginary field of discriminant $\Delta_{K} \equiv 1 \mod 4$. We take an example of each such elliptic curve over $\QQ$ with \textit{j}-invariant equal to one of the five above, namely, \texttt{121.b1}, \texttt{361.a1}, \texttt{1849.b1}, \texttt{4489.b1}, \texttt{26569.a1}. Running code provided by Lozano-Robledo, we see that the conductor of each of the elliptic curves is equal to $1$. Hence, $\delta = \frac{\Delta_{K}-1}{4}$ is an odd integer. By Theorem 9.3 in \cite{al-rCMGRs}, $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to $\mathcal{N}_{\delta,1}(2^{\infty}) = \left\langle C_{\delta,1}(2^{\infty}), \begin{bmatrix} -1 & 0 \\ 1 & 1 \end{bmatrix} \right\rangle$ where

\begin{center}$C_{\delta,1}(2^{\infty}) = \left\{ \begin{bmatrix} a+b & b \\ \delta b & a \end{bmatrix} \colon a,b \in \ZZ_{2} | \texttt{a and b not both even} \right\}.$\end{center}

Note that setting $a = -1$ and $b = 0$ shows that $\operatorname{-Id} \in \overline{\rho}_{E,2^{\infty}}(G_{\Q})$ for each of the five elliptic curves. Let $d$ be a non-zero, squarefree integer and let $E^{(d)}$ be the quadratic twist of $E$ by $d$. If $\operatorname{-Id}$ is contained in every index-$2$ subgroup of $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$, then $\overline{\rho}_{E^{(d)},2^{\infty}}(G_{\Q})$ contains $\operatorname{-Id}$. To see why this is true, note that $\overline{\rho}_{E^{(d)},2^{\infty}}(G_{\Q})$ is the same as $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$, up to multiplication of some elements of $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ by $\operatorname{-Id}$. Thus, $\overline{\rho}_{E^{(d)},2^{\infty}}(G_{\Q})$ is a subgroup of $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ of index $1$ or $2$ depending on whether or not $\overline{\rho}_{E^{(d)},2^{\infty}}(G_{\Q})$ contains $\operatorname{-Id}$. If on the other hand, all subgroups of $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ of index $2$ contain $\operatorname{-Id}$, then $\operatorname{-Id}$ is contained in $\overline{\rho}_{E^{(d)},2^{\infty}}(G_{\Q})$.

Let $H$ be a subgroup of $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ of index $2$. Then $H$ is normal and hence, the squares of all elements of $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ are contained in $H$. Note that
$$\left(\begin{bmatrix} -1 & 0 \\ 1 & 1 \end{bmatrix} \cdot \begin{bmatrix} a+1 & 1 \\ \delta & a \end{bmatrix}\right)^{2} = \begin{bmatrix} a^{2}+a-\delta & 0 \\ 0 & a^{2}+a - \delta \end{bmatrix}.$$
Let $p(x) = x^{2} + x -  \delta + 1$. Then $p(0) = 0$ in $\ZZ / 2 \ZZ$ because $\delta$ is odd and $p'(0) = 1 \neq 0 \mod 2$. By Hensel's lemma, there is a unique solution $\alpha \in \ZZ_{2}$ to the equality $x^{2} + x - \delta = -1$. Hence, $\begin{bmatrix} -1 & 0 \\ 0 & -1 \end{bmatrix} = \begin{bmatrix} \alpha^{2} + \alpha - \delta & 0 \\ 0 & \alpha^{2} + \alpha - \delta \end{bmatrix}$ is a square in $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$. Thus, $H$ contains $\operatorname{-Id}$ and so, $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ contains $\operatorname{-Id}$.
\end{proof}

\begin{corollary}
Let $E/\QQ$ be an elliptic curve with complex multiplication. Suppose that $E$ does not have a point of order $2$ defined over $\QQ$. Then $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to $\mathcal{N}_{\delta,1}(G_{\Q})$ or $\mathcal{N}_{\delta,3}(G_{\Q})$.
\end{corollary}

\begin{proof}
In this case, $\textit{j}_{E} \neq 1728$. If $\textit{j}_{E} = 0$, then the corollary is proven simply by observing Theorem 1.8 in \cite{al-rCMGRs}. So we may assume that $\textit{j}_{E} \neq 0, 1728$. By Lemma \ref{lemma odd graphs}, $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ contains $\operatorname{-Id}$. In other words, $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is not affected by quadratic twisting. Thus, if $E$ does not contain a cyclic, $\QQ$-rational subgroup of order $27$, then $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to $\mathcal{N}_{\delta, 1}(2^{\infty})$. On the other hand, suppose that $E$ does contain a cyclic, $\QQ$-rational subgroup of order $27$. Then $\textit{j}_{E} = -12288000$ and $E$ has CM by an order with $\Delta_{K} = -3$ and $f = 3$. Again, $\Delta_{K}f^{2}$ is not divisible by $8$ and by Theorem 9.3 in \cite{al-rCMGRs}, $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to $\mathcal{N}_{\delta,3}(G_{\Q})$.
\end{proof}

\subsection{$R_{4}(14)$ graphs}

Let $E/\QQ$ be the elliptic curve with LMFDB notation \texttt{49.a1}. Then $\textit{j}_{E} = 16581375$. Running code provided by Lozano-Robledo, we see that $E$ has complex multiplication by an order of $K = \QQ(\sqrt{-7})$ with discriminant $\Delta_{K} = -7$ and conductor $f = 2$. Then $\delta = \frac{-7 \cdot 2^{2}}{4} = -7$. Theorem 9.3 in \cite{al-rCMGRs} says that, by the fact that $\Delta_{K} f^{2} = -7 \cdot 2^{2}$ is not divisible by $8$, $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to $\mathcal{N}_{-7,0}(2^{\infty}) = \left\langle C_{-7,0}(2^{\infty}), \begin{bmatrix} -1 & 0 \\ 0 & 1 \end{bmatrix} \right\rangle$ where
$$C_{-7,0}(2^{\infty}) = \left\langle \begin{bmatrix} a & b \\ -7b & a \end{bmatrix} \colon 2 \nmid a^{2}+b^{2} \right\rangle.$$
We will prove that $\operatorname{-Id}$ is contained in all subgroups of $\mathcal{N}_{-7,0}(2^{\infty})$ of index $2$. Note that
$$\left(\begin{bmatrix} -1 & 0 \\ 0 & 1 \end{bmatrix} \cdot \begin{bmatrix} 0 & b \\ -7b & 0 \end{bmatrix}\right)^{2} = \begin{bmatrix} 7b^{2} & 0 \\ 0 & 7b^{2} \end{bmatrix}.$$

\begin{lemma}[Generalized Hensel's Lemma]\label{Hensel}
Let $p$ be a prime and let $f(x)$ be a polynomial with integer coefficients. Suppose that $f(a) \equiv 0 (\mod p^{j})$, $p^{\tau} \mid \mid f'(a)$, and that $j \geq 2\tau + 1$. Then there is a unique $t$ (modulo $p$) such that $f(a+tp^{j-\tau}) \equiv 0 (\mod p^{j+1})$

\end{lemma}

Consider the polynomial $f(x) = 7x^{2}+1$. Then $f(1) = 8 \equiv 0 \mod 8$. Next we have $f'(x) = 14x$. Letting $\tau = 1$ and $j = 3$, we have that $j \geq 2\tau + 1$. So there is a unique $t$ modulo $2$ such that $f(1+t \cdot 2^{2}) \equiv 0 \mod 2^{4}$. Moreover, $1 + t \cdot 2^{2}$ is odd and so, $f'(1+t \cdot 2^{2})$ is odd. We can use Lemma \ref{Hensel} again to find a lift of $1$ to level $5$ which is a root of $f(x)$. Continuing this process inductively, we find lifts of $1$ to all levels and a root of $f(x)$ to all levels. Hence, there is a solution to $7x^{2} = -1$ at all level $\ZZ / 2^{N} \ZZ$. Hence, $\operatorname{-Id}$ is an element of all subgroups of $\mathcal{N}_{-7,0}(2^{\infty}$ of index $2$. Thus, quadratic twisting does not affect $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$. Thus, if $\textit{j}_{E} = -3375$, then $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to $\mathcal{N}_{-7,0}(2^{\infty})$.

Let $E'/\QQ$ be an elliptic curve with $\textit{j}_{E} = -3375$. Then $E'$ is $2$-isogenous to an elliptic curve with \textit{j}-invariant equal to $16581375$. By Corollary \ref{contains -Id}, $\overline{\rho}_{E',2^{\infty}}(G_{\Q})$ contains $\operatorname{-Id}$ and hence, $\overline{\rho}_{E',2^{\infty}}(G_{\Q})$ is not affected by quadratic twisting. Using code provided by Lozano-Robledo, we see that $E'$ has complex multiplication by an order of $K = \QQ(\sqrt{-7})$ with discriminant $\Delta_{K} = -7$ and conductor $f = 1$. Again, by the fact that $\Delta_{K} \cdot f^{2}$ is not divisible by $8$, Theorem 9.3 in \cite{al-rCMGRs} says that $\overline{\rho}_{E',2^{\infty}}(G_{\Q})$ is conjugate to $\mathcal{N}_{-7,1}(2^{\infty})$.

\subsection{$\textit{j} = 8000$}

Let $E/\QQ$ be the elliptic curve with LMFDB label \texttt{256.a1}. Then $\textit{j}_{E} = 8000$. There are two elliptic curves in the $\QQ$-isogeny class of $E$; $E$ is $2$-isogenous to an elliptic curve $E'$, also with $\textit{j}_{E'} = 8000$. Using code provided by Lozano-Robledo, we see that $E$ has complex multiplication by an order of $K = \QQ(\sqrt{-2})$ with $\Delta_{K} = -8$ and conductor $f = 1$. We compute that $\delta = \frac{-8 \cdot 1^{2}}{4} = -2$. By part 2 of Theorem 1, $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is a group of level $8$. Moreover, there is an $\epsilon \in \{\pm 1\}$ and an $\alpha \in \{3, 5\}$ such that $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to one of the following eight subgroups of $\operatorname{GL}(2, \ZZ_{2})$
$$\left\langle \begin{bmatrix} \epsilon & 0 \\ 0 & -\epsilon \end{bmatrix}, \begin{bmatrix} \alpha & 0 \\ 0 & \alpha \end{bmatrix}, \begin{bmatrix} 1 & 1 \\ -2 & 1 \end{bmatrix} \right\rangle, \left\langle \begin{bmatrix} \epsilon & 0 \\ 0 & -\epsilon \end{bmatrix}, \begin{bmatrix} \alpha & 0 \\ 0 & \alpha \end{bmatrix}, \begin{bmatrix} -1 & -1 \\ 2 & -1 \end{bmatrix} \right\rangle.$$
A quick computation reveals that all four groups with $\alpha = 5$ are conjugate over $\operatorname{GL}(2, \ZZ / 8 \ZZ)$ and contain $\operatorname{-Id}$. If $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to $H_{1} = \left\langle \begin{bmatrix} \epsilon & 0 \\ 0 & -\epsilon \end{bmatrix}, \begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix}, \begin{bmatrix} 1 & 1 \\ -2 & 1 \end{bmatrix} \right\rangle$ then by Corollary \ref{contains -Id}, $\overline{\rho}_{E',2^{\infty}}(G_{\Q})$ also contains $\operatorname{-Id}$ and hence, $\overline{\rho}_{E',2^{\infty}}(G_{\Q})$ is also conjugate to $H_{1}$.

Another quick computation reveals that $H_{2} = \left\langle \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & -1 \end{bmatrix}, \begin{bmatrix} 1 & 1 \\ -2 & 1 \end{bmatrix} \right\rangle$ is conjugate to the group $\left\langle \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & -1 \end{bmatrix}, \begin{bmatrix} -1 & -1 \\ 2 & -1 \end{bmatrix} \right\rangle$ over $\operatorname{GL}(2, \ZZ / \ZZ)$ and $H_{3} = \left\langle \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} -1 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 1 \\ -2 & 1 \end{bmatrix} \right\rangle$ is conjugate to the group $\left\langle \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} -1 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} -1 & -1 \\ 2 & -1 \end{bmatrix} \right\rangle$ over $\operatorname{GL}(2, \ZZ / 8 \ZZ)$ but $H_{2}$ is not conjugate to $H_{3}$ over $\operatorname{GL}(2, \ZZ / 8 \ZZ)$. The groups $H_{2}$ and $H_{3}$ are index-$2$ subgroups of $H_{1}$ that do not contain $\operatorname{-Id}$. In other words, $H_{1}$, $H_{2}$, and $H_{3}$ are quadratic twists. Suppose that $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to $H_{2}$. To make use of Lemma \ref{2-adic determination}, we note that $H_{2}$ is conjugate to $\left\langle \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} -1 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & -2 \\ 1 & 1 \end{bmatrix} \right\rangle$. By Lemma \ref{2-adic determination}, $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to $\left\langle \begin{bmatrix} 3 & 0 \\ 0 & 3 \end{bmatrix}, \begin{bmatrix} -1 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & -1 \\ 2 & 1 \end{bmatrix} \right\rangle$ which is in turn conjugate to $H_{3}$.

\subsection{$R_{4}(6)$ graphs}

Let $E/\QQ$ be an elliptic curve with CM with a $\QQ$-rational subgroup of order $6$. Then $\textit{j}_{E} = 0$ or $54000$. All elliptic curves over $\QQ$ in the $\QQ$-isogeny class of $E$ have CM by an order of $K = \QQ(\sqrt{-3})$ with discriminant $\Delta_{K} = -3$. The isogeny graph associated to $E$ with the $\textit{j}$-invariant of the respective curves is below
\begin{center} \begin{tikzcd}
{E_{1}, \textit{j}_{E_{1}} = 0} \arrow[d, no head, "2"'] \arrow[rr, no head, "3"] &  & {E_{2}, \textit{j}_{E_{2}} = 0} \arrow[d, no head, "2"] \\
{E_{3}, \textit{j}_{E_{3}} = 54000} \arrow[rr, no head, "3"']            &  & {E_{4}, \textit{j}_{E_{4}} = 54000}           
\end{tikzcd} \end{center}
Suppose that $\textit{j}_{E} = 0$. Then by Theorem 1.8 in \cite{al-rCMGRs}, the image of the $2$-adic Galois representation attached to $E$ is conjugate to
$$\left\langle \begin{bmatrix} a+b & b \\ -b & a \end{bmatrix}, \begin{bmatrix} 0 & 1 \\ 1 & 0 \end{bmatrix} : \texttt{a is odd and b is even} \right\rangle.$$
Suppose on the other hand that $\textit{j}_{E} = 54000$. Running code provided by Lozano-Robledo, we see that $E$ has CM by an order with conductor equal to $f = 2$. Thus, $\Delta_{K} \cdot f^{2} = -12$ is not divisible by $8$. By Theorem 9.3 in \cite{al-rCMGRs}, $\rho_{E,2^{\infty}}(G_{\Q})$ is conjugate to $$\mathcal{N}_{-3,0}(2^{\infty}) = \left\langle \begin{bmatrix} a & b \\ -3b & a \end{bmatrix}, \begin{bmatrix} -1 & 0 \\ 0 & 1 \end{bmatrix} : \texttt{a+b is odd} \right\rangle.$$

\subsection{\textit{j} = 1728}

Let $E/\QQ$ be an elliptic curve with $\textit{j}_{E} = 1728$. Then $E$ has CM by a an order of $K = \QQ(i)$ with discriminant $\Delta_{K} = -4$ and conductor $f = 1$. Then $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to a subgroup of $G_{1} = \left\langle \begin{bmatrix} a & b \\ -b & a \end{bmatrix}, \begin{bmatrix} -1 & 0 \\ 0 & 1 \end{bmatrix} : a^{2}+b^{2} \not \equiv 0 \mod 2 \right\rangle$. Let

\begin{itemize}
    \item $G_{2,a} = \left\langle \operatorname{-Id}, 3 \cdot \operatorname{Id}, \begin{bmatrix} 1 & 2 \\ -2 & 1 \end{bmatrix} \right\rangle$
    \item $G_{2,b} = \left\langle \operatorname{-Id}, 3 \cdot \operatorname{Id}, \begin{bmatrix} 2 & 1 \\ -1 & 2 \end{bmatrix} \right\rangle$
    \item $G_{4,a} = \left\langle 5 \cdot \operatorname{Id}, \begin{bmatrix} 1 & 2 \\ -2 & 1 \end{bmatrix} \right\rangle$
    \item $G_{4,b} = \left\langle 5 \cdot \operatorname{Id}, \begin{bmatrix} -1 & -2 \\ 2 & -1 \end{bmatrix} \right\rangle$
    \item $G_{4,c} = \left\langle 3 \cdot \operatorname{Id}, \begin{bmatrix} 2 & -1 \\ 1 & 2 \end{bmatrix} \right\rangle$
    \item $G_{4,d} = \left\langle 3 \cdot \operatorname{Id}, \begin{bmatrix} -2 & 1 \\ -1 & -2 \end{bmatrix} \right\rangle$
\end{itemize}
and let $\Gamma = \left\{c_{1} = \begin{bmatrix} 1 & 0 \\ 0 & -1 \end{bmatrix}, c_{-1} = \begin{bmatrix} -1 & 0 \\ 0 & 1 \end{bmatrix}, c_{1}' = \begin{bmatrix} 0 & 1 \\ 1 & 0 \end{bmatrix}, c_{-1}' = \begin{bmatrix} 0 & -1 \\ -1 & 0 \end{bmatrix} \right\}$. Then by Theorem 1.7 in \cite{al-rCMGRs}, $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is generated by one of $G_{1}$, $G_{2,a}$, $G_{2b}$, $G_{4,a}$, $G_{4,b}$, $G_{4,c}$, $G_{4,d}$, and one element of $\Gamma$. The group $G_{1}$ is all of $\mathcal{N}_{-1,0}(2^{\infty})$. It is easy to see that $\left\langle G_{2,a}, c_{1} \right\rangle = \left\langle G_{2,a}, c_{-1} \right\rangle$ and $\left\langle G_{2,b}, c_{1} \right\rangle = \left\langle G_{2,b}, c_{-1} \right\rangle$. Note that $\left\langle G_{4,a}, c_{1} \right\rangle = \left\langle 5 \cdot \operatorname{Id}, \begin{bmatrix} 1 & 2 \\ -2 & 1 \end{bmatrix}, c_{1} \right\rangle = \left\langle 5 \cdot \operatorname{Id}, c_{1} \cdot \begin{bmatrix} 1 & 2 \\ -2 & 1 \end{bmatrix} \cdot c_{1}^{-1}, c_{1} \right\rangle = \left\langle 5 \cdot \operatorname{Id}, \begin{bmatrix} 1 & -2 \\ 2 & 1 \end{bmatrix}, c_{1} \right\rangle$. After switching the orders of the generators of $\operatorname{GL}(2, \ZZ_{2})$, we see that this last group is conjugate to the group $\left\langle 5 \cdot \operatorname{Id}, \begin{bmatrix} 1 & 2 \\ -2 & 1  \end{bmatrix}, c_{-1} \right\rangle = \left\langle G_{4,a}, c_{-1} \right\rangle$. Note that $\left\langle G_{4,a}, c_{1}' \right\rangle = \left\langle 5 \cdot \operatorname{Id}, \begin{bmatrix} 1 & 2 \\ -2 & 1
\end{bmatrix}, \begin{bmatrix} 0 & 1 \\ 1 & 0 \end{bmatrix} \right\rangle$ is conjugate to the group $\left\langle 5 \cdot \operatorname{Id}, c_{1} \cdot \begin{bmatrix} 1 & 2 \\ -2 & 1 \end{bmatrix} \cdot c_{1}^{-1}, c_{1} \cdot \begin{bmatrix} 0 & 1 \\ 1 & 0 \end{bmatrix} \cdot c_{1}^{-1} \right\rangle = \left\langle 5 \cdot \operatorname{Id}, \begin{bmatrix} 1 & -2 \\ 2 & 1 \end{bmatrix}, \begin{bmatrix} 0 & -1 \\ -1 & 0 \end{bmatrix} \right\rangle$. After switching the order of the generators, this last group is conjugate to $\left\langle 5 \cdot \operatorname{Id}, \begin{bmatrix} 1 & 2 \\ -2 & 1 \end{bmatrix}, \begin{bmatrix} 0 & -1 \\ -1 & 0 \end{bmatrix} \right\rangle = \left\langle G_{4,a}, c_{-1}' \right\rangle$. Making similar computations, we see that $\left\langle G_{4,x}, c_{1} \right\rangle$ is conjugate to $\left\langle G_{4,x}, c_{-1} \right\rangle$ and $\left\langle G_{4,x}, c_{1}' \right\rangle$ is conjugate to $\left\langle G_{4,x}, c_{-1}' \right\rangle$ for $x = b$, $c$, and $d$. Hence, we work with the case that $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to $G_{1}$, $\left\langle G_{2,a}, c_{1} \right\rangle$, $\left\langle G_{2,a}, c_{1}' \right\rangle$, $\left\langle G_{2,b}, c_{1} \right\rangle$, $\left\langle G_{2,b}, c_{1}' \right\rangle$, $\left\langle G_{4,a}, c_{1} \right\rangle$, $\left\langle G_{4,a}, c_{1}' \right\rangle$, $\left\langle G_{4,b}, c_{1} \right\rangle$, $\left\langle G_{4,b}, c_{1}' \right\rangle$, $\left\langle G_{4,c}, c_{1} \right\rangle$, $\left\langle G_{4,c}, c_{1}' \right\rangle$, $\left\langle G_{4,d}, c_{1} \right\rangle$, or $\left\langle G_{4,d}, c_{1}' \right\rangle$.

If $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to one of $\left\langle \operatorname{-Id}, 3 \cdot \operatorname{Id}, \begin{bmatrix} 1 & 2 \\ -2 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & -1 \end{bmatrix} \right\rangle$, $\left\langle 5 \cdot \operatorname{Id}, \begin{bmatrix} 1 & 2 \\ -2 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & -1 \end{bmatrix} \right\rangle$, or $\left\langle 5 \cdot \operatorname{Id}, \begin{bmatrix} -1 & -2 \\ 2 & -1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 0 & -1 \end{bmatrix} \right\rangle$, then $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ reduces modulo $2$ to the trivial group and hence, $E$ has full two-torsion defined over $\QQ$. Next, if $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to one of $\left\langle \operatorname{-Id}, 3 \cdot \operatorname{Id}, \begin{bmatrix} 1 & 2 \\ -2 & 1 \end{bmatrix}, \begin{bmatrix} 0 & 1 \\ 1 & 0 \end{bmatrix} \right\rangle$, $\left\langle 5 \cdot \operatorname{Id}, \begin{bmatrix} 1 & 2 \\ -2 & 1 \end{bmatrix}, \begin{bmatrix} 0 & 1 \\ 1 & 0 \end{bmatrix} \right\rangle$, or $\left\langle 5 \cdot \operatorname{Id}, \begin{bmatrix} -1 & -2 \\ 2 & -1 \end{bmatrix}, \begin{bmatrix} 0 & 1 \\ 1 & 0 \end{bmatrix} \right\rangle$, then using magma, we see that $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to a subgroup of $\left\langle \begin{bmatrix} \ast & \ast \\ 0 & \ast \end{bmatrix} \right\rangle \subseteq \operatorname{GL}(2, \ZZ / 4 \ZZ)$. Thus, $E$ has a cyclic, $\QQ$-rational subgroup of order $4$. On the other hand, if $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to any one of the remaining seven groups, then $E(\QQ)_{\texttt{tors}} \cong \ZZ / 2 \ZZ$ and $E$ does not have a cyclic, $\QQ$-rational subgroup of order $4$.

We start with classifying the $2$-adic images of the elliptic curves that are $\QQ$-isogenous to elliptic curves defined over $\QQ$ with full two-torsion defined over $\QQ$ and \textit{j}-invariant equal to $1728$. 

\begin{itemize}
    \item $\overline{\rho}_{E,2^{\infty}}(G_{\Q}) \cong \left\langle \operatorname{-Id}, 3 \cdot \operatorname{Id}, \begin{bmatrix} 1 & 0 \\ 0 & -1 \end{bmatrix}, \begin{bmatrix} 1 & 2 \\ -2 & 1 \end{bmatrix} \right\rangle$
    
    By Lemma \ref{2-adic determination}, $\overline{\rho}_{E / \left\langle Q_{2} \right\rangle, 2^{\infty}}(G_{\Q})$ is conjugate to $H_{Q_{2}} = \left\langle \operatorname{-Id}, 3 \cdot \operatorname{Id}, \begin{bmatrix} 1 & 0 \\ 0 & -1 \end{bmatrix}, \begin{bmatrix} 1 & 1 \\ -4 & 1 \end{bmatrix} \right\rangle$. Switching the order of $P$ and $Q$, we see that $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to $\left\langle \operatorname{-Id}, 3 \cdot \operatorname{Id}, \begin{bmatrix} -1 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & -2 \\ 2 & 1 \end{bmatrix} \right\rangle$ and hence, by Lemma \ref{2-adic determination}, $\overline{\rho}_{E / \left\langle P_{2} \right\rangle, 2^{\infty}}(G_{\Q})$ is conjugate to $H_{P_{2}} = \left\langle \operatorname{-Id}, 3 \cdot \operatorname{Id}, \begin{bmatrix} -1 & 0 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & -1 \\ 4 & 1 \end{bmatrix} \right\rangle$. The conjugation of all generators of $H_{P_{2}}$ by $\begin{bmatrix} 1 & 0 \\ 0 & -1 \end{bmatrix}$ generate we see that $H_{Q_{2}}$. Hence, $H_{P_{2}}$ is conjugate (actually, equal) to $H_{Q_{2}}$. Finally, rewriting $E[2^{\infty}] = \left\langle P_{2^{\infty}}, P_{2^{\infty}}+Q_{2^{\infty}} \right\rangle$, we see that $\overline{\rho}_{E,2^{\infty}}(G_{\Q})$ is conjugate to $\left\langle \operatorname{-Id}, 3 \cdot \operatorname{Id}, \begin{bmatrix} 1 & 2 \\ 0 & -1 \end{bmatrix}, \begin{bmatrix} 3 & 4 \\ -2 & -1 \end{bmatrix} \right\rangle$. Thus, $\overline{\rho}_{E / \left\langle P_{2}+Q_{2} \right\rangle, 2^{\infty}}(G_{\Q})$ is conjugate to $H_{P_{2}+Q_{2}} = \left\langle \operatorname{-Id}, 3 \cdot \operatorname{Id}, \begin{bmatrix} 1 & 1 \\ 0 & -1 \end{bmatrix}, \begin{bmatrix} 3 & 2 \\ -4 & -1 \end{bmatrix}\right\rangle$. Note that $H_{P_{2}+Q_{2}}$ is not conjugate to $H_{P_{2}}$ and $E/\left\langle P_{2} \right\rangle(\QQ)_{\text{tors}} \cong E/\left\langle Q_{2} \right\rangle(\QQ)_{\text{tors}} \cong E/\left\langle P_{2}+Q_{2} \right\rangle(\QQ)_{\text{tors}} \cong \ZZ / 2 \ZZ$ and all three elliptic curves $E / \left\langle P_{2} \right\rangle$, $E / \left\langle Q_{2} \right\rangle$, and $E / \left\langle P_{2}+Q_{2} \right\rangle$ have $\QQ$-rational, cyclic subgroups of order $4$.
\end{itemize}
\newpage

\section{Odd-degree graphs}. 

Let $E/\QQ$ be an elliptic curve with complex multiplication. Suppose that $E$ does not have a point of order $2$ defined over $\QQ$. By Corollary \ref{odd-degree graphs}, the image of the $2$-adic Galois representation attached to all elliptic curves over $\QQ$ in the $\QQ$-isogeny class of $E$ are the same, up to conjugation. Thus, classifying the $2$-adic images of the isogeny-torsion graphs that do not have a point of order $2$ defined over $\QQ$ will be a rather quick task.

\subsection{$L_{4}$ Graphs}

Let $E/\QQ$ be an elliptic curve such that the isogeny-torsion graph associated to $E$ is of $L_{4}$ type. We may assume that $E$ has split Cartan modulo $3$. Then  $\textit{j}_{E} = 0$. By Theorem 1.8 in \cite{al-rCMGRs}, the image of the $2$-adic Galois representation attached to $E$ is conjugate to $H = \left\langle \operatorname{-Id}, \begin{bmatrix} 0 & 1 \\ 1 & 0 \end{bmatrix}, \begin{bmatrix} 7 & 4 \\ -4 & 3 \end{bmatrix}, \begin{bmatrix} 2 & 1 \\ -1 & 1 \end{bmatrix} \right\rangle$. By Lemma \ref{2-adic determination}, the image of all elliptic curves in the $\QQ$-isogeny class of $E$ is conjugate to $H$.

\subsection{$L_{2}(p)$ graphs with CM}

\begin{itemize}
    \item $L_{2}(163)$ graph
    
    Let $E/\QQ$ be an elliptic curve with a $\QQ$-rational subgroup of order $163$. Then the \textit{j}-invariant of $E$ is equal to $-262537412640768000$ and $E$ has CM by an order of discriminant $\Delta_{K} = -163$ and conductor $f = 1$. Moreover, there are two elliptic curves over $\QQ$ in the $\QQ$-isogeny class of $E$. Using code by Lozano-Robledo, we see that the image of the $2$-adic Galois representation attached to $E$ is of level $2$, conjugate to $\operatorname{GL}(2, \ZZ / 2 \ZZ)$. By Theorem 1.1 of \cite{al-rCMGRs}, the image of the $2$-adic Galois representation attached to $E$ (and of the other elliptic curve over $\QQ$ in the $\QQ$-isogeny class of $E$) is conjugate to
    $$\left\langle \begin{bmatrix} a+b & b \\ -41b & a \end{bmatrix}, \begin{bmatrix} -1 & 0 \\ 1 & 1 \end{bmatrix} : \texttt{a and b not both even} \right\rangle.$$
    
    \item $L_{2}(67)$ graph
    
    Let $E/\QQ$ be an elliptic curve with a $\QQ$-rational subgroup of order $67$. Then the \textit{j}-invariant of $E$ is equal to $-147197952000$ and $E$ has CM by an order of discriminant $\Delta_{K} = -67$ and conductor $f = 1$. Moreover, there are two elliptic curves over $\QQ$ in the $\QQ$-isogeny class of $E$. Using code by Lozano-Robledo, we see that the image of the $2$-adic Galois representation attached to $E$ is of level $2$, conjugate to $\operatorname{GL}(2, \ZZ / 2 \ZZ)$. By Theorem 1.1 of \cite{al-rCMGRs}, the image of the $2$-adic Galois representation attached to $E$ (and of the other elliptic curve over $\QQ$ in the $\QQ$-isogeny class of $E$) is conjugate to
    $$\left\langle \begin{bmatrix} a+b & b \\ -17b & a \end{bmatrix}, \begin{bmatrix} -1 & 0 \\ 1 & 1 \end{bmatrix} : \texttt{a and b not both even} \right\rangle.$$
    
    \item $L_{2}(43)$ graph
    
    Let $E/\QQ$ be an elliptic curve with a $\QQ$-rational subgroup of order $43$. Then the \textit{j}-invariant of $E$ is equal to $-884736000$ and $E$ has CM by an order of discriminant $\Delta_{K} = -43$ and conductor $f = 1$. Moreover, there are two elliptic curves over $\QQ$ in the $\QQ$-isogeny class of $E$. Using code by Lozano-Robledo, we see that the image of the $2$-adic Galois representation attached to $E$ is of level $2$, conjugate to $\operatorname{GL}(2, \ZZ / 2 \ZZ)$. By Theorem 1.1 of \cite{al-rCMGRs}, the image of the $2$-adic Galois representation attached to $E$ (and of the other elliptic curve over $\QQ$ in the $\QQ$-isogeny class of $E$) is conjugate to
    $$\left\langle \begin{bmatrix} a+b & b \\ -11b & a \end{bmatrix}, \begin{bmatrix} -1 & 0 \\ 1 & 1 \end{bmatrix} : \texttt{a and b not both even} \right\rangle.$$
    
    \item $L_{2}(19)$ graph
    
    Let $E/\QQ$ be an elliptic curve with a $\QQ$-rational subgroup of order $19$. Then the \textit{j}-invariant of $E$ is equal to $-884736$ and $E$ has CM by an order of discriminant $\Delta_{K} = -19$ and conductor $f = 1$. Moreover, there are two elliptic curves over $\QQ$ in the $\QQ$-isogeny class of $E$. Using code by Lozano-Robledo, we see that the image of the $2$-adic Galois representation attached to $E$ is of level $2$, conjugate to $\operatorname{GL}(2, \ZZ / 2 \ZZ)$. By Theorem 1.1 of \cite{al-rCMGRs}, the image of the $2$-adic Galois representation attached to $E$ (and of the other elliptic curve over $\QQ$ in the $\QQ$-isogeny class of $E$) is conjugate to
    $$\left\langle \begin{bmatrix} a+b & b \\ -5b & a \end{bmatrix}, \begin{bmatrix} -1 & 0 \\ 1 & 1 \end{bmatrix} : \texttt{a and b not both even} \right\rangle.$$
    
    \item $L_{2}(11)$ graph
    
    Let $E/\QQ$ be an elliptic curve with a $\QQ$-rational subgroup of order $11$. Then the \textit{j}-invariant of $E$ is equal to $-32768$ and $E$ has CM by an order of discriminant $\Delta_{K} = -11$ and conductor $f = 1$. Moreover, there are two elliptic curves over $\QQ$ in the $\QQ$-isogeny class of $E$. Using code by Lozano-Robledo, we see that the image of the $2$-adic Galois representation attached to $E$ is of level $2$, conjugate to $\operatorname{GL}(2, \ZZ / 2 \ZZ)$. By Theorem 1.1 of \cite{al-rCMGRs}, the image of the $2$-adic Galois representation attached to $E$ (and of the other elliptic curve over $\QQ$ in the $\QQ$-isogeny class of $E$) is conjugate to
    $$\left\langle \begin{bmatrix} a+b & b \\ -3b & a \end{bmatrix}, \begin{bmatrix} -1 & 0 \\ 1 & 1 \end{bmatrix} : \texttt{a and b not both even} \right\rangle.$$
    
    \item $L_{2}(3)$ graph
    
    Let $E/\QQ$ be an elliptic curve with CM such that the isogeny-torsion graph associated to $E$ is of $L_{2}(3)$ type. Then $\textit{j}_{E} = 0$. By Theorem 1.8 in \cite{al-rCMGRs} and Lemma \ref{2-adic determination}, the image of the $2$-adic Galois representation attached to both elliptic curves over $\QQ$ in the $\QQ$-isogeny class of $E$ is conjugate to $$\left\langle \operatorname{-Id}, \begin{bmatrix} 0 & 1 \\ 1 & 0 \end{bmatrix}, \begin{bmatrix} 7 & 4 \\ -4 & 3 \end{bmatrix}, \begin{bmatrix} 2 & 1 \\ -1 & 1 \end{bmatrix} \right\rangle.$$
    
    \end{itemize}
\subsection{$R_{4}(pq)$ graphs with CM}
    
    \begin{itemize}
        \item $R_{4}(14)$ Graphs
        
        Let $E/\QQ$ be an elliptic curve with a $\QQ$-rational subgroup of order $14$. Then $\textit{j}_{E} = -3375$ or $\textit{j}_{E} = 16581375$. All elliptic curves in the $\QQ$-isogeny class of $E$ have CM by an order of discriminant $-7$. The isogeny graph associated to $E$ with the \textit{j}-invariant of the respective curves is below.
\begin{center}
\begin{tikzcd}
{E_{1}, \textit{j}_{E_{1}} = -3375} \arrow[dd, no head, "2"'] \arrow[rr, no head, "7"] &  & {E_{2}, \textit{j}_{E_{2}} = -3375} \arrow[dd, no head, "2"] \\
                                                                     &  &                                                     \\
{E_{3}, \textit{j}_{E_{3}} = 16581375} \arrow[rr, no head, "7"']              &  & {E_{4}, \textit{j}_{E_{4}} = 16581375}             
\end{tikzcd}
\end{center}
Suppose that $\textit{j}_{E} = -3375$. Running code provided by Lozano-Robledo, we see that $E$ has CM by an order with conductor equal to $1$. Moreover, the code outputs that the level of definition of the $2$-adic image attached to $E$ is equal to $8$ and the reduction of the $2$-adic image modulo $8$ is a group of order $32$. By Theorem 1.1 in \cite{al-rCMGRs}, the image of the mod-$8$ Galois representation and hence, the image of the $2$-adic Galois representation attached to $E$ is conjugate to
$$\left\langle \begin{bmatrix} a+b & b \\ -2b & a \end{bmatrix}, \begin{bmatrix} -1 & 0 \\ 1 & 1 \end{bmatrix} : \texttt{a is odd and b is even} \right\rangle.$$
Now suppose that $\textit{j}_{E} = 16581375$. Running the same code, we see that $E$ has CM by an order with conductor equal to $2$. Moreover, the code outputs that the level of definition of the $2$-adic image attached to $E$ is equal to $8$ and the reduction of the $2$-adic image modulo $8$ is a group of order $64$. By Theorem 1.1 in \cite{al-rCMGRs}, the image of the mod-$8$ Galois representation and hence, the image of the $2$-adic Galois representation attached to $E$ is conjugate to
$$\left\langle \begin{bmatrix} a & b \\ -7b & a \end{bmatrix}, \begin{bmatrix} -1 & 0 \\ 0 & 1 \end{bmatrix} : \texttt{a+b is odd} \right\rangle.$$

\item $R_{4}(6)$ graphs


\end{itemize}

\subsection{$L_{2}(2)$ graph}

Let $E/\QQ$ be an elliptic curve with CM such that the isogeny graph associated to $E$ is of $L_{2}(2)$ type. Then each elliptic curve over $\QQ$ in the $\QQ$-isogeny class of $E$ has CM by an order with discriminant $-8$. Moreover, $\textit{j}_{E} = 8000$ or $1728$. Supose that $\textit{j}_{E} = 1728$. Then by 

Suppose that $\textit{j}_{E} = 8000$. Running code provided by Lozano-Robledo, we see that $E$ has CM by an order with conductor $1$.

VERY CONFUSED



\newpage

\subsection{\textit{j} = 0}

Let $E/\QQ$ be an elliptic curve defined over $\QQ$ with $\textit{j}_{E} = 0$. By Theorem 1.8 in \cite{al-rCMGRs}, the image of the $2$-adic Galois representation attached to $E$ is conjugate to one of two groups,
\begin{itemize}

\item $G_{1} := \left\langle
\begin{bmatrix} 0 & 1 \\ 1 & 0 \\ \end{bmatrix},
\begin{bmatrix} 7 & 4 \\ -4 & 3 \\ \end{bmatrix},
\begin{bmatrix} 3 & 6 \\ -6 & -3 \\ \end{bmatrix}, -I
\right\rangle$

\item $G_{2} := \left\langle
\begin{bmatrix} 0 & 1 \\ 1 & 0 \\ \end{bmatrix},
\begin{bmatrix} 7 & 4 \\ -4 & 3 \\ \end{bmatrix},
\begin{bmatrix} 2 & 1 \\ -1 & 1 \\ \end{bmatrix}, -I
\right\rangle$


\end{itemize}


The reduction of $G_{1}$ modulo $2$ is the subgroup of $\operatorname{GL}(2, \ZZ / 2 \ZZ)$ generated by $\begin{bmatrix} 0 & 1 \\ 1 & 0 \end{bmatrix}$ and the reduction of $G_{2}$ modulo $2$ is $\operatorname{GL}(2, \ZZ / 2 \ZZ)$. This shows that an elliptic curve $E/\QQ$ with $\textit{j}_{E} = 0$ has a point of order $2$ defined over $\QQ$ if and only if the image of the $2$-adic Galois representation attached to $E$ is conjugate to $G_{1}$.

If $E$ does not have a point of order $2$ defined over $\QQ$, then by Table \ref{tab-CMgraphs}, the isogeny graph associated to the $\QQ$-isogeny class of $E$ is of $L_{4}$ type or of $L_{2}(3)$ type. By Lemma \ref{2-adic determination}, the image of the $2$-adic Galois representation attached to each elliptic curve on an isogeny graph of type $L_{4}$ or $L_{2}(3)$ is conjugate to the same group; namely, $G_{2}$.

If $E$ has a point of order $2$ defined over $\QQ$, then by Table \ref{tab-CMgraphs}, the isogeny graph associated to the $\QQ$-isogeny class of $E$ is of $R_{4}(6)$ type. There are four elliptic curves in the $\QQ$-isogeny class, two with \textit{j}-invariant equal to $0$ and two with \textit{j}-invariant equal to $54000$. Let us label the elliptic curves in the $\QQ$-isogeny class that have \textit{j}-invariant $0$ as $E_{1}$ and $E_{2}$ and the elliptic curves in the $\QQ$-isogeny class that have \textit{j}-invariant $54000$ as $E_{3}$ and $E_{4}$. Then the isogeny graph of $E$ is of the form

\begin{center} \begin{tikzcd}
{E_{1}, \textit{j}_{E_{1}} = 0} \arrow[rr, "3", no head] \arrow[d, "2"', no head] &  & {E_{2}, \textit{j}_{E_{2}} = 0} \arrow[d, "2", no head] \\
{E_{3}, \textit{j}_{E_{3}}=54000} \arrow[rr, "3"', no head]              &  & {E_{4}, \textit{j}_{E_{4}}=54000}             
\end{tikzcd} \end{center}

As stated before, the image of the $2$-adic Galois representation attached to $E_{1}$ and $E_{2}$ is conjugate to $G_{1}$. Let us now compute the image of the $2$-adic Galois representation attached to $E_{3}$ and $E_{4}$. Let $P_{2^{\infty}}$ and $Q_{2^{\infty}}$ be generators of $E[2^{\infty}]$ such that the image of the $2$-adic Galois representation attached to $E_{1}$ is equal to $G_{1}$. If we rewrite the generators of $E[2^{\infty}] = \left\langle P_{2^{\infty}}, P_{2^{\infty}} + Q_{2^{\infty}} \right\rangle$, then the image of the $2$-adic Galois representation attached to $E_{1}$ is equal to
$$\left\langle
\begin{bmatrix} -1 & 0 \\ 1 & 1 \\ \end{bmatrix},
\begin{bmatrix} 11 & 12 \\ -4 & -1 \\ \end{bmatrix},
\begin{bmatrix} 9 & 18 \\ -6 & -9 \\ \end{bmatrix}, -I
\right\rangle.$$
By Lemma \ref{2-adic determination}, the image of the $2$-adic Galois representation attached to $E_{3}$ and $E_{4}$ is conjugate to
$$\left\langle
\begin{bmatrix} -1 & 0 \\ 2 & 1 \\ \end{bmatrix},
\begin{bmatrix} 11 & 6 \\ -8 & -1 \\ \end{bmatrix},
\begin{bmatrix} 9 & 9 \\ -12 & -9 \\ \end{bmatrix}, -I
\right\rangle.$$
Alternatively, we can make use of the fact that an elliptic curve with \textit{j}-invariant equal to $54000$ has CM by an order $\mathcal{O}_{K,f}$ with discriminant $-12 = 2^{2} \cdot -3 = f^{2} \cdot \Delta_{K}$. Hence, the conductor $f$ of the order $\mathcal{O}_{K,f}$ is equal to $2$.

In this case, $\Delta_{K} \cdot f^{2}$ is divisible by $4$ and so $\delta = \frac{\Delta_{K} \cdot f^{2}}{4} = -3$. Let us set $\phi = 0$. Following Theorem 1.1 in \cite{al-rCMGRs}, the image of the $2$-adic Galois representations attached to $E_{3}$ and $E_{4}$ are conjugate to
$$\mathcal{N}_{\delta, \phi}(N)$$
\newpage

	\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.7}{
    \begin{tabular}{ |c|c|c|c|c| }
    \hline
    Field & Discriminant & Conductor & $\delta$ & graph \\
    \hline
    $\QQ(\sqrt{-1})$ & $-4$ & $1$ & $-1$ & 5 \\
	\hline
	$\QQ(\sqrt{-2})$ & $-8$ & $2$ & $-8$ & 5 \\
	\hline
	$\QQ(\sqrt{-3})$ & $-3$ & $3$ & $-9$ & 5 \\
	\hline
	$\QQ(\sqrt{-7})$ & $-7$ & $7$ & $-98$ & 5 \\
	\hline
	$\QQ(\sqrt{-11})$ & $-11$ & $11$ & $-363$ & 5 \\
	\hline
	$\QQ(\sqrt{-19})$ & $-19$ & $19$ & $-1805$ & 5 \\
	\hline
	$\QQ(\sqrt{-43})$ & $-43$ & $43$ & $20339$ & 5 \\
	\hline
	$\QQ(\sqrt{-67})$ & $-67$ & $67$ & $-78608$ & 5 \\
	\hline
	$\QQ(\sqrt{-163})$ & $-163$ & $163$ & $-1089329$ & 5 \\
	\hline
\end{tabular}}
	\caption{CM graphs}
 	\label{CM graphs}
\end{table}
\end{center}
	
	\newpage
	
	\section{S Graphs}
	
	\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.7}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Isogeny Graph & $E_{1}$ & $E_{2}$ & $E_{3}$ & $E_{4}$ & $E_{5}$ & $E_{6}$ & $E_{7}$ & $E_{8}$ & Isogeny-Torsion Graph & Example Isogeny Class\\
    \hline
    \multirow{8}*{\includegraphics[scale=0.25]{Snew}} &
    \multirow{2}*{$\operatorname{H}_{8}$} & \multirow{2}*{$\operatorname{H}_{8}$} & \multirow{2}*{$\operatorname{H}_{13}$} & \multirow{2}*{$\operatorname{H}_{13}$} & \multirow{2}*{$\operatorname{H}_{13}$} & \multirow{2}*{$\operatorname{H}_{13}$} & \multirow{2}*{$\operatorname{H}_{13}$} & \multirow{2}*{$\operatorname{H}_{13}$} & $([2,6],[2,2],[6],[2],[6],[2],[6],[2])$ & \texttt{630.f} \\
    \cline{10-11}
    & & & & & & & & & $([2,2],[2,2],[2],[2],[2],[2],[2],[2])$ & \texttt{3630.w} \\
    \cline{2-11}
    & $\operatorname{H}_{8a}$ & $\operatorname{H}_{8a}$ & $\operatorname{H}_{13a}$ & $\operatorname{H}_{13a}$ & $\operatorname{H}_{13a}$ & $\operatorname{H}_{13a}$ & $\operatorname{H}_{13a}$ & $\operatorname{H}_{13a}$ & $([2,2],[2,2],[2],[2],[2],[2],[2],[2])$ & \texttt{450.d} \\
    \cline{2-11}
    & $\operatorname{H}_{8b}$ & $\operatorname{H}_{8b}$ & $\operatorname{H}_{13b}$ & $\operatorname{H}_{13b}$ & $\operatorname{H}_{13b}$ & $\operatorname{H}_{13b}$ & $\operatorname{H}_{13b}$ & $\operatorname{H}_{13b}$ & $([2,2],[2,2],[2],[2],[2],[2],[2],[2])$ & \texttt{14400.o} \\
    \cline{2-11}
    & \multirow{2}*{$\operatorname{H}_{8c}$} & \multirow{2}*{$\operatorname{H}_{8c}$} & \multirow{2}*{$\operatorname{H}_{13c}$} & \multirow{2}*{$\operatorname{H}_{13c}$} & \multirow{2}*{$\operatorname{H}_{13e}$} & \multirow{2}*{$\operatorname{H}_{13e}$} & \multirow{2}*{$\operatorname{H}_{13g}$} & \multirow{2}*{$\operatorname{H}_{13g}$} & $([2,6],[2,2],[6],[2],[6],[2],[6],[2])$ & \texttt{30.a} \\
    \cline{10-11}
    & & & & & & & & & $([2,2],[2,2],[2],[2],[2],[2],[2],[2])$ & \texttt{240.b} \\
    \cline{2-11}
    & \multirow{2}*{$\operatorname{H}_{8d}$} & \multirow{2}*{$\operatorname{H}_{8d}$} & \multirow{2}*{$\operatorname{H}_{13h}$} & \multirow{2}*{$\operatorname{H}_{13h}$} & \multirow{2}*{$\operatorname{H}_{13d}$} & \multirow{2}*{$\operatorname{H}_{13d}$} & \multirow{2}*{$\operatorname{H}_{13f}$} & \multirow{2}*{$\operatorname{H}_{13f}$} & $([2,6],[2,2],[12],[4],[6],[2],[6],[2])$ & \texttt{90.c} \\
    \cline{10-11}
    & & & & & & & & & $([2,2],[2,2],[4],[4],[2],[2],[2],[2])$ & \texttt{150.b} \\
    \hline
    

    
\end{tabular}}
\caption{2-adic Images of S Graphs}
\label{2-adic Images of S Graphs Table}
\end{table}
\end{center}
	
	\begin{proposition}\label{2-adic Images of S Graphs}
	Let $\mathcal{E}$ be a $\QQ$-isogeny class of elliptic curves defined over $\QQ$. Suppose that the isogeny graph associated to $\mathcal{E}$ is of type $S$. Then the classification of $2$-adic images associated to the elliptic curves over $\QQ$ in $\mathcal{E}$ are in Table \ref{2-adic Images of S Graphs Table}.
	\end{proposition}
	
	\begin{proof}

	We need to prove that there are no examples other than the ones from Table \ref{2-adic Images of S Graphs Table}. Let $E/\QQ$ be an elliptic curve with full two-torsion defined over $\QQ$. Suppose that the isogeny graph associated to the $\QQ$-isogeny class of $E$ is of type $\mathcal{S}$. Then $E$ has a $\QQ$-rational subgroup of order $3$ and the image of the mod-$2$ Galois representation attached to $E$ is trivial. 
	
	In the RZB database, the full lift of the trivial subgroup of $\operatorname{GL}(2, \ZZ / 2 \ZZ)$ is denoted $\operatorname{H}_{8}$. Referring to the RZB database (or the corresponding website), we see that there are eight modular curves that minimally cover $\operatorname{X}_{8}$, namely, $\operatorname{X}_{24}$, $\operatorname{X}_{25}$, $\operatorname{X}_{38}$, $\operatorname{X}_{46}$, $\operatorname{X}_{8a}$, $\operatorname{X}_{8b}$, $\operatorname{X}_{8c}$, and $\operatorname{X}_{8d}$.
	
	******************
	
	By NEWPAPER, the image of the mod-$2^{2} \cdot 3$ Galois representation attached to $E$ is not conjugate to a subgroup of $\operatorname{H}_{24} \times B(3)'$ or $\operatorname{H}_{25} \times B(3)'$. By NEWPAPER, the image of the mod-$2^{3} \cdot 3$ Galois representation attached to $E$ is not conjugate to a subgroup of $\operatorname{H}_{38} \times B(3)'$ or $\operatorname{H}_{46} \times B(3)'$.
	
	Using the RZB database, we see that the subgroups of $\operatorname{GL}(2, \ZZ / 8 \ZZ)$ that reduce modulo $4$ to $\operatorname{H}_{8b}$ are $\operatorname{H}_{38b}$, $\operatorname{H}_{46b}$, and the full lift of $\operatorname{H}_{8b}$ to level $8$. Using the RZB database, we see that the subgroups of $\operatorname{GL}(2, \ZZ / 8 \ZZ)$ that reduce modulo $4$ to $\operatorname{H}_{8d}$ are $\operatorname{H}_{38a}$, $\operatorname{H}_{38c}$, $\operatorname{H}_{38d}$, $\operatorname{H}_{46a}$, $\operatorname{H}_{46c}$, $\operatorname{H}_{46d}$, and the full lift of $\operatorname{H}_{8d}$ to level $8$. Using the RZB database, we see that there is a single subgroup of $\operatorname{GL}(2, \ZZ / 16 \ZZ)$ that reduces modulo $8$ to $\operatorname{H}_{8a}$, namely, the full lift of $\operatorname{H}_{8a}$ to level $16$. Similarly, using the RZB database, we see that there is a single subgroup of $\operatorname{GL}(2, \ZZ / 16 \ZZ)$ that reduces modulo $8$ to $\operatorname{H}_{8c}$, namely, the full lift of $\operatorname{H}_{8c}$ to level $16$.
	
	This means that the $2$-adic image of the Galois representation attached to $E$ is conjugate to $\operatorname{H}_{8a}$, $\operatorname{H}_{8b}$, $\operatorname{H}_{8c}$, $\operatorname{H}_{8d}$, or $\operatorname{H}_{8}$. Finally, by NEWPAPER, the image of the mod-$2^{2} \cdot 3$ Galois representation attached to $E$ is not conjugate to a subgroup of $\operatorname{H}_{8b} \times B(3)$ and the image of the mod-$2^{3} \cdot 3$ Galois representation attached to $E$ is not conjugate to a subgroup of $\operatorname{H}_{8a} \times B(3)$. All other examples are possible as can be seen in Table \ref{2-adic Images of S Graphs Table}.
	
	*******************
	\end{proof}
	
	\section{$R_{k}$ Graphs}
	
	\subsection{$R_{6}$ Graphs}
	
	\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.7}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \hline
    
    Isogeny Graph & $E_{1}$ & $E_{2}$ & $E_{3}$ & $E_{4}$ & $E_{5}$ & $E_{6}$ & Isogeny-Torsion Graph & Example Isogeny Class \\
    \hline
    \multirow{4}*{\includegraphics[scale=0.25]{R6new.jpg}} & \multirow{2}*{$\operatorname{H}_{16}$} & \multirow{2}*{$\operatorname{H}_{17}$} & \multirow{2}*{$\operatorname{H}_{16}$} & \multirow{2}*{$\operatorname{H}_{17}$} & \multirow{2}*{$\operatorname{H}_{16}$} & \multirow{2}*{$\operatorname{H}_{17}$} & $([6],[6],[6],[6],[2],[2])$ & \texttt{14.a} \\
    \cline{8-9}
    & & & & & & & $([2],[2],[2],[2],[2],[2])$ & \texttt{98.a} \\
    \cline{2-9}
    & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & $([6],[6],[6],[6],[2],[2])$ & \texttt{2394.j} \\
    \cline{8-9}
    & & & & & & & $([2],[2],[2],[2],[2],[2])$ & \texttt{271950.do} \\
    \hline
    
	\end{tabular}}
\caption{2-adic Images of $R_{6}$ Graphs}
\label{2-adic Images of R6 Graphs Table}
\end{table}
\end{center}

\begin{proposition}\label{2-adic Images of R_{6} Graphs}
	Let $\mathcal{E}$ be a $\QQ$-isogeny class of elliptic curves defined over $\QQ$. Suppose that the isogeny graph associated to $\mathcal{E}$ is of type $R_{6}$. Then the classification of $2$-adic images associated to the elliptic curves over $\QQ$ in $\mathcal{E}$ are in Table \ref{2-adic Images of R6 Graphs Table}.

\end{proposition}

\begin{proof}
We need to prove that there are no examples other than the ones from Table \ref{2-adic Images of R_{6} Graphs}. Let $E/\QQ$ be an elliptic curve that contains a $\QQ$-rational subgroup of order $18$. Then the image of the mod-$2$ Galois representation attached to $E$ is of order $2$.

In the RZB database, the full lift of the subgroup of $\operatorname{GL}(2, \ZZ / 2 \ZZ)$ of order $2$ is denoted $\operatorname{H}_{6}$. Referring to the RZB database (or the corresponding website), we see that there are twelve subgroups of $\operatorname{GL}(2, \ZZ_{2})$ that minimally cover $\operatorname{H}_{6}$, namely, all groups $\operatorname{H}_{8}$ to $\operatorname{H}_{19}$.

If the image of the $2$-adic Galois representation attached to $E$ is conjugate to $\operatorname{H}_{16}$, then $E$ is $2$-isogenous to an elliptic curve over $\QQ$ whose $2$-adic image is conjugate to $\operatorname{H}_{17}$. There are four subgroups of $\operatorname{GL}(2, \ZZ_{2})$ that minimally cover $\operatorname{H}_{16}$, namely, $\operatorname{H}_{29}$, $\operatorname{H}_{38}$, $\operatorname{H}_{40}$, and $\operatorname{H}_{42}$. Note that by Lemma \ref{2-adic determination}, if the image of the $2$-adic Galois representation attached to $E$ is not conjugate to $\operatorname{H}_{16}$, then the image of the $2$-adic Galois representation attached to any elliptic curve in the $\QQ$-isogeny class of $E$ is not conjugate to $\operatorname{H}_{17}$.

Thus, to prove that Table \ref{2-adic Images of R6 Graphs Table} is complete, we just need to prove that the image of the mod-$2^{N} \cdot 9$ Galois representation is not conjugate to a subgroup of any of the groups
$\operatorname{H}_{i} \times B(9)'$ where $i$ is any integer in $[8, 15]$ or $i = 18, 19, 29, 38, 40,$ or $42$.


*************************************************************

By NEWPAPER, there are no elliptic curves over $\QQ$ such that the image of the mod-$2^{N} \cdot 9$ Galois representation is conjugate to $\operatorname{H}_{i} \times B(9)'$ where $i$ is any integer in $[8, 15]$ or $i = 18, 19, 29, 38, 40,$ or $42$.

*************************************************************
\end{proof}

\subsection{$R_{4}$ Graphs}


\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.7}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    
    Isogeny Graph & $pq$ & $E_{1}$ & $E_{2}$ & $E_{3}$ & $E_{4}$ & Isogeny-Torsion Graph & Example Isogeny Class \\
    \hline
    \multirow{24}*{\includegraphics[scale=0.10]{Rk Graph.png}} & \multirow{2}*{$21$} & \multirow{2}*{$\operatorname{H}_{4}$} & \multirow{2}*{$\operatorname{H}_{4}$} & \multirow{2}*{$\operatorname{H}_{4}$} & \multirow{2}*{$\operatorname{H}_{4}$} & $([3],[3],[1],[1])$ & \texttt{162.b} \\
    \cline{7-8}
    & & & & & & $([1],[1],[1],[1])$ & \texttt{1296.f} \\
    \cline{2-8}
    & \multirow{3}*{$15$} & \multirow{3}*{$\operatorname{H}_{4}$} & 
    \multirow{3}*{$\operatorname{H}_{4}$} & \multirow{3}*{$\operatorname{H}_{4}$} & \multirow{3}*{$\operatorname{H}_{4}$} & $([5],[5],[1],[1])$ & \texttt{50.a} \\
    \cline{7-8}
    & & & & & & $([3],[3],[1],[1])$ & \texttt{50.b} \\
    \cline{7-8}
    & & & & & & $([1],[1],[1],[1])$ & \texttt{400.d} \\
    \cline{2-8}
    & \multirow{5}*{$10$} & \multirow{2}*{$\operatorname{H}_{15}$} & \multirow{2}*{$\operatorname{H}_{19}$} & \multirow{2}*{$\operatorname{H}_{15}$} & \multirow{2}*{$\operatorname{H}_{19}$} & $([10],[10],[2],[2])$ & \texttt{66.c} \\
    \cline{7-8}
    & & & & & & $([2],[2],[2],[2])$ & \texttt{198.c} \\
    \cline{3-8}
    & & $\operatorname{H}_{14}$ & $\operatorname{H}_{14}$ & $\operatorname{H}_{14}$ & $\operatorname{H}_{14}$ & $([2],[2],[2],[2])$ & \texttt{1734.d} \\
    \cline{3-8}
    & & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & $([10],[10],[2],[2])$ & \texttt{150.c} \\
\cline{7-8}
& & & & & & $([2],[2],[2],[2])$ & \texttt{150.a} \\
\cline{2-8}
& \multirow{14}*{$6$} & \multirow{2}*{$\operatorname{H}_{16}$} & \multirow{2}*{$\operatorname{H}_{17}$} & \multirow{2}*{$\operatorname{H}_{16}$} & \multirow{2}*{$\operatorname{H}_{17}$} & $([6],[6],[2],[2])$ & \texttt{34.a} \\
    \cline{7-8}
    & & & & & & $([2],[2],[2],[2])$ & \texttt{272.d} \\
    \cline{3-8}
    & & \multirow{2}*{$\operatorname{H}_{15}$} & \multirow{2}*{$\operatorname{H}_{19}$} & \multirow{2}*{$\operatorname{H}_{15}$} & \multirow{2}*{$\operatorname{H}_{19}$} & $([6],[6],[2],[2])$ & \texttt{66.a} \\
    \cline{7-8}
    & & & & & & $([2],[2],[2],[2])$ & \texttt{528.d} \\
    \cline{3-8}
    & & \multirow{2}*{$\operatorname{H}_{9d}$} & \multirow{2}*{$\operatorname{H}_{10d}$} & \multirow{2}*{$\operatorname{H}_{9d}$} & \multirow{2}*{$\operatorname{H}_{10d}$} & $([6],[6],[2],[2])$ & \texttt{130.a} \\
    \cline{7-8}
    & & & & & & $([2],[2],[2],[2])$ & \texttt{320.a} \\
    \cline{3-8}
    & & \multirow{2}*{$\operatorname{H}_{9c}$} & \multirow{2}*{$\operatorname{H}_{10a}$} & \multirow{2}*{$\operatorname{H}_{9c}$} & \multirow{2}*{$\operatorname{H}_{10a}$} & $([6],[6],[2],[2])$ & \texttt{20.a} \\
    \cline{7-8}
    & & & & & & $([2],[2],[2],[2])$ & \texttt{80.b} \\
    \cline{3-8}
    & & $\operatorname{H}_{9b}$ & $\operatorname{H}_{10b}$ & $\operatorname{H}_{9b}$ & $\operatorname{H}_{10b}$ & $([2],[2],[2],[2])$ & \texttt{1600.c} \\
    \cline{3-8}
    & & $\operatorname{H}_{9a}$ & $\operatorname{H}_{10c}$ & $\operatorname{H}_{9a}$ & $\operatorname{H}_{10c}$ & $([2],[2],[2],[2])$ & \texttt{100.a} \\
    \cline{3-8}
    & & \multirow{2}*{$\operatorname{H}_{9}$} & \multirow{2}*{$\operatorname{H}_{10}$} & \multirow{2}*{$\operatorname{H}_{9}$} & \multirow{2}*{$\operatorname{H}_{10}$} & $([6],[6],[2],[2])$ & \texttt{180.a} \\
    \cline{7-8}
    & & & & & & $([2],[2],[2],[2])$ & \texttt{650.l} \\
    \cline{3-8}
    & & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & \multirow{2}*{$\operatorname{H}_{6}$} & $([6],[6],[2],[2])$ & \texttt{84.b} \\
    \cline{7-8}
    & & & & & & $([2],[2],[2],[2])$ & \texttt{336.b} \\
    \hline
    \end{tabular}}
\caption{2-adic Images of $R_{4}$ Graphs}
\label{2-adic Images of R4 Graphs Table}
\end{table}
\end{center}


\newpage

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.7}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    Isogeny Graph & $p$ & $E_{1}$ & $E_{2}$ & $E_{3}$ & Isogeny-Torsion Graph & Example Isogeny Class \\
    \hline
    \multirow{5}*{\includegraphics[scale=0.1]{L3 Graph.png}} & \multirow{2}*{$5$} & \multirow{2}*{$\operatorname{H}_{1}$} & \multirow{2}*{$\operatorname{H}_{1}$} & \multirow{2}*{$\operatorname{H}_{1}$} & $([5],[5],[1])$ & \texttt{11.a} \\
    \cline{6-7}
    & & & & & $([1],[1],[1])$ & \texttt{99.d} \\
    \cline{2-7}
    & \multirow{3}*{$3$} & \multirow{3}*{$\operatorname{H}_{1}$} & \multirow{3}*{$\operatorname{H}_{1}$} & \multirow{3}*{$\operatorname{H}_{1}$} & $([9],[3],[1])$ & \texttt{54.b} \\
    \cline{6-7}
    & & & & & $([3],[3],[1])$ & \texttt{19.a} \\
    \cline{6-7}
    & & & & & $([1],[1],[1])$ & \texttt{175.b} \\
    \hline
    
    
\end{tabular}}
\caption{2-adic Images of $L_{3}$ Graphs}
\label{2-adic Images of L3 Graphs Table}
\end{table}
\end{center}


\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1}
\scalebox{0.7}{
    \begin{tabular}{|c|c|c|c|c|c|}

\hline

Isogeny Graph & $p$ & $E_{1}$ & $E_{2}$ & Isogeny-Torsion Graph & Example Isogeny Class \\
    \hline

\multirow{48}*{\includegraphics[scale=0.075]{L2 Graph.png}} & $37$ & $\operatorname{H}_{1}$ & $\operatorname{H}_{1}$ & $([1],[1])$ & \texttt{1225.b} \\
\cline{2-6}
& $17$ & $\operatorname{H}_{1}$ & $\operatorname{H}_{1}$ & $([1],[1])$ & \texttt{14450.b} \\
\cline{2-6}
& \multirow{2}*{$13$} & $\operatorname{H}_{1}$ & $\operatorname{H}_{1}$ & $([1],[1])$ & \texttt{147.b} \\
\cline{3-6}
& & $\operatorname{H}_{4}$ & $\operatorname{H}_{4}$ & $([1],[1])$ & \texttt{11094.g} \\
\cline{2-6}
& \multirow{3}*{$11$} & $\operatorname{H}_{3}$ & $\operatorname{H}_{3}$ & $([1],[1])$ & \texttt{121.a} \\
\cline{3-6}
& & $\operatorname{H}_{3a}$ & $\operatorname{H}_{3a}$ & $([1],[1])$ & \texttt{7744.c} \\
\cline{3-6}
& & $\operatorname{H}_{3b}$ & $\operatorname{H}_{3b}$ & $([1],[1])$ & \texttt{121.c} \\
\cline{2-6}
& \multirow{13}*{$7$} & \multirow{2}*{$\operatorname{H}_{1}$} & \multirow{2}*{$\operatorname{H}_{1}$} & $([7],[1])$ & \texttt{26.b} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{208.d} \\
\cline{3-6}
& & $\operatorname{H}_{2}$ & $\operatorname{H}_{2}$ & $([1],[1])$ & \texttt{1922.c} \\
\cline{3-6}
& & $\operatorname{H}_{2a}$ & $\operatorname{H}_{2a}$ & $([1],[1])$ & \texttt{3969.d} \\
\cline{3-6}
& & $\operatorname{H}_{2b}$ & $\operatorname{H}_{2b}$ & $([1],[1])$ & \texttt{1922.e} \\
\cline{3-6}
& & $\operatorname{H}_{3}$ & $\operatorname{H}_{3}$ & $([1],[1])$ & \texttt{507.b} \\
\cline{3-6}
& & $\operatorname{H}_{3a}$ & $\operatorname{H}_{3a}$ & $([1],[1])$ & \texttt{87616.w} \\
\cline{3-6}
& & $\operatorname{H}_{3b}$ & $\operatorname{H}_{3b}$ & $([1],[1])$ & \texttt{1369.d} \\
\cline{3-6}
& & $\operatorname{H}_{4}$ & $\operatorname{H}_{4}$ & $([1],[1])$ & \texttt{11094.i} \\
\cline{3-6}
& & $\operatorname{H}_{5}$ & $\operatorname{H}_{5}$ & $([1],[1])$ & \texttt{12482.f} \\
\cline{3-6}
& & $\operatorname{H}_{20}$ & $\operatorname{H}_{20}$ & $([1],[1])$ & \texttt{338.c} \\
\cline{3-6}
& & $\operatorname{H}_{20a}$ & $\operatorname{H}_{20a}$ & $([1],[1])$ & \texttt{10816.u1} \\
\cline{3-6}
& & $\operatorname{H}_{20b}$ & $\operatorname{H}_{20b}$ & $([1],[1])$ & \texttt{338.e} \\
\cline{2-6}
& \multirow{5}*{$5$} & \multirow{2}*{$\operatorname{H}_{1}$} & \multirow{2}*{$\operatorname{H}_{1}$} & $([5],[1])$ & \texttt{38.b} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{75.c} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{4}$} & \multirow{2}*{$\operatorname{H}_{4}$} & $([5],[1])$ & \texttt{38350.t} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{6400.d} \\
\cline{3-6}
& & $\operatorname{H}_{7}$ & $\operatorname{H}_{7}$ & $([1],[1])$ & \texttt{14450.h} \\
\cline{2-6}
& \multirow{23}*{$3$} & \multirow{2}*{$\operatorname{H}_{1}$} & \multirow{2}*{$\operatorname{H}_{1}$} & $([3],[1])$ & \texttt{44.a} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{176.a} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{2}$} & \multirow{2}*{$\operatorname{H}_{2}$} & $([3],[1])$ & \texttt{324.a} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{196.a} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{2a}$} & \multirow{2}*{$\operatorname{H}_{2a}$} & $([3],[1])$ & \texttt{196.b} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{784.d} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{2b}$} & \multirow{2}*{$\operatorname{H}_{2b}$} & $([3],[1])$ & \texttt{1922.b} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{3136.h} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{3}$} & \multirow{2}*{$\operatorname{H}_{3}$} & $([3],[1])$ & \texttt{324.d} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{242.b} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{3a}$} & \multirow{2}*{$\operatorname{H}_{3a}$} & $([3],[1])$ & \texttt{1058.b} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{5184.z} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{3b}$} & \multirow{2}*{$\operatorname{H}_{3b}$} & $([3],[1])$ & \texttt{242.a} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{1296.a} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{4}$} & \multirow{2}*{$\operatorname{H}_{4}$} & $([3],[1])$ & \texttt{350.e} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{350.a} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{5}$} & \multirow{2}*{$\operatorname{H}_{5}$} & $([3],[1])$ & \texttt{1682.b} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{1682.i} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{20}$} & \multirow{2}*{$\operatorname{H}_{20}$} & $([3],[1])$ & \texttt{162.a} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{1296.c} \\
\cline{3-6}
& & $\operatorname{H}_{20a}$ & $\operatorname{H}_{20a}$ & $([1],[1])$ & \texttt{5184.c} \\
\cline{3-6}
& & \multirow{2}*{$\operatorname{H}_{20b}$} & \multirow{2}*{$\operatorname{H}_{20b}$} & $([3],[1])$ & \texttt{162.d} \\
\cline{5-6}
& & & & $([1],[1])$ & \texttt{1296.l} \\
\cline{3-6}
\hline
\end{tabular}}
\caption{2-adic Images of odd-degree $L_{2}$ Graphs}
\label{2-adic Images of L2 Graphs Table Odd}
\end{table}
\end{center}

\newpage

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.7}{
    \begin{tabular}{|c|c|c|}

\hline

Isogeny-Torsion Graph & $E$ & Example Isogeny Class \\
    \hline
\multirow{22}*{$([1])$} & $\operatorname{H}_{1}$ & \texttt{37.a} \\
\cline{2-3}
& $\operatorname{H}_{2} = \texttt{2.2.0.1}$ & \texttt{392.a} \\
\cline{2-3}
& $\operatorname{H}_{2a} = \texttt{4.4.0.2}$ & \texttt{392.c} \\
\cline{2-3}
& $\operatorname{H}_{2b} = \texttt{8.4.0.1}$ & \texttt{3136.b} \\
\cline{2-3}
& $\operatorname{H}_{3} = \texttt{4.2.0.1}$ & \texttt{567.a} \\
\cline{2-3}
& $\operatorname{H}_{3a} = \texttt{4.4.0.3}$ & \texttt{2738.b} \\
\cline{2-3}
& $\operatorname{H}_{3b} = \texttt{8.4.0.2}$ & \texttt{2116.c} \\
\cline{2-3}
& $\operatorname{H}_{4} = \texttt{8.2.0.1}$ & \texttt{200.a} \\
\cline{2-3}
& $\operatorname{H}_{5} = \texttt{8.2.0.2}$ & \texttt{1682.a} \\
\cline{2-3}
& $\operatorname{H}_{7} = \texttt{4.4.0.1}$ & \texttt{216.a} \\
\cline{2-3}
& $\operatorname{H}_{20} = \texttt{4.8.0.2}$ & \texttt{648.d} \\
\cline{2-3}
& $\operatorname{H}_{20a} = \texttt{8.16.0.3}$ & \texttt{5184.u} \\
\cline{2-3}
& $\operatorname{H}_{20b} = \texttt{4.16.0.2}$ & \texttt{648.b} \\
\cline{2-3}
& $\operatorname{H}_{22} = \texttt{8.8.0.1}$ & \texttt{44800.r} \\
\cline{2-3}
& $\operatorname{H}_{55} = \texttt{8.16.0.1}$ & \texttt{3388.f} \\
\cline{2-3}
& $\operatorname{H}_{56} = \texttt{16.16.0.1}$ & \texttt{3628800.bg} \\
\cline{2-3}
& $\operatorname{H}_{57} = \texttt{16.16.0.2}$ & \texttt{6400.b} \\
\cline{2-3}
& $\operatorname{H}_{57a} = \texttt{32.32.0.3}$ & \texttt{6400.p} \\
\cline{2-3}
& $\operatorname{H}_{57b} = \texttt{32.32.0.4}$ & \texttt{6400.c} \\
\cline{2-3}
& $\operatorname{H}_{177}$ & $y^{2} = x^{3} - 340750x - 76560000$ \\
\cline{2-3}
& $\operatorname{H}_{178} = \texttt{32.32.0.1}$ & \texttt{20736.e} \\
\cline{2-3}
& $\operatorname{H}_{441}$ & $y^{2}+y = x^{3} - 3014658660x+150916472601529$ \\
\hline

\end{tabular}}
\caption{2-adic Images of $L_{1}$ Graphs}
\label{2-adic Images of L1 Graphs}
\end{table}
\end{center}

\newpage

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.53}{
    \begin{tabular}{|c|c|c|c|c|c|c|}

\hline

Isogeny Graph & Isogeny-Torsion Graph & $E_{1}$ & $E_{2}$ & $E_{3}$ & $E_{4}$ & Example Isogeny Class \\
\hline
\multirow{60}*{\includegraphics[scale=0.1]{T4 Graph.png}} &

\multirow{7}*{$([2,2],[4],[4],[2])$} & $\operatorname{H}_{24e}$ & $\operatorname{H}_{32l}$ & $\operatorname{H}_{27h}$ & $\operatorname{H}_{32i}$ & \texttt{205a} \\
\cline{3-7}
& & $\operatorname{H}_{61h}$ & $\operatorname{H}_{116l}$ & $\operatorname{H}_{95a}$ & $\operatorname{H}_{116i}$ & \texttt{291.b} \\
\cline{3-7}
& & $\operatorname{H}_{66e}$ & $\operatorname{H}_{79h}$ & $\operatorname{H}_{94d}$ & $\operatorname{H}_{79i}$ & \texttt{1120.i} \\
\cline{3-7}
& & $\operatorname{H}_{67c}$ & $\operatorname{H}_{115e}$ & $\operatorname{H}_{60d}$ & $\operatorname{H}_{115g}$ & \texttt{40.a} \\
\cline{3-7}
& & $\operatorname{H}_{209b}$ & $\operatorname{H}_{222a}$ & $\operatorname{H}_{241d}$ & $\operatorname{H}_{241c}$ & \texttt{514.b} \\
\cline{3-7}
& & $\operatorname{H}_{210b}$ & $\operatorname{H}_{221a}$ & $\operatorname{H}_{242d}$ & $\operatorname{H}_{242b}$ & \texttt{17.a} \\
\cline{3-7}
& & $\operatorname{H}_{214b}$ & $\operatorname{H}_{226d}$ & $\operatorname{H}_{231c}$ & $\operatorname{H}_{226c}$ & \text{84320.k} \\
\cline{2-7}

& \multirow{14}*{$([2,2],[4],[2],[2])$} & $\operatorname{H}_{8d}$ & $\operatorname{H}_{13h}$ & $\operatorname{H}_{13d}$ & $\operatorname{H}_{13f}$ & \texttt{33.a} \\
\cline{3-7}
& & $\operatorname{H}_{38a}$ & $\operatorname{H}_{34a}$ & $\operatorname{H}_{34d}$ & $\operatorname{H}_{44b}$ & \texttt{392.d} \\
\cline{3-7}
& & $\operatorname{H}_{38c}$ & $\operatorname{H}_{44c}$ & $\operatorname{H}_{34h}$ & $\operatorname{H}_{34e}$ & \texttt{112.b} \\
\cline{3-7}
& & $\operatorname{H}_{38d}$ & $\operatorname{H}_{34f}$ & $\operatorname{H}_{34g}$ & $\operatorname{H}_{44d}$ & \texttt{56.a} \\
\cline{3-7}
& & $\operatorname{H}_{46a}$ & $\operatorname{H}_{33c}$ & $\operatorname{H}_{33d}$ & $\operatorname{H}_{48b}$ & \texttt{288.b} \\
\cline{3-7}
& & $\operatorname{H}_{46c}$ & $\operatorname{H}_{48c}$ & $\operatorname{H}_{33h}$ & $\operatorname{H}_{33f}$ & \texttt{96.b} \\
\cline{3-7}
& & $\operatorname{H}_{46d}$ & $\operatorname{H}_{33e}$ & $\operatorname{H}_{33g}$ & $\operatorname{H}_{48d}$ & \texttt{66.b} \\
\cline{3-7}
& & $\operatorname{H}_{24d}$ & $\operatorname{H}_{32e}$ & $\operatorname{H}_{32f}$ & $\operatorname{H}_{27d}$ & \texttt{2200.e} \\
\cline{3-7}
& & $\operatorname{H}_{61d}$ & $\operatorname{H}_{116e}$ & $\operatorname{H}_{116f}$ & $\operatorname{H}_{95e}$ & \texttt{28227.e} \\
\cline{3-7}
& & $\operatorname{H}_{66d}$ & $\operatorname{H}_{79b}$ & $\operatorname{H}_{79d}$ & $\operatorname{H}_{94f}$ & \texttt{2240.l} \\
\cline{3-7}
& & $\operatorname{H}_{67b}$ & $\operatorname{H}_{115a}$ & $\operatorname{H}_{115d}$ & $\operatorname{H}_{60b}$ & \texttt{200.c} \\
\cline{3-7}
& & $\operatorname{H}_{209c}$ & $\operatorname{H}_{241e}$ & $\operatorname{H}_{241h}$ & $\operatorname{H}_{222c}$ & \texttt{132098.b} \\
\cline{3-7}
& & $\operatorname{H}_{210c}$ & $\operatorname{H}_{242h}$ & $\operatorname{H}_{242e}$ & $\operatorname{H}_{221c}$ & \texttt{289.a} \\
\cline{3-7}
& & $\operatorname{H}_{214d}$ & $\operatorname{H}_{226e}$ & $\operatorname{H}_{226h}$ & $\operatorname{H}_{231a}$ & \texttt{168640.bg} \\

\cline{2-7}

& \multirow{39}*{$([2,2],[2],[2],[2])$} & $\operatorname{H}_{8b}$ & $\operatorname{H}_{13b}$ & $\operatorname{H}_{13b}$ & $\operatorname{H}_{13b}$ & \texttt{1089.j}\\
\cline{3-7}
& & $\operatorname{H}_{38b}$ & $\operatorname{H}_{34c}$ & $\operatorname{H}_{44a}$ & $\operatorname{H}_{34b}$ & \texttt{3136.q} \\
\cline{3-7}
& & $\operatorname{H}_{46b}$ & $\operatorname{H}_{33a}$ & $\operatorname{H}_{33b}$ & $\operatorname{H}_{48a}$ & \texttt{576.h} \\
\cline{3-7}
& & $\operatorname{H}_{24}$ & $\operatorname{H}_{32}$ & $\operatorname{H}_{32}$ & $\operatorname{H}_{27}$ & \texttt{1845.e} \\
\cline{3-7}
& & $\operatorname{H}_{61}$ & $\operatorname{H}_{116}$ & $\operatorname{H}_{116}$ & $\operatorname{H}_{95}$ & \texttt{7275.i} \\
\cline{3-7}
& & $\operatorname{H}_{66}$ & $\operatorname{H}_{79}$ & $\operatorname{H}_{79}$ & $\operatorname{H}_{94}$ & \texttt{10080.h} \\
\cline{3-7}
& & $\operatorname{H}_{67}$ & $\operatorname{H}_{115}$ & $\operatorname{H}_{115}$ & $\operatorname{H}_{60}$ & \texttt{360.a} \\
\cline{3-7}
& & $\operatorname{H}_{209}$ & $\operatorname{H}_{241}$ & $\operatorname{H}_{241}$ & $\operatorname{H}_{222}$ & \texttt{4626.d} \\
\cline{3-7}
& & $\operatorname{H}_{210}$ & $\operatorname{H}_{242}$ & $\operatorname{H}_{242}$ & $\operatorname{H}_{221}$ & \texttt{153.d} \\
\cline{3-7}
& & $\operatorname{H}_{214}$ & $\operatorname{H}_{226}$ & $\operatorname{H}_{226}$ & $\operatorname{H}_{231}$ & \texttt{421600.o} \\
\cline{3-7}
& & $\operatorname{H}_{24a}$ & $\operatorname{H}_{32a}$ & $\operatorname{H}_{32a}$ & $\operatorname{H}_{27b}$ & \texttt{7200.bz} \\
\cline{3-7}
& & $\operatorname{H}_{24b}$ & $\operatorname{H}_{32h}$ & $\operatorname{H}_{32h}$ & $\operatorname{H}_{27e}$ & \texttt{1025.c} \\
\cline{3-7}
& & $\operatorname{H}_{24c}$ & $\operatorname{H}_{32k}$ & $\operatorname{H}_{32j}$ & $\operatorname{H}_{27g}$ & \texttt{960.d} \\
\cline{3-7}
& & $\operatorname{H}_{24f}$ & $\operatorname{H}_{32g}$ & $\operatorname{H}_{32g}$ & $\operatorname{H}_{27f}$ & \texttt{936.h} \\
\cline{3-7}
& & $\operatorname{H}_{24g}$ & $\operatorname{H}_{32b}$ & $\operatorname{H}_{32b}$ & $\operatorname{H}_{27a}$ & \texttt{14400.ex} \\
\cline{3-7}
& & $\operatorname{H}_{24h}$ & $\operatorname{H}_{32d}$ & $\operatorname{H}_{32c}$ & $\operatorname{H}_{27c}$ & \texttt{2400.b} \\
\cline{3-7}
& & $\operatorname{H}_{61a}$ & $\operatorname{H}_{116h}$ & $\operatorname{H}_{116h}$ & $\operatorname{H}_{95c}$ & \texttt{873.c} \\
\cline{3-7}
& & $\operatorname{H}_{61b}$ & $\operatorname{H}_{116g}$ & $\operatorname{H}_{116g}$ & $\operatorname{H}_{95d}$ & \texttt{6066.e} \\
\cline{3-7}
& & $\operatorname{H}_{61c}$ & $\operatorname{H}_{116c}$ & $\operatorname{H}_{116d}$ & $\operatorname{H}_{95f}$ & \texttt{161376.y} \\
\cline{3-7}
& & $\operatorname{H}_{61e}$ & $\operatorname{H}_{116b}$ & $\operatorname{H}_{116b}$ & $\operatorname{H}_{95g}$ & \texttt{84681.j} \\
\cline{3-7}
& & $\operatorname{H}_{61f}$ & $\operatorname{H}_{116a}$ & $\operatorname{H}_{116a}$ & $\operatorname{H}_{95h}$ & $y^{2} = x^{3} - 134002596x + 596756613760$ \\
\cline{3-7}
& & $\operatorname{H}_{61g}$ & $\operatorname{H}_{116k}$ & $\operatorname{H}_{116j}$ & $\operatorname{H}_{95b}$ & \texttt{7872.k} \\
\cline{3-7}
& & $\operatorname{H}_{66a}$ & $\operatorname{H}_{79e}$ & $\operatorname{H}_{79g}$ & $\operatorname{H}_{94a}$ & \texttt{39200.bo} \\
\cline{3-7}
& & $\operatorname{H}_{66b}$ & $\operatorname{H}_{79f}$ & $\operatorname{H}_{79f}$ & $\operatorname{H}_{94e}$ & \texttt{7840.m} \\
\cline{3-7}
& & $\operatorname{H}_{66c}$ & $\operatorname{H}_{79a}$ & $\operatorname{H}_{79c}$ & $\operatorname{H}_{94c}$ & \texttt{5600.j} \\
\cline{3-7}
& & $\operatorname{H}_{66f}$ & $\operatorname{H}_{79j}$ & $\operatorname{H}_{79j}$ & $\operatorname{H}_{94b}$ & \texttt{15680.cb} \\
\cline{3-7}
& & $\operatorname{H}_{67a}$ & $\operatorname{H}_{115f}$ & $\operatorname{H}_{115h}$ & $\operatorname{H}_{60c}$ & \texttt{320.d} \\
\cline{3-7}
& & $\operatorname{H}_{67d}$ & $\operatorname{H}_{115c}$ & $\operatorname{H}_{115b}$ & $\operatorname{H}_{60a}$ & \texttt{1600.o} \\
\cline{3-7}
& & $\operatorname{H}_{209a}$ & $\operatorname{H}_{241a}$ & $\operatorname{H}_{241b}$ & $\operatorname{H}_{222b}$ & \texttt{16448.k} \\
\cline{3-7}
& & $\operatorname{H}_{209d}$ & $\operatorname{H}_{241f}$ & $\operatorname{H}_{241g}$ & $\operatorname{H}_{222d}$ & $y^{2} = x^{3} - 5794082476x + 169747287967440$ \\
\cline{3-7}
& & $\operatorname{H}_{210a}$ & $\operatorname{H}_{242a}$ & $\operatorname{H}_{242c}$ & $\operatorname{H}_{221b}$ & \texttt{1088.i} \\
\cline{3-7}
& & $\operatorname{H}_{210d}$ & $\operatorname{H}_{242f}$ & $\operatorname{H}_{221d}$ & $\operatorname{H}_{242g}$ & \texttt{18496.i} \\
\cline{3-7}
& & $\operatorname{H}_{214a}$ & $\operatorname{H}_{226a}$ & $\operatorname{H}_{2226b}$ & $\operatorname{H}_{231d}$ & $y^{2} = x^{3} - 248504206997764x - 1507817332544964967680$ \\
\cline{3-7}
& & $\operatorname{H}_{214c}$ & $\operatorname{H}_{226f}$ & $\operatorname{H}_{226g}$ & $\operatorname{H}_{231b}$ & \texttt{$y^{2} = x^{3} - 62126051749441x - 188477166568120620960$} \\
\cline{3-7}
& & $\operatorname{H}_{8}$ & $\operatorname{H}_{13}$ & $\operatorname{H}_{13}$ & $\operatorname{H}_{13}$ & \texttt{315.a} \\
\cline{3-7}
& & $\operatorname{H}_{38}$ & $\operatorname{H}_{34}$ & $\operatorname{H}_{34}$ & $\operatorname{H}_{44}$ & \texttt{350.b} \\
\cline{3-7}
& & $\operatorname{H}_{46}$ & $\operatorname{H}_{33}$ & $\operatorname{H}_{33}$ & $\operatorname{H}_{48}$ & \texttt{198.a} \\
\cline{3-7}
& & $\operatorname{H}_{8a}$ & $\operatorname{H}_{13a}$ & $\operatorname{H}_{13a}$ & $\operatorname{H}_{13a}$ & \texttt{1800.c} \\
\cline{3-7}
& & $\operatorname{H}_{8c}$ & $\operatorname{H}_{13g}$ & $\operatorname{H}_{13e}$ & $\operatorname{H}_{13c}$ & \texttt{120.a} \\
\hline
\end{tabular}}
\caption{2-adic Images of $T_{4}$ Graphs}
\label{2-adic Images of T4 Graphs}
\end{table}
\end{center}

\subsection{$2$-adic images of $T_{4}$ graphs not in LMFDB}

There are four classes of $2$-adic images of non-CM elliptic curves over $\QQ$ whose associated isogeny graph is of type $T_{4}$ and which are not found in the LMFDB. To classify these $2$-adic images, we use the example of the elliptic curve in the isogeny graph with full two-torsion defined over $\QQ$ provided by the RZB database and its associated $2$-adic image. Let $E/\QQ$ be such an elliptic curve. We will say that $P_{2}$ and $Q_{2}$ are distinct points on $E$ of order $2$. The points $P_{2}$ and $Q_{2}$ are defined over $\QQ$ as $E$ has full two torsion defined over $\QQ$. As the isogeny graph associated to the $\QQ$-isogeny class of $E$ is of type $T_{4}$, the only finite, cyclic, $\QQ$-rational subgroups of $E$ are the four groups generated by $P_{2}$, $Q_{2}$, $P_{2}+Q_{2}$, and $\mathcal{O}$. It remains to compute the image of the $2$-adic Galois representation attached to $E / \left\langle Q_{2} \right\rangle$, $E / \left\langle P_{2} \right\rangle$, and $E / \left\langle P_{2} + Q_{2} \right\rangle$. By \cite{rouse} all that needs to be done is to compute the image of the mod-$32$ Galois representation attached to the elliptic curve in question.

\begin{enumerate}
    \item $\operatorname{H}_{61f} = \left\langle
    \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix},
    \begin{bmatrix} 1 & 2 \\ 6 & 7 \end{bmatrix},
    \begin{bmatrix} 3 & 6 \\ 10 & 5 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 12 & 3 \end{bmatrix}
    \right\rangle \subseteq \operatorname{GL}(2, \ZZ / 16 \ZZ)$
    
    Note that the transpose of $\operatorname{H}_{61f}$ is conjugate to $\operatorname{H}_{61f}$ in $\operatorname{GL}(2, \ZZ / 16 \ZZ)$. Let $E/\QQ$ be an elliptic curve such that the image of the $2$-adic Galois representation attached to $E$ is conjugate to $\operatorname{H}_{61f}$. By Lemma \ref{group lifting}, the image of the mod-$64$ Galois representation attached to $E$ is conjugate to
    $$\hat{H} = \left\langle
    \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix},
    \begin{bmatrix} 1 & 2 \\ 6 & 7 \end{bmatrix},
    \begin{bmatrix} 3 & 6 \\ 10 & 5 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 12 & 3 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix}
    \right\rangle$$
    where $\left\langle\begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix}\right\rangle$ is the kernel of the reduction by $16$ map from $\operatorname{GL}(2, \ZZ / 64 \ZZ)$ to $\operatorname{GL}(2, \ZZ / 16 \ZZ)$. Moreover, $E$ has full two-torsion defined over $\QQ$. Let $P_{2}$ and $Q_{2}$ be points on $E$ of order $2$. Then $P_{2}$, $Q_{2}$, and $P_{2}+Q_{2}$ generate the non-trivial, finite, cyclic, $\QQ$-rational subgroups of $E$. We compute the $2$-adic Galois representations attached to $E / \left\langle Q_{2} \right\rangle$, $E / \left\langle P_{2} \right\rangle$, and $E / \left\langle P_{2} + Q_{2} \right\rangle$.
    
    \begin{itemize}
        \item $E/\left\langle Q_{2} \right\rangle$
        
        By Corollary \ref{2-adic image determination corollary}, the image of the mod-$32$ Galois representation attached to $E/\left\langle Q_{2} \right\rangle$ is conjugate to
    $$H' = \left\langle
    \begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix},
    \begin{bmatrix} 1 & 1 \\ 12 & 7 \end{bmatrix},
    \begin{bmatrix} 3 & 3 \\ 20 & 5 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 24 & 3 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix}
    \right\rangle.$$
    Note that the transpose of $H'$ is conjugate to $H'$ in $\operatorname{GL}(2, \ZZ / 32 \ZZ)$. Looking this group up in the RZB database, we see that it has label $\operatorname{H}_{116a}$. The level of $\operatorname{H}_{116a}$ is equal to $32$.
    
    \item $E/ \left\langle P_{2} \right\rangle$
    
    By Corollary \ref{2-adic image determination corollary}, the image of the mod-$32$ Galois representation attached to $E$ is conjugate to
    $$H' = \left\langle
    \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 3 \\ 4 & 1 \end{bmatrix},
    \begin{bmatrix} 5 & 5 \\ 12 & 3 \end{bmatrix},
    \begin{bmatrix} 3 & 6 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix}
    \right\rangle.$$
    Note that the transpose of $H'$ is conjugate to $H'$ in $\operatorname{GL}(2, \ZZ / 32 \ZZ)$. Looking this group up in the RZB database, we see that it is conjugate to the group $\operatorname{H}_{116a}$.
    
    \item $E/\left\langle P_{2} + Q_{2} \right\rangle$
    
    By Corollary \ref{2-adic image determination corollary}, the image of the mod-$32$ Galois representation attached to $E/ \left\langle P_{2}+Q_{2} \right\rangle$ is conjugate to
    $$H' = \left\langle
    \begin{bmatrix} 1 & -2 \\ 0 & 5 \end{bmatrix},
    \begin{bmatrix} -5 & -5 \\ 12 & 13 \\ \end{bmatrix},
    \begin{bmatrix} -7 & -3 \\ 20 & 15 \\ \end{bmatrix},
    \begin{bmatrix} -11 & -7 \\ 24 & 15 \\ \end{bmatrix},
    \begin{bmatrix} 17 & 8 \\ 0 & 1 \\ \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \\ \end{bmatrix},
    \begin{bmatrix} -15 & -8 \\ 32 & 17 \\ \end{bmatrix},
    \begin{bmatrix} 1 & -8 \\ 0 & 17 \\ \end{bmatrix}
    \right\rangle.$$
    Note that the transpose of $H'$ is conjugate to $H'$ in $\operatorname{GL}(2, \ZZ / 32 \ZZ)$. Looking this group in the RZB database, we see that it is conjugate to group $\operatorname{H}_{95h}$. The level of $\operatorname{H}_{95h}$ is equal to $16$.
    \end{itemize}
    
    \item $\operatorname{H}_{209d} = \left\langle \begin{bmatrix} 1 & 2 \\ 14 & 5 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 12 & 5 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 7 \end{bmatrix} \right\rangle \subseteq \operatorname{GL}(2, \ZZ / 16 \ZZ)$

    Note that the transpose of $\operatorname{H}_{209d}$ is conjugate to $\operatorname{H}_{209d}$ in $\operatorname{GL}(2, \ZZ / 16 \ZZ)$. Let $E/\QQ$ be an elliptic curve such that the image of the $2$-adic Galois representation attached to $E$ is conjugate to $\operatorname{H}_{209d}$. By Lemma \ref{group lifting}, the image of the mod-$64$ Galois representation attached to $E$ is conjugate to
        $$\hat{H} = \left\langle \begin{bmatrix} 1 & 2 \\ 14 & 5 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 12 & 5 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 7 \end{bmatrix},\begin{bmatrix} 17 & 0 \\ 0 & 1 \\ \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \\ \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \\ \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \\ \end{bmatrix} \right\rangle$$
    where $\left\langle \begin{bmatrix} 17 & 0 \\ 0 & 1 \\ \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \\ \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \\ \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \\ \end{bmatrix} \right\rangle$ is the kernel of the reduction by $16$ map from $\operatorname{GL}(2, \ZZ / 64 \ZZ)$ to $\operatorname{GL}(2, \ZZ / 16 \ZZ)$. Moreover, $E$ has full two-torsion defined over $\QQ$. Let $P_{2}$ and $Q_{2}$ be points on $E$ of order $2$. Then $P_{2}$, $Q_{2}$, and $P_{2}+Q_{2}$ generate the non-trivial, finite, cyclic, $\QQ$-rational subgroups of $E$. We compute the $2$-adic Galois representations attached to $E / \left\langle Q_{2} \right\rangle$, $E / \left\langle P_{2} \right\rangle$, and $E / \left\langle P_{2} + Q_{2} \right\rangle$.
    
    \begin{itemize}
        \item $E / \left\langle Q_{2} \right\rangle$
        
        
    By Corollary \ref{2-adic image determination corollary}, the image of the mod-$32$ Galois representation attached to $E / \left\langle Q_{2} \right\rangle$ is conjugate to
    $$H' = \left\langle \begin{bmatrix} 1 & 1 \\ 28 & 5 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 24 & 5 \end{bmatrix}, \begin{bmatrix} 3 & 0 \\ 0 & 7 \end{bmatrix},\begin{bmatrix} 17 & 0 \\ 0 & 1 \\ \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \\ \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \\ \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 32 & 1 \\ \end{bmatrix} \right\rangle.$$
    Note that $H'$ is not conjugate to the transpose of $H'$ in $\operatorname{GL}(2,\ZZ / 32 \ZZ)$. Looking up the transpose of $H'$ in the RZB database, we see that the transpose of $H'$ is conjugate to $\operatorname{H}_{241g}$. The level of $\operatorname{H}_{241g}$ is equal to $32$.
    
    \item $E / \left\langle P_{2} \right\rangle$
    
    By Corollary \ref{2-adic image determination corollary}, the image of the mod-$32$ Galois representation attached to $E$ is conjugate to
    $$H' = \left\langle
    \begin{bmatrix} 5 & 7 \\ 4 & 1 \end{bmatrix},
    \begin{bmatrix} 5 & 6 \\ 0 & 3 \end{bmatrix},
    \begin{bmatrix} 7 & 0 \\ 0 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}
    \right\rangle.$$
    Note that $H'$ is not conjugate to the transpose of $H'$ in $\operatorname{GL}(2, \ZZ / 32 \ZZ)$. Searching for the transpose of $H'$ in the RZB database, we see that the transpose of $H'$ is conjugate to $\operatorname{H}_{241f}$. The level of $\operatorname{H}_{241f}$ is equal to $32$.
    
    \item $E / \left\langle P_{2}+Q_{2} \right\rangle$
    
    By Corollary \ref{2-adic image determination corollary}, the image of the mod-$32$ Galois representation attached to $E/\left\langle P_{2}+Q_{2} \right\rangle$ is conjugate to
    $$H' = \left\langle
    \begin{bmatrix} -13 & -8 \\ 28 & 19 \end{bmatrix},
    \begin{bmatrix} -9 & -7 \\ 24 & 17 \end{bmatrix},
    \begin{bmatrix} 3 & -2 \\ 0 & 7 \end{bmatrix},
    \begin{bmatrix} 17 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & -8 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} -15 & -8 \\ 32 & 17 \end{bmatrix}
    \right\rangle.$$
    Searching for the transpose of $H'$ in the RZB database, we see that the transpose of $H'$ is conjugate to $\operatorname{H}_{222d}$. The level of $\operatorname{H}_{222d}$ is equal to $16$.
    
    \end{itemize}
    
    
    \item $\operatorname{H}_{214a} = \left\langle \begin{bmatrix} 3 & 6 \\ 6 & 11 \end{bmatrix}, \begin{bmatrix} 1 & 2 \\ 14 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 6 \\ 2 & 1 \end{bmatrix} \right\rangle \subseteq \operatorname{GL}(2, \ZZ / 16 \ZZ)$
    
    Note that the transpose of $\operatorname{H}_{214a}$ is conjugate to $\operatorname{H}_{214a}$ in $\operatorname{GL}(2, \ZZ / 16 \ZZ)$. Let $E/\QQ$ be an elliptic curve such that the image of the $2$-adic Galois representation attached to $E$ is conjugate to $\operatorname{H}_{214a}$. By Lemma \ref{group lifting}, the image of the mod-$64$ Galois representation attached to $E$ is conjugate to
        $$\hat{H} = \left\langle \begin{bmatrix} 3 & 6 \\ 6 & 11 \end{bmatrix}, \begin{bmatrix} 1 & 2 \\ 14 & 7 \end{bmatrix}, \begin{bmatrix} 1 & 6 \\ 2 & 1 \end{bmatrix}, \begin{bmatrix} 17 & 0 \\ 0 & 1 \\ \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \\ \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \\ \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \\ \end{bmatrix} \right\rangle$$
    where $\left\langle \begin{bmatrix} 17 & 0 \\ 0 & 1 \\ \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \\ \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \\ \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \\ \end{bmatrix} \right\rangle$ is the kernel of the reduction by $16$ map from $\operatorname{GL}(2, \ZZ / 64 \ZZ)$ to $\operatorname{GL}(2, \ZZ / 16 \ZZ)$. Moreover, $E$ has full two-torsion defined over $\QQ$. Let $P_{2}$ and $Q_{2}$ be points on $E$ of order $2$. Then $P_{2}$, $Q_{2}$, and $P_{2}+Q_{2}$ generate the non-trivial, finite, cyclic, $\QQ$-rational subgroups of $E$. We compute the $2$-adic Galois representations attached to $E / \left\langle Q_{2} \right\rangle$, $E / \left\langle P_{2} \right\rangle$, and $E / \left\langle P_{2} + Q_{2} \right\rangle$.
    
    \begin{itemize}
        \item $E / \left\langle Q_{2} \right\rangle$
        
        By Lemma \ref{2-adic image determination corollary}, the image of the mod-$32$ Galois representation attached to $E / \left\langle Q_{2} \right\rangle$ is conjugate to
        $$H' = \left\langle
        \begin{bmatrix} 3 & 3 \\ 12 & 11 \end{bmatrix},
        \begin{bmatrix} 1 & 1 \\ 28 & 7 \end{bmatrix},
        \begin{bmatrix} 1 & 3 \\ 4 & 1 \end{bmatrix},
        \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0  \\ 32 & 1 \end{bmatrix}
        \right\rangle.$$
        Searching for the transpose of $H'$ in the RZB database, we see that the image of the $2$-adic Galois representation attached to $E / \left\langle Q_{2} \right\rangle$ is conjugate to $\operatorname{H}_{226a}$. Note that the level of $\operatorname{H}_{226a}$ is equal to $16$.
        
        \item $E / \left\langle P_{2} \right\rangle$
        
        By Lemma \ref{2-adic image determination corollary}, the image of the mod-$32$ Galois representation attached to $E / \left\langle P_{2} \right\rangle$ is conjugate to
        $$H' = \left\langle
        \begin{bmatrix} 11 & 3 \\ 12 & 3  \end{bmatrix},
        \begin{bmatrix} 7 & 7 \\ 4 & 1  \end{bmatrix},
        \begin{bmatrix} 1 & 1 \\ 12 & 1  \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17  \end{bmatrix},
        \begin{bmatrix} 17 & 0 \\ 0 & 1  \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 32 & 1  \end{bmatrix},
        \begin{bmatrix} 1 & 8 \\ 0 & 1  \end{bmatrix}
        \right\rangle$$
        Searching for the transpose of $H'$ in the RZB database, we see that the image of the $2$-adic Galois representation attached to $E$ is conjugate to $\operatorname{H}_{226b}$. The level of $\operatorname{H}_{226b}$ is equal to $16$.
        
        \item $E / \left\langle P_{2} + Q_{2} \right\rangle$
        By Lemma \ref{2-adic image determination corollary}, the image of the mod-$32$ Galois representation attached to $E / \left\langle P_{2}+Q_{2} \right\rangle$ is conjugate to
        $$H' =
        \left\langle
        \begin{bmatrix} -3 & -4 \\ 12 & 17 \end{bmatrix},
        \begin{bmatrix} -13 & -9 \\ 28 & 21 \end{bmatrix},
        \begin{bmatrix} -1 & 2 \\ 4 & 3 \end{bmatrix},
        \begin{bmatrix} 17 & 8 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & -8 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} -15 & -8 \\ 32 & 17 \end{bmatrix}
        \right\rangle.$$
        Searching for the transpose of $H'$ in the RZB database, we see that the transpose of $H'$ is conjugate to $\operatorname{H}_{231d}$. Note that the level of $\operatorname{H}_{231d}$ is equal to $16$.
        
    \end{itemize}
    
    \item $\operatorname{H}_{214c} = \left\langle
    \begin{bmatrix} 3 & 12 \\ 0 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 4 \\ 0 & 15 \end{bmatrix},
    \begin{bmatrix} 1 & 2 \\ 2 & 9 \end{bmatrix}
    \right\rangle \subseteq \operatorname{GL}(2, \ZZ / 16 \ZZ)$
    
    Note that the transpose of $\operatorname{H}_{214c}$ is conjugate to $\operatorname{H}_{214c}$. Let $E/\QQ$ be an elliptic curve such that the image of the $2$-adic Galois representation attached to $E$ is conjugate to $\operatorname{H}_{214c}$. By Lemma \ref{group lifting}, the image of the mod-$64$ Galois representation attached to $E$ is conjugate to
    $$\hat{H} = \left\langle
    \begin{bmatrix} 3 & 12 \\ 0 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 4 \\ 0 & 15 \end{bmatrix},
    \begin{bmatrix} 1 & 2 \\ 2 & 9 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix}
    \right\rangle$$
    where $\left\langle\begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix}\right\rangle$ is the kernel of the reduction by $16$ map from $\operatorname{GL}(2, \ZZ / 64 \ZZ)$ to $\operatorname{GL}(2, \ZZ / 16 \ZZ)$. Moreover, $E$ has full two-torsion defined over $\QQ$. Let $P_{2}$ and $Q_{2}$ be points on $E$ of order $2$. Then $P_{2}$, $Q_{2}$, and $P_{2}+Q_{2}$ generate the non-trivial, finite, cyclic, $\QQ$-rational subgroups of $E$. We compute the $2$-adic Galois representations attached to $E / \left\langle Q_{2} \right\rangle$, $E / \left\langle P_{2} \right\rangle$, and $E / \left\langle P_{2} + Q_{2} \right\rangle$.
    
    \begin{itemize}
        \item $E / \left\langle Q_{2} \right\rangle$
        
        By Corollary \ref{2-adic image determination corollary}, the image of the mod-$32$ Galois representation attached to $E / \left\langle Q_{2} \right\rangle$ is conjugate to
        $$H' = \left\langle
        \begin{bmatrix} 3 & 6 \\ 0 & 3 \end{bmatrix},
        \begin{bmatrix} 1 & 2 \\ 0 & 15 \end{bmatrix},
        \begin{bmatrix} 1 & 1 \\ 4 & 9 \end{bmatrix},
        \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}
        \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
        \right\rangle.$$
        Searching the RZB database for the transpose of $H'$, we see that the transpose of $H'$ is conjugate to $\operatorname{H}_{226f}$. Note that the level of $\operatorname{H}_{226f}$ is equal to $16$.
        
        \item $E / \left\langle P_{2} \right\rangle$
        
        By Corollary \ref{2-adic image determination corollary}, the image of the mod-$32$ Galois representation attached to $E / \left\langle P_{2} \right\rangle$ is conjugate to
        $$H' = 
        \left\langle
        \begin{bmatrix} 3 & 0 \\ 24 & 3 \end{bmatrix},
        \begin{bmatrix} 15 & 0 \\ 8 & 1 \end{bmatrix},
        \begin{bmatrix} 9 & 1 \\ 4 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
        \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix},
        \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix}
        \right\rangle.$$
        Searching the RZB database for the transpose of $H'$, we see that the transpose of $H'$ is conjugate to $\operatorname{H}_{226g}$. The level of $\operatorname{H}_{226g}$ is equal to $16$.
    
    \item $E / \left\langle P_{2} + Q_{2} \right\rangle$
    
    By Corollary \ref{2-adic image determination corollary}, the image of the mod-$32$ Galois representation attached to $E / \left\langle P_{2}+Q_{2} \right\rangle$ is conjugate to
    $$H' = \left\langle
    \begin{bmatrix} 3 & 6 \\ 0 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & -5 \\ 0 & 15 \end{bmatrix},
    \begin{bmatrix} -1 & -4 \\ 4 & 11 \end{bmatrix},
    \begin{bmatrix} 17 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & -8 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} -15 & -8 \\ 32 & 17 \end{bmatrix}
    \right\rangle.$$
    Searching the RZB database for the transpose of $H'$, we see that the transpose of $H'$ is conjugate to $\operatorname{H}_{231b}$. Note that the level of $\operatorname{H}_{231b}$ is equal to $16$.
    \end{itemize}
    
\end{enumerate}

\newpage

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.5}
\scalebox{0.3}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline

Isogeny Graph & Isogeny-Torsion Graph & $E_{1}$ & $E_{2}$ & $E_{3}$ & $E_{4}$ & $E_{5}$ & $E_{6}$ & Example Isogeny Class \\
\hline
\multirow{81}*{\includegraphics[scale=0.13]{T6 Graph.png}} &

\multirow{5}*{$([2,4],[8],[4],[2,2],[2],[2])$} & $\operatorname{H}_{98e}$ & $\operatorname{H}_{102p}$ & $\operatorname{H}_{120d}$ & $\operatorname{H}_{101d}$ & $\operatorname{H}_{122c}$ & $\operatorname{H}_{85l}$ & \texttt{21.a} \\
\cline{3-9}
& & $\operatorname{H}_{188c}$ & $\operatorname{H}_{230e}$ & $\operatorname{H}_{236b}$ & $\operatorname{H}_{200b}$ & $\operatorname{H}_{202g}$ & $\operatorname{H}_{217c}$ & \texttt{42.a} \\
\cline{3-9}
& & $\operatorname{H}_{200a}$ & $\operatorname{H}_{202h}$ & $\operatorname{H}_{217b}$ & $\operatorname{H}_{188d}$ & $\operatorname{H}_{236h}$ & $\operatorname{H}_{230b}$ & \texttt{336.d} \\
\cline{3-9}
& & $\operatorname{H}_{204h}$ & $\operatorname{H}_{197h}$ & $\operatorname{H}_{234b}$ & $\operatorname{H}_{190d}$ & $\operatorname{H}_{219g}$ & $\operatorname{H}_{228h}$ & \texttt{48.a} \\
\cline{3-9}
& & $\operatorname{H}_{181e}$ & $\operatorname{H}_{223d}$ & $\operatorname{H}_{229g}$ & $\operatorname{H}_{203f}$ & $\operatorname{H}_{233a}$ & $\operatorname{H}_{199f}$ & \texttt{102.c} \\
\cline{2-9}

& \multirow{8}*{$([2,4],[4],[4],[2,2],[2],[2])$} & $\operatorname{H}_{203e}$ & $\operatorname{H}_{233b}$ & $\operatorname{H}_{199e}$ & $\operatorname{H}_{181f}$ & $\operatorname{H}_{223h}$ & $\operatorname{H}_{229c}$ & \texttt{816.b} \\
\cline{3-9}
& & $\operatorname{H}_{190c}$ & $\operatorname{H}_{219c}$ & $\operatorname{H}_{228b}$ & $\operatorname{H}_{204f}$ & $\operatorname{H}_{234a}$ & $\operatorname{H}_{197g}$ & \texttt{24.a} \\
\cline{3-9}
& & $\operatorname{H}_{62a}$ & $\operatorname{H}_{78j}$ & $\operatorname{H}_{75j}$ & $\operatorname{H}_{100h}$ & $\operatorname{H}_{117k}$ & $\operatorname{H}_{117k}$ & \texttt{3696.e} \\
\cline{3-9}
& & $\operatorname{H}_{99g}$ & $\operatorname{H}_{119d}$ & $\operatorname{H}_{84k}$ & $\operatorname{H}_{87d}$ & $\operatorname{H}_{121c}$ & $\operatorname{H}_{86j}$ & \texttt{240.c} \\
\cline{3-9}
& & $\operatorname{H}_{100e}$ & $\operatorname{H}_{117d}$ & $\operatorname{H}_{117d}$ & $\operatorname{H}_{62b}$ & $\operatorname{H}_{78i}$ & $\operatorname{H}_{75i}$ & \texttt{1848.g} \\
\cline{3-9}
& & $\operatorname{H}_{87c}$ & $\operatorname{H}_{121d}$ & $\operatorname{H}_{86l}$ & $\operatorname{H}_{99h}$ & $\operatorname{H}_{119b}$ & $\operatorname{H}_{84l}$ & \texttt{120.b} \\
\cline{3-9}
& & $\operatorname{H}_{101b}$ & $\operatorname{H}_{85k}$ & $\operatorname{H}_{122d}$ & $\operatorname{H}_{98h}$ & $\operatorname{H}_{120b}$ & $\operatorname{H}_{102o}$ & \texttt{210.c} \\
\cline{3-9}
& & $\operatorname{H}_{25n}$ & $\operatorname{H}_{36n}$ & $\operatorname{H}_{36n}$ & $\operatorname{H}_{25h}$ & $\operatorname{H}_{36l}$ & $\operatorname{H}_{36l}$ & \texttt{231.a} \\
\cline{2-9}

& \multirow{24}*{$([2,2],[4],[2],[2,2],[2],[2])$} & $\operatorname{H}_{25i}$ & $\operatorname{H}_{36h}$ & $\operatorname{H}_{36f}$ & $\operatorname{H}_{25l}$ & $\operatorname{H}_{36m}$ & $\operatorname{H}_{36m}$ & \texttt{1287.e} \\
\cline{3-9}
& & $\operatorname{H}_{62e}$ & $\operatorname{H}_{78g}$ & $\operatorname{H}_{75f}$ & $\operatorname{H}_{100j}$ & $\operatorname{H}_{117l}$ & $\operatorname{H}_{117l}$ & \texttt{14784.ci} \\
\cline{3-9}
& & $\operatorname{H}_{62f}$ & $\operatorname{H}_{75g}$ & $\operatorname{H}_{78h}$ & $\operatorname{H}_{100i}$ & $\operatorname{H}_{117c}$ & $\operatorname{H}_{117c}$ & \texttt{14784.z} \\
\cline{3-9}
& & $\operatorname{H}_{87l}$ & $\operatorname{H}_{86o}$ & $\operatorname{H}_{121e}$ & $\operatorname{H}_{99n}$ & $\operatorname{H}_{119l}$ & $\operatorname{H}_{84c}$ & \texttt{1200.o} \\
\cline{3-9}
& & $\operatorname{H}_{98n}$ & $\operatorname{H}_{120f}$ & $\operatorname{H}_{102l}$ & $\operatorname{H}_{101o}$ & $\operatorname{H}_{122k}$ & $\operatorname{H}_{85d}$ & \texttt{147.a} \\
\cline{3-9}
& & $\operatorname{H}_{101l}$ & $\operatorname{H}_{85p}$ & $\operatorname{H}_{122e}$ & $\operatorname{H}_{98p}$ & $\operatorname{H}_{102h}$ & $\operatorname{H}_{120l}$ & \texttt{1008.l} \\
\cline{3-9}
& & $\operatorname{H}_{99m}$ & $\operatorname{H}_{84p}$ & $\operatorname{H}_{119f}$ & $\operatorname{H}_{87p}$ & $\operatorname{H}_{121l}$ & $\operatorname{H}_{86d}$ & \texttt{2880.bb} \\
\cline{3-9}
& & $\operatorname{H}_{100a}$ & $\operatorname{H}_{117b}$ & $\operatorname{H}_{117i}$ & $\operatorname{H}_{62g}$ & $\operatorname{H}_{78d}$ & $\operatorname{H}_{75d}$ & \texttt{142296.bm} \\
\cline{3-9}
& & $\operatorname{H}_{98m}$ & $\operatorname{H}_{102k}$ & $\operatorname{H}_{120h}$ & $\operatorname{H}_{101m}$ & $\operatorname{H}_{122l}$ & $\operatorname{H}_{85c}$ & \texttt{2352.v} \\
\cline{3-9}
& & $\operatorname{H}_{99p}$ & $\operatorname{H}_{119h}$ & $\operatorname{H}_{84o}$ & $\operatorname{H}_{87m}$ & $\operatorname{H}_{121k}$ & $\operatorname{H}_{86b}$ & \texttt{2880.x} \\
\cline{3-9}
& & $\operatorname{H}_{101j}$ & $\operatorname{H}_{122f}$ & $\operatorname{H}_{85m}$ & $\operatorname{H}_{98o}$ & $\operatorname{H}_{102g}$ & $\operatorname{H}_{120j}$ & \texttt{63.a} \\
\cline{3-9}
& & $\operatorname{H}_{87k}$ & $\operatorname{H}_{121f}$ & $\operatorname{H}_{86n}$ & $\operatorname{H}_{99o}$ & $\operatorname{H}_{119j}$ & $\operatorname{H}_{84d}$ & \texttt{600.c} \\
\cline{3-9}
& & $\operatorname{H}_{203b}$ & $\operatorname{H}_{199h}$ & $\operatorname{H}_{233c}$ & $\operatorname{H}_{181h}$ & $\operatorname{H}_{223c}$ & $\operatorname{H}_{229d}$ & \texttt{3264.m} \\
\cline{3-9}
& & $\operatorname{H}_{190a}$ & $\operatorname{H}_{219a}$ & $\operatorname{H}_{228e}$ & $\operatorname{H}_{204d}$ & $\operatorname{H}_{234g}$ & $\operatorname{H}_{197c}$ & \texttt{144.b} \\
\cline{3-9}
& & $\operatorname{H}_{181b}$ & $\operatorname{H}_{229e}$ & $\operatorname{H}_{223f}$ & $\operatorname{H}_{203c}$ & $\operatorname{H}_{233f}$ & $\operatorname{H}_{199a}$ & \texttt{13872.bm} \\
\cline{3-9}
& & $\operatorname{H}_{181a}$ & $\operatorname{H}_{223b}$ & $\operatorname{H}_{229b}$ & $\operatorname{H}_{203d}$ & $\operatorname{H}_{233e}$ & $\operatorname{H}_{199b}$ & \texttt{1734.j} \\
\cline{3-9}
& & $\operatorname{H}_{200d}$ & $\operatorname{H}_{217a}$ & $\operatorname{H}_{202f}$ & $\operatorname{H}_{188g}$ & $\operatorname{H}_{236c}$ & $\operatorname{H}_{230a}$ & \texttt{1344.q} \\
\cline{3-9}
& & $\operatorname{H}_{190b}$ & $\operatorname{H}_{228a}$ & $\operatorname{H}_{219f}$ & $\operatorname{H}_{204a}$ & $\operatorname{H}_{234f}$ & $\operatorname{H}_{197d}$ & \texttt{72.a} \\
\cline{3-9}
& & $\operatorname{H}_{200c}$ & $\operatorname{H}_{202e}$ & $\operatorname{H}_{217d}$ & $\operatorname{H}_{188h}$ & $\operatorname{H}_{236f}$ & $\operatorname{H}_{230f}$ & \texttt{1344.i} \\
\cline{3-9}
& & $\operatorname{H}_{188b}$ & $\operatorname{H}_{230h}$ & $\operatorname{H}_{236g}$ & $\operatorname{H}_{200e}$ & $\operatorname{H}_{202c}$ & $\operatorname{H}_{217h}$ & \texttt{294.g} \\
\cline{3-9}
& & $\operatorname{H}_{203a}$ & $\operatorname{H}_{233d}$ & $\operatorname{H}_{199g}$ & $\operatorname{H}_{181g}$ & $\operatorname{H}_{223e}$ & $\operatorname{H}_{229h}$ & \texttt{3264.bc} \\
\cline{3-9}
& & $\operatorname{H}_{188a}$ & $\operatorname{H}_{236a}$ & $\operatorname{H}_{230d}$ & $\operatorname{H}_{200f}$ & $\operatorname{H}_{202d}$ & $\operatorname{H}_{217f}$ & \texttt{2352.l} \\
\cline{3-9}
& & $\operatorname{H}_{204c}$ & $\operatorname{H}_{234c}$ & $\operatorname{H}_{197e}$ & $\operatorname{H}_{190g}$ & $\operatorname{H}_{219d}$ & $\operatorname{H}_{228c}$ & \texttt{192.b} \\
\cline{3-9}
& & $\operatorname{H}_{204b}$ & $\operatorname{H}_{197f}$ & $\operatorname{H}_{234d}$ & $\operatorname{H}_{190h}$ & $\operatorname{H}_{219h}$ & $\operatorname{H}_{228g}$ & \texttt{192.d} \\
\cline{2-9}

& \multirow{44}*{$([2,2],[2],[2],[2,2],[2],[2])$} & $\operatorname{H}_{25g}$ & $\operatorname{H}_{36i}$ & $\operatorname{H}_{36i}$ & $\operatorname{H}_{25e}$ & $\operatorname{H}_{36k}$ & $\operatorname{H}_{36k}$ & \texttt{6720.b} \\
\cline{3-9}
& & $\operatorname{H}_{25c}$ & $\operatorname{H}_{36j}$ & $\operatorname{H}_{36j}$ & $\operatorname{H}_{25f}$ & $\operatorname{H}_{36e}$ & $\operatorname{H}_{36c}$ & \texttt{990.c} \\
\cline{3-9}
& & $\operatorname{H}_{25m}$ & $\operatorname{H}_{36g}$ & $\operatorname{H}_{36g}$ & $\operatorname{H}_{25m}$ & $\operatorname{H}_{36g}$ & $\operatorname{H}_{36g}$ & \texttt{53361.q} \\
\cline{3-9}
& & $\operatorname{H}_{62}$ & $\operatorname{H}_{78}$ & $\operatorname{H}_{75}$ & $\operatorname{H}_{100}$ & $\operatorname{H}_{117}$ & $\operatorname{H}_{117}$ & \texttt{5544.s} \\
\cline{3-9}
& & $\operatorname{H}_{25d}$ & $\operatorname{H}_{36d}$ & $\operatorname{H}_{36d}$ & $\operatorname{H}_{25d}$ & $\operatorname{H}_{36d}$ & $\operatorname{H}_{36d}$ & \texttt{54450.bw} \\
\cline{3-9}
& & $\operatorname{H}_{25b}$ & $\operatorname{H}_{36q}$ & $\operatorname{H}_{36p}$ & $\operatorname{H}_{25j}$ & $\operatorname{H}_{36s}$ & $\operatorname{H}_{36t}$ & \texttt{990.b} \\
\cline{3-9}
& & $\operatorname{H}_{98}$ & $\operatorname{H}_{102}$ & $\operatorname{H}_{120}$ & $\operatorname{H}_{101}$ & $\operatorname{H}_{122}$ & $\operatorname{H}_{85}$ & \texttt{525.d} \\
\cline{3-9}
& & $\operatorname{H}_{87}$ & $\operatorname{H}_{121}$ & $\operatorname{H}_{86}$ & $\operatorname{H}_{99}$ & $\operatorname{H}_{119}$ & $\operatorname{H}_{84}$ & \texttt{1989.e} \\
\cline{3-9}
& & $\operatorname{H}_{25a}$ & $\operatorname{H}_{36r}$ & $\operatorname{H}_{36o}$ & $\operatorname{H}_{25k}$ & $\operatorname{H}_{36b}$ & $\operatorname{H}_{36a}$ & \texttt{693.d} \\
\cline{3-9}
& & $\operatorname{H}_{25}$ & $\operatorname{H}_{36}$ & $\operatorname{H}_{36}$ & $\operatorname{H}_{25}$ & $\operatorname{H}_{36}$ & $\operatorname{H}_{36}$ & \texttt{3465.l} \\
\cline{3-9}
& & $\operatorname{H}_{87i}$ & $\operatorname{H}_{121j}$ & $\operatorname{H}_{86a}$ & $\operatorname{H}_{99j}$ & $\operatorname{H}_{119e}$ & $\operatorname{H}_{84n}$ & \texttt{720.d} \\
\cline{3-9}
& & $\operatorname{H}_{87b}$ & $\operatorname{H}_{121p}$ & $\operatorname{H}_{86e}$ & $\operatorname{H}_{99c}$ & $\operatorname{H}_{119p}$ & $\operatorname{H}_{84e}$ & \texttt{1800.n} \\
\cline{3-9}
& & $\operatorname{H}_{98d}$ & $\operatorname{H}_{120n}$ & $\operatorname{H}_{102a}$ & $\operatorname{H}_{101a}$ & $\operatorname{H}_{85e}$ & $\operatorname{H}_{122m}$ & \texttt{22050.df} \\
\cline{3-9}
& & $\operatorname{H}_{62h}$ & $\operatorname{H}_{78b}$ & $\operatorname{H}_{75h}$ & $\operatorname{H}_{100f}$ & $\operatorname{H}_{117h}$ & $\operatorname{H}_{117m}$ & \texttt{25872.cs} \\
\cline{3-9}
& & $\operatorname{H}_{98g}$ & $\operatorname{H}_{102c}$ & $\operatorname{H}_{120o}$ & $\operatorname{H}_{101f}$ & $\operatorname{H}_{122n}$ & $\operatorname{H}_{85g}$ & \texttt{7056.p} \\
\cline{3-9}
& & $\operatorname{H}_{87g}$ & $\operatorname{H}_{121o}$ & $\operatorname{H}_{86f}$ & $\operatorname{H}_{99f}$ & $\operatorname{H}_{119o}$ & $\operatorname{H}_{84g}$ & \texttt{14400.db} \\
\cline{3-9}
& & $\operatorname{H}_{98f}$ & $\operatorname{H}_{102d}$ & $\operatorname{H}_{120m}$ & $\operatorname{H}_{101h}$ & $\operatorname{H}_{122o}$ & $\operatorname{H}_{85h}$ & \texttt{441.f} \\
\cline{3-9}
& & $\operatorname{H}_{98b}$ & $\operatorname{H}_{102m}$ & $\operatorname{H}_{120c}$ & $\operatorname{H}_{101g}$ & $\operatorname{H}_{122b}$ & $\operatorname{H}_{85j}$ & \texttt{1344.g} \\
\cline{3-9}
& & $\operatorname{H}_{87a}$ & $\operatorname{H}_{121m}$ & $\operatorname{H}_{86g}$ & $\operatorname{H}_{99d}$ & $\operatorname{H}_{119n}$ & $\operatorname{H}_{84f}$ & \texttt{3600.t} \\
\cline{3-9}
& & $\operatorname{H}_{62j}$ & $\operatorname{H}_{78c}$ & $\operatorname{H}_{75b}$ & $\operatorname{H}_{100d}$ & $\operatorname{H}_{117a}$ & $\operatorname{H}_{117j}$ & $y^{2} = x^{3} + x^{2} - 87851969x - 102107357409$ \\
\cline{3-9}
& & $\operatorname{H}_{87f}$ & $\operatorname{H}_{121a}$ & $\operatorname{H}_{86k}$ & $\operatorname{H}_{99a}$ & $\operatorname{H}_{119c}$ & $\operatorname{H}_{84j}$ & \texttt{960.j} \\
\cline{3-9}
& & $\operatorname{H}_{87n}$ & $\operatorname{H}_{121h}$ & $\operatorname{H}_{86p}$ & $\operatorname{H}_{99l}$ & $\operatorname{H}_{119i}$ & $\operatorname{H}_{84a}$ & \texttt{4800.cd} \\
\cline{3-9}
& & $\operatorname{H}_{62c}$ & $\operatorname{H}_{78e}$ & $\operatorname{H}_{75a}$ & $\operatorname{H}_{100c}$ & $\operatorname{H}_{117n}$ & $\operatorname{H}_{117o}$ & \texttt{8280.g} \\
\cline{3-9}
& & $\operatorname{H}_{98j}$ & $\operatorname{H}_{120e}$ & $\operatorname{H}_{102j}$ & $\operatorname{H}_{101i}$ & $\operatorname{H}_{85b}$ & $\operatorname{H}_{122j}$ & \texttt{1470.q} \\
\cline{3-9}
& & $\operatorname{H}_{181}$ & $\operatorname{H}_{223}$ & $\operatorname{H}_{229}$ & $\operatorname{H}_{203}$ & $\operatorname{H}_{233}$ & $\operatorname{H}_{199}$ & \texttt{306.b} \\
\cline{3-9}
& & $\operatorname{H}_{190}$ & $\operatorname{H}_{219}$ & $\operatorname{H}_{228}$ & $\operatorname{H}_{204}$ & $\operatorname{H}_{234}$ & $\operatorname{H}_{197}$ & \texttt{600.h} \\
\cline{3-9}
& & $\operatorname{H}_{87j}$ & $\operatorname{H}_{121i}$ & $\operatorname{H}_{86c}$ & $\operatorname{H}_{99i}$ & $\operatorname{H}_{119g}$ & $\operatorname{H}_{84m}$ & \texttt{360.b} \\
\cline{3-9}
& & $\operatorname{H}_{98i}$ & $\operatorname{H}_{102e}$ & $\operatorname{H}_{120i}$ & $\operatorname{H}_{101n}$ & $\operatorname{H}_{122g}$ & $\operatorname{H}_{85o}$ & \texttt{4032.h} \\
\cline{3-9}
& & $\operatorname{H}_{87o}$ & $\operatorname{H}_{121g}$ & $\operatorname{H}_{86m}$ & $\operatorname{H}_{99k}$ & $\operatorname{H}_{119k}$ & $\operatorname{H}_{84b}$ & \texttt{4800.r} \\
\cline{3-9}
& & $\operatorname{H}_{62d}$ & $\operatorname{H}_{78f}$ & $\operatorname{H}_{75c}$ & $\operatorname{H}_{100b}$ & $\operatorname{H}_{117f}$ & $\operatorname{H}_{117e}$ & \texttt{16560.h} \\
\cline{3-9}
& & $\operatorname{H}_{98c}$ & $\operatorname{H}_{102n}$ & $\operatorname{H}_{120a}$ & $\operatorname{H}_{101e}$ & $\operatorname{H}_{122a}$ & $\operatorname{H}_{85i}$ & \texttt{1344.s} \\
\cline{3-9}
& & $\operatorname{H}_{98k}$ & $\operatorname{H}_{102i}$ & $\operatorname{H}_{120g}$ & $\operatorname{H}_{101k}$ & $\operatorname{H}_{122i}$ & $\operatorname{H}_{85a}$ & \texttt{5880.z} \\
\cline{3-9}
& & $\operatorname{H}_{98a}$ & $\operatorname{H}_{102b}$ & $\operatorname{H}_{120p}$ & $\operatorname{H}_{101c}$ & $\operatorname{H}_{122p}$ & $\operatorname{H}_{85f}$ & \texttt{28224.fk} \\
\cline{3-9}
& & $\operatorname{H}_{188}$ & $\operatorname{H}_{236}$ & $\operatorname{H}_{230}$ & $\operatorname{H}_{200}$ & $\operatorname{H}_{202}$ & $\operatorname{H}_{217}$ & \texttt{126.a} \\
\cline{3-9}
& & $\operatorname{H}_{87e}$ & $\operatorname{H}_{121b}$ & $\operatorname{H}_{86i}$ & $\operatorname{H}_{99b}$ & $\operatorname{H}_{119a}$ & $\operatorname{H}_{84i}$ & \texttt{960.c} \\
\cline{3-9}
& & $\operatorname{H}_{62i}$ & $\operatorname{H}_{78a}$ & $\operatorname{H}_{75e}$ & $\operatorname{H}_{100g}$ & $\operatorname{H}_{117p}$ & $\operatorname{H}_{117g}$ & \texttt{12936.m} \\
\cline{3-9}
& & $\operatorname{H}_{98l}$ & $\operatorname{H}_{120k}$ & $\operatorname{H}_{102f}$ & $\operatorname{H}_{101p}$ & $\operatorname{H}_{85n}$ & $\operatorname{H}_{122h}$ & \texttt{2070.b} \\
\cline{3-9}
& & $\operatorname{H}_{87h}$ & $\operatorname{H}_{121n}$ & $\operatorname{H}_{86h}$ & $\operatorname{H}_{99e}$ & $\operatorname{H}_{119m}$ & $\operatorname{H}_{84h}$ & \texttt{14400.cm} \\
\cline{3-9}
& & $\operatorname{H}_{181c}$ & $\operatorname{H}_{223a}$ & $\operatorname{H}_{229f}$ & $\operatorname{H}_{203g}$ & $\operatorname{H}_{233h}$ & $\operatorname{H}_{199c}$ & \texttt{55488.cr} \\
\cline{3-9}
& & $\operatorname{H}_{190e}$ & $\operatorname{H}_{219e}$ & $\operatorname{H}_{228d}$ & $\operatorname{H}_{204g}$ & $\operatorname{H}_{234h}$ & $\operatorname{H}_{197b}$ & \texttt{576.b} \\
\cline{3-9}
& & $\operatorname{H}_{181d}$ & $\operatorname{H}_{223g}$ & $\operatorname{H}_{229a}$ & $\operatorname{H}_{203h}$ & $\operatorname{H}_{233g}$ & $\operatorname{H}_{199d}$ & \texttt{55488.m} \\
\cline{3-9}
& & $\operatorname{H}_{188f}$ & $\operatorname{H}_{236d}$ & $\operatorname{H}_{230g}$ & $\operatorname{H}_{200g}$ & $\operatorname{H}_{202b}$ & $\operatorname{H}_{217g}$ & \texttt{9408.bw} \\
\cline{3-9}
& & $\operatorname{H}_{188e}$ & $\operatorname{H}_{236e}$ & $\operatorname{H}_{230c}$ & $\operatorname{H}_{200h}$ & $\operatorname{H}_{202a}$ & $\operatorname{H}_{217e}$ & \texttt{9408.n} \\
\cline{3-9}
& & $\operatorname{H}_{190f}$ & $\operatorname{H}_{219b}$ & $\operatorname{H}_{228f}$ & $\operatorname{H}_{204e}$ & $\operatorname{H}_{234e}$ & $\operatorname{H}_{197a}$ & \texttt{576.d} \\
\hline
\end{tabular}}
\caption{2-adic Images of $T_{6}$ Graphs}
\label{2-adic Images of T6 Graphs}
\end{table}
\end{center}

\newpage

\subsection{$2$-adic images of $T_{6}$ graphs not in LMFDB}

There is one example of a $2$-adic images of non-CM elliptic curves over $\QQ$ such that the isogeny graph is of $T_{6}$ type and the example isogeny class is not in the LMFDB.
$$\operatorname{H}_{62j} = \left\langle
\begin{bmatrix} 3 & 6 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 0 \\ 4 & 7 \end{bmatrix}
\right\rangle \subseteq \operatorname{GL}(2, \ZZ / 8 \ZZ)$$
Note that $\operatorname{H}_{62j}$ is conjugate to its transpose in $\operatorname{GL}(2, \ZZ / 8 \ZZ)$. Note that the reduction of $E$ modulo $2$ is the trivial subgroup of $\operatorname{GL}(2, \ZZ / 2 \ZZ)$. Thus, $E$ has full two-torsion defined over $\QQ$. We can say that $E[2] = \left\langle P_{2}, Q_{2} \right\rangle$ and both $P_{2}$ and $Q_{2}$ are points of order $2$ defined over $\QQ$. Note that the reduction of $\operatorname{H}_{62j}$ modulo $4$ is upper triangular. Hence, an elliptic curve $E/\QQ$ such that the image of the $2$-adic Galois representation attached to $E$ is conjugate to $\operatorname{H}_{62j}$ has a $4$-isogeny. In this form, $E[4] = \left\langle P_{4}, Q_{4} \right\rangle$ and $P_{4}$ generates a cyclic, $\QQ$-rational subgroup of $E$ of order $4$. We prefer to rearrange the generators of $E[2^{\infty}]$ so that the cyclic, $\QQ$-rational subgroup of $E$ of order $4$ is generated by $Q_{4}$. 

\begin{itemize}

\item $E / \left\langle P_{2} \right\rangle$

By Lemma \ref{group lifting}, the image of the mod-$64$ Galois representation attached to $E$ is conjugate to
$$\overline{H} = \left\langle
\begin{bmatrix} 3 & 6 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 0 \\ 4 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}
\right\rangle.$$
By Lemma \ref{2-adic determination}, the image of the mod-$32$ Galois representation attached to $E / \left\langle P_{2} \right\rangle$ is conjugate to
$$H' = \left\langle
\begin{bmatrix} 3 & 3 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 0 \\ 8 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
\right\rangle.$$
Note that
$$H' = \left\langle
\begin{bmatrix} 3 & 3 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 0 \\ 8 & 7 \end{bmatrix},
\begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
\begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
\right\rangle$$
the full lift of $\left\langle \begin{bmatrix} 3 & 3 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 0 \\ 8 & 7 \end{bmatrix} \right\rangle$ of level $16$ to level $32$ and
$$H' \neq \left\langle
\begin{bmatrix} 3 & 3 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 0 \\ 8 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}
\right\rangle$$
the full lift of $\left\langle \begin{bmatrix} 3 & 3 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 0 \\ 8 & 7 \end{bmatrix} \right\rangle$ of level $8$ to level $32$. Searching the RZB database for the transpose of the group $H'$, we see that the image of the $2$-adic Galois representation to $E / \left\langle P_{2} \right\rangle$ is conjugate to $\operatorname{H}_{78c}$.

\item $E / \left\langle P_{2} + Q_{2} \right\rangle$

We need to rewrite the generators of $E[2]$ as $E[2] = \left\langle P_{2}, P_{2}+Q_{2} \right\rangle$ and hence, the generators of $E[8]$ as $E[8] = \left\langle P_{8}, P_{8}+Q_{8} \right\rangle$. In this case,
$$H = \left\langle
\begin{bmatrix} 3 & 2 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & -2 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 3 & -4 \\ 4 & 11 \end{bmatrix}
\right\rangle.$$
By Lemma \ref{group lifting}, the image of the mod-$64$ Galois representation attached to $E$ is conjugate to
$$\overline{H} = \left\langle
\begin{bmatrix} 3 & 2 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & -2 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 3 & -4 \\ 4 & 11 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}
\right\rangle.$$
By Lemma \ref{2-adic determination}, the image of the mod-$32$ Galois representation attached to $E / \left\langle P_{2}+Q_{2} \right\rangle$ is conjugate to
$$H' = \left\langle
\begin{bmatrix} 3 & 1 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & -1 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 3 & -2 \\ 8 & 11 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
\right\rangle.$$
Note that
$$H' = \left\langle
\begin{bmatrix} 3 & 1 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & -1 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 3 & -2 \\ 8 & 11 \end{bmatrix},
\begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
\begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
\right\rangle$$
the full lift of $\left\langle \begin{bmatrix} 3 & 1 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & -1 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 3 & -2 \\ 8 & 11 \end{bmatrix} \right\rangle$ from level $8$ to level $32$. Moreover,
$H'$ is not conjugate to
$$\left\langle
\begin{bmatrix} 3 & 1 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & -1 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 3 & -2 \\ 8 & 11 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}
\right\rangle$$
the full lift of $\left\langle \begin{bmatrix} 3 & 1 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 3 & -1 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 3 & -2 \\ 8 & 11 \end{bmatrix} \right\rangle$ from level $8$ to level $32$. Searching the RZB database for the transpose of $H'$ in $\operatorname{GL}(2, \ZZ / 16 \ZZ)$, we see that it is conjugate to $\operatorname{H}_{75b}$.

\item $E / \left\langle Q_{2} \right\rangle$ 

We need to rewrite the image of the mod-$8$ Galois representation attached to $E$ as
$$H = \left\langle
\begin{bmatrix} 7 & 0 \\ 6 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 4 \\ 0 & 7 \end{bmatrix}
\right\rangle.$$
By Lemma \ref{group lifting}, the image of the mod-$64$ Galois representation attached to $E$ is conjugate to
$$\overline{H} = \left\langle
\begin{bmatrix} 7 & 0 \\ 6 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 4 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}
\right\rangle.$$
By Lemma \ref{2-adic determination}, the image of the mod-$32$ Galois representation attached to $E / \left\langle Q_{2} \right\rangle$ is conjugate to
$$H' = \left\langle
\begin{bmatrix} 7 & 0 \\ 12 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 2 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
\right\rangle.$$
Note that
$$H' \neq \left\langle
\begin{bmatrix} 7 & 0 \\ 12 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 2 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 4 & 1 \end{bmatrix}
\right\rangle \subseteq \operatorname{GL}(2, \ZZ / 8 \ZZ)$$
which is the full lift of $\left\langle \begin{bmatrix} 7 & 0 \\ 12 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 2 \\ 0 & 7 \end{bmatrix} \right\rangle \subseteq \operatorname{GL}(2, \ZZ / 8 \ZZ)$ to level $32$.
$$H' = \left\langle
\begin{bmatrix} 7 & 0 \\ 12 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 2 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}
\right\rangle$$
which is the full lift of $\left\langle \begin{bmatrix} 7 & 0 \\ 12 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 2 \\ 0 & 7 \end{bmatrix} \right\rangle \subseteq \operatorname{GL}(2, \ZZ / 16 \ZZ)$ to level $32$. In other words, $H'$ is a group of level $16$. Searching the RZB database for the transpose of $H'$ in $\operatorname{GL}(2, \ZZ / 16 \ZZ)$, we see that it is conjugate to $\operatorname{H}_{100d}$.

\item $E / \left\langle Q_{4} \right\rangle$

To use Lemma \ref{2-adic determination}, we need to rewrite the generators of $E[8]$ as $\left\langle Q_{8}, P_{8} \right\rangle$ and thus, $E[4] = \left\langle Q_{4}, P_{4} \right\rangle$. In this case, the image of the mod-$8$ Galois representation attached to $E$ is conjugate to
$$H = \left\langle
\begin{bmatrix} 7 & 0 \\ 6 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 4 \\ 0 & 7 \end{bmatrix}
\right\rangle.$$
By Lemma \ref{group lifting}, the image of the mod-$64$ Galois representation attached to $E$ is conjugate to
$$\overline{H} = \left\langle
\begin{bmatrix} 7 & 0 \\ 6 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 4 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}
\right\rangle.$$
By Lemma \ref{2-adic determination}, the image of the mod-$32$ Galois representation attached to $E / \left\langle Q_{4} \right\rangle$ is conjugate to
$$H' = \left\langle
\begin{bmatrix} 7 & 0 \\ 24 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 1 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
\right\rangle.$$
Note that
$$H' = \left\langle
\begin{bmatrix} 7 & 0 \\ 24 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 1 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
\begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
\right\rangle$$
the full lift of $\left\langle
\begin{bmatrix} 7 & 0 \\ 24 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 1 \\ 0 & 7 \end{bmatrix} \right\rangle$ from level $16$ to level $32$. Moreover,
$$H' \neq \left\langle
\begin{bmatrix} 7 & 0 \\ 24 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 1 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}
\right\rangle$$
the full lift of $\left\langle \begin{bmatrix} 7 & 0 \\ 24 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 1 \\ 0 & 7 \end{bmatrix} \right\rangle$ from level $8$ to level $32$. Searching the RZB database for the transpose of $H'$ in $\operatorname{GL}(2, \ZZ / 16 \ZZ)$, we see that the image of the $2$-adic Galois representation attached to $E / \left\langle Q_{4} \right\rangle$ is conjugate to $\operatorname{H}_{117a}$.

\item $E / \left\langle P_{2} + Q_{4} \right\rangle$

To use Lemma \ref{2-adic determination}, we need to rewrite the generators of $E[8]$ as $\left\langle P_{8}, P_{4} + Q_{8} \right\rangle$ and thus, $E[4] = \left\langle P_{4}, P_{2}+Q_{4} \right\rangle$. In this case, the image of the mod-$8$ Galois representation attached to $E$ is conjugate to
$$H = \left\langle
\begin{bmatrix} 3 & 0 \\ 6 & 7 \end{bmatrix},
\begin{bmatrix} 5 & 4 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 4 \\ 0 & 7 \end{bmatrix}
\right\rangle.$$
By Lemma \ref{group lifting}, the image of the mod-$64$ Galois representation attached to $E$ is conjugate to
$$\overline{H} = \left\langle
\begin{bmatrix} 3 & 0 \\ 6 & 7 \end{bmatrix},
\begin{bmatrix} 5 & 4 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 4 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}
\right\rangle.$$
By Lemma \ref{2-adic determination}, the image of the mod-$32$ Galois representation attached to $E / \left\langle P_{2} + Q_{4} \right\rangle$ is conjugate to
$$H' =\left\langle
\begin{bmatrix} 3 & 0 \\ 24 & 7 \end{bmatrix},
\begin{bmatrix} 5 & 1 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 1 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 2 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
\right\rangle.$$
Note that
$$H' =\left\langle
\begin{bmatrix} 3 & 0 \\ 24 & 7 \end{bmatrix},
\begin{bmatrix} 5 & 1 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 1 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
\begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
\right\rangle$$
the full lift of $\left\langle
\begin{bmatrix} 3 & 0 \\ 24 & 7 \end{bmatrix},
\begin{bmatrix} 5 & 1 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 1 \\ 0 & 7 \end{bmatrix}
\right\rangle$ from level $16$ to level $32$. Moreover,
$$H' \neq \left\langle
\begin{bmatrix} 3 & 0 \\ 24 & 7 \end{bmatrix},
\begin{bmatrix} 5 & 1 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 1 \\ 0 & 7 \end{bmatrix},
\begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
\begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
\begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}
\right\rangle$$
the full lift of $\left\langle
\begin{bmatrix} 3 & 0 \\ 24 & 7 \end{bmatrix},
\begin{bmatrix} 5 & 1 \\ 0 & 3 \end{bmatrix},
\begin{bmatrix} 5 & 0 \\ 0 & 5 \end{bmatrix},
\begin{bmatrix} 7 & 1 \\ 0 & 7 \end{bmatrix} \right\rangle$ from level $8$ to level $32$. Searching the RZB database for the transpose of $H'$ in $\operatorname{GL}(2, \ZZ / 16 \ZZ)$, we see that the image of the $2$-adic Galois representation attached to $E / \left\langle P_{2} + Q_{4} \right\rangle$ is conjugate to $\operatorname{H}_{117j}$.
\end{itemize}

\newpage

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.5}
\scalebox{0.5}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline

Isogeny Graph & Isogeny-Torsion Graph & $E_{1}$ & $E_{2}$ & $E_{3}$ & $E_{4}$ & $E_{5}$ & $E_{6}$ & $E_{7}$ & $E_{8}$ & Example Isogeny Class \\
\hline
\multirow{53}*{\includegraphics[scale=0.15]{T8 Graph.png}} 

& $([2,8],[8],[8],[2,4],[4],[2,2],[2],[2])$ & $\operatorname{H}_{193n}$ & $\operatorname{H}_{235l}$ & $\operatorname{H}_{235l}$ & $\operatorname{H}_{189d}$ & $\operatorname{H}_{207n}$ & $\operatorname{H}_{192i}$ & $\operatorname{H}_{211m}$ & $\operatorname{H}_{211m}$ & \texttt{210.e} \\
\cline{2-11}

& $([2,4],[8],[4],[2,4],[4],[2,2],[2],[2])$ & $\operatorname{H}_{194l}$ & $\operatorname{H}_{213i}$ & $\operatorname{H}_{227i}$ & $\operatorname{H}_{183i}$ & $\operatorname{H}_{205h}$ & $\operatorname{H}_{208a}$ & $\operatorname{H}_{243g}$ & $\operatorname{H}_{243g}$ & \texttt{1230.f} \\
\cline{2-11}

& $([2,4],[4],[4],[2,4],[8],[2,2],[2],[2])$ & $\operatorname{H}_{215c}$ & $\operatorname{H}_{240l}$ & $\operatorname{H}_{240l}$ & $\operatorname{H}_{187d}$ & $\operatorname{H}_{195l}$ & $\operatorname{H}_{185h}$ & $\operatorname{H}_{225g}$ & $\operatorname{H}_{212h}$ & \texttt{15.a} \\
\cline{2-11}

& \multirow{4}*{$([2,4],[4],[4],[2,4],[4],[2,2],[2],[2])$} & $\operatorname{H}_{96t}$ & $\operatorname{H}_{118l}$ & $\operatorname{H}_{118l}$ & $\operatorname{H}_{58i}$ & $\operatorname{H}_{92h}$ & $\operatorname{H}_{96o}$ & $\operatorname{H}_{118i}$ & $\operatorname{H}_{118i}$ & \texttt{195.a} \\
\cline{3-11}
& & $\operatorname{H}_{208c}$ & $\operatorname{H}_{243d}$ & $\operatorname{H}_{243d}$ & $\operatorname{H}_{183d}$ & $\operatorname{H}_{205i}$ & $\operatorname{H}_{194k}$ & $\operatorname{H}_{213h}$ & $\operatorname{H}_{227k}$ & \texttt{510.e} \\
\cline{3-11}
& & $\operatorname{H}_{185g}$ & $\operatorname{H}_{225h}$ & $\operatorname{H}_{212i}$ & $\operatorname{H}_{187k}$ & $\operatorname{H}_{195h}$ & $\operatorname{H}_{215l}$ & $\operatorname{H}_{240h}$ & $\operatorname{H}_{240h}$ & \texttt{240.d} \\
\cline{3-11}
& & $\operatorname{H}_{192g}$ & $\operatorname{H}_{211s}$ & $\operatorname{H}_{211s}$ & $\operatorname{H}_{189e}$ & $\operatorname{H}_{207l}$ & $\operatorname{H}_{193i}$ & $\operatorname{H}_{235i}$ & $\operatorname{H}_{235i}$ & \texttt{1680.j} \\
\cline{2-11}

& \multirow{9}*{$([2,2],[4],[2],[2,2],[2],[2,2],[2],[2])$} & $\operatorname{H}_{96g}$ & $\operatorname{H}_{118f}$ & $\operatorname{H}_{118c}$ & $\operatorname{H}_{58c}$ & $\operatorname{H}_{92d}$ & $\operatorname{H}_{96p}$ & $\operatorname{H}_{118j}$ & $\operatorname{H}_{118j}$ & \texttt{7605.h} \\
\cline{3-11}
& & $\operatorname{H}_{185l}$ & $\operatorname{H}_{225k}$ & $\operatorname{H}_{212f}$ & $\operatorname{H}_{187j}$ & $\operatorname{H}_{195b}$ & $\operatorname{H}_{215k}$ & $\operatorname{H}_{240d}$ & $\operatorname{H}_{240d}$ & \texttt{1200.e} \\
\cline{3-11}
& & $\operatorname{H}_{192j}$ & $\operatorname{H}_{211p}$ & $\operatorname{H}_{211c}$ & $\operatorname{H}_{189b}$ & $\operatorname{H}_{207c}$ & $\operatorname{H}_{193j}$ & $\operatorname{H}_{235j}$ & $\operatorname{H}_{235j}$ & \texttt{20160.cz} \\
\cline{3-11}
& & $\operatorname{H}_{193g}$ & $\operatorname{H}_{235f}$ & $\operatorname{H}_{235c}$ & $\operatorname{H}_{189c}$ & $\operatorname{H}_{207k}$ & $\operatorname{H}_{192h}$ & $\operatorname{H}_{211h}$ & $\operatorname{H}_{211h}$ & \texttt{1470.j} \\
\cline{3-11}
& & $\operatorname{H}_{208e}$ & $\operatorname{H}_{243b}$ & $\operatorname{H}_{243e}$ & $\operatorname{H}_{183c}$ & $\operatorname{H}_{205d}$ & $\operatorname{H}_{194d}$ & $\operatorname{H}_{213a}$ & $\operatorname{H}_{227d}$ & \texttt{130050.fr} \\
\cline{3-11}
& & $\operatorname{H}_{185i}$ & $\operatorname{H}_{212g}$ & $\operatorname{H}_{225j}$ & $\operatorname{H}_{187h}$ & $\operatorname{H}_{195f}$ & $\operatorname{H}_{215d}$ & $\operatorname{H}_{240m}$ & $\operatorname{H}_{240m}$ & \texttt{75.b} \\
\cline{3-11}
& & $\operatorname{H}_{194g}$ & $\operatorname{H}_{213k}$ & $\operatorname{H}_{227e}$ & $\operatorname{H}_{183j}$ & $\operatorname{H}_{205c}$ & $\operatorname{H}_{208i}$ & $\operatorname{H}_{243l}$ & $\operatorname{H}_{243l}$ & \texttt{50430.ba} \\
\cline{3-11}
& & $\operatorname{H}_{215g}$ & $\operatorname{H}_{240j}$ & $\operatorname{H}_{240f}$ & $\operatorname{H}_{187c}$ & $\operatorname{H}_{195c}$ & $\operatorname{H}_{185b}$ & $\operatorname{H}_{225b}$ & $\operatorname{H}_{212b}$ & \texttt{225.b} \\
\cline{3-11}
& & $\operatorname{H}_{194h}$ & $\operatorname{H}_{227g}$ & $\operatorname{H}_{213f}$ & $\operatorname{H}_{183a}$ & $\operatorname{H}_{205b}$ & $\operatorname{H}_{208g}$ & $\operatorname{H}_{243p}$ & $\operatorname{H}_{243p}$ & \texttt{277440.dv} \\
\cline{2-11}

& \multirow{37}*{$([2,2],[2],[2],[2,2],[2],[2,2],[2],[2])$} & $\operatorname{H}_{96}$ & $\operatorname{H}_{118}$ & $\operatorname{H}_{118}$ & $\operatorname{H}_{58}$ & $\operatorname{H}_{92}$ & $\operatorname{H}_{96}$ & $\operatorname{H}_{118}$ & $\operatorname{H}_{118}$ & \texttt{6435.i} \\
\cline{3-11}
& & $\operatorname{H}_{96h}$ & $\operatorname{H}_{118d}$ & $\operatorname{H}_{118d}$ & $\operatorname{H}_{58d}$ & $\operatorname{H}_{92c}$ & $\operatorname{H}_{96h}$ & $\operatorname{H}_{118d}$ & $\operatorname{H}_{118d}$ & \texttt{2925.d} \\
\cline{3-11}
& & $\operatorname{H}_{96m}$ & $\operatorname{H}_{118v}$ & $\operatorname{H}_{118v}$ & $\operatorname{H}_{58k}$ & $\operatorname{H}_{92i}$ & $\operatorname{H}_{96e}$ & $\operatorname{H}_{118t}$ & $\operatorname{H}_{118q}$ & \texttt{975.i} \\
\cline{3-11}
& & $\operatorname{H}_{96c}$ & $\operatorname{H}_{118s}$ & $\operatorname{H}_{118o}$ & $\operatorname{H}_{58b}$ & $\operatorname{H}_{92a}$ & $\operatorname{H}_{96r}$ & $\operatorname{H}_{118n}$ & $\operatorname{H}_{118n}$ & \texttt{585.g} \\
\cline{3-11}
& & $\operatorname{H}_{96a}$ & $\operatorname{H}_{118e}$ & $\operatorname{H}_{118a}$ & $\operatorname{H}_{58f}$ & $\operatorname{H}_{92f}$ & $\operatorname{H}_{96j}$ & $\operatorname{H}_{118h}$ & $\operatorname{H}_{118h}$ & \texttt{486720.dr} \\
\cline{3-11}
& & $\operatorname{H}_{96l}$ & $\operatorname{H}_{118x}$ & $\operatorname{H}_{118x}$ & $\operatorname{H}_{58h}$ & $\operatorname{H}_{92k}$ & $\operatorname{H}_{96s}$ & $\operatorname{H}_{118w}$ & $\operatorname{H}_{118w}$ & \texttt{40560.h} \\
\cline{3-11}
& & $\operatorname{H}_{96n}$ & $\operatorname{H}_{118u}$ & $\operatorname{H}_{118u}$ & $\operatorname{H}_{58a}$ & $\operatorname{H}_{92b}$ & $\operatorname{H}_{96q}$ & $\operatorname{H}_{118m}$ & $\operatorname{H}_{118m}$ & \texttt{2535.k} \\
\cline{3-11}
& & $\operatorname{H}_{192}$ & $\operatorname{H}_{211}$ & $\operatorname{H}_{211}$ & $\operatorname{H}_{189}$ & $\operatorname{H}_{207}$ & $\operatorname{H}_{193}$ & $\operatorname{H}_{235}$ & $\operatorname{H}_{235}$ & \texttt{25410.bl} \\
\cline{3-11}
& & $\operatorname{H}_{192a}$ & $\operatorname{H}_{211q}$ & $\operatorname{H}_{211l}$ & $\operatorname{H}_{189f}$ & $\operatorname{H}_{207e}$ & $\operatorname{H}_{193e}$ & $\operatorname{H}_{235o}$ & $\operatorname{H}_{235s}$ & \texttt{7350.w} \\
\cline{3-11}
& & $\operatorname{H}_{192b}$ & $\operatorname{H}_{211b}$ & $\operatorname{H}_{211e}$ & $\operatorname{H}_{189g}$ & $\operatorname{H}_{207f}$ & $\operatorname{H}_{193f}$ & $\operatorname{H}_{235r}$ & $\operatorname{H}_{235p}$ & \texttt{1050.c} \\
\cline{3-11}
& & $\operatorname{H}_{192d}$ & $\operatorname{H}_{211i}$ & $\operatorname{H}_{211o}$ & $\operatorname{H}_{189m}$ & $\operatorname{H}_{207b}$ & $\operatorname{H}_{193k}$ & $\operatorname{H}_{235t}$ & $\operatorname{H}_{235q}$ & \texttt{25200.p} \\
\cline{3-11}
& & $\operatorname{H}_{192c}$ & $\operatorname{H}_{211f}$ & $\operatorname{H}_{211a}$ & $\operatorname{H}_{189n}$ & $\operatorname{H}_{207a}$ & $\operatorname{H}_{193l}$ & $\operatorname{H}_{235n}$ & $\operatorname{H}_{235m}$ & \texttt{3150.bp} \\
\cline{3-11}
& & $\operatorname{H}_{96k}$ & $\operatorname{H}_{118g}$ & $\operatorname{H}_{118g}$ & $\operatorname{H}_{58e}$ & $\operatorname{H}_{92g}$ & $\operatorname{H}_{96i}$ & $\operatorname{H}_{118k}$ & $\operatorname{H}_{118k}$ & \texttt{12480.n} \\
\cline{3-11}
& & $\operatorname{H}_{96b}$ & $\operatorname{H}_{118b}$ & $\operatorname{H}_{118b}$ & $\operatorname{H}_{58j}$ & $\operatorname{H}_{92e}$ & $\operatorname{H}_{96b}$ & $\operatorname{H}_{118b}$ & $\operatorname{H}_{118b}$ & \texttt{187200.hl} \\
\cline{3-11}
& & $\operatorname{H}_{185}$ & $\operatorname{H}_{225}$ & $\operatorname{H}_{212}$ & $\operatorname{H}_{187}$ & $\operatorname{H}_{195}$ & $\operatorname{H}_{215}$ & $\operatorname{H}_{240}$ & $\operatorname{H}_{240}$ & \texttt{735.c} \\
\cline{3-11}
& & $\operatorname{H}_{194}$ & $\operatorname{H}_{213}$ & $\operatorname{H}_{227}$ & $\operatorname{H}_{183}$ & $\operatorname{H}_{205}$ & $\operatorname{H}_{208}$ & $\operatorname{H}_{243}$ & $\operatorname{H}_{243}$ & \texttt{1530.b} \\
\cline{3-11}
& & $\operatorname{H}_{96d}$ & $\operatorname{H}_{118p}$ & $\operatorname{H}_{118p}$ & $\operatorname{H}_{58g}$ & $\operatorname{H}_{92j}$ & $\operatorname{H}_{96f}$ & $\operatorname{H}_{118r}$ & $\operatorname{H}_{118r}$ & \texttt{38025.cm} \\
\cline{3-11}
& & $\operatorname{H}_{192n}$ & $\operatorname{H}_{211j}$ & $\operatorname{H}_{211j}$ & $\operatorname{H}_{189l}$ & $\operatorname{H}_{207j}$ & $\operatorname{H}_{193a}$ & $\operatorname{H}_{235k}$ & $\operatorname{H}_{235k}$ & \texttt{6720.j} \\
\cline{3-11}
& & $\operatorname{H}_{194i}$ & $\operatorname{H}_{213j}$ & $\operatorname{H}_{227l}$ & $\operatorname{H}_{183l}$ & $\operatorname{H}_{205e}$ & $\operatorname{H}_{208b}$ & $\operatorname{H}_{243k}$ & $\operatorname{H}_{243k}$ & \texttt{69360.q} \\
\cline{3-11}
& & $\operatorname{H}_{185e}$ & $\operatorname{H}_{225i}$ & $\operatorname{H}_{212e}$ & $\operatorname{H}_{187l}$ & $\operatorname{H}_{195e}$ & $\operatorname{H}_{215j}$ & $\operatorname{H}_{240c}$ & $\operatorname{H}_{240c}$ & \texttt{4800.bz} \\
\cline{3-11}
& & $\operatorname{H}_{185k}$ & $\operatorname{H}_{225e}$ & $\operatorname{H}_{212k}$ & $\operatorname{H}_{187e}$ & $\operatorname{H}_{195g}$ & $\operatorname{H}_{215b}$ & $\operatorname{H}_{240k}$ & $\operatorname{H}_{240k}$ & \texttt{960.l} \\
\cline{3-11}
& & $\operatorname{H}_{208l}$ & $\operatorname{H}_{243f}$ & $\operatorname{H}_{243a}$ & $\operatorname{H}_{183f}$ & $\operatorname{H}_{205a}$ & $\operatorname{H}_{194a}$ & $\operatorname{H}_{213b}$ & $\operatorname{H}_{227c}$ & \texttt{252150.c} \\
\cline{3-11}
& & $\operatorname{H}_{194f}$ & $\operatorname{H}_{213g}$ & $\operatorname{H}_{227j}$ & $\operatorname{H}_{183e}$ & $\operatorname{H}_{205l}$ & $\operatorname{H}_{208h}$ & $\operatorname{H}_{243c}$ & $\operatorname{H}_{243c}$ & \texttt{16320.bw} \\
\cline{3-11}
& & $\operatorname{H}_{185f}$ & $\operatorname{H}_{225l}$ & $\operatorname{H}_{212l}$ & $\operatorname{H}_{187a}$ & $\operatorname{H}_{195a}$ & $\operatorname{H}_{215a}$ & $\operatorname{H}_{240p}$ & $\operatorname{H}_{240p}$ & \texttt{4800.t} \\
\cline{3-11}
& & $\operatorname{H}_{192e}$ & $\operatorname{H}_{211r}$ & $\operatorname{H}_{211g}$ & $\operatorname{H}_{189k}$ & $\operatorname{H}_{207g}$ & $\operatorname{H}_{193b}$ & $\operatorname{H}_{235h}$ & $\operatorname{H}_{235h}$ & \texttt{630.a} \\
\cline{3-11}
& & $\operatorname{H}_{192m}$ & $\operatorname{H}_{211d}$ & $\operatorname{H}_{211d}$ & $\operatorname{H}_{189h}$ & $\operatorname{H}_{207i}$ & $\operatorname{H}_{193c}$ & $\operatorname{H}_{235a}$ & $\operatorname{H}_{235e}$ & \texttt{47040.ha} \\
\cline{3-11}
& & $\operatorname{H}_{194j}$ & $\operatorname{H}_{213e}$ & $\operatorname{H}_{227f}$ & $\operatorname{H}_{183h}$ & $\operatorname{H}_{205f}$ & $\operatorname{H}_{208d}$ & $\operatorname{H}_{243m}$ & $\operatorname{H}_{243m}$ & \texttt{8670.v} \\
\cline{3-11}
& & $\operatorname{H}_{192l}$ & $\operatorname{H}_{211t}$ & $\operatorname{H}_{211t}$ & $\operatorname{H}_{189i}$ & $\operatorname{H}_{207m}$ & $\operatorname{H}_{193m}$ & $\operatorname{H}_{235g}$ & $\operatorname{H}_{235g}$ & \texttt{6720.bq} \\
\cline{3-11}
& & $\operatorname{H}_{192k}$ & $\operatorname{H}_{211k}$ & $\operatorname{H}_{211k}$ & $\operatorname{H}_{189a}$ & $\operatorname{H}_{207d}$ & $\operatorname{H}_{193h}$ & $\operatorname{H}_{235d}$ & $\operatorname{H}_{235d}$ & \texttt{141120.gt} \\
\cline{3-11}
& & $\operatorname{H}_{185c}$ & $\operatorname{H}_{225a}$ & $\operatorname{H}_{212c}$ & $\operatorname{H}_{187f}$ & $\operatorname{H}_{195d}$ & $\operatorname{H}_{215f}$ & $\operatorname{H}_{240e}$ & $\operatorname{H}_{240i}$ & \texttt{14400.cj} \\
\cline{3-11}
& & $\operatorname{H}_{192f}$ & $\operatorname{H}_{211n}$ & $\operatorname{H}_{211n}$ & $\operatorname{H}_{189j}$ & $\operatorname{H}_{207h}$ & $\operatorname{H}_{193d}$ & $\operatorname{H}_{235b}$ & $\operatorname{H}_{235b}$ & \texttt{4410.t} \\
\cline{3-11}
& & $\operatorname{H}_{208k}$ & $\operatorname{H}_{243n}$ & $\operatorname{H}_{243j}$ & $\operatorname{H}_{183b}$ & $\operatorname{H}_{205k}$ & $\operatorname{H}_{194b}$ & $\operatorname{H}_{213c}$ & $\operatorname{H}_{227b}$ & \texttt{196800.ii} \\
\cline{3-11}
& & $\operatorname{H}_{185a}$ & $\operatorname{H}_{225d}$ & $\operatorname{H}_{212d}$ & $\operatorname{H}_{187b}$ & $\operatorname{H}_{195j}$ & $\operatorname{H}_{215e}$ & $\operatorname{H}_{240a}$ & $\operatorname{H}_{240n}$ & \texttt{2880.y} \\
\cline{3-11}
& & $\operatorname{H}_{208f}$ & $\operatorname{H}_{243i}$ & $\operatorname{H}_{243o}$ & $\operatorname{H}_{183g}$ & $\operatorname{H}_{205g}$ & $\operatorname{H}_{194c}$ & $\operatorname{H}_{213d}$ & $\operatorname{H}_{227a}$ & \texttt{6150.r} \\
\cline{3-11}
& & $\operatorname{H}_{185d}$ & $\operatorname{H}_{225c}$ & $\operatorname{H}_{212a}$ & $\operatorname{H}_{187g}$ & $\operatorname{H}_{195i}$ & $\operatorname{H}_{215h}$ & $\operatorname{H}_{240b}$ & $\operatorname{H}_{240o}$ & \texttt{45.a} \\
\cline{3-11}
& & $\operatorname{H}_{185j}$ & $\operatorname{H}_{225f}$ & $\operatorname{H}_{212j}$ & $\operatorname{H}_{187i}$ & $\operatorname{H}_{195k}$ & $\operatorname{H}_{215i}$ & $\operatorname{H}_{240g}$ & $\operatorname{H}_{240g}$ & \texttt{960.a} \\
\cline{3-11}
& & $\operatorname{H}_{194e}$ & $\operatorname{H}_{213l}$ & $\operatorname{H}_{227h}$ & $\operatorname{H}_{183k}$ & $\operatorname{H}_{205j}$ & $\operatorname{H}_{208j}$ & $\operatorname{H}_{243h}$ & $\operatorname{H}_{243h}$ & \texttt{16320.m} \\
\hline
\end{tabular}}
\caption{2-adic Images of $T_{8}$ Graphs}
\label{2-adic Images of T8 Graphs}
\end{table}
\end{center}



\newpage

\subsection{$2$-adic images of $L_{2}(2)$ graphs not in LMFDB}

There are seven examples of $2$-adic images of non-CM elliptic curves over $\QQ$ such that the isogeny graph is of $L_{2}(2)$ and the example elliptic curve is not in the LMFDB. Given an elliptic curve $E/\QQ$ such that the image of the $2$-adic Galois representation attached to $E$ is conjugate to the group $H$, we just need to compute the image of the $2$-adic Galois representation attached to $E / \left\langle Q_{2} \right\rangle$. 

\begin{enumerate}
    \item $\operatorname{H}_{350} = \left\langle
    \begin{bmatrix}
    1 & 3 \\ 10 & 15 \\
    \end{bmatrix},
    \begin{bmatrix}
    1 & 6 \\ 2 & 11 \\
    \end{bmatrix},
    \begin{bmatrix}
    1 & 5 \\ 12 & 7 \\
    \end{bmatrix},
    \begin{bmatrix}
    1 & 2 \\ 2 & 11 \\
    \end{bmatrix}
    \right\rangle \subseteq \operatorname{GL}(2, \ZZ / 16 \ZZ)$
    
    Note that $\operatorname{H}_{350}$ is conjugate to its transpose in $\operatorname{GL}(2, \ZZ / 16 \ZZ)$. To use Lemma \ref{2-adic determination}, we have to rewrite the generators of $E[2]$ as $E[2] = \left\langle Q_{2}, P_{2} \right\rangle$. In this case, the image of the mod-$16$ Galois representation attached to $E$ is conjugate to
    $$H = \left\langle \begin{bmatrix}
    15 & 10 \\ 3 & 1 \\
    \end{bmatrix},
    \begin{bmatrix}
    11 & 2 \\ 6 & 1 \\
    \end{bmatrix},
    \begin{bmatrix}
    7 & 12 \\ 5 & 1 \\
    \end{bmatrix},
    \begin{bmatrix}
    11 & 2 \\ 2 & 1 \\
    \end{bmatrix} \right\rangle.$$
    By Lemma \ref{group lifting}, the image of the mod-$64$ Galois representation attached to $E$ is conjugate to
    $$\overline{H} = \left\langle \begin{bmatrix}
    15 & 10 \\ 3 & 1 \\
    \end{bmatrix},
    \begin{bmatrix}
    11 & 2 \\ 6 & 1 \\
    \end{bmatrix},
    \begin{bmatrix}
    7 & 12 \\ 5 & 1 \\
    \end{bmatrix},
    \begin{bmatrix}
    11 & 2 \\ 2 & 1 \\
    \end{bmatrix},
    \begin{bmatrix}
    17 & 0 \\ 0 & 1
    \end{bmatrix},
    \begin{bmatrix}
    1 & 0 \\ 0 & 17
    \end{bmatrix},
    \begin{bmatrix}
    1 & 16 \\ 0 & 1
    \end{bmatrix},
    \begin{bmatrix}
    1 & 0 \\ 16 & 1
    \end{bmatrix}
    \right\rangle.$$
    By Lemma \ref{2-adic determination}, the image of the mod-$32$ Galois representation attached to $E / \left\langle P_{2} \right\rangle$ is conjugate to
    $$H' = \left\langle
    \begin{bmatrix} 15 & 5 \\ 6 & 1 \end{bmatrix},
    \begin{bmatrix} 11 & 1 \\ 12 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 6 \\ 10 & 1 \end{bmatrix},
    \begin{bmatrix} 11 & 1 \\ 4 & 1 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
    \right\rangle.$$
    Looking up the transpose of $H'$ in the RZB database, we see that the image of the mod-$32$ Galois representation attached to $E / \left\langle P_{2} \right\rangle$ is conjugate to $\operatorname{H}_{284}$.
    
    \item $\operatorname{H}_{323} = \left\langle
    \begin{bmatrix} 1 & 0 \\ 2 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 1 \\ 10 & 15 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 4 & 5 \end{bmatrix},
    \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix}
    \right\rangle \subseteq \operatorname{GL}(2, \ZZ / 16 \ZZ)$
    
    Note that $\operatorname{H}_{323}$ is conjugate to its transpose in $\operatorname{GL}(2, \ZZ / 16 \ZZ)$. To use Lemma \ref{2-adic determination}, we have to rewrite the generators of $E[2]$ as $E[2] = \left\langle Q_{2}, P_{2} \right\rangle$. In this case, the image of the mod-$16$ Galois representation attached to $E$ is conjugate to
    $$H = \left\langle
    \begin{bmatrix} 3 & 2 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 15 & 10 \\ 1 & 1 \end{bmatrix},
    \begin{bmatrix} 5 & 4 \\ 0 & 1 \end{bmatrix}, \begin{bmatrix} 1 & 0 \\ 4 & 1 \end{bmatrix} \right\rangle.$$
    By Lemma \ref{group lifting}, the image of the mod-$64$ Galois representation attached to $E$ is conjugate to
    $$\overline{H} = \left\langle
    \begin{bmatrix} 3 & 2 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 15 & 10 \\ 1 & 1 \end{bmatrix},
    \begin{bmatrix} 5 & 4 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 4 & 1 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
    \right\rangle.$$
    By Lemma \ref{2-adic determination}, the image of the mod-$32$ Galois representation attached to $E / \left\langle P_{2} \right\rangle$ is conjugate to
    $$H' = \left\langle
    \begin{bmatrix} 3 & 1 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 15 & 5 \\ 2 & 1 \end{bmatrix},
    \begin{bmatrix} 5 & 2 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
    \right\rangle.$$
    Looking up the transpose of $H'$ in the RZB databse, we see that the image of the mod-$32$ Galois representation attached to $E / \left\langle P_{2} \right\rangle$ is conjugate to $\operatorname{H}_{288}$.
    \item $\operatorname{H}_{324} = \left\langle
    \begin{bmatrix} 1 & 0 \\ 2 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 1 \\ 10 & 15 \end{bmatrix},
    \begin{bmatrix} 1 & 5 \\ 10 & 15 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 4 & 5 \end{bmatrix}
    \right\rangle \subseteq \operatorname{GL}(2, \ZZ / 16 \ZZ)$
    
    Note that $H$ is conjugate to its transpose in $\operatorname{GL}(2, \ZZ / 16 \ZZ)$. To use Lemma \ref{2-adic determination}, we have to rewrite the generators of $E[2]$ as $E[2] = \left\langle Q_{2}, P_{2} \right\rangle$. In this case, the image of the mod-$16$ Galois representation attached to $E$ is conjugate to
    $$H = \left\langle
    \begin{bmatrix} 3 & 2 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 15 & 10 \\ 1 & 1 \end{bmatrix},
    \begin{bmatrix} 15 & 10 \\ 5 & 1 \end{bmatrix},
    \begin{bmatrix} 5 & 4 \\ 0 & 1 \end{bmatrix},
    \right\rangle.$$
    By Lemma \ref{group lifting}, the image of the mod-$64$ Galois representation attached to $E$ is conjugate to
    $$\overline{H} = \left\langle
    \begin{bmatrix} 3 & 2 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 15 & 10 \\ 1 & 1 \end{bmatrix},
    \begin{bmatrix} 15 & 10 \\ 5 & 1 \end{bmatrix},
    \begin{bmatrix} 5 & 4 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
    \right\rangle.$$
    By Lemma \ref{2-adic determination}, the image of the mod-$32$ Galois representation attached to $E / \left\langle P_{2} \right\rangle$ is conjugate to
    $$H' = \left\langle
    \begin{bmatrix} 3 & 1 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 15 & 5 \\ 2 & 1 \end{bmatrix},
    \begin{bmatrix} 15 & 5 \\ 10 & 1 \end{bmatrix},
    \begin{bmatrix} 5 & 2 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
    \right\rangle.$$
    Searching the RZB database for the transpose of $H'$, we see that the image of the $2$-adic Galois representation attached to $E / \left\langle P_{2} \right\rangle$ is conjugate to $\operatorname{H}_{291}$.
    
    \item $\operatorname{H}_{295} = \left\langle
    \begin{bmatrix} 7 & 14 \\ 0 & 1 \end{bmatrix}
    \begin{bmatrix} 7 & 0 \\ 0 & 7 \end{bmatrix}
    \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix}
    \begin{bmatrix} 1 & 5 \\ 6 & 3 \end{bmatrix}
    \right\rangle \subseteq \operatorname{GL}(2, \ZZ / 16 \ZZ)$
    
    Note that $H$ is not conjugate to its transpose in $\operatorname{GL}(2, \ZZ / 16 \ZZ)$. In other words, the image of the mod-$16$ Galois representation attached to an elliptic curve $E/\QQ$ is conjugate to $\operatorname{H}_{295}$ if its image is conjugate to
    $$H = \left\langle
    \begin{bmatrix} 7 & 0 \\ 14 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 0 \\ 0 & 7 \end{bmatrix},
    \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 6 \\ 5 & 3 \end{bmatrix}
    \right\rangle.$$
    By Lemma \ref{group lifting}, the image of the mod-$32$ Galois representation attached to $E$ is conjugate to
    $$\overline{H} = \left\langle
    \begin{bmatrix} 7 & 0 \\ 14 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 0 \\ 0 & 7 \end{bmatrix},
    \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 6 \\ 5 & 3 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
    \right\rangle.$$
    By Lemma \ref{2-adic determination}, the image of the mod-$32$ Galois representation attached to $E / \left\langle P_{2} \right\rangle$ is conjugate to
    $$H' = \left\langle
    \begin{bmatrix} 7 & 0 \\ 28 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 0 \\ 0 & 7 \end{bmatrix},
    \begin{bmatrix} 5 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 3 \\ 10 & 3 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
    \right\rangle.$$
    Searching the RZB databse for the transpose of $H'$, we see that the image of the $2$-adic Galois representation attached to $E / \left\langle P_{2} \right\rangle$ is conjugate to $\operatorname{H}_{297}$.
    
    \item $\operatorname{H}_{97} = \left\langle
    \begin{bmatrix} 1 & 3 \\ 0 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 3 \\ 2 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 1 \\ 6 & 3 \end{bmatrix}
    \right\rangle \subseteq \operatorname{GL}(2, \ZZ / 8 \ZZ)$
    
    Note that $H$ is conjugate to its transpose in $\operatorname{GL}(2, \ZZ / 8 \ZZ)$. To use Lemma \ref{2-adic determination}, we have to rewrite the generators of $E[2]$ as $E[2] = \left\langle Q_{2}, P_{2} \right\rangle$. In this case, the image of the mod-$8$ Galois representation attached to $E$ is conjugate to
    $$H = \left\langle
    \begin{bmatrix} 7 & 0 \\ 3 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 2 \\ 3 & 1 \end{bmatrix},
    \begin{bmatrix} 3 & 6 \\ 1 & 1 \end{bmatrix}
    \right\rangle.$$
    By Lemma \ref{group lifting}, the image of the mod-$64$ Galois representation attached to $E$ is conjugate to
    $$\overline{H} = \left\langle
    \begin{bmatrix} 7 & 0 \\ 3 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 2 \\ 3 & 1 \end{bmatrix},
    \begin{bmatrix} 3 & 6 \\ 1 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 8 & 1 \end{bmatrix}
    \right\rangle.$$
    By Lemma \ref{2-adic determination}, the image of the mod-$32$ Galois representation attached to $E / \left\langle P_{2} \right\rangle$ is conjugate to
    $$H' = \left\langle
    \begin{bmatrix} 7 & 0 \\ 6 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 1 \\ 6 & 1 \end{bmatrix},
    \begin{bmatrix} 3 & 3 \\ 2 & 1 \end{bmatrix},
    \begin{bmatrix} 9 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 9 \end{bmatrix},
    \begin{bmatrix} 1 & 4 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
    \right\rangle.$$
    The group $H'$ is simply the full lift of the group 
    $$\left\langle
    \begin{bmatrix} 7 & 0 \\ 6 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 1 \\ 6 & 1 \end{bmatrix},
    \begin{bmatrix} 3 & 3 \\ 2 & 1 \end{bmatrix}
    \right\rangle \subseteq \operatorname{GL}(2, \ZZ / 8 \ZZ)$$
    to level $32$, which, in turn is conjugate to $H$ over $\operatorname{GL}(2, \ZZ / 8 \ZZ)$. Hence, the image of the $2$-adic Galios representation attached to $E / \left\langle P_{2} \right\rangle$ is conjugate to $\operatorname{H}_{97}$ also
    
    \item $\operatorname{H}_{113} = \left\langle
    \begin{bmatrix} 1 & 3 \\ 12 & 3 \end{bmatrix},
    \begin{bmatrix} 1 & 1 \\ 12 & 7 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 4 & 5 \end{bmatrix},
    \begin{bmatrix} 1 & 3 \\ 14 & 7 \end{bmatrix}
    \right\rangle \subseteq \operatorname{GL}(2, \ZZ / 16 \ZZ)$
    
    Note that $H$ is conjugate to its transpose in $\operatorname{GL}(2, \ZZ / 16 \ZZ)$. To use Lemma \ref{2-adic determination}, we have to rewrite the generators of $E[2]$ as $E[2] = \left\langle Q_{2}, P_{2} \right\rangle$. In this case, the image of the mod-$16$ Galois representation attached to $E$ is conjugate to
    $$H = \left\langle
    \begin{bmatrix} 3 & 12 \\ 3 & 1\end{bmatrix},
    \begin{bmatrix} 7 & 12 \\ 1 & 1\end{bmatrix},
    \begin{bmatrix} 5 & 4 \\ 0 & 1\end{bmatrix},
    \begin{bmatrix} 7 & 14 \\ 3 & 1\end{bmatrix}
    \right\rangle.$$
    By Lemma \ref{group lifting}, the image of the mod-$64$ Galois representation attached to $E$ is conjugate to
    $$\overline{H} = \left\langle
    \begin{bmatrix} 3 & 12 \\ 3 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 12 \\ 1 & 1 \end{bmatrix},
    \begin{bmatrix} 5 & 4 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 14 \\ 3 & 1 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
    \right\rangle.$$
    By Lemma \ref{2-adic determination}, the image of the mod-$32$ Galois representation attached to $E$ is conjugate to
    $$H' = \left\langle
    \begin{bmatrix} 3 & 6 \\ 6 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 6 \\ 2 & 1 \end{bmatrix},
    \begin{bmatrix} 5 & 2 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 7 & 7 \\ 6 & 1 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
    \right\rangle.$$
    Searching the RZB database for the transpose of $H'$, we see that the image of the $2$-adic Galois representation attached to $E / \left\langle P_{2} \right\rangle`$ is conjugate to $\operatorname{H}_{114}$.
    
    \item $\operatorname{H}_{302} =
    \left\langle
    \begin{bmatrix} 13 & 7 \\ 2 & 3 \end{bmatrix},
    \begin{bmatrix} 3 & 3 \\ 2 & 1 \end{bmatrix},
    \begin{bmatrix} 13 & 10 \\ 2 & 3 \end{bmatrix}
    \right\rangle \subseteq \operatorname{GL}(2, \ZZ / 16 \ZZ)$
    
    Note that $H$ is conjugate to its conjugate in $\operatorname{GL}(2, \ZZ / 16 \ZZ)$. To use Lemma \ref{2-adic determination}, we have to rewrite the generators of $E[2]$ as $E[2] = \left\langle Q_{2}, P_{2} \right\rangle$. In this case, the image of the mod-$16$ Galois representation attached to $E$ is conjugate to
    $$H = \left\langle
    \begin{bmatrix} 3 & 2 \\ 7 & 13 \end{bmatrix},
    \begin{bmatrix} 1 & 2 \\ 3 & 3 \end{bmatrix},
    \begin{bmatrix} 3 & 2 \\ 10 & 13 \end{bmatrix}
    \right\rangle.$$
    By Lemma \ref{group lifting}, the image of the mod-$64$ Galois representation attached to $E$ is conjugate to
    $$\overline{H} = \left\langle
    \begin{bmatrix} 3 & 2 \\ 7 & 13 \end{bmatrix},
    \begin{bmatrix} 1 & 2 \\ 3 & 3 \end{bmatrix},
    \begin{bmatrix} 3 & 2 \\ 10 & 13 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 16 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 16 & 1 \end{bmatrix}
    \right\rangle.$$
    By Lemma \ref{2-adic determination}, the image of the mod-$32$ Galois representation attached to $E / \left\langle P_{2} \right\rangle$ is conjugate to
    $$H' = \left\langle
    \begin{bmatrix} 3 & 1 \\ 14 & 13 \end{bmatrix},
    \begin{bmatrix} 1 & 1 \\ 6 & 3 \end{bmatrix},
    \begin{bmatrix} 3 & 1 \\ 20 & 13 \end{bmatrix},
    \begin{bmatrix} 17 & 0 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 0 & 17 \end{bmatrix},
    \begin{bmatrix} 1 & 8 \\ 0 & 1 \end{bmatrix},
    \begin{bmatrix} 1 & 0 \\ 32 & 1 \end{bmatrix}
    \right\rangle.$$
    Searching the RZB database for the transpose of $H'$, we see that the image of the $2$-adic Galois representation attached to $E / \left\langle P_{2} \right\rangle$ is conjugate to $\operatorname{H}_{326}$.
\end{enumerate}

	

\bibliography{bibliography}
\bibliographystyle{plain}

\begin{tikzcd}
E_{1} \arrow[r, "5", no head] & E_{2} \arrow[r, "5", no head] & E_{3}
\end{tikzcd}

\begin{tikzcd}
E_{1} \arrow[r, "5", no head] \arrow[d, "2"', no head] & E_{2} \arrow[d, "2", no head] \\
E_{3} \arrow[r, "5"', no head]                & E_{4}               
\end{tikzcd}

\begin{tikzcd}
E_{1} \arrow[r, "5", no head] \arrow[d, "3"', no head] & E_{2} \arrow[d, "3", no head] \\
E_{3} \arrow[r, "5"', no head]                & E_{4}               
\end{tikzcd}

\begin{tikzcd}
\mathbb{Z} / 7 \mathbb{Z} \arrow[r, no head, "7"] & \mathcal{O}
\end{tikzcd}

\begin{tikzcd}
\mathbb{Z} / 9 \mathbb{Z} \arrow[r, "3", no head] & \mathbb{Z} / 3 \mathbb{Z} \arrow[r, "3", no head] & \mathcal{O}
\end{tikzcd}

\begin{tikzcd}
\mathbb{Z} / 10 \mathbb{Z} \arrow[r, "2", no head] \arrow[d, "5"', no head] & \mathbb{Z} / 10 \mathbb{Z} \arrow[d, "5", no head] \\
\mathbb{Z} / 2 \mathbb{Z} \arrow[r, "2"', no head]                 & \mathbb{Z} / 2 \mathbb{Z}                
\end{tikzcd}

\begin{tikzcd}
                                           &  & \mathbb{Z} / 12 \mathbb{Z} \arrow[d, "2"', no head] \arrow[rr, "3", no head]                                                     &  & \mathbb{Z} / 4 \mathbb{Z} \arrow[d, "2", no head]                                                     &  &                           \\
                                           &  & \mathbb{Z} / 2 \mathbb{Z} \times \mathbb{Z} / 6 \mathbb{Z} \arrow[rr, "3", no head] \arrow[lld, "2"', no head] \arrow[rrd, "2"', no head] &  & \mathbb{Z} / 2 \mathbb{Z} \times \mathbb{Z} / 2 \mathbb{Z} \arrow[lld, "2", no head] \arrow[rrd, "2", no head] &  &                           \\
\mathbb{Z} / 6 \mathbb{Z} \arrow[rr, "3"', no head] &  & \mathbb{Z} / 2 \mathbb{Z}                                                                                      &  & \mathbb{Z} / 6 \mathbb{Z} \arrow[rr, "3"', no head]                                                   &  & \mathbb{Z} / 2 \mathbb{Z}
\end{tikzcd}

\begin{tikzcd}
                          & \mathbb{Z} / 8 \mathbb{Z} \arrow[d, no head]                                              &                                                                                 & \mathbb{Z} / 2 \mathbb{Z}                                                       &                           \\
                          & \mathbb{Z} / 2 \mathbb{Z} \times \mathbb{Z} / 8 \mathbb{Z} \arrow[ld, no head] \arrow[rd, no head] &                                                                                 & \mathbb{Z} / 2 \mathbb{Z} \times \mathbb{Z} / 2 \mathbb{Z} \arrow[rd, no head] \arrow[u, no head] &                           \\
\mathbb{Z} / 8 \mathbb{Z} &                                                                                  & \mathbb{Z} / 2 \mathbb{Z} \times \mathbb{Z} / 4 \mathbb{Z} \arrow[d, no head] \arrow[ru, no head] &                                                                                 & \mathbb{Z} / 2 \mathbb{Z} \\
                          &                                                                                  & \mathbb{Z} / 4 \mathbb{Z}                                                       &                                                                                 &                          
\end{tikzcd}

\begin{tikzcd}
E/\mathbb{Q} \arrow[rr, "\left\langle Q_{p^{m}} \right\rangle"] &  & E'/\mathbb{Q}
\end{tikzcd}

\begin{tikzcd}
                        & \operatorname{H}_{235l}                                 &                                              & \operatorname{H}_{211m}                      &                         \\
                        & \operatorname{H}_{193n} \arrow[u, no head] \arrow[ld, no head] \arrow[rd, no head] &                                              & \operatorname{H}_{192i} \arrow[u, no head] \arrow[rd, no head] &                         \\
\operatorname{H}_{235l} &                                                         & \operatorname{H}_{189d} \arrow[d, no head] \arrow[ru, no head] &                                              & \operatorname{H}_{211m} \\
                        &                                                         & \operatorname{H}_{207n}                      &                                              &                        
\end{tikzcd}

\begin{tikzcd}
\mathbb{Z} / m \mathbb{Z} \arrow[r, no head, "3"] & \left\{ \mathcal{O} \right\}
\end{tikzcd}

$m = 1$ or $3$

\vspace{5mm}

\begin{tikzcd}
\mathbb{Z} / m \mathbb{Z} \arrow[r, no head, "3"] & \mathbb{Z} / m \mathbb{Z} \arrow[r, no head, "3"] & \mathbb{Z} / m \mathbb{Z} \arrow[r, no head, "3"] & \left\{ \mathcal{O} \right\}
\end{tikzcd}

$m = 1$ or $3$

\vspace{5mm}

\begin{tikzcd}
\mathbb{Z} / 2m \mathbb{Z} \arrow[r, "2", no head] \arrow[d, "3"', no head] & \mathbb{Z} / 2m \mathbb{Z} \arrow[d, "3", no head] \\
\mathbb{Z} / 2 \mathbb{Z} \arrow[r, "2"', no head]                 & \mathbb{Z} / 2 \mathbb{Z}                
\end{tikzcd}

$m = 1$ or $3$




\begin{table}[h!]
 	\renewcommand{\arraystretch}{1.2}
 	\begin{tabular}{|c|c|}
 	\hline
 		Classification of --- & Extension to $\mathbb{Q}$-isogeny classes, Classification of --- \\
 		\hline
 		$\operatorname{X}_{0}(N)$ (Kenku) & isogeny graphs \\
 		\hline
 		$E(\mathbb{Q})_{\texttt{tors}}$ (Mazur) & isogeny-torsion graphs (GC, ÁL-R) \\
 		\hline
 		$\overline{\rho}_{E,2^{\infty}}(G_{\mathbb{Q}})$ (RZB, ÁL-R) & $2$-adic Galois images of isogeny-torsion graphs (ongoing) \\
 		\hline
 	\end{tabular}
 \end{table}

\begin{tikzcd}
E_{1} \arrow[d, "p"', no head] \arrow[r, "2", no head] & E_{2} \arrow[d, "p", no head] \\
E_{3} \arrow[r, "2"', no head]                & E_{4}               
\end{tikzcd}

\newpage

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.7}{
    \begin{tabular}{|c|c|c|}

\hline

Isogeny-Torsion Graph & Reductive $2$-adic classification & $2$-adic classification \\
    \hline
\multirow{14}*{$([1])$} & \multirow{6}*{$\operatorname{H}_{1}$} & $\operatorname{H}_{2}$ \\
\cline{3-3}
& & $\operatorname{H}_{3}$ \\
\cline{3-3}
& & $\operatorname{H}_{4}$ \\
\cline{3-3}
& & $\operatorname{H}_{5}$ \\
\cline{3-3}
& & $\operatorname{H}_{7}$ \\
\cline{3-3}
& & $\operatorname{H}_{20}$ \\
\cline{2-3}
& \multirow{2}*{$\operatorname{H}_{7}$} & $\operatorname{H}_{22}$ \\
\cline{3-3}
& & $\operatorname{H}_{55}$ \\
\cline{2-3}
& \multirow{2}*{$\operatorname{H}_{22}$} & $\operatorname{H}_{56}$ \\
\cline{3-3}
& & $\operatorname{H}_{57}$ \\
\cline{2-3}
& $\operatorname{H}_{55}$ & $\operatorname{H}_{441}$ \\
\cline{2-3}
& \multirow{2}*{$\operatorname{H}_{56}$} & $\operatorname{H}_{177}$ \\
\cline{3-3}
& & $\operatorname{H}_{178}$ \\
\hline
\end{tabular}}
\caption{Reductions of $L_{1}$ Graphs}
\label{Reductions of L1 Graphs}
\end{table}
\end{center}

\newpage

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.7}{
    \begin{tabular}{|c|c|c|}

\hline

Isogeny-Torsion Graph & Reductive $2$-adic classification & $2$-adic classification \\
    \hline
\multirow{9}*{\includegraphics[scale=0.1]{T4 Graph.png}} & \multirow{3}*{$(\operatorname{H}_{8}, \operatorname{H}_{13}, \operatorname{H}_{13}, \operatorname{H}_{13})$} & $(\operatorname{H}_{24}, \operatorname{H}_{27}, \operatorname{H}_{32}, \operatorname{H}_{32})$ \\
\cline{3-3}
& & $(\operatorname{H}_{38}, \operatorname{H}_{34}, \operatorname{H}_{34}, \operatorname{H}_{44})$ \\
\cline{3-3}
& & $(\operatorname{H}_{46}, \operatorname{H}_{33}, \operatorname{H}_{33}, \operatorname{H}_{48})$ \\
\cline{2-3}
& \multirow{3}*{$(\operatorname{H}_{24}, \operatorname{H}_{27}, \operatorname{H}_{32}, \operatorname{H}_{32})$} & $(\operatorname{H}_{61}, \operatorname{H}_{95}, \operatorname{H}_{116}, \operatorname{H}_{116})$ \\
\cline{3-3}
& & $(\operatorname{H}_{66}, \operatorname{H}_{79}, \operatorname{H}_{79}, \operatorname{H}_{94})$ \\
\cline{3-3}
& & $(\operatorname{H}_{67}, \operatorname{H}_{60}, \operatorname{H}_{115}, \operatorname{H}_{115})$ \\
\cline{2-3}
& \multirow{2}*{$(\operatorname{H}_{61}, \operatorname{H}_{95}, \operatorname{H}_{116}, \operatorname{H}_{116})$} & $(\operatorname{H}_{209}, \operatorname{H}_{222}, \operatorname{H}_{241}, \operatorname{H}_{241})$ \\
\cline{3-3}
& & $(\operatorname{H}_{210}, \operatorname{H}_{221}, \operatorname{H}_{242}, \operatorname{H}_{242})$ \\
\cline{2-3}
& $(\operatorname{H}_{66}, \operatorname{H}_{79}, \operatorname{H}_{79}, \operatorname{H}_{94})$ & $(\operatorname{H}_{214}, \operatorname{H}_{226}, \operatorname{H}_{226}, \operatorname{H}_{231})$ \\
\hline
\end{tabular}}
\caption{Reductions of $T_{4}$ Graphs}
\label{Reductions of T4 Graphs}
\end{table}
\end{center}

\newpage

\begin{center}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\scalebox{0.6}{
    \begin{tabular}{|c|c|c|}

\hline

Isogeny-Torsion Graph & Reductive $2$-adic classification & $2$-adic classification \\
    \hline
\multirow{53}*{\includegraphics[scale=0.1]{L22 graph.png}} & \multirow{9}*{$(\operatorname{H}_{6}, \operatorname{H}_{6})$} & $(\operatorname{H}_{9}, \operatorname{H}_{10})$ \\
\cline{3-3}
& & $(\operatorname{H}_{11}, \operatorname{H}_{11})$ \\
\cline{3-3}
& & $(\operatorname{H}_{12}, \operatorname{H}_{12})$ \\
\cline{3-3}
& & $(\operatorname{H}_{14}, \operatorname{H}_{14})$ \\
\cline{3-3}
& & $(\operatorname{H}_{15}, \operatorname{H}_{19})$ \\
\cline{3-3}
& & $(\operatorname{H}_{16}, \operatorname{H}_{17})$ \\
\cline{3-3}
& & $(\operatorname{H}_{18}, \operatorname{H}_{18})$ \\
\cline{3-3}
& & $(\operatorname{H}_{23}, \operatorname{H}_{43})$ \\
\cline{3-3}
& & $(\operatorname{H}_{26}, \operatorname{H}_{28})$ \\
\cline{2-3}
& $(\operatorname{H}_{9}, \operatorname{H}_{10})$ & $(\operatorname{H}_{37}, \operatorname{H}_{42})$ \\
\cline{2-3}
& \multirow{10}*{$(\operatorname{H}_{11}, \operatorname{H}_{11})$} & $(\operatorname{H}_{29}, \operatorname{H}_{41})$ \\
\cline{3-3}
& & $(\operatorname{H}_{35}, \operatorname{H}_{49})$ \\
\cline{3-3}
& & $(\operatorname{H}_{39}, \operatorname{H}_{45})$ \\
\cline{3-3}
& & $(\operatorname{H}_{47}, \operatorname{H}_{47})$ \\
\cline{3-3}
& & $(\operatorname{H}_{50}, \operatorname{H}_{50})$ \\
\cline{3-3}
& & $(\operatorname{H}_{63}, \operatorname{H}_{70})$ \\
\cline{3-3}
& & $(\operatorname{H}_{73}, \operatorname{H}_{90})$ \\
\cline{3-3}
& & $(\operatorname{H}_{77}, \operatorname{H}_{80})$ \\
\cline{3-3}
& & $(\operatorname{H}_{81}, \operatorname{H}_{83})$ \\
\cline{3-3}
& & $(\operatorname{H}_{97}, \operatorname{H}_{97})$ \\
\cline{2-3}
& \multirow{4}*{$(\operatorname{H}_{12}, \operatorname{H}_{12})$} & $(\operatorname{H}_{30}, \operatorname{H}_{30})$ \\
\cline{3-3}
& & $(\operatorname{H}_{31}, \operatorname{H}_{31})$ \\
\cline{3-3}
& & $(\operatorname{H}_{40}, \operatorname{H}_{40})$ \\
\cline{3-3}
& & $(\operatorname{H}_{89}, \operatorname{H}_{93})$ \\
\cline{2-3}
& \multirow{6}*{$(\operatorname{H}_{23}, \operatorname{H}_{43})$} & $(\operatorname{H}_{64}, \operatorname{H}_{64})$ \\
\cline{3-3}
& & $(\operatorname{H}_{65}, \operatorname{H}_{71})$ \\
\cline{3-3}
& & $(\operatorname{H}_{68}, \operatorname{H}_{74})$ \\
\cline{3-3}
& & $(\operatorname{H}_{69}, \operatorname{H}_{91})$ \\
\cline{3-3}
& & $(\operatorname{H}_{76}, \operatorname{H}_{82})$ \\
\cline{3-3}
& & $(\operatorname{H}_{191}, \operatorname{H}_{196})$ \\
\cline{2-3}
& $(\operatorname{H}_{30}, \operatorname{H}_{30})$ & $(\operatorname{H}_{103}, \operatorname{H}_{104})$ \\
\cline{2-3}
& \multirow{4}*{$(\operatorname{H}_{39}, \operatorname{H}_{45})$} & $(\operatorname{H}_{105}, \operatorname{H}_{112})$ \\
\cline{3-3}
& & $(\operatorname{H}_{106}, \operatorname{H}_{111})$ \\
\cline{3-3}
& & $(\operatorname{H}_{107}, \operatorname{H}_{110})$ \\
\cline{3-3}
& & $(\operatorname{H}_{109}, \operatorname{H}_{124})$ \\
\cline{2-3}
& $(\operatorname{H}_{37}, \operatorname{H}_{42})$ & $(\operatorname{H}_{108}, \operatorname{H}_{123})$ \\
\cline{2-3}
& $(\operatorname{H}_{50}, \operatorname{H}_{50})$ & $(\operatorname{H}_{113}, \operatorname{H}_{114})$ \\
\cline{2-3}
& $(\operatorname{H}_{63}, \operatorname{H}_{70})$ & $(\operatorname{H}_{302}, \operatorname{H}_{326})$ \\
\cline{2-3}
& $(\operatorname{H}_{65}, \operatorname{H}_{71})$ & $(\operatorname{H}_{318}, \operatorname{H}_{328})$ \\
\cline{2-3}
& \multirow{3}*{$(\operatorname{H}_{69}, \operatorname{H}_{91})$} & $(\operatorname{H}_{288}, \operatorname{H}_{323})$ \\
\cline{3-3}
& & $(\operatorname{H}_{289}, \operatorname{H}_{320})$ \\
\cline{3-3}
& & $(\operatorname{H}_{291}, \operatorname{H}_{324})$ \\
\cline{2-3}
& \multirow{2}*{$(\operatorname{H}_{73}, \operatorname{H}_{90})$} & $(\operatorname{H}_{281}, \operatorname{H}_{349})$ \\
\cline{3-3}
& & $(\operatorname{H}_{284}, \operatorname{H}_{350})$ \\
\cline{2-3}
& $(\operatorname{H}_{77}, \operatorname{H}_{80})$ & $(\operatorname{H}_{216}, \operatorname{H}_{224})$ \\
\cline{2-3}
& \multirow{2}*{$(\operatorname{H}_{81}, \operatorname{H}_{83})$} & $(\operatorname{H}_{218}, \operatorname{H}_{237})$ \\
\cline{3-3}
& & $(\operatorname{H}_{220}, \operatorname{H}_{232})$ \\
\cline{2-3}
& \multirow{3}*{$(\operatorname{H}_{89}, \operatorname{H}_{93})$} & $(\operatorname{H}_{295}, \operatorname{H}_{297})$ \\
\cline{3-3}
& & $(\operatorname{H}_{556}, \operatorname{H}_{563})$ \\
\cline{3-3}
& & $(\operatorname{H}_{558}, \operatorname{H}_{566})$ \\
\cline{2-3}
& \multirow{2}*{$(\operatorname{H}_{97}, \operatorname{H}_{97})$} & $(\operatorname{H}_{304}, \operatorname{H}_{309})$ \\
\cline{3-3}
& & $(\operatorname{H}_{308}, \operatorname{H}_{312})$ \\
\cline{2-3}
& $(\operatorname{H}_{108}, \operatorname{H}_{123})$ & $(\operatorname{H}_{238}, \operatorname{H}_{239})$ \\
\cline{2-3}
& $(\operatorname{H}_{288}, \operatorname{H}_{323})$ & $(\operatorname{H}_{619}, \operatorname{H}_{649})$ \\
\hline
\end{tabular}}
\caption{Reductions of $L_{2}$ Graphs}
\label{Reductions of L2 Graphs}
\end{table}
\end{center}

\bibliography{bibliography}
\bibliographystyle{plain}

\end{document}


Searching for quadratic subfields of QQ(E[3]) for S graphs

EE:=EllipticCurve("240b");

E:=WeierstrassModel(EE);
Q:=Rationals();
D:=DivisionPolynomial(E,3);
Degree(D) eq 12;
S:=SplittingField(D);
Degree(S) eq 12;
#Roots(D,S);

a1:=Roots(D,S)[1,2];
B<x>:=PolynomialRing(S);
f:=DivisionPolynomial(E,3);
K:=ext<S|x^2-Evaluate(f,a1)>;
F:=AbsoluteField(K);
Degree(F) eq 12;

DD:=DefiningPolynomial(Subfields(F,2)[1,1]);
SquarefreeFactorization(Integers()!Discriminant(DD));
SquarefreeFactorization($1);

DD:=DefiningPolynomial(Subfields(F,2)[2,1]);
SquarefreeFactorization(Integers()!Discriminant(DD));
SquarefreeFactorization($1);

DD:=DefiningPolynomial(Subfields(F,2)[3,1]);
SquarefreeFactorization(Integers()!Discriminant(DD));
SquarefreeFactorization($1);

\fi
